Variational Analysis in the Wasserstein Space

We study optimization problems whereby the optimization variable is a probability measure. Since the space of probability measures is not a vector space, many classical methods for optimization (e.g., gradients) do not directly apply. Thus, one typically resorts to the abstract machinery of infinite-dimensional analysis or other ad-hoc methodologies, not tailored to the space of probability measures, which however involve projections or rely on convexity-type assumptions. We believe instead that these problems call for a comprehensive methodological framework for calculus in the space of probability measures. In this work, we combine ideas from optimal transport, variational analysis, and Wasserstein gradient flows to equip the Wasserstein space (i.e., the space of probability measures endowed with the Wasserstein distance) with a variational structure, both by combining and extending existing results and introducing novel tools. Our theoretical analysis culminates in general necessary optimality conditions. These conditions (i) resemble the optimality conditions in Euclidean spaces, such as the KKT conditions, (ii) are intuitive, informative, and easy to study, and (iii) yield closed-form solutions or can be used to design computationally attractive algorithms. We accompany our theoretical results with numerous examples and present applications to machine learning, drug discovery, and distributionally robust optimization.

==> elements/cor_chain_rule_linear_body.tex <==
Consider the proper functionals $\objective_{1},\objective_{2}:\Pp{2}{\reals^d}\to\realsBar$,  $\rho_1,\rho_2\geq0$, and $\varFixed\in\Pp{2}{\reals^d}$. Then,
$
    \subgradientRegular{(\rho_1\objective_1 + \rho_2\objective_2)}(\varFixed)
    \supseteq
    \rho_1\subgradientRegular{\objective_1}(\varFixed)
    +
    \rho_2\subgradientRegular{\objective_2}(\varFixed).
$
If additionally $\objective_2$ is differentiable at $\varFixed$,
$\subgradientRegular{(\rho_1\objective_1 + \rho_2\objective_2)}(\varFixed)
= \rho_1\subgradientRegular{\objective_1}(\varFixed) + \rho_2\gradient{}{\objective_2}(\varFixed)$ and{, if $\objective_2$ is
differentiable on a Wasserstein neighborhood of $\varFixed$ with
$\varGeneric \mapsto \gradient{}{\objective_2}(\varGeneric)$ continuous at $\varFixed$ (convergence in Wasserstein in the argument and in the value),}
$\subgradient{(\rho_1\objective_1 + \rho_2\objective_2)}(\varFixed)
    = \rho_1\subgradient{\objective_1}(\varFixed) + \rho_2\gradient{}{\objective_2}(\varFixed).
$


==> elements/cor_chain_rule_linear_title.tex <==
Linear combination rule%

==> elements/cor_first_order_optimality_conditions_diff_body.tex <==
Let $\feasibleSet \subseteq \Pp{2}{\reals^d}$, $\objective:\Pp{2}{\reals^d}\to\realsBar$ be proper, and $\varOptimal \in \feasibleSet$ be a local minimum of $\objective$ over $\feasibleSet$.
\begin{enumerate}
\item
    \uniqueLabel{item:cor_first_order:regular}
    If $\objective$ is differentiable at $\varOptimal$, then $-\gradient{}{\objective}(\varOptimal)\in\normalConeRegular{\feasibleSet}{\varOptimal}\subseteq{}\normalCone{\feasibleSet}{\varOptimal}$.
\item
    \uniqueLabel{item:cor_first_order:strong}
    If $\objective$ is strongly differentiable at $\varOptimal$, then $-\gradientStrong{}{\objective}(\varOptimal)\in \normalConeRegularStrong{\feasibleSet}{\varOptimal}\subseteq{}\normalConeStrong{\feasibleSet}{\varOptimal}$.
\end{enumerate}


==> elements/cor_first_order_optimality_conditions_diff_proof.tex <==
{%
For~\ref{item:cor_first_order:regular}, let $\objective$ be differentiable at $\varOptimal$. By~\cref{proposition:prop_differentiability_properties}\ref{item:gradient_uniqueness}, $-\gradient{}{\objective}(\varOptimal) \in \subgradientRegular{(-\objective)}(\varOptimal)$, so, applying~\cref{definition:def_sub_sup_differentiability}\ref{item:subgradient:regular} to $-\objective$, for any $\varGeneric \in \feasibleSet$ sufficiently close to $\varOptimal$ and $\varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varOptimal}{\varGeneric}}$ we have
\begin{equation*}
    \innerProduct{-\gradient{}{\objective}(\varOptimal)}{\varTangent}_{\varOptimal}
    \leq
    -\bigl(\objective(\varGeneric) - \objective(\varOptimal)\bigr) + \onotation{\wassersteinDistance{\varOptimal}{\varGeneric}{2}}
    \leq
    \onotation{\wassersteinDistance{\varOptimal}{\varGeneric}{2}},
\end{equation*}
where the last inequality follows from local optimality of $\varOptimal$.
Hence, $-\gradient{}{\objective}(\varOptimal) \in \normalConeRegular{\feasibleSet}{\varOptimal} \subseteq \normalCone{\feasibleSet}{\varOptimal}$, which proves~\ref{item:cor_first_order:regular}.
}
%
{%
The proof of~\ref{item:cor_first_order:strong} is analogous, replacing differentiability with strong differentiability (\cref{definition:def_strong_differentiability}), so that $-\gradientStrong{}{\objective}(\varOptimal) \in \subgradientRegularStrong{(-\objective)}(\varOptimal)$, $\setPlansOptimal{\varOptimal}{\varGeneric}$ with $\setPlans{\varOptimal}{\varGeneric}$, and the regular normal cone with its strong counterpart (\cref{definition:def_fuzzy_normal_cone}).
Since $\wassersteinDistance{\varOptimal}{\varGeneric}{2} \leq \norm{\varTangent}_{\varOptimal}$ for every $\varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlans{\varOptimal}{\varGeneric}}$, the $\onotation{\norm{\varTangent}_{\varOptimal}}$ condition still forces $\varGeneric\convergenceWasserstein\varOptimal$ as $\norm{\varTangent}_{\varOptimal}\to0$, and the same argument applies.
}


==> elements/cor_first_order_optimality_conditions_diff_title.tex <==
First-order optimality conditions, the differentiable case%

==> elements/cor_functional_variance_body.tex <==
Consider the functional $\objective: \Pp{2}{\reals^d} \to \realsBar$,
$
\objective(\varGeneric)
\coloneqq
\variance{x \sim \varGeneric}{V(x)}
$, {where $V \in \C{2}{\reals^d}{}$ is such that both $V$ and $V^2$ have uniformly bounded Hessians (i.e., there exists $M>0$ so that $\norm{\hessian{}{V}(x)} \leq M$ and $\norm{\hessian{}{(V^2)}(x)} \leq M$ for all $x \in \reals^d$).
Then, $\objective$ is real-valued and, at every $\varFixed \in \Pp{2}{\reals^d}$, differentiable, with gradient}
$
{
\gradient{}{\objective}(\varFixed)
\localEquiv{\varFixed}
\pushforward{(\identity{}, 2(V - \expectedValue{x\sim\varFixed}{V(x)})\gradient{}{V})}{\varFixed}.
}
$


==> elements/cor_functional_variance_proof.tex <==
{%
\emph{Step 1 (growth and convexity estimates).}
Since $\norm{\hessian{}{V}(x)} \leq M$ for all $x \in \reals^d$, a
second-order Taylor expansion around $0$ gives $\abs{V(x)} \leq A +
B\norm{x}^2$ for some $A, B > 0$, the gradient bound
$\norm{\gradient{}{V}(x)} \leq \norm{\gradient{}{V}(0)} + M\norm{x}$, and
$\lambda$-convexity of $V$ with $\lambda = -M$; since $\hessian{}{(V^2)}$
is uniformly bounded as well, the same three properties hold for $V^2$.
In particular, $\objective_1(\varGeneric) \coloneqq
\expectedValue{x\sim\varGeneric}{V(x)^2}$ and $\objective_2(\varGeneric)
\coloneqq \expectedValue{x\sim\varGeneric}{V(x)}$ are finite for every
$\varGeneric \in \Pp{2}{\reals^d}$, so $\objective = \objective_1 -
\objective_2^2$ is real-valued and, since $\abs{V}$ and $V^2$ are
continuous with at most quadratic growth, $\objective_1$ and
$\objective_2$ are continuous in Wasserstein (cf.
\cref{section:ot_wasserstein:background}).

\emph{Step 2 (differentiability of the two terms).}
By \cref{proposition:prop_functional_expected_value}, applied to $V$ and
to $V^2$ (both proper and continuous, hence lower semicontinuous, and, by
Step 1, $\lambda$-convex, differentiable, and bounded above by $A +
B\norm{x}^2$), the functionals $\objective_2$ and $\objective_1$
are differentiable at every $\varGeneric \in \Pp{2}{\reals^d}$, with
gradients $\gradient{}{\objective_2}(\varGeneric) \localEquiv{\varGeneric}
\pushforward{(\identity{}, \gradient{}{V})}{\varGeneric}$ and
$\gradient{}{\objective_1}(\varGeneric) \localEquiv{\varGeneric}
\pushforward{(\identity{}, 2V\gradient{}{V})}{\varGeneric}$. With $g(t) =
t^2$ (so that $g(+\infty) = +\infty$ and $g$ is continuously
differentiable) and $\objective_2$ continuous in Wasserstein by Step 1, the
chain rule for the differentiable case
(\cref{proposition:prop_calculus}\ref{prop_calculus_chain_rule:differentiable})
shows that $\objective_2^2 = \comp{\objective_2}{g}$ is differentiable at
every $\varGeneric$, with gradient
$2\expectedValue{x\sim\varGeneric}{V(x)}\pushforward{(\identity{},
\gradient{}{V})}{\varGeneric} = \pushforward{(\identity{},
2\expectedValue{x\sim\varGeneric}{V(x)}\gradient{}{V})}{\varGeneric}$; by
\cref{definition:def_differentiability}, $-\objective_2^2$ is then
differentiable as well, with gradient $\pushforward{(\identity{},
-2\expectedValue{x\sim\varGeneric}{V(x)}\gradient{}{V})}{\varGeneric}$.

\emph{Step 3 (sum rule).}
By the sum rule
(\cref{proposition:prop_calculus}\ref{prop_calculus_sum_rule}), applied to
$\objective = \objective_1 + (-\objective_2^2)$ (with $\objective_1$
continuous in Wasserstein by Step 1),
$\subgradientRegular{\objective}(\varFixed) \ni
\gradient{}{\objective_1}(\varFixed) \localSum{\varTangentCoupling}
\gradient{}{(-\objective_2^2)}(\varFixed)$; applied to $-\objective =
(-\objective_1) + \objective_2^2$, it likewise yields
$\subgradientRegular{(-\objective)}(\varFixed) \ni
\gradient{}{(-\objective_1)}(\varFixed) \localSum{\varTangentCoupling}
\gradient{}{\objective_2^2}(\varFixed)$, which, by Step 4 below, is the
negation of the former element. Hence, $\objective$ is differentiable at
every $\varFixed \in \Pp{2}{\reals^d}$
(\cref{definition:def_differentiability}).

\emph{Step 4 (the formula).}
All the variations above are induced by maps anchored at $\varFixed$, so
in each sum the coupling $\varTangentCoupling$ is unique and the sum is
induced by the pointwise sum of the maps. Therefore,
$
\gradient{}{\objective}(\varFixed)
\localEquiv{\varFixed}
\pushforward{(\identity{}, 2V\gradient{}{V} -
2\expectedValue{x\sim\varFixed}{V(x)}\gradient{}{V})}{\varFixed}
=
\pushforward{(\identity{}, 2(V -
\expectedValue{x\sim\varFixed}{V(x)})\gradient{}{V})}{\varFixed}.
$
}

==> elements/cor_functional_variance_title.tex <==
Variance%

==> elements/cor_subgradients_horizon_body.tex <==
{%
Each of the functionals $\objective\colon\Pp{2}{\reals^d}\to\reals$ below is Lipschitz on bounded subsets of $\Pp{2}{\reals^d}$ (in the Wasserstein distance) and, in particular, strictly continuous:
\begin{enumerate}[leftmargin=*]
\item the potential energy $\objective(\varGeneric)=\expectedValue{x\sim\varGeneric}{V(x)}$, with $V$ satisfying the assumptions of \cref{proposition:prop_functional_expected_value} and $V(x)\le C(1+\norm{x}^2)$ for some $C>0$;
\item the interaction energy $\objective(\varGeneric)=\tfrac12\expectedValue{(x,y)\sim\varGeneric\times\varGeneric}{U(x-y)}$, with $U$ as in \cref{proposition:prop_functional_interaction};
\item the squared Wasserstein distance $\objective(\varGeneric)=\tfrac12\wassersteinDistance{\varGeneric}{\varReference}{2}^2$ to a fixed $\varReference\in\Pp{2}{\reals^d}$, as in \cref{proposition:prop_wassersteindistance_general_subgradient};
\item the variance $\objective(\varGeneric)=\variance{x\sim\varGeneric}{V(x)}$, with $V$ as in \cref{corollary:cor_functional_variance}.
\end{enumerate}
In particular, all these functionals have trivial horizon subgradient, $\subgradientHzn{\objective}(\varFixed)\localEquiv{\varFixed}\{\localZero{\varFixed}\}$, at every $\varFixed\in\Pp{2}{\reals^d}$.
}


==> elements/cor_subgradients_horizon_proof.tex <==
{%
We prove that each of the four functionals is Lipschitz on bounded subsets of $\Pp{2}{\reals^d}$. Strict continuity at any $\varFixed$ is then immediate, as the closed ball $\closedWassersteinBall{\varFixed}{r}{2}$ is a bounded neighborhood of $\varFixed$, and \cref{proposition:prop_subgradients_horizon_trivial} yields the trivial horizon subgradient. Throughout, $m_2(\varGeneric)\coloneqq\int_{\reals^d}\norm{x}^2\,\d\varGeneric(x)$ denotes the second moment, which is bounded on bounded sets.
For $\varGeneric_1,\varGeneric_2\in\Pp{2}{\reals^d}$, we fix an optimal transport plan $\varPlanGeneric\in\setPlansOptimal{\varGeneric_1}{\varGeneric_2}$, so that $\int_{\reals^d\times\reals^d}\norm{x-y}^2\,\d\varPlanGeneric(x, y)=\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}^2$, with $x$- and $y$-marginals $\varGeneric_1$ and $\varGeneric_2$.

\emph{Step~1 (a transport estimate).}
We first record an estimate used repeatedly: if $\phi\colon\reals^d\to\reals$ satisfies
$
\abs{\phi(x)-\phi(y)}\le c\,(1+\norm{x}+\norm{y})\norm{x-y}+c\,\norm{x-y}^2
$
for all $x,y\in\reals^d$ and some $c>0$, then $\varGeneric\mapsto\int_{\reals^d}\phi(x)\,\d\varGeneric(x)$ is finite on $\Pp{2}{\reals^d}$ and Lipschitz on bounded sets. Indeed, letting $x\to y$ shows that $\phi$ is continuous, and $y=0$ gives $\abs{\phi(x)}\le c'(1+\norm{x}^2)$, so that $\int_{\reals^d}\abs{\phi(x)}\,\d\varGeneric(x)\le c'(1+m_2(\varGeneric))<\infty$. Integrating the growth condition against $\varPlanGeneric$ and using Cauchy--Schwarz,
\begin{align*}
&\abs{\int_{\reals^d}\phi(x)\,\d\varGeneric_1(x)-\int_{\reals^d}\phi(x)\,\d\varGeneric_2(x)}
\\&\qquad\qquad\qquad=\abs{\int_{\reals^d\times\reals^d}\big(\phi(x)-\phi(y)\big)\,\d\varPlanGeneric(x, y)}
\\
&\le c\,\norm{1+\norm{x}+\norm{y}}_{L^2(\varPlanGeneric)}\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}+c\,\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}^2
\\&\le c\big(1+m_2(\varGeneric_1)^{1/2}+m_2(\varGeneric_2)^{1/2}\big)\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}+c\,\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}^2,
\end{align*}
using $\norm{x-y}_{L^2(\varPlanGeneric)}=\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}$. On a bounded set, $m_2$ and $\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}$ are bounded, so the right-hand side is at most a constant multiple of $\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}$.

\emph{Step~2 (potential energy).}
Since $V$ is $\lambda$-convex with $V(x)\le C(1+\norm{x}^2)$, the proper convex function $W\coloneqq V-\tfrac{\lambda}{2}\norm{\cdot}^2$ is bounded above by $C_1(1+\norm{\cdot}^2)$, hence finite, and therefore continuous and subdifferentiable, on $\reals^d$, with $\subgradient{V}(x)=\subgradient{W}(x)+\lambda x$. Fix $p_0\in\subgradient{W}(0)$. Since $p_0$ is a subgradient of $W$ at $0$, the subgradient inequality $W(x)\ge W(0)+\innerProduct{p_0}{x}$ and Cauchy--Schwarz give the lower bound $W(x)\ge W(0)-\norm{p_0}\norm{x}$ for all $x\in\reals^d$. Now fix $x\in\reals^d$ and $p\in\subgradient{W}(x)$; we may assume $p\neq 0$, as the bound below is trivial otherwise. By definition of subgradient, $W(y)\ge W(x)+\innerProduct{p}{y-x}$ for all $y\in\reals^d$; evaluating this inequality at $y=x+t\tfrac{p}{\norm{p}}$ for $t>0$ and using $\innerProduct{p}{\tfrac{p}{\norm{p}}}=\norm{p}$, we obtain
\begin{equation*}
t\norm{p}=\innerProduct{p}{t\tfrac{p}{\norm{p}}}\le W\big(x+t\tfrac{p}{\norm{p}}\big)-W(x).
\end{equation*}
To bound the right-hand side, the quadratic growth $W(\cdot)\le C_1(1+\norm{\cdot}^2)$ with $\norm{x+t\tfrac{p}{\norm{p}}}\le\norm{x}+t$ gives $W\big(x+t\tfrac{p}{\norm{p}}\big)\le C_1\big(1+(\norm{x}+t)^2\big)$, while the lower bound above gives $-W(x)\le-W(0)+\norm{p_0}\norm{x}$; hence
\begin{equation*}
t\norm{p}\le C_1\big(1+(\norm{x}+t)^2\big)-W(0)+\norm{p_0}\norm{x}.
\end{equation*}
Choosing $t=1+\norm{x}$, so that $\norm{x}+t=1+2\norm{x}$, and dividing the previous inequality by $1+\norm{x}$,
\begin{align*}
\norm{p}
&\le\frac{C_1\big(1+(1+2\norm{x})^2\big)-W(0)+\norm{p_0}\norm{x}}{1+\norm{x}}
\\
&=\frac{C_1\big(2+4\norm{x}+4\norm{x}^2\big)-W(0)+\norm{p_0}\norm{x}}{1+\norm{x}}
\\
&\le\frac{4C_1(1+\norm{x})^2}{1+\norm{x}}+\frac{\abs{W(0)}}{1+\norm{x}}+\frac{\norm{p_0}\norm{x}}{1+\norm{x}}
\\
&\le 4C_1(1+\norm{x})+\abs{W(0)}+\norm{p_0}
\\
&\le c_0(1+\norm{x}),
\end{align*}
where $c_0\coloneqq 4C_1+\abs{W(0)}+\norm{p_0}$: the third line uses $2+4\norm{x}+4\norm{x}^2\le 4(1+\norm{x})^2$ and $-W(0)\le\abs{W(0)}$, the fourth uses $1+\norm{x}\ge 1$ and $\norm{x}\le 1+\norm{x}$, and the last uses $\abs{W(0)}+\norm{p_0}\le\big(\abs{W(0)}+\norm{p_0}\big)(1+\norm{x})$. Consequently, since $\subgradient{V}(x)=\subgradient{W}(x)+\lambda x$, every $s\in\subgradient{V}(x)$ satisfies $\norm{s}\le c_0'(1+\norm{x})$ with $c_0'\coloneqq c_0+\abs{\lambda}$. By $\lambda$-convexity, $V(x)-V(y)\le\innerProduct{s_x}{x-y}-\tfrac{\lambda}{2}\norm{x-y}^2$ for $s_x\in\subgradient{V}(x)$, and symmetrically; hence
\begin{equation*}
\abs{V(x)-V(y)}\le c_0'(1+\norm{x}+\norm{y})\norm{x-y}+\tfrac{\abs{\lambda}}{2}\norm{x-y}^2,
\end{equation*}
which is the condition of Step~1 with $\phi=V$. Thus $\objective$ is finite and Lipschitz on bounded sets.

\emph{Step~3 (interaction energy).}
Since $U\in\C{2}{\reals^d}{}$ has bounded Hessian, $\norm{\gradient{}{U}(z)}\le a_0+M\norm{z}$ with $a_0\coloneqq\norm{\gradient{}{U}(0)}$, and $\abs{U(z)}\le\abs{U(0)}+a_0\norm{z}+\tfrac{M}{2}\norm{z}^2$; in particular $\objective$ is finite on $\Pp{2}{\reals^d}$. Coupling $\varGeneric_1\times\varGeneric_1$ with $\varGeneric_2\times\varGeneric_2$ through $\varPlanGeneric\times\varPlanGeneric$,
\begin{equation*}
\objective(\varGeneric_1)-\objective(\varGeneric_2)=\tfrac12\int_{\reals^d\times\reals^d}\!\int_{\reals^d\times\reals^d}\big(U(x-x')-U(y-y')\big)\,\d\varPlanGeneric(x,y)\,\d\varPlanGeneric(x',y').
\end{equation*}
A point of the segment between $x-x'$ and $y-y'$ has norm at most $\norm{x}+\norm{x'}+\norm{y}+\norm{y'}$, and $\norm{(x-x')-(y-y')}\le\norm{x-y}+\norm{x'-y'}$, so the mean value theorem gives
\begin{equation*}
\abs{U(x-x')-U(y-y')}\le\big(a_0+M(\norm{x}+\norm{x'}+\norm{y}+\norm{y'})\big)\big(\norm{x-y}+\norm{x'-y'}\big).
\end{equation*}
By Cauchy--Schwarz over $\varPlanGeneric\times\varPlanGeneric$, using $\norm{\norm{x-y}+\norm{x'-y'}}_{L^2(\varPlanGeneric\times\varPlanGeneric)}\le2\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}$ and $\norm{a_0+M(\norm{x}+\norm{x'}+\norm{y}+\norm{y'})}_{L^2(\varPlanGeneric\times\varPlanGeneric)}\le a_0+2M(m_2(\varGeneric_1)^{1/2}+m_2(\varGeneric_2)^{1/2})$,
\begin{equation*}
\abs{\objective(\varGeneric_1)-\objective(\varGeneric_2)}\le\big(a_0+2M(m_2(\varGeneric_1)^{1/2}+m_2(\varGeneric_2)^{1/2})\big)\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2},
\end{equation*}
so $\objective$ is Lipschitz on bounded sets.

\emph{Step~4 (Wasserstein distance).}
The triangle inequality gives $\abs{\wassersteinDistance{\varGeneric_1}{\varReference}{2}-\wassersteinDistance{\varGeneric_2}{\varReference}{2}}\le\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}$, so
\begin{align*}
\abs{\objective(\varGeneric_1)-\objective(\varGeneric_2)}
&=\tfrac12\abs{\wassersteinDistance{\varGeneric_1}{\varReference}{2}-\wassersteinDistance{\varGeneric_2}{\varReference}{2}}\big(\wassersteinDistance{\varGeneric_1}{\varReference}{2}+\wassersteinDistance{\varGeneric_2}{\varReference}{2}\big)
\\
&\le\tfrac12\big(\wassersteinDistance{\varGeneric_1}{\varReference}{2}+\wassersteinDistance{\varGeneric_2}{\varReference}{2}\big)\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}.
\end{align*}
The prefactor is bounded on bounded sets, so $\objective$ is Lipschitz on bounded sets.

\emph{Step~5 (variance).}
Write $\objective=g\circ(\objective_1,\objective_2)$, where $\objective_1(\varGeneric)\coloneqq\int_{\reals^d} V(x)^2\,\d\varGeneric(x)$, $\objective_2(\varGeneric)\coloneqq\int_{\reals^d} V(x)\,\d\varGeneric(x)$, and $g(a,b)\coloneqq a-b^2$. Since $V$ and $V^2$ have uniformly bounded Hessians, Taylor expansions around $0$ give, for some $A,B,c>0$ and all $x\in\reals^d$, the quadratic bounds $\abs{V(x)}\le A+B\norm{x}^2$ and $V(x)^2\le A+B\norm{x}^2$, together with the gradient bounds $\norm{\gradient{}{V}(x)}\le c(1+\norm{x})$ and $\norm{\gradient{}{(V^2)}(x)}\le c(1+\norm{x})$. By the mean value theorem---a point of the segment between $x$ and $y$ having norm at most $\norm{x}+\norm{y}$---both $\abs{V(x)-V(y)}$ and $\abs{V^2(x)-V^2(y)}$ are at most $c''(1+\norm{x}+\norm{y})\norm{x-y}$, so $V$ and $V^2$ satisfy the condition of Step~1. Hence, $\objective_1$ and $\objective_2$ are Lipschitz on bounded sets; they are also bounded there (by $A+B\,m_2(\varGeneric)$), so $(\objective_1(\varGeneric),\objective_2(\varGeneric))$ ranges in a bounded set $S\subseteq\reals^2$. Since $g(a,b)=a-b^2$ is continuously differentiable, it is Lipschitz on the bounded set $S$: there is a constant $L_S\ge 0$ such that $\abs{g(a)-g(a')}\le L_S\big(\abs{a_1-a_1'}+\abs{a_2-a_2'}\big)$ for all $a=(a_1,a_2),\,a'=(a_1',a_2')\in S$. Applying this bound with $a=(\objective_1(\varGeneric_1),\objective_2(\varGeneric_1))$ and $a'=(\objective_1(\varGeneric_2),\objective_2(\varGeneric_2))$,
\begin{equation*}
\abs{\objective(\varGeneric_1)-\objective(\varGeneric_2)}\le L_S\big(\abs{\objective_1(\varGeneric_1)-\objective_1(\varGeneric_2)}+\abs{\objective_2(\varGeneric_1)-\objective_2(\varGeneric_2)}\big),
\end{equation*}
and, since $\objective_1$ and $\objective_2$ are Lipschitz on bounded sets, so is $\objective$.
}


==> elements/cor_subgradients_horizon_title.tex <==
Some horizon subgradients%

==> elements/def_almost_linear_structure_wass_body.tex <==
Given $\varFixed \in \Pp{2}{\reals^d}$, $\varTangent_1, \varTangent_2 \in \PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$, and $\tau \in \reals$,
we define:
\begin{enumerate}[leftmargin=*]
\item \emph{A ``local'' zero:}
\label{item:local-zero}
$
\localZero{\varFixed}
\coloneqq
\varFixed\times\delta_0.
$

\item \emph{A scalar multiplication\footnote{We highlight the distinction between our multiplication, which affects the displacement of the probability mass but not the total mass, and the multiplication in the space of signed measures, which instead merely affects the amount of probability mass at each location without displacing it. As we never operate in the space of signed measures, the notational override does not create ambiguity.}:}
\label{item:local-scale}
$
\tau \varTangent_1
\coloneqq
\pushforward{(\projection{1}{}, \tau \projection{2}{})}{\varTangent_1}.
$

\item \emph{An addition:} For $\varTangentCoupling\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}$,
\label{item:local-sum}
$
\varTangent_1
\localSum{\varTangentCoupling}
\varTangent_2
\coloneqq
\pushforward{(\projection{1}{}, \projection{2}{} + \projection{3}{})}{\varTangentCoupling}.
$
\end{enumerate}


==> elements/def_almost_linear_structure_wass_title.tex <==
An ``almost linear'' structure of the space of variations%

==> elements/def_differentiability_body.tex <==
A functional $\objective: \Pp{2}{\reals^d} \to \realsBar$ is \emph{differentiable} at $\varFixed \in \Pp{2}{\reals^d}$ if
$
-\subgradientRegular{(-\objective)}(\varFixed)
\cap
\subgradientRegular{\objective}(\varFixed) \neq \emptyset.
$

==> elements/def_differentiability_title.tex <==
Differentiable functional%

==> elements/def_extremal_body.tex <==
Let $\Omega_1,\Omega_2 \subseteq \Pp{2}{\reals^d}$ be nonempty sets and let $\varFixed\in\Omega_1\cap\Omega_2$.
%
The probability measure $\varFixed$ is a local extremal point of $(\Omega_1,\Omega_2)$ if there is a \WikipediaLink{https://en.wikipedia.org/wiki/Neighbourhood_(mathematics)}{neighborhood} $U$ of $\varFixed$ so that for all $\varepsilon>0$ there is $a\in\reals^d$ with $\norm{a}<\varepsilon$ such that
$
\left(\pushforward{(\identity{}+a)}{\Omega_1}\right)\cap \Omega_2\cap U = \emptyset
$.
In this case, $(\Omega_1,\Omega_2,\varFixed)$ is called extremal.

==> elements/def_extremal_title.tex <==
Extremal system%


==> elements/def_fuzzy_normal_cone_body.tex <==
    The \emph{strong regular normal cone} of $\feasibleSet \subseteq \Pp{2}{\reals^d}$ at $\varFixed \in \feasibleSet$, denoted by $\normalConeRegularStrong{\feasibleSet}{\varFixed}$, contains all the $\varTangentFixed \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ such that for all $\varGeneric \in \feasibleSet$, one has $\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed} \leq \onotation{\norm{\varTangent}_{\varFixed}}$ for $\varTangent\in\pushforward{(\projection{1}{}, \projection{2}{}- \projection{1}{})}{\setPlans{\varFixed}{\varGeneric}}$.
The \emph{strong normal cone} of $\feasibleSet$ at $\varFixed$, denoted by $\normalConeStrong{\feasibleSet}{\varFixed}$, is the limit of strong regular normals; i.e., $\varTangentFixed \in \PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$ belongs to $\normalConeStrong{\feasibleSet}{\varFixed}$ if there exist $(\varGeneric_n)_{n\in\naturals} \subseteq \feasibleSet$, $\varGeneric_n \convergenceWasserstein \varFixed$, and $\varTangent_n \in \normalConeRegularStrong{\feasibleSet}{\varGeneric_n}$ so that $\varTangent_n \convergenceWasserstein \varTangentFixed$.


==> elements/def_fuzzy_normal_cone_title.tex <==
Strong normal cone%

==> elements/def_normal_cone_body.tex <==
The \emph{regular normal cone} of $\feasibleSet \subseteq \Pp{2}{\reals^d}$ at $\varFixed \in \feasibleSet$, denoted by $\normalConeRegular{\feasibleSet}{\varFixed}$,
contains all the
$\varTangentFixed \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ such that for all $\varGeneric \in \feasibleSet$, one has
$
\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed} \leq \onotation{\norm{\varTangent}_{\varFixed}}
$
for $\varTangent\in\pushforward{(\projection{1}{}, \projection{2}{}- \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$.
The \emph{normal cone} of $\feasibleSet$ at $\varFixed$, denoted by $\normalCone{\feasibleSet}{\varFixed}$, is the limit of regular normals; i.e., $\varTangentFixed \in \PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$ belongs to $\normalCone{\feasibleSet}{\varFixed}$ if there exist 
$(\varGeneric_n)_{n\in\naturals}\subset \feasibleSet$,
$\varGeneric_n \convergenceWasserstein \varFixed$,
$\varTangent_n \in \normalConeRegular{\feasibleSet}{\varGeneric_n}$
so that 
$\varTangent_n \convergenceWasserstein \varTangentFixed$.



==> elements/def_normal_cone_title.tex <==
Normal cone%

==> elements/def_snc_body.tex <==
A set $\feasibleSet$ is \gls*{acr:snc} at $\varFixed \in \feasibleSet$ if for any sequence $(\varGeneric_n)_{n \in \naturals} \subseteq \feasibleSet$, $\varGeneric_n\convergenceWasserstein\varFixed$ and $\varTangent_n\in\normalConeRegularStrong{\feasibleSet}{\varGeneric_n}$ so that $\varTangent_n\convergenceNarrow\varTangent{}\in\Pp{2}{\reals^d\times\reals^d}$, we have $\varTangent_n \convergenceWasserstein\varTangent$.


==> elements/def_snc_title.tex <==
Sequential normal compactness%

==> elements/def_strong_differentiability_body.tex <==
{%
    A functional $\objective: \Pp{2}{\reals^d} \to \realsBar$ is \emph{strongly differentiable} at $\varFixed \in \Pp{2}{\reals^d}$ if
    $
    -\subgradientRegularStrong{(-\objective)}(\varFixed)
    \cap
    \subgradientRegularStrong{\objective}(\varFixed) \neq \emptyset.
    $}


==> elements/def_strong_differentiability_title.tex <==
Strongly differentiable functional%

==> elements/def_strong_sub_sup_differentiability_body.tex <==
Consider a functional $\objective: \Pp{2}{\reals^d} \to \realsBar$ and a probability measure $\varFixed \in \Pp{2}{\reals^d}$ with $\objective(\varFixed) \in \reals$. We say that:
\begin{enumerate}
\item
    \uniqueLabel{item:strong_subgradient:regular}
    {$\varTangentFixed \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ is a \emph{strong regular subgradient of $\objective$ at $\varFixed$}, written $\varTangentFixed \in \subgradientRegularStrong{\objective}(\varFixed)$, if for all $\varGeneric \in \Pp{2}{\reals^d}$ and all $\varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlans{\varFixed}{\varGeneric}}$, it holds that
    $
    \objective(\varGeneric) - \objective(\varFixed) \geq \innerProduct{\varTangentFixed}{\varTangent}_{\varFixed} + \onotation{\norm{\varTangent}_{\varFixed}}.
    $}
\item
    \uniqueLabel{item:strong_subgradient}
    $\varTangentFixed \in \PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$ is a \emph{strong (general) subgradient of $\objective$ at $\varFixed$}, written $\varTangentFixed \in \subgradientStrong{\objective}(\varFixed)$, if there are sequences $\varGeneric_n \convergenceWasserstein \varFixed$ with $\objective(\varGeneric_n)\to\objective(\varFixed)$ and $\varTangent_n \in \subgradientRegularStrong{\objective}(\varGeneric_n)$ with $\varTangent_n \convergenceWasserstein \varTangentFixed$.
\end{enumerate}


==> elements/def_strong_sub_sup_differentiability_title.tex <==
Strong subgradient%

==> elements/def_sub_sup_differentiability_body.tex <==
Consider a functional $\objective: \Pp{2}{\reals^d} \to \realsBar$ and a probability measure $\varFixed \in \Pp{2}{\reals^d}$ with $\objective(\varFixed) \in \reals$. We say that:
\begin{enumerate}
\item 
\uniqueLabel{item:subgradient:regular}
$\varTangentFixed \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ is a \emph{regular subgradient of $\objective$ at $\varFixed$}, written $\varTangentFixed \in \subgradientRegular{\objective}(\varFixed)$, if for all $\varGeneric \in \Pp{2}{\reals^d}$ and all $\varTangent \in \pushforward{(\pi_1, \pi_2 - \pi_1)}{\setPlansOptimal{\varFixed}{\varGeneric}}$, it holds that
$
    \objective(\varGeneric) 
    -
    \objective(\varFixed) 
    \geq
    \innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
    +
    \onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}.
$
Then, $\objective$ is regularly subdifferentiable at $\varFixed$.
\item
\uniqueLabel{item:subgradient}
$\varTangentFixed \in \PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$
is a \emph{(general) subgradient of $\objective$ at $\varFixed$}, written $\varTangentFixed \in \subgradient{\objective}(\varFixed)$, if there are sequences $\varGeneric_n \convergenceWasserstein \varFixed$ with $\objective(\varGeneric_n)\to\objective(\varFixed)$ and $\varTangent_n \in \subgradientRegular{\objective}(\varGeneric_n)$ with $\varTangent_n \convergenceWasserstein \varTangentFixed$. 
Then, $\objective$ is subdifferentiable at $\varFixed$.
\end{enumerate}

==> elements/def_sub_sup_differentiability_horizon_body.tex <==
For $\objective: \Pp{2}{\reals^d} \to \realsBar$ and any $\varFixed \in \Pp{2}{\reals^d}$ at which $\objective(\varFixed) \in \reals$, 
we say that $\varTangent\in\PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$ is a \emph{horizon subgradient of $\objective$ at $\varFixed$}, $\varTangent \in \subgradientHzn{\objective}(\varFixed)$, if there exists $\boldsymbol{\varTangent} \in\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ such that $\pushforward{T}{\boldsymbol{\varTangent}} = \varTangent$ and $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = 0$, with $T$ as in \eqref{equation:extraction-map-epigraph}.

==> elements/def_sub_sup_differentiability_horizon_title.tex <==
Wasserstein horizon subgradients%

==> elements/def_sub_sup_differentiability_title.tex <==
Wasserstein subgradients%

==> elements/def_tangent_cone_body.tex <==
The \emph{tangent cone} of $\feasibleSet \subseteq \Pp{2}{\reals^d}$ at $\varFixed \in \feasibleSet$, denoted by $\tangentCone{\feasibleSet}{\varFixed}$, is the set of all the $\varTangentFixed \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ such that for some $(\varGeneric_n)_{n \in \naturals} \subseteq \feasibleSet$, $\varGeneric_n \convergenceWasserstein \varFixed$, $(\varTangent_n)_{n \in \naturals} \subseteq \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$, $\varTangent_n\in\pushforward{(\projection{1}{}, \projection{2}{}- \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric_n}}$ and $\tau_n \fromAbove 0$, one has
$
\wassersteinDistance{\frac{1}{\tau_n}\varTangent_n}{ \varTangentFixed}{\varFixed}\to 0
$.

==> elements/def_tangent_cone_title.tex <==
Tangent cone%

==> elements/def_wasserstein_space_local_optimum_body.tex <==
A functional $\objective: \Pp{2}{\reals^d} \to \realsBar$ attains a local minimum over a constraint set $\feasibleSet \subseteq \Pp{2}{\reals^d}$ at $\varOptimal \in \feasibleSet$ if there exists $\varepsilon>0$ such that for all $\varGeneric \in \wassersteinBall{\varOptimal}{\varepsilon}{2} \cap \feasibleSet$ we have 
$
\objective(\varGeneric) \geq \objective(\varOptimal).
$

==> elements/def_wasserstein_space_local_optimum_title.tex <==
Local optimality in the Wasserstein space%

==> elements/eps_to_exact_normal_body.tex <==
Let $\varFixed\in\Omega\subseteq\Pp{2}{\reals^d}$, with $\Omega$ nonempty and locally closed around $\varFixed$. Let $\varepsilon\geq0$ and $\sigma>0$ and let $\varTangent_\varepsilon\in\PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$ such that, for all $\varGeneric\in\Omega$, one has $\innerProduct{\varTangent_\varepsilon}{\varTangent}_{\varFixed}\leq\varepsilon\norm{\varTangent}_{\varFixed}+\onotation{\norm{\varTangent}_{\varFixed}}$ for $\varTangent\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varFixed}{\varGeneric}}$.
Then, there is $\tilde\varGeneric\in\Omega$ so that $\wassersteinDistance{\varFixed}{\tilde\varGeneric}{2}\leq\sigma$ and $\varTangent\in\normalConeRegularStrong{\Omega}{\tilde\varGeneric}$ so that $\wassersteinDistance{\varTangent}{\varTangent_\varepsilon}{2}\leq\varepsilon+\sigma$.


==> elements/eps_to_exact_normal_proof.tex <==
We divide the proof into steps.
If $\norm{\varTangent_\varepsilon}_{\varFixed}\leq\varepsilon+\sigma$, then $\varTangent\coloneqq\localZero{\varFixed}\in\normalConeRegularStrong{\Omega}{\varFixed}$ and $\tilde\varGeneric\coloneqq\varFixed$ satisfy these bounds, since $\wassersteinDistance{\varTangent}{\varTangent_\varepsilon}{2}\leq\wassersteinDistance{\localZero{\varFixed}}{\varTangent_\varepsilon}{\varFixed}=\norm{\varTangent_\varepsilon}_{\varFixed}\leq\varepsilon+\sigma$. Hence, throughout the proof we assume $\norm{\varTangent_\varepsilon}_{\varFixed}>\varepsilon+\sigma$.

\emph{Step 1 (Reduction and epigraphical lift).}
We lift the problem to $\Pp{2}{\epigraphSpace}$, where $\epigraphSpace\coloneqq\reals^d\times\reals^d\times\reals^d\times\reals$ and we read the coordinates $(\bar x,\varTangentReals_\varepsilon,x,\beta)$ as a base point $\bar x$, the value $\varTangentReals_\varepsilon$ of the candidate normal $\varTangent_\varepsilon$ at $\bar x$, a moved point $x\in\Omega$, and an epigraphical variable $\beta\in\reals$.
Let
\begin{align*}
    \Lambda_1
    &\coloneqq\left\{\varTangentCoupling\times\delta_\beta\in\Pp{2}{\reals^d\times\reals^d\times\reals^d\times\reals}
    \st
    \pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega,\;
    \beta\geq 0\right\},
    \\
    \Lambda_2
    &\coloneqq
    \biggl\{
    \varTangentCoupling\times\delta_\beta\in\Pp{2}{\reals^d\times\reals^d\times\reals^d\times\reals}
    \st
    \pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling}=\varTangent_\varepsilon,
    \\&
    \qquad
    \beta
    \leq
    \int_{\reals^d\times\reals^d\times\reals^d}\innerProduct{\varTangentReals_\varepsilon}{x-\bar x}
    \d\varTangentCoupling(\bar x,\varTangentReals_\varepsilon,x)
    -(\varepsilon+\sigma)
    \sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{x-\bar x}^2\d\varTangentCoupling(\bar x,\varTangentReals_\varepsilon,x)}
    \biggr\}.
\end{align*}
Both sets are nonempty (e.g., $\bar\varTangentCoupling\times\delta_0\in\Lambda_1\cap\Lambda_2$, where $\bar\varTangentCoupling\coloneqq\pushforward{(\projection{1}{},\projection{2}{},\projection{1}{})}{\varTangent_\varepsilon}$ corresponds to the optimal transport plan $\pushforward{(\identity{},\identity{})}{\varFixed}$ of $\varFixed$ with itself). They are also locally closed around $\bar\varTangentCoupling\times\delta_0$: $\Lambda_2$ is closed since $\pushforward{(\projection{1}{},\projection{2}{})}{}$ is $1$-Lipschitz with respect to $\wassersteinDistance{}{}{2}$ and the second-moment functionals defining its $\beta$-bound are continuous in Wasserstein, while $\Lambda_1$ inherits local closedness from $\Omega$ through the $1$-Lipschitz marginal $\pushforward{\projection{3}{}}{}$ and the closedness of $\beta\geq0$.

\emph{Step 2 (Extremality and the extremal principle).}
We now show that $\bar\varTangentCoupling\times\delta_0$ is a local extremal point of $(\Lambda_1,\Lambda_2)$.
By hypothesis,
\[
\limsup_{\substack{\varGeneric\in\Omega,\,\varTangent\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varFixed}{\varGeneric}}\\\norm{\varTangent}_{\varFixed}\to0}} \frac{\innerProduct{\varTangent_\varepsilon}{\varTangent}_{\varFixed}}{\norm{\varTangent}_{\varFixed}}\leq \varepsilon .
\]
Thus, there exists a neighborhood $U$ of $\bar{\varTangentCoupling}\times\delta_0$ such that, for every $\varTangentCoupling\times\delta_\beta\in U$ with $\pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling}=\varTangent_\varepsilon$ and $\pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega$, the induced variation $\varTangent\coloneqq\pushforward{(\projection{1}{},\projection{3}{}-\projection{1}{})}{\varTangentCoupling}$ of $\Omega$ at $\varFixed$ satisfies
\begin{equation}\label{eq:eps_normal_cone:extremality}
    \begin{aligned}
    \int_{\reals^d\times\reals^d\times\reals^d}\innerProduct{\varTangentReals_\varepsilon}{x-\bar x}
    \d\varTangentCoupling(\bar x,\varTangentReals_\varepsilon,x)
    &\leq
    \innerProduct{\varTangent_\varepsilon}{\varTangent}_{\varFixed}
    \\
    &\leq
    (\varepsilon+\sigma)
    \norm{\varTangent}_{\varFixed}
    \\
    &=
    (\varepsilon+\sigma)
    \sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{x-\bar x}^2\d\varTangentCoupling(\bar x,\varTangentReals_\varepsilon,x)}.
    \end{aligned}
\end{equation}
where the first inequality follows from the definition of inner product and the second from the $\varepsilon$-normality of $\varTangent_\varepsilon$, applicable because $\norm{\varTangent}_{\varFixed}^2=\int_{\reals^d\times\reals^d\times\reals^d}\norm{x-\bar x}^2\d\varTangentCoupling(\bar x,\varTangentReals_\varepsilon,x)$ is small for $\varTangentCoupling\times\delta_\beta\in U$ and $\pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega$.
%
We claim $\pushforward{(\identity{}+(0,0,0,a))}{\Lambda_1}\cap\Lambda_2\cap U=\emptyset$ for all $a>0$, so that $(\Lambda_1,\Lambda_2,\bar\varTangentCoupling\times\delta_0)$ is extremal in the sense of~\cref{definition:def_extremal}. Indeed, a point $\varTangentCoupling\times\delta_\beta$ in this intersection lies in $\Lambda_2$, so $\pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling}=\varTangent_\varepsilon$.
It is also the $(0,0,0,a)$-shift of a point of $\Lambda_1$, i.e., $\varTangentCoupling\times\delta_{\beta-a}\in\Lambda_1$, so $\pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega$ and $\beta-a\geq0$. Since $\pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega$,~\eqref{eq:eps_normal_cone:extremality} together with the $\beta$-bound defining $\Lambda_2$ forces $\beta\leq0$, contradicting $\beta\geq a>0$.
Therefore, \cref{theorem:th_extremal_principle} applied to $(\Lambda_1,\Lambda_2,\bar\varTangentCoupling\times\delta_0)$ with accuracy $\sigma>0$ yields points $\varTangentCoupling_i\times\delta_{\beta_i}\in\Lambda_i$ with
\begin{equation}\label{eq:eps_normal_cone:close_points}
    \sqrt{\wassersteinDistance{\bar\varTangentCoupling}{\varTangentCoupling_i}{2}^2+\abs{\beta_i}^2}<\sigma,
    \qquad i\in\{1,2\},
\end{equation}
and tangent vectors $\boldsymbol{\varTangent}_i$ at $\varTangentCoupling_i\times\delta_{\beta_i}$, with $\norm{\boldsymbol{\varTangent}_i}_{\varTangentCoupling_i\times\delta_{\beta_i}}=1$, that are $\sigma$-close to the strong regular normal cone $\normalConeRegularStrong{\Lambda_i}{\varTangentCoupling_i\times\delta_{\beta_i}}$, and a transport plan $\varPlanGeneric_{\boldsymbol\varTangent}\in\setPlans{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_2}$ with $\pushforward{(\projection{1}{},\projection{3}{})}{\varPlanGeneric_{\boldsymbol\varTangent}}\in\setPlansOptimal{\varTangentCoupling_1\times\delta_{\beta_1}}{\varTangentCoupling_2\times\delta_{\beta_2}}$ such that
\begin{equation}\label{eq:eps_normal_cone:cancellation}
    \int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol{\varTangentReals}_1+\boldsymbol{\varTangentReals}_2}^2\d\varPlanGeneric_{\boldsymbol\varTangent}(\boldsymbol{\zeta}_1,\boldsymbol{\zeta}_2)=0.
\end{equation}
For $i\in\{1,2\}$ we fix $\boldsymbol{\varTangent}_i^{\parallel}\in\normalConeRegularStrong{\Lambda_i}{\varTangentCoupling_i\times\delta_{\beta_i}}$ with $\wassersteinDistance{\boldsymbol{\varTangent}_i}{\boldsymbol{\varTangent}_i^{\parallel}}{\varTangentCoupling_i\times\delta_{\beta_i}}\leq\sigma$.

\emph{Step 3 (Structure of the lifted normals).}
We write the arrow of $\boldsymbol{\varTangent}_i^{\parallel}$ in coordinates as $\boldsymbol{\zeta}_i=(\boldsymbol{w}_i,\varTangentReals_i,\lambda_i^{\beta})$, with $\boldsymbol{w}_i$ the $(\bar x,\varTangentReals_\varepsilon)$-component, $\varTangentReals_i$ the $x$-component, and $\lambda_i^{\beta}$ the (scalar) $\beta$-component.
We let $\lambda_i\coloneqq\expectedValue{\boldsymbol{\varTangent}_i^{\parallel}}{\lambda_i^{\beta}}$.
We record two facts.

\emph{Fact 1.}
By~\cref{theorem:th_extremal_principle}, $\boldsymbol{\varTangent}_1$ and $\boldsymbol{\varTangent}_2$ are induced by a common optimal transport plan $\varPlanGeneric$ and a single fixed shift $\boldsymbol{a}$ between $\varTangentCoupling_1\times\delta_{\beta_1}$ and $\varTangentCoupling_2\times\delta_{\beta_2}$.
As these have Dirac $\beta$-marginals, $\varPlanGeneric$ couples the $\beta$-coordinate by $\delta_{(\beta_1,\beta_2)}$ and $\boldsymbol{a}$ has a constant $\beta$-component.
Thus, the $\beta$-component of the arrow of $\boldsymbol{\varTangent}_i$ is a constant $c_i$ $\almostEverywhere{\boldsymbol{\varTangent}_i}$. Since $\wassersteinDistance{\boldsymbol{\varTangent}_i}{\boldsymbol{\varTangent}_i^{\parallel}}{\varTangentCoupling_i\times\delta_{\beta_i}}\leq\sigma$, the $\beta$-arrow $\lambda_i^{\beta}$ of $\boldsymbol{\varTangent}_i^{\parallel}$ obeys $\int_{\epigraphSpace\times\epigraphSpace}(\lambda_i^{\beta}-c_i)^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)\leq\sigma^2$; in particular $\abs{\lambda_i-c_i}\leq\sigma$ and
\begin{equation*}
\int_{\epigraphSpace\times\epigraphSpace}(\lambda_i^{\beta}-\lambda_i)^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)
=\int_{\epigraphSpace\times\epigraphSpace}(\lambda_i^{\beta}-c_i)^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)-(\lambda_i-c_i)^2
\leq\sigma^2 .
\end{equation*}
Hence, since $\int_{\epigraphSpace\times\epigraphSpace}(\lambda_i^{\beta})^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)=\lambda_i^2+\int_{\epigraphSpace\times\epigraphSpace}(\lambda_i^{\beta}-\lambda_i)^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)$, we have $\int_{\epigraphSpace\times\epigraphSpace}(\lambda_i^{\beta})^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)=\lambda_i^2+\rho_i$ with $0\leq\rho_i\leq\sigma^2$. So,
\begin{equation}\label{eq:eps_normal_cone:norm_decomposition}
\norm{\boldsymbol{\varTangent}_i^{\parallel}}_{\varTangentCoupling_i\times\delta_{\beta_i}}^2
=\int_{\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol{w}_i}^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)
+\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_i}^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)
+\lambda_i^2+\rho_i.
\end{equation}

\emph{Fact 2.}
By the structure of $\Lambda_1$,~\cref{proposition:prop_normal_cone_product}\ref{item:product:cylinder} gives $\boldsymbol{w}_1=0$ $\almostEverywhere{\boldsymbol{\varTangent}_1^{\parallel}}$.

\emph{Step 4 (Extraction of the $\Omega$-normal).}
By the structure of $\Lambda_1$,~\cref{proposition:prop_normal_cone_product} (\ref{item:product:delta} for the $\delta_\beta$-factor, \ref{item:product:cylinder} for the free block) we have $\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1^{\parallel}} \in \normalConeRegularStrong{\Omega}{\tilde\varGeneric}$ with $\tilde\varGeneric\coloneqq\pushforward{\projection{3}{}}{\varTangentCoupling_1}$.

\emph{Step 5 (Controlling $\varTangent_\varepsilon$ through $\Lambda_2$).}
We use the normal $\boldsymbol{\varTangent}_2^{\parallel}\in\normalConeRegularStrong{\Lambda_2}{\varTangentCoupling_2\times\delta_{\beta_2}}$ to control $\varTangent_\varepsilon$; its base has $x$-coordinate $x_2$, its arrow has components $(\boldsymbol{w}_2,\varTangentReals_2,\lambda_2^\beta)$, and $\lambda_2=\expectedValue{\boldsymbol{\varTangent}_2^{\parallel}}{\lambda_2^\beta}$.
Its $(\bar x,\varTangentReals_\varepsilon)$-component $\boldsymbol{w}_2$ is small.
Indeed, by~\eqref{eq:eps_normal_cone:cancellation}, the $(\bar x,\varTangentReals_\varepsilon)$-component of the arrow of $\boldsymbol{\varTangent}_2$ equals, in norm along $\varPlanGeneric_{\boldsymbol\varTangent}$, that of $\boldsymbol{\varTangent}_1$, which is within $\sigma$ of $\boldsymbol{w}_1$ (the $(\bar x,\varTangentReals_\varepsilon)$-projection is $1$-Lipschitz and $\wassersteinDistance{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_1^{\parallel}}{}\leq\sigma$); as $\boldsymbol{w}_1=0$ (Fact~2) and $\boldsymbol{\varTangent}_2^{\parallel}$ is likewise within $\sigma$ of $\boldsymbol{\varTangent}_2$, we get $\bigl(\int_{\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol{w}_2}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\bigr)^{1/2}\leq 2\sigma$, i.e., $\int_{\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol{w}_2}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\leq 4\sigma^2$.

Since $\boldsymbol{\varTangent}_2^{\parallel}\in\normalConeRegularStrong{\Lambda_2}{\varTangentCoupling_2\times\delta_{\beta_2}}$, every coupling $\boldsymbol\varTangentCoupling\in\Pp{2}{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}$ with $\pushforward{(\projection{1}{},\projection{2}{})}{\boldsymbol\varTangentCoupling}=\boldsymbol{\varTangent}_2^{\parallel}$ and $\pushforward{(\projection{1}{}+\projection{3}{})}{\boldsymbol\varTangentCoupling}\in\Lambda_2$ satisfies
\begin{equation}\label{eq:eps_subdifferential:regular_cone_lambda_2}
    \int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\boldsymbol{\bar\varTangentReals}}{\boldsymbol\varTangentReals'}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})
    \leq
    \onotation{\left(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol\varTangentReals'}^2\d\boldsymbol\varTangentCoupling(\boldsymbol{q})\right)^{1/2}},
\end{equation}
where $\boldsymbol{q}$ denotes a generic point of $\epigraphSpace\times\epigraphSpace\times\epigraphSpace$: its three blocks are a base point of $\boldsymbol{\varTangent}_2^{\parallel}$, the arrow $\boldsymbol{\bar\varTangentReals}$ that $\boldsymbol{\varTangent}_2^{\parallel}$ attaches to it (that is, $\boldsymbol{\bar\varTangentReals}=\boldsymbol{\zeta}_2$ in the coordinates of Step~3), and a displacement $\boldsymbol{\varTangentReals}'$.
%
We now use~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} for displacements $\boldsymbol\varTangentReals'=(0,0,\varTangentReals',\Delta\beta)$ with $\Delta\beta\in\reals$.
For such $\boldsymbol\varTangentReals'$ the arrow component $\boldsymbol{w}_2$ is paired with the zero displacement on the $(\bar x,\varTangentReals_\varepsilon)$-coordinates and drops out, so the left-hand side of~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} equals $\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_2}{\varTangentReals'}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})+\lambda_2\,\Delta\beta$.
Testing with $\varTangentReals'=0$ and $\Delta\beta\leq 0$ (admissible since lowering $\beta$ preserves membership in $\Lambda_2$) gives $\lambda_2\Delta\beta\leq\onotation{\abs{\Delta\beta}}$ for all $\Delta\beta\leq 0$ and so $\lambda_2\geq 0$.
Moreover, since $\varTangentCoupling_2\times\delta_{\beta_2}\in\Lambda_2$, we have
\begin{equation}\label{eq:proof_eps_normal_cone:beta2_inequality}
    \beta_{2}
    \leq
    \int_{\reals^d\times\reals^d\times\reals^d} \innerProduct{\varTangentReals_\varepsilon}{x_2-\bar x}\d\varTangentCoupling_2(\bar x,\varTangentReals_\varepsilon,x_2)
    -(\varepsilon+\sigma)\sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{x_2-\bar x}^2\d\varTangentCoupling_2(\bar x,\varTangentReals_\varepsilon,x_2)} .
\end{equation}
We distinguish two cases.

\subparagraph{Case (a): $\lambda_2=0$.}
Set $\varTangentCoupling_t'\coloneqq\pushforward{(\projection{\bar{x}}{},\projection{\varTangentReals_{\varepsilon}}{},\projection{x_2}{}+t\projection{\varTangentReals_2}{})}{\boldsymbol{\varTangent}_2^{\parallel}}$, and let
\begin{equation*}
    R(t)
    \coloneqq
    \int_{\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_\varepsilon}{x_2+t\varTangentReals_2-\bar x}\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)
    -(\varepsilon+\sigma)\sqrt{\int_{\epigraphSpace\times\epigraphSpace}\norm{x_2+t\varTangentReals_2-\bar x}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)}.
\end{equation*}
As $R$ has an affine and a square-root term, $R(t)-R(0)=O(t)$.
Set $\beta_t'\coloneqq\beta_2+\bigl(R(t)-R(0)\bigr)$.
Since $\beta_2\leq R(0)$ by~\eqref{eq:proof_eps_normal_cone:beta2_inequality}, we have $\beta_t'\leq R(t)$, so $\varTangentCoupling_t'\times\delta_{\beta_t'}\in\Lambda_2$ for $t\geq 0$. The associated displacement is $(0,0,t\varTangentReals_2,\beta_t'-\beta_2)$ with $\beta_t'-\beta_2=R(t)-R(0)=O(t)$, induced by
\begin{equation*}
\boldsymbol\varTangentCoupling_t'
\coloneqq
\pushforward{\big(
(\projection{\bar x}{},\projection{\varTangentReals_\varepsilon}{},\projection{x_2}{},\beta_2),
(\projection{\boldsymbol{w}_2}{},\projection{\varTangentReals_2}{},\projection{\lambda_2^\beta}{}),
(0,0,\,t\projection{\varTangentReals_2}{},\,\beta_t'-\beta_2)
\big)}{\boldsymbol{\varTangent}_2^{\parallel}},
\end{equation*}
which satisfies $\pushforward{(\projection{1}{},\projection{2}{})}{\boldsymbol\varTangentCoupling_t'}=\boldsymbol{\varTangent}_2^{\parallel}$ and $\pushforward{(\projection{1}{}+\projection{3}{})}{\boldsymbol\varTangentCoupling_t'}=\varTangentCoupling_t'\times\delta_{\beta_t'}\in\Lambda_2$ by construction, so~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} applies to it.
Since $\lambda_2=0$, the left-hand side of~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} equals $t\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_2}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)$ and its right-hand side is $\onotation{t}$.
Dividing by $t>0$ and letting $t\fromAbove0$ gives $\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_2}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)=0$. Then~\eqref{eq:eps_normal_cone:norm_decomposition}, with $\lambda_2=0$, $\rho_2\leq\sigma^2$, and $\int_{\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol{w}_2}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\leq4\sigma^2$, gives $\norm{\boldsymbol{\varTangent}_2^{\parallel}}_{\varTangentCoupling_2\times\delta_{\beta_2}}^2\leq5\sigma^2$.
Since $\boldsymbol{\varTangent}_2^{\parallel}$ is $\sigma$-close to $\boldsymbol{\varTangent}_2$, this gives $\norm{\boldsymbol{\varTangent}_2}_{\varTangentCoupling_2\times\delta_{\beta_2}}\leq(1+\sqrt5)\,\sigma$, contradicting $\norm{\boldsymbol{\varTangent}_2}_{\varTangentCoupling_2\times\delta_{\beta_2}}=1$ for $\sigma$ sufficiently small.
Thus, $\lambda_2>0$.

\subparagraph{Case (b): $\lambda_2>0$.}
Suppose without loss of generality that~\eqref{eq:proof_eps_normal_cone:beta2_inequality} holds with equality.
%
Indeed, if the inequality is strict, choosing the displacement $\varTangentReals'=0$, $\Delta\beta>0$ in~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} yields $\lambda_2\leq 0$ and so a contradiction.
%
For $t\geq 0$ we perturb the $x$-coordinate of $\boldsymbol{\varTangent}_2^{\parallel}$ along the direction $\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon$ by setting $\varTangentCoupling_t\coloneqq\pushforward{(\projection{\bar x}{},\projection{\varTangentReals_\varepsilon}{},\projection{x_2}{}+t(\lambda_2\projection{\varTangentReals_\varepsilon}{}+\projection{\varTangentReals_2}{}))}{\boldsymbol{\varTangent}_2^{\parallel}}$, and define
\begin{align*}
    \beta_t
    &\coloneqq
    \int_{\reals^d\times\reals^d\times\reals^d} \innerProduct{\varTangentReals_\varepsilon}{x-\bar x}\d\varTangentCoupling_t(\bar x,\varTangentReals_\varepsilon,x)
    - (\varepsilon+\sigma)\sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{x-\bar x}^2\d\varTangentCoupling_t(\bar x,\varTangentReals_\varepsilon,x)}
    \\
    &=
    \int_{\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_\varepsilon}{x_2+t(\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon)-\bar x}\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)
    \\
    &\qquad
    -(\varepsilon+\sigma)
    \sqrt{\int_{\epigraphSpace\times\epigraphSpace}\norm{x_2+t(\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon)-\bar x}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)}.
\end{align*}
Since the inequality~\eqref{eq:proof_eps_normal_cone:beta2_inequality} holds with equality, we have $\varTangentCoupling_t\times\delta_{\beta_t}\in\Lambda_2$.
%
The associated displacement is $\boldsymbol\varTangentReals'=\big(0,0,\,t(\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon),\,\beta_t-\beta_2\big)\in\epigraphSpace$, induced by
\begin{equation*}
\boldsymbol\varTangentCoupling_t
\coloneqq
\pushforward{\big(
(\projection{\bar x}{},\projection{\varTangentReals_\varepsilon}{},\projection{x_2}{},\beta_2),
(\projection{\boldsymbol{w}_2}{},\projection{\varTangentReals_2}{},\projection{\lambda_2^\beta}{}),
(0,0,\,t(\lambda_2\projection{\varTangentReals_\varepsilon}{}+\projection{\varTangentReals_2}{}),\,\beta_t-\beta_2)
\big)}{\boldsymbol{\varTangent}_2^{\parallel}}.
\end{equation*}
By construction, $\boldsymbol\varTangentCoupling_t\in\Pp{2}{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}$,  $\pushforward{(\projection{1}{},\projection{2}{})}{\boldsymbol\varTangentCoupling_t}=\boldsymbol{\varTangent}_2^{\parallel}$, and $\pushforward{(\projection{1}{}+\projection{3}{})}{\boldsymbol\varTangentCoupling_t}=\varTangentCoupling_t\times\delta_{\beta_t}\in\Lambda_2$, so~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} applies to it.
We expand $\beta_t$ in $t$ as $\beta_t=I(t)-(\varepsilon+\sigma)N(t)$, where
\begin{align*}
    I(t)&\coloneqq\int_{\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_\varepsilon}{x_2+t(\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon)-\bar x}\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)
    =I(0)+t\int_{\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_\varepsilon}{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2),
    \\
    N(t)&\coloneqq\biggl(\int_{\epigraphSpace\times\epigraphSpace}\norm{x_2+t(\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon)-\bar x}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\biggr)^{1/2}.
\end{align*}
The map $I$ is affine in $t$.
The map $w\mapsto\bigl(\int_{\epigraphSpace\times\epigraphSpace}\norm{w}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\bigr)^{1/2}$ is a seminorm, so its triangle inequality applied to the splitting $x_2+t(\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon)-\bar x=(x_2-\bar x)+t(\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon)$ gives, for $t\geq0$,
\begin{equation*}
    N(t)\leq N(0)+t\biggl(\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\biggr)^{1/2}.
\end{equation*}
As~\eqref{eq:proof_eps_normal_cone:beta2_inequality} holds with equality, $\beta_2=I(0)-(\varepsilon+\sigma)N(0)$, so $\beta_t-\beta_2=\bigl(I(t)-I(0)\bigr)-(\varepsilon+\sigma)\bigl(N(t)-N(0)\bigr)$. Substituting and multiplying by $\lambda_2\geq0$,
\begin{equation}
\begin{aligned}
    \lambda_2(\beta_t-\beta_2)
    &\geq
    \lambda_2 t
    \int_{\epigraphSpace\times\epigraphSpace}
    \innerProduct{\varTangentReals_\varepsilon}{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)
    \\
    &\qquad\qquad\qquad
    -\lambda_2 t (\varepsilon+\sigma)\biggl(\int_{\epigraphSpace\times\epigraphSpace} \norm{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\biggr)^{1/2}.
    \label{eq:eps_normal_cone:beta_t_lower}
\end{aligned}
\end{equation}
Moreover, $\abs{\beta_t-\beta_2}=O(t)$, since $I$ is affine and $N$ Lipschitz in $t$.
%
Hence,
\begin{equation}\label{eq:eps_normal_cone:beta_t_bound}
    \int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol\varTangentReals'}^2\d\boldsymbol\varTangentCoupling_t(\boldsymbol{q})
    =
    t^2\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)
    +\abs{\beta_t-\beta_2}^2
    =
    O(t^2).
\end{equation}
The inner product in~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} is
\begin{equation}\label{eq:eps_normal_cone:inner_t}
    \int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_2}{t(\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon)}\d\boldsymbol\varTangentCoupling_t(\boldsymbol{q})
    =
    t\int_{\epigraphSpace\times\epigraphSpace} \innerProduct{\varTangentReals_2}{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2).
\end{equation}
By~\eqref{eq:eps_normal_cone:inner_t} and~\eqref{eq:eps_normal_cone:beta_t_lower}, the left-hand side of~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} is bounded below by $t\,Q$, where
\begin{equation}\label{eq:eps_normal_cone:Q_def}
\begin{aligned}
    Q
    &\coloneqq
    \int_{\epigraphSpace\times\epigraphSpace} \innerProduct{\varTangentReals_2}{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)
    +\lambda_2\int_{\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_\varepsilon}{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)
    \\
    &-\lambda_2 (\varepsilon+\sigma)\sqrt{\int_{\epigraphSpace\times\epigraphSpace} \norm{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)}
    \\
    &=
    \int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)
    -\lambda_2 (\varepsilon+\sigma)\sqrt{\int_{\epigraphSpace\times\epigraphSpace} \norm{\varTangentReals_2+\lambda_2\varTangentReals_\varepsilon}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)}.
\end{aligned}
\end{equation}
The right-hand side of~\eqref{eq:eps_subdifferential:regular_cone_lambda_2} is $\onotation{\left(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol\varTangentReals'}^2\d\boldsymbol\varTangentCoupling_t(\boldsymbol{q})\right)^{1/2}}=\onotation{t}$ by~\eqref{eq:eps_normal_cone:beta_t_bound}. Hence, $t\,Q\leq\onotation{t}$.
We divide by $t>0$ and let $t\fromAbove0$ to get $Q\leq0$ or equivalently
\begin{equation}\label{eq:eps_normal_cone:v2_over_lambda_close}
    \sqrt{\int_{\epigraphSpace\times\epigraphSpace} \norm{\tfrac{\varTangentReals_2}{\lambda_2}+\varTangentReals_\varepsilon}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)}
    \leq
    \varepsilon+\sigma.
\end{equation}
Thus, $\hat\varTangent_2\coloneqq-\tfrac{1}{\lambda_2}\pushforward{(\projection{\bar x}{},\projection{\varTangentReals_2}{})}{\boldsymbol{\varTangent}_2^{\parallel}}$ satisfies $\wassersteinDistance{\varTangent_\varepsilon}{\hat\varTangent_2}{\varFixed}\leq\varepsilon+\sigma$.

\emph{Step 6 (Lower bound on $\lambda_2$).}
It remains to transfer the bound from $\hat\varTangent_2$ to $\varTangent\coloneqq\tfrac1{\lambda_2}\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1^{\parallel}}$, which requires a lower bound on $\lambda_2$.
By~\eqref{eq:eps_normal_cone:norm_decomposition}, $\rho_2\leq\sigma^2$ (Fact~1), and $\int_{\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol{w}_2}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\leq4\sigma^2$ (Step~5),
$
    \norm{\boldsymbol{\varTangent}_2^{\parallel}}_{\varTangentCoupling_2\times\delta_{\beta_2}}^2\leq\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_2}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)+\lambda_2^2+5\sigma^2,
$
while $\norm{\boldsymbol{\varTangent}_2^{\parallel}}_{\varTangentCoupling_2\times\delta_{\beta_2}}\geq\norm{\boldsymbol{\varTangent}_2}_{\varTangentCoupling_2\times\delta_{\beta_2}}-\sigma=1-\sigma$. Moreover, applying triangle inequality to~\eqref{eq:eps_normal_cone:v2_over_lambda_close}, and $\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_\varepsilon}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)=\norm{\varTangent_\varepsilon}_{\varFixed}^2$ gives
\begin{equation*}
    \biggl(\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_2}^2\d\boldsymbol{\varTangent}_2^{\parallel}(\boldsymbol{\zeta}_2)\biggr)^{1/2}\leq\lambda_2\bigl(\norm{\varTangent_\varepsilon}_{\varFixed}+\varepsilon+\sigma\bigr).
\end{equation*}
Overall, $(1-\sigma)^2\leq\lambda_2^2\bigl(\norm{\varTangent_\varepsilon}_{\varFixed}+\varepsilon+\sigma\bigr)^2+\lambda_2^2+5\sigma^2$, so $\lambda_2\geq c\,\sqrt{(1-\sigma)^2-5\sigma^2}$ with $c\coloneqq\bigl(1+(\norm{\varTangent_\varepsilon}_{\varFixed}+\varepsilon+\sigma)^2\bigr)^{-1/2}$.
In particular, for $\sigma\leq\tfrac14$ (so that $(1-\sigma)^2-5\sigma^2\geq\tfrac14$) we have $\lambda_2\geq c/2>0$, so $\lambda_2$ is bounded away from $0$ and $\tfrac1{\lambda_2}\leq\tfrac2c$.

\emph{Step 7 (Closeness of $\varTangent$ to $\varTangent_\varepsilon$).}
Recall $\varTangent\coloneqq\tfrac{1}{\lambda_2}\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1^{\parallel}}$.
Since $\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1^{\parallel}}\in\normalConeRegularStrong{\Omega}{\tilde\varGeneric}$ (Step~4), the regular normal cone is a cone, and $\lambda_2>0$, we have $\varTangent\in\normalConeRegularStrong{\Omega}{\tilde\varGeneric}$.
As $\varTangent$ is based at $\tilde\varGeneric$ while $\hat\varTangent_2$ and $\varTangent_\varepsilon$ are based at $\varFixed$, the triangle inequality gives $\wassersteinDistance{\varTangent}{\varTangent_\varepsilon}{2}\leq\wassersteinDistance{\varTangent}{\hat\varTangent_2}{2}+\wassersteinDistance{\hat\varTangent_2}{\varTangent_\varepsilon}{2}$.
Since $\wassersteinDistance{\hat\varTangent_2}{\varTangent_\varepsilon}{\varFixed}\leq\varepsilon+\sigma$ by~\eqref{eq:eps_normal_cone:v2_over_lambda_close}, it remains to bound $\wassersteinDistance{\varTangent}{\hat\varTangent_2}{2}$.

Glue the transport plan $\varPlanGeneric_{\boldsymbol\varTangent}$ with the two transport plans realizing the $\sigma$-closeness of $\boldsymbol{\varTangent}_i$ to $\boldsymbol{\varTangent}_i^{\parallel}$, along their shared $\boldsymbol{\varTangent}_1$- and $\boldsymbol{\varTangent}_2$-marginals.
This yields a transport plan $\theta\in\Pp{2}{\mathbb{S}}$, $\mathbb{S}\coloneqq(\epigraphSpace\times\epigraphSpace)^4$, that carries $\boldsymbol{\varTangent}_1^{\parallel},\boldsymbol{\varTangent}_1,\boldsymbol{\varTangent}_2,\boldsymbol{\varTangent}_2^{\parallel}$.
{We write a generic point of $\mathbb{S}$ as
$(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})$:
each entry is a pair (base point, arrow) in
$\epigraphSpace\times\epigraphSpace$, and under $\theta$ the four pairs have
laws $\boldsymbol{\varTangent}_1^{\parallel}$, $\boldsymbol{\varTangent}_1$,
$\boldsymbol{\varTangent}_2$, and $\boldsymbol{\varTangent}_2^{\parallel}$,
respectively. Since the $\sigma$-closeness of $\boldsymbol{\varTangent}_i$ to
$\boldsymbol{\varTangent}_i^{\parallel}$ is measured in the Wasserstein
distance at their common base $\varTangentCoupling_i\times\delta_{\beta_i}$,
which couples variations with a common base point, $\boldsymbol{q}_i$ and
$\boldsymbol{q}_i^{\parallel}$ share their base $\almostEverywhere{\theta}$. The
integrands below use only some components of these pairs, in the coordinates
of Step~1 for the bases and of Step~3 for the arrows: $x_1$ is the
$x$-coordinate (the moved point) of the common base of
$\boldsymbol{q}_1^{\parallel}$ and $\boldsymbol{q}_1$, whereas $\bar x_2$ and
$x_2$ are the $\bar x$- and $x$-coordinates of the common base of
$\boldsymbol{q}_2$ and $\boldsymbol{q}_2^{\parallel}$; finally,
$\varTangentReals_i$ and $\varTangentReals_i^{\parallel}$ are the
$x$-components of the arrows of $\boldsymbol{q}_i$ and
$\boldsymbol{q}_i^{\parallel}$, respectively.}
Under $\theta$, $\varTangent$ has base point $x_1\sim\tilde\varGeneric$ and arrow $\tfrac1{\lambda_2}\varTangentReals_1^{\parallel}$, whereas $\hat\varTangent_2=-\tfrac1{\lambda_2}\pushforward{(\projection{\bar x}{},\projection{\varTangentReals_2}{})}{\boldsymbol{\varTangent}_2^{\parallel}}$ has base point $\bar x_2\sim\varFixed$ and arrow $-\tfrac1{\lambda_2}\varTangentReals_2^{\parallel}$.
Therefore, $\theta$ induces a coupling of $\varTangent$ and $\hat\varTangent_2$ and so
\begin{equation*}
    \wassersteinDistance{\varTangent}{\hat\varTangent_2}{2}^2
    \leq
    \int_{\mathbb{S}}\norm{x_1-\bar x_2}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})
    +\tfrac1{\lambda_2^2}\int_{\mathbb{S}}\norm{\varTangentReals_1^{\parallel}+\varTangentReals_2^{\parallel}}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel}) .
\end{equation*}
We bound the two integrals separately. For the arrows, the triangle inequality in $\Lp{2}{\mathbb{S}}{\theta}$ together with $\varTangentReals_1=-\varTangentReals_2$ (see~\eqref{eq:eps_normal_cone:cancellation}) gives
\begin{align*}
    \Bigl(\int_{\mathbb{S}}\norm{\varTangentReals_1^{\parallel}+\varTangentReals_2^{\parallel}}^2&\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})\Bigr)^{1/2}
    \\
    &\leq
    \Bigl(\int_{\mathbb{S}}\norm{\varTangentReals_1^{\parallel}-\varTangentReals_1}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})\Bigr)^{1/2}
    \\
    &+\Bigl(\int_{\mathbb{S}}\norm{\varTangentReals_1+\varTangentReals_2}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})\Bigr)^{1/2}
    \\
    &+\Bigl(\int_{\mathbb{S}}\norm{\varTangentReals_2-\varTangentReals_2^{\parallel}}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})\Bigr)^{1/2}
    \leq2\sigma,
\end{align*}
where the first and third terms are each at most $\sigma$ by the $\sigma$-closeness of $\boldsymbol{\varTangent}_i$ to $\boldsymbol{\varTangent}_i^{\parallel}$ and the middle one vanishes. For the base points, the triangle inequality gives
\begin{align*}
    \Bigl(\int_{\mathbb{S}}\norm{x_1-\bar x_2}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})\Bigr)^{1/2}
    &\leq
    \Bigl(\int_{\mathbb{S}}\norm{x_1-x_2}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})\Bigr)^{1/2}
    \\&+
    \Bigl(\int_{\mathbb{S}}\norm{x_2-\bar x_2}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})\Bigr)^{1/2},
\end{align*}
where $x_2$ is the moved point of $\varTangentCoupling_2$. The first term is at most $2\sigma$, as, under $\theta$, $x_1$ and $x_2$ are coupled by the optimal transport plan between $\varTangentCoupling_1\times\delta_{\beta_1}$ and $\varTangentCoupling_2\times\delta_{\beta_2}$, and these two points are each within $\sigma$ of $\bar\varTangentCoupling\times\delta_0$ by~\eqref{eq:eps_normal_cone:close_points}.
The second term equals $\bigl(\int_{\reals^d\times\reals^d\times\reals^d}\norm{x_2-\bar x}^2\d\varTangentCoupling_2(\bar x,\varTangentReals_\varepsilon,x_2)\bigr)^{1/2}\leq\sqrt2\,\sigma$, since $(\bar x,\varTangentReals_\varepsilon,x_2)\mapsto x_2-\bar x$ is $\sqrt2$-Lipschitz, $x_2=\bar x$ $\almostEverywhere{\bar\varTangentCoupling}$, and $\wassersteinDistance{\bar\varTangentCoupling}{\varTangentCoupling_2}{2}<\sigma$ by~\eqref{eq:eps_normal_cone:close_points}. Hence $\bigl(\int_{\mathbb{S}}\norm{x_1-\bar x_2}^2\d\theta(\boldsymbol{q}_1^{\parallel},\boldsymbol{q}_1,\boldsymbol{q}_2,\boldsymbol{q}_2^{\parallel})\bigr)^{1/2}\leq(2+\sqrt2)\,\sigma$.
Combining the two bounds and using $\lambda_2\geq c/2$ (Step~6) gives
\begin{equation*}
    \wassersteinDistance{\varTangent}{\hat\varTangent_2}{2}
    \leq
    (2+\sqrt2)\,\sigma+\frac{2\sigma}{\lambda_2}
    \leq
    \Bigl(2+\sqrt2+\tfrac4c\Bigr)\sigma.
\end{equation*}
Overall, $\wassersteinDistance{\varTangent}{\varTangent_\varepsilon}{2}\leq(\varepsilon+\sigma)+\bigl(2+\sqrt2+\tfrac4c\bigr)\sigma=\varepsilon+C\sigma$ with $C\coloneqq3+\sqrt2+\tfrac4c$.

\emph{Step 8 (Conclusion).}
Since $\projection{3}{}$ is $1$-Lipschitz and $\pushforward{\projection{3}{}}{\bar\varTangentCoupling}=\varFixed$, \eqref{eq:eps_normal_cone:close_points} gives $\wassersteinDistance{\varFixed}{\tilde\varGeneric}{2}\leq\wassersteinDistance{\bar\varTangentCoupling}{\varTangentCoupling_1}{2}<\sigma$. We have thus produced, at the accuracy $\sigma$, $\tilde\varGeneric\in\Omega$ and $\varTangent\in\normalConeRegularStrong{\Omega}{\tilde\varGeneric}$ with $\wassersteinDistance{\varFixed}{\tilde\varGeneric}{2}<\sigma$ and $\wassersteinDistance{\varTangent}{\varTangent_\varepsilon}{2}\leq\varepsilon+C\sigma$. For $\sigma\leq\tfrac14$ we have $c\geq c_0\coloneqq\bigl(1+(\norm{\varTangent_\varepsilon}_{\varFixed}+\varepsilon+\tfrac14)^2\bigr)^{-1/2}$, hence $C\leq C_0\coloneqq3+\sqrt2+4/c_0$; the constant $C_0$ is larger than $1$ and depends only on $\norm{\varTangent_\varepsilon}_{\varFixed}$ and $\varepsilon$. Given the target $\sigma>0$ of the statement, running the construction at accuracy $s\coloneqq\min\{\sigma/C_0,\tfrac14\}\leq\tfrac14$ in place of $\sigma$ then yields $\wassersteinDistance{\varFixed}{\tilde\varGeneric}{2}<s\leq\sigma$ and $\wassersteinDistance{\varTangent}{\varTangent_\varepsilon}{2}\leq\varepsilon+C_0 s\leq\varepsilon+\sigma$, which proves the lemma.


==> elements/eps_to_exact_normal_title.tex <==
From approximate to exact regular normals%


==> elements/ex_functional_expected_value_body.tex <==
Consider the same functional $\objective$ as in \cref{sec:introduction}, namely $\objective(\varGeneric) \coloneqq\expectedValue{x \sim \varGeneric}{\innerProduct{\theta}{x}}$ and $V(x) \coloneqq \innerProduct{\theta}{x}$ in \cref{proposition:prop_functional_expected_value}. Since $V$ is a linear function, it satisfies all the assumptions of \cref{proposition:prop_functional_expected_value}, and in particular $\objective$ is differentiable with $\gradient{}{\objective}(\varGeneric) \localEquiv{\varGeneric} \pushforward{(\identity{}, \theta)}{\varGeneric}$; moreover, its subdifferential is the singleton $\subgradient{\objective}(\varGeneric) = \{\gradient{}{\objective}(\varGeneric)\}$.

==> elements/ex_functional_expected_value_title.tex <==
Expected values of linear functions%

==> elements/ex_functional_interaction_body.tex <==
Consider $U(z) = \frac{1}{2}\innerProduct{Qz}{z}$ for symmetric\footnote{Otherwise, the term $\frac{1}{2}(Q + Q^\top)$ appears in the expression of the subgradient.} $Q \in \reals^{d\times d}$. Then, $U$ is twice continuously differentiable with $\gradient{}{U}(z) = Qz$ and constant (and, thus, bounded) Hessian $Q$. In virtue of \cref{proposition:prop_functional_interaction}, the functional $\objective(\varGeneric) = \frac{1}{2}\expectedValue{(x, y) \sim \varGeneric\times\varGeneric}{U(x - y)}$ is differentiable with
$
\gradient{}{\objective}(\varGeneric) \localEquiv{\varGeneric}
\pushforward{(\identity{}, Q(\identity{} - \expectedValue{x \sim \varGeneric}{x}))}{\varGeneric}.
$

==> elements/ex_functional_interaction_title.tex <==
Quadratic interaction energies%

==> elements/ex_functional_optimal_transport_body.tex <==
Consider $c(x,y)=h(x-y)$ for $h:\reals^d\to\nonnegativeReals$ strictly convex and twice continuously differentiable with bounded Hessian, with $h(0)=0$ and $\gradient{}h(0)=0$ (so that $c\geq0$). Then $\gradient{x}{c}(x,y)=\gradient{}h(x-y)$ and, by strict convexity of $h$, $y\mapsto\gradient{x}{c}(x,y)$ is injective. Thus, $c$ satisfies the assumptions of \cref{proposition:prop_functional_optimal_transport} and the subgradient of
$
\objective(\varGeneric)
\coloneqq
\wassersteinDistance{\varGeneric}{\varReference}{c}
$
at $\varFixed$ is
$
\emptyset\neq
\subgradient{\objective}(\varFixed)
\localSubseteq{\varFixed}
\pushforward{(\projection{1}{}, \comp{(\projection{1}{}-\projection{2}{})}{\gradient{}h})}{\setPlansOptimalCost{\varFixed}{\varReference}{c}}
$.
Moreover, $\objective$ is differentiable whenever $\setPlansOptimalCost{\varFixed}{\varReference}{c}$ is a singleton and induced by an optimal transport map and, in particular, at all absolutely continuous measures.


==> elements/ex_functional_optimal_transport_title.tex <==
Strictly convex transportation cost%

==> elements/ex_non_subdifferentiability_regular_wasserstein_singletonplans_body.tex <==
Let \textcolor{ETHblue}{$\varFixed \coloneqq \delta_{(0,0)}$} (\textcolor{ETHblue}{blue} in the picture) and \textcolor{ETHred}{$\varReference \coloneqq \frac{1}{2}\delta_{(-1, 0)} + \frac{1}{2}\delta_{(1, 0)}$} (\textcolor{ETHred}{red} in the picture).
Applying the definition of Wasserstein distance (cf. \eqref{definition:wasserstein-distance}), $\objective(\textcolor{ETHblue}{\varFixed})\coloneqq\frac{1}{2}\wassersteinDistance{\textcolor{ETHblue}{\varFixed}}{\textcolor{ETHred}{\varReference}}{2}^2 = \frac{1}{2}$, and there is a unique optimal transport plan between $\varFixed$ and $\varReference$; in particular, $\setPlansOptimal{\textcolor{ETHblue}{\varFixed}}{\textcolor{ETHred}{\varReference}} = \{\textcolor{ETHblue}{\varFixed}\times\textcolor{ETHred}{\varReference}\}$.
We now show that $\objective(\varGeneric) = \frac{1}{2}\wassersteinDistance{\varGeneric}{\textcolor{ETHred}{\varReference}}{2}^2$ is not regularly subdifferentiable at $\textcolor{ETHblue}{\varFixed}$.
By \cref{proposition:prop_wassersteindistance_regular_subgradient_must_be_plan}\ref{item:prop_wassersteindistance_regular_subgradient_must_be_plan:regular_necessary}, it suffices to prove that
$$\varTangent \coloneqq \pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{(\textcolor{ETHblue}{\varFixed}\times\textcolor{ETHred}{\varReference})} = \frac{1}{2}\delta_{((0,0),(-1,0))} + \frac{1}{2}\delta_{((0,0),(1,0))}$$
is not a regular subgradient of $\objective$.

\vspace{0.5\baselineskip}

\begin{center}
\begin{minipage}{.69\textwidth}
Consider $\textcolor{ETHgreen}{\varGeneric_n\coloneqq\frac{1}{2}\delta_{(-\frac{1}{n},-\frac{1}{n})}+\frac{1}{2}\delta_{(\frac{1}{n},\frac{1}{n})}}$. Then, there is a unique optimal transport plan
$\setPlansOptimal{\textcolor{ETHblue}{\varFixed}}{\textcolor{ETHgreen}{\varGeneric_n}} = \{\textcolor{ETHblue}{\varFixed}\times\textcolor{ETHgreen}{\varGeneric_n}\}$, and
$\objective(\textcolor{ETHgreen}{\varGeneric_n})=\frac{1}{2}\wassersteinDistance{\textcolor{ETHgreen}{\varGeneric_n}}{\textcolor{ETHred}{\varReference}}{2}^2=\frac{1}{2}((1-\frac{1}{n})^2+\frac{1}{n^2})=\frac{1}{2}-\frac{1}{n}+\frac{1}{n^2}$,
and
$\wassersteinDistance{\textcolor{ETHblue}{\varFixed}}{\textcolor{ETHgreen}{\varGeneric_n}}{2}=(\frac{1}{n^2}+\frac{1}{n^2})^{1/2}=\frac{\sqrt{2}}{n}$.
We now show that such a sequence contradicts \cref{definition:def_sub_sup_differentiability}\ref{item:subgradient:regular} by proving that, along this ``direction'', $\varTangent$ does not lower bound $\objective$. For this, we consider the variations $\varTangent_n \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\textcolor{ETHblue}{\varFixed}}{\textcolor{ETHgreen}{\varGeneric_n}}}$. Using the expressions of $\textcolor{ETHblue}{\varFixed}$ and $\textcolor{ETHgreen}{\varGeneric_n}$, we conclude that the only variation between $\varFixed$ and $\varGeneric_n$ is
\end{minipage}
\begin{minipage}{.3\textwidth}
\centering
\includegraphics[width=.9\linewidth]{figures/fig_subgradients/regular_wass_discrete.pdf}
\end{minipage}
\end{center}

$$\varTangent_n\coloneqq\pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{(\textcolor{ETHblue}{\varFixed}\times\textcolor{ETHgreen}{\varGeneric_n})} = \frac{1}{2}\delta_{((0,0),(-\frac{1}{n}, -\frac{1}{n}))} + \frac{1}{2}\delta_{((0,0),(\frac{1}{n}, \frac{1}{n}))}.$$
With this, we compute the inner product between $\varTangent$ and $\varTangent_n$:
$$
{\innerProduct{\varTangent}{\varTangent_n}_{\varFixed}
    =
    \max_{\varTangentCoupling \in \setPlansCommonMarginal{\varTangent}{\varTangent_n}{1}}
    \int_{\reals^2\times\reals^2\times\reals^2} \innerProduct{\varTangentReals}{\varTangentReals_n} \d\varTangentCoupling(x, \varTangentReals, \varTangentReals_n).}
$$
The coupling $\varTangentCoupling$ is fully parametrized by a single coefficient $\tau \in [0,1]$, and the max reduces to a line search:
    \begin{align*}
    \innerProduct{\varTangent}{\varTangent_n}_{\varFixed}
    =
    \max_{\tau \in [0, 1]} \frac{\tau}{2}&\left(\innerProduct{(1, 0)}{\left(\frac{1}{n}, \frac{1}{n}\right)} + \innerProduct{(-1, 0)}{\left(-\frac{1}{n},-\frac{1}{n}\right)}\right)
    \\&{+ \frac{(1 - \tau)}{2}\left(\innerProduct{(1, 0)}{\left(-\frac{1}{n}, -\frac{1}{n}\right)} + \innerProduct{(-1, 0)}{\left(\frac{1}{n}, \frac{1}{n}\right)}\right)
    =
    \frac{1}{n}.}
    \end{align*}
Thus,
$$
    {\liminf_{n\to\infty}
    \frac{\objective(\textcolor{ETHgreen}{\varGeneric_n}) - \objective(\textcolor{ETHblue}{\varFixed})-\innerProduct{\varTangent}{\varTangent_n}_{\varFixed}}{\wassersteinDistance{\varFixed}{\textcolor{ETHgreen}{\varGeneric_n}}{2}}
    =
    \liminf_{n\to\infty}
    \frac{-\frac{2}{n}+\frac{1}{n^2}}{\frac{\sqrt{2}}{n}}
    =
    -\sqrt{2}
    <
    0}
$$
and so $\objective(\textcolor{ETHgreen}{\varGeneric_n}) - \objective(\textcolor{ETHblue}{\varFixed}) < \innerProduct{\varTangent}{\varTangent_n}_{\varFixed} + \onotation{\wassersteinDistance{\textcolor{ETHblue}{\varFixed}}{\textcolor{ETHgreen}{\varGeneric_n}}{2}}$.
That is, $\objective$ is not regularly subdifferentiable at $\varFixed$
and, in particular, uniqueness of the optimal transport plan does not imply regular subdifferentiability.


==> elements/ex_non_subdifferentiability_regular_wasserstein_singletonplans_title.tex <==
Non regular-subdifferentiability of the squared Wasserstein distance%

==> elements/ex_subdifferentiability_via_gaussians_wasserstein_body.tex <==
Let $\objective: \Pp{2}{\reals^d} \to \realsBar$, $\objective(\varGeneric) \coloneqq \frac{1}{2}\wassersteinDistance{\varGeneric}{\varReference}{2}^2$ and fix
$
\varFixed
=
\delta_{0}
$ and
$
\varReference
=
\gaussian{0}{\eye{d}}
$ being the Gaussian centered in $0$ with covariance matrix $\eye{d}$, the identity matrix in $\reals^{d\times d}$.
In this case, there is a unique transport plan $\varFixed\times\varReference$ from $\varFixed$ to $\varReference$, but it is not induced by a transport map (indeed, the mass at 0 needs to be split, see the picture below for an intuition).
Here, we show that $\varTangent \coloneqq \pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{(\varFixed\times\varReference)}$ belongs to the general subgradient $\subgradient{\objective}(\varFixed)$.
To do so, we approximate $\delta_0$ with Gaussians with vanishing variance.
Specifically, consider the sequence $\varGeneric_n = \gaussian{0}{\frac{1}{n^2}\eye{d}}$ so that $\wassersteinDistance{\varFixed}{\varGeneric_n}{2} = \frac{\sqrt{d}}{n} \fromAbove 0$ and $\varGeneric_n\convergenceWasserstein\varFixed$ and $\objective(\varGeneric_n)\to\objective(\varFixed)$.
Since both $\varReference$ and $\varGeneric_n$ are Gaussians, the set of optimal transport plans is a singleton $\setPlansOptimal{\varGeneric_n}{\varReference} = \{\pushforward{(\identity{}, T_n)}{\varGeneric_n}\}$, and the unique optimal transport plan is induced by the optimal transport map $T_n(x) = nx$.
By~\cref{proposition:prop_wassersteindistance_regular_subgradient_must_be_plan}, $\objective$ is differentiable at $\varGeneric_n$ and, in particular,
$
\varTangent_n \coloneqq \pushforward{(\identity{}, \identity{} - T_n)}{\varGeneric_n} \in \subgradientRegular{\objective}(\varGeneric_n).
$
{
We now show that $\varTangent_n \convergenceWasserstein \varTangent$ and so $\varTangent$ is a (general) subgradient of $\objective$ at $\varFixed$. For this, we observe that
$\varPlanGeneric_{\varTangent}=\pushforward{(\projection{1}{},\projection{1}{}-\comp{\projection{2}{}}{T_n},\projection{2}{},\projection{2}{}-\comp{\projection{2}{}}{T_n})}{(\varFixed\times\varGeneric_n)}$ is a (possibly suboptimal) transport plan between $\varTangent$ and $\varTangent_n$.
Indeed, using $\varFixed\times\varReference=\varFixed\times(\pushforward{T_n}{\varGeneric_n})=\pushforward{(\projection{1}{},\comp{\projection{2}{}}{T_n})}{(\varFixed\times\varGeneric_n)}$, we can compute the first marginal as $
\pushforward{(\projection{1}{},\projection{2}{})}{\varPlanGeneric_{\varTangent}}
=
\pushforward{(\projection{1}{},\projection{1}{}-\comp{\projection{2}{}}{T_n})}{(\varFixed\times\varGeneric_n)}=\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{
\pushforward{(\projection{1}{},\comp{\projection{2}{}}{T_n})}{(\varFixed\times\varGeneric_n)}
}=\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{(\varFixed\times\varReference)}=\varTangent$ and the second marginal as
$
\pushforward{(\projection{3}{},\projection{4}{})}{\varPlanGeneric_{\varTangent}}
=
\pushforward{(\projection{2}{},\projection{2}{}-\comp{\projection{2}{}}{T_n})}{(\varFixed\times\varGeneric_n)}
=
\pushforward{(\identity{},\identity{}-T_n)}{(\pushforward{\projection{2}{}}{(\varFixed\times\varGeneric_n)})}
=
\pushforward{(\identity{},\identity{}-T_n)}{\varGeneric_n}
=
\varTangent_n
$.
Given this transport plan, we can bound the Wasserstein distance between $\varTangent$ and $\varTangent_n$ as
\vspace{-\baselineskip}
\begin{center}
\begin{minipage}{.75\textwidth}
\begin{align*}
\wassersteinDistance{\varTangent}{\varTangent_n}{2}^2
&\leq
\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d}
\norm{x_1-x_2}^2
\\
&\qquad
+\norm{\varTangentReals_1-\varTangentReals_2}^2\d\varPlanGeneric_{\varTangent}(x_1,\varTangentReals_1,x_2,\varTangentReals_2)
\\
&=
\int_{\reals^d\times\reals^d}
\norm{\bar x-x_n}^2
\\
&\qquad
+\norm{(\bar x-T_n(x_n))-(x_n-T_n(x_n))}^2\d(\varFixed\times\varGeneric_n)(\bar x,x_n)
\\
&=
2\int_{\reals^d}\norm{x_n}^2\d\varGeneric_n(x_n)
\\
&=\frac{2d}{n^2},
\end{align*}
\end{minipage}
\hfill
\begin{minipage}{.24\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/fig_geometry/gauss.pdf}
\end{minipage}
\end{center}
where we used that $\varFixed=\delta_0$ and so $\bar x=0$ for $\varFixed$-almost all $\bar x$.
This implies that $\wassersteinDistance{\varTangent}{\varTangent_n}{2}\fromAbove 0$ and so $\varTangent_n\convergenceWasserstein\varTangent$. Thus, $\varTangent\in\subgradient{\objective}(\varFixed)$ and the squared Wasserstein distance is subdifferentiable at $\varFixed$.
}


==> elements/ex_subdifferentiability_via_gaussians_wasserstein_title.tex <==
Subgradients via Gaussian mollification%

==> elements/fuzzy-intersection_body.tex <==
    Let $\Omega_1, \Omega_2 \subseteq \Pp{2}{\reals^d}$ be arbitrary sets locally closed around $\varFixed \in \Omega_1 \cap \Omega_2$, and let $\varTangentFixed \in \normalConeRegularStrong{\Omega_1\cap\Omega_2}{\varFixed}$.
    Then for any $\varepsilon > 0$ there are $\lambda \geq 0$, $\varGeneric_i \in \Omega_i \cap \wassersteinBall{\varFixed}{\varepsilon}{2}$, $\varGeneric_2' \in \Omega_2\cap\wassersteinBall{\varFixed}{2\varepsilon}{2}$, variations $\varTangent_1\in\PpLocal{2}{\reals^d\times\reals^d}{\varGeneric_1}$ and $\varTangent_2\in\PpLocal{2}{\reals^d\times\reals^d}{\varGeneric_2}$ that are $\varepsilon$-close with respect to $\wassersteinDistance{}{}{2}$ to $\normalConeRegularStrong{\Omega_1}{\varGeneric_1}$ and $\normalConeRegularStrong{\Omega_2}{\varGeneric_2'}$ respectively, and $\varPlanGeneric \in \setPlans{\varTangentFixed}{\varTangent_1, \varTangent_2}$ so that
    $\int_{(\reals^d\times\reals^d)^3}\norm{\bar{x}-x_1}^2\d\varPlanGeneric(\bar{x}, \bar{\varTangentReals}, x_1, \varTangentReals_1, x_2, \varTangentReals_2)\leq\varepsilon^2$,
    $\int_{(\reals^d\times\reals^d)^3}\norm{\bar{x}-x_2}^2\d\varPlanGeneric(\bar{x}, \bar{\varTangentReals}, x_1, \varTangentReals_1, x_2, \varTangentReals_2)\leq\varepsilon^2$,
    and
    \begin{equation}
    \label{eq:lemma-fuzzy:the-statement}
    \int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
    \norm{\lambda \bar{\varTangentReals} - (\varTangentReals_1 + \varTangentReals_2)}^2
    \d\varPlanGeneric(\bar{x}, \bar{\varTangentReals}, x_1, \varTangentReals_1, x_2, \varTangentReals_2)
    =
    0.
    \end{equation}
    Moreover,
    \begin{equation}
    \label{eq:lemma-fuzzy:nontriviality}
        \max\{\lambda,\norm{\varTangent_1}_{\varGeneric_1}\}=1 .
    \end{equation}


==> elements/fuzzy-intersection_proof.tex <==
We divide the proof into steps.
%
We mirror the proof of~\cref{lemma:eps_to_exact_normal}, applying the extremal principle in  $\epigraphSpace=\reals^d\times\reals^d\times\reals^d\times\reals$.

\emph{Step 1 (Epigraphical lift).}
As in~\cref{lemma:eps_to_exact_normal}, we read the coordinates $(\bar x,\bar\varTangentReals,x,\beta)$ of $\epigraphSpace$ as a base point $\bar x$, the value $\bar\varTangentReals$ of the candidate normal $\varTangentFixed$ at $\bar x$, a moved point $x$, and an epigraphical variable $\beta$. For $\varTangentCoupling\in\Pp{2}{\reals^d\times\reals^d\times\reals^d}$ we define
\begin{align*}
    \Lambda_1
    &\coloneqq\Bigl\{\varTangentCoupling\times\delta_\beta\in\Pp{2}{\reals^d\times\reals^d\times\reals^d\times\reals}
    \st
    \pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega_1,\;\beta\geq 0\Bigr\},
    \\
    \Lambda_2
    &\coloneqq\Bigl\{
    \varTangentCoupling\times\delta_\beta\in\Pp{2}{\reals^d\times\reals^d\times\reals^d\times\reals}
    \st
    \pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling}=\varTangentFixed,\;
    \pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega_2,
    \\
    &\qquad\qquad
    \beta\leq\int_{\reals^d\times\reals^d\times\reals^d}\innerProduct{\bar\varTangentReals}{x-\bar x}\d\varTangentCoupling(\bar x,\bar\varTangentReals,x)
    -\varepsilon\sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{x-\bar x}^2\d\varTangentCoupling(\bar x,\bar\varTangentReals,x)}
    \Bigr\}.
\end{align*}
Both sets are nonempty. Indeed, $\bar\varTangentCoupling\times\delta_0\in\Lambda_1\cap\Lambda_2$, where $\bar\varTangentCoupling\coloneqq\pushforward{(\projection{1}{},\projection{2}{},\projection{1}{})}{\varTangentFixed}$ corresponds to the moved point coinciding with the base point $\varFixed\in\Omega_1\cap\Omega_2$.
They are also locally closed around $\bar\varTangentCoupling\times\delta_0$, by the same continuity and closedness arguments as in~\cref{lemma:eps_to_exact_normal}: $\Lambda_2$ is closed since $\pushforward{(\projection{1}{},\projection{2}{})}{}$ is $1$-Lipschitz with respect to $\wassersteinDistance{}{}{2}$ and the expected value is continuous in Wasserstein, while $\Lambda_1$ inherits local closedness from $\Omega_1$.

\emph{Step 2 (Extremality and the extremal principle).}
We claim that $\bar\varTangentCoupling\times\delta_0$ is a local extremal point of $(\Lambda_1,\Lambda_2)$. Since $\varTangentFixed\in\normalConeRegularStrong{\Omega_1\cap\Omega_2}{\varFixed}$, there is a neighborhood $U$ of $\bar\varTangentCoupling\times\delta_0$ such that every $\varTangentCoupling\times\delta_\beta\in U$ with $\pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling}=\varTangentFixed$ and $\pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega_1\cap\Omega_2$, with induced variation $\varTangent\coloneqq\pushforward{(\projection{1}{},\projection{3}{}-\projection{1}{})}{\varTangentCoupling}$ of $\Omega_1\cap\Omega_2$ at $\varFixed$, satisfies
\begin{equation}\label{eq:lemma-fuzzy:linearization}
\begin{aligned}
    \int_{\reals^d\times\reals^d\times\reals^d}\innerProduct{\bar\varTangentReals}{x-\bar x}\d\varTangentCoupling(\bar x,\bar\varTangentReals,x)
    \leq
    \innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
    \leq
    \varepsilon\norm{\varTangent}_{\varFixed}
    =
    \varepsilon\sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{x-\bar x}^2\d\varTangentCoupling(\bar x,\bar\varTangentReals,x)},
\end{aligned}
\end{equation}
the first inequality since $\varTangentCoupling$ is one admissible coupling of $\varTangentFixed$ and $\varTangent$, and the second by the strong regular normal cone inequality, which gives $\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}\leq\onotation{\norm{\varTangent}_{\varFixed}}\leq\varepsilon\norm{\varTangent}_{\varFixed}$ on $U$ small enough.
For any $a>0$, a point $\varTangentCoupling\times\delta_\beta\in\pushforward{(\identity{}+(0,0,0,a))}{\Lambda_1}\cap\Lambda_2\cap U$ lies in $\Lambda_2$ (so $\pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling}=\varTangentFixed$ and $\pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega_2$) and is the $(0,0,0,a)$-shift of a point of $\Lambda_1$ (i.e., $\varTangentCoupling\times\delta_{\beta-a}\in\Lambda_1$, so $\pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega_1$ and $\beta-a\geq0$).
Then $\pushforward{\projection{3}{}}{\varTangentCoupling}\in\Omega_1\cap\Omega_2$, so~\eqref{eq:lemma-fuzzy:linearization} applies and the definition of $\Lambda_2$ forces $\beta\leq\int_{\reals^d\times\reals^d\times\reals^d}\innerProduct{\bar\varTangentReals}{x-\bar x}\d\varTangentCoupling(\bar x,\bar\varTangentReals,x)-\varepsilon\sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{x-\bar x}^2\d\varTangentCoupling(\bar x,\bar\varTangentReals,x)}\leq0$. Thus, $\beta\leq0$, contradicting $\beta\geq a>0$. Hence, $\pushforward{(\identity{}+(0,0,0,a))}{\Lambda_1}\cap\Lambda_2\cap U=\emptyset$ for all $a>0$, and $\bar\varTangentCoupling\times\delta_0$ is extremal in the sense of~\cref{definition:def_extremal}.
%
Therefore,~\cref{theorem:th_extremal_principle}, applied to $(\Lambda_1,\Lambda_2,\bar\varTangentCoupling\times\delta_0)$ at accuracy $\sigma$, yields points $\varTangentCoupling_i\times\delta_{\beta_i}\in\Lambda_i$ with
\begin{equation}\label{eq:lemma-fuzzy:close_points}
    \sqrt{\wassersteinDistance{\bar\varTangentCoupling}{\varTangentCoupling_i}{2}^2+\abs{\beta_i}^2}<\sigma,\qquad i\in\{1,2\},
\end{equation}
variations $\boldsymbol{\varTangent}_i$ at $\varTangentCoupling_i\times\delta_{\beta_i}$ (with $\norm{\boldsymbol{\varTangent}_i}_{\varTangentCoupling_i\times\delta_{\beta_i}}=1$) that are $\sigma$-close to $\normalConeRegularStrong{\Lambda_i}{\varTangentCoupling_i\times\delta_{\beta_i}}$, and a transport plan $\varPlanGeneric_{\boldsymbol\varTangent}\in\setPlans{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_2}$ with $\pushforward{(\projection{1}{},\projection{3}{})}{\varPlanGeneric_{\boldsymbol\varTangent}}\in\setPlansOptimal{\varTangentCoupling_1\times\delta_{\beta_1}}{\varTangentCoupling_2\times\delta_{\beta_2}}$ such that
\begin{equation}\label{eq:lemma-fuzzy:cancellation}
    \int_{(\epigraphSpace\times\epigraphSpace)^2}\norm{\boldsymbol{\varTangentReals}_1+\boldsymbol{\varTangentReals}_2}^2\d\varPlanGeneric_{\boldsymbol\varTangent}(\boldsymbol{\zeta}_1,\boldsymbol{\zeta}_2)=0.
\end{equation}
We fix $\boldsymbol{\varTangent}_i^{\parallel}\in\normalConeRegularStrong{\Lambda_i}{\varTangentCoupling_i\times\delta_{\beta_i}}$ with $\wassersteinDistance{\boldsymbol{\varTangent}_i}{\boldsymbol{\varTangent}_i^{\parallel}}{\varTangentCoupling_i\times\delta_{\beta_i}}\leq\sigma$, and set $\varGeneric_1\coloneqq\pushforward{\projection{3}{}}{\varTangentCoupling_1}\in\Omega_1$ and $\varGeneric_2\coloneqq\pushforward{\projection{3}{}}{\varTangentCoupling_2}\in\Omega_2$.

\emph{Step 3 (Structure of the lifted normals).}
We write the arrow of $\boldsymbol{\varTangent}_i^{\parallel}$ in coordinates as $\boldsymbol{\zeta}_i=(\boldsymbol{w}_i,\varTangentReals_i,\lambda_i^{\beta})$, with $\boldsymbol{w}_i$ the $(\bar x,\bar\varTangentReals)$-component, $\varTangentReals_i$ the $x$-component, and $\lambda_i^{\beta}$ the (scalar) $\beta$-component; we denote by $x_i$ the moved-point coordinate of the base of $\boldsymbol{\varTangent}_i^{\parallel}$, set $\lambda_i\coloneqq\expectedValue{\boldsymbol{\varTangent}_i^{\parallel}}{\lambda_i^{\beta}}$.
We now recall Facts~1 and~2 of the proof of~\cref{lemma:eps_to_exact_normal} (with $\bar\varTangentReals$ playing the role of $\varTangentReals_\varepsilon$). First, by \cref{theorem:th_extremal_principle} the $\beta$-arrow of $\boldsymbol{\varTangent}_i$ is $\almostEverywhere{\boldsymbol{\varTangent}_i}$ a constant $c_i$, and $\boldsymbol{\varTangentReals}_1=-\boldsymbol{\varTangentReals}_2$ gives $c_1=-c_2$. Consequently, the $\beta$-arrow $\lambda_i^{\beta}$ of $\boldsymbol{\varTangent}_i^{\parallel}$ is $\almostEverywhere{\boldsymbol{\varTangent}_i^{\parallel}}$ within $\sigma$ of its mean $\lambda_i$ (and $\abs{\lambda_i-c_i}\leq\sigma$), which yields the norm decomposition
\begin{equation}\label{eq:lemma-fuzzy:norm_decomposition}
    \norm{\boldsymbol{\varTangent}_i^{\parallel}}_{\varTangentCoupling_i\times\delta_{\beta_i}}^2
    =\int_{\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol{w}_i}^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)
    +\int_{\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals_i}^2\d\boldsymbol{\varTangent}_i^{\parallel}(\boldsymbol{\zeta}_i)
    +\lambda_i^2+\rho_i,\qquad 0\leq\rho_i\leq\sigma^2.
\end{equation}
Second, by the structure of $\Lambda_1$, $\boldsymbol{w}_1=0$ $\almostEverywhere{\boldsymbol{\varTangent}_1^{\parallel}}$.

\emph{Step 4 (Normal to $\Omega_1$).}
By the structure of $\Lambda_1$,~\cref{proposition:prop_normal_cone_product} (\ref{item:product:delta} for the $\delta_\beta$-factor, \ref{item:product:cylinder} for the free block) we have $\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1^{\parallel}}\in\normalConeRegularStrong{\Omega_1}{\varGeneric_1}$ and $\lambda_1\leq 0$.

\emph{Step 5 (Normal to $\Omega_2$).}
We extract from $\boldsymbol{\varTangent}_2^{\parallel}$ a normal to $\Omega_2$. Since $\boldsymbol{\varTangent}_2^{\parallel}\in\normalConeRegularStrong{\Lambda_2}{\varTangentCoupling_2\times\delta_{\beta_2}}$, every coupling $\boldsymbol\varTangentCoupling\in\Pp{2}{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}$ with $\pushforward{(\projection{1}{},\projection{2}{})}{\boldsymbol\varTangentCoupling}=\boldsymbol{\varTangent}_2^{\parallel}$ and $\pushforward{(\projection{1}{}+\projection{3}{})}{\boldsymbol\varTangentCoupling}\in\Lambda_2$ satisfies
\begin{equation}\label{eq:lemma-fuzzy:regular_cone_lambda_2}
    \int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\boldsymbol{\bar\varTangentReals}}{\boldsymbol\varTangentReals'}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})
    \leq
    \onotation{\left(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{\boldsymbol\varTangentReals'}^2\d\boldsymbol\varTangentCoupling(\boldsymbol{q})\right)^{1/2}},
\end{equation}
where $\boldsymbol{q}$ denotes a generic point of $\epigraphSpace\times\epigraphSpace\times\epigraphSpace$: its three blocks are a base point of $\boldsymbol{\varTangent}_2^{\parallel}$, the arrow $\boldsymbol{\bar\varTangentReals}$ that $\boldsymbol{\varTangent}_2^{\parallel}$ attaches to it (that is, $\boldsymbol{\bar\varTangentReals}=\boldsymbol{\zeta}_2$ in the coordinates of Step~3), and a displacement $\boldsymbol{\varTangentReals}'$.
We will use it only for displacements $\boldsymbol\varTangentReals'=(0,0,\varTangentReals',\Delta\beta)$, for which it holds $\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\boldsymbol{\bar\varTangentReals}}{\boldsymbol\varTangentReals'}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})=\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_2}{\varTangentReals'}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})+\lambda_2\,\Delta\beta$.
%
Testing $\varTangentReals'=0$ with a constant $\Delta\beta\leq0$, admissible since lowering $\beta$ preserves membership in $\Lambda_2$, gives $\lambda_2\Delta\beta\leq\onotation{\abs{\Delta\beta}}$ for all $\Delta\beta\leq0$, whence $\lambda_2\geq0$. Next, fix $\varGeneric'\in\Omega_2$ and a variation $\varTangent'\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varGeneric_2}{\varGeneric'}}$.
Let $\boldsymbol\varTangentCoupling$ be a coupling as above whose displacement has $x$-component $\varTangentReals'$ realizing $\varTangent'$. Define
\begin{equation}\label{eq:lemma-fuzzy:beta-prime}
\begin{aligned}
    \beta'&\coloneqq\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\bar\varTangentReals}{x_2+\varTangentReals'-\bar x}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})
    -\varepsilon\Bigl(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{x_2+\varTangentReals'-\bar x}^2\d\boldsymbol\varTangentCoupling(\boldsymbol{q})\Bigr)^{1/2},
    \\
    \beta_0'&\coloneqq\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\bar\varTangentReals}{x_2-\bar x}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})
    -\varepsilon\Bigl(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{x_2-\bar x}^2\d\boldsymbol\varTangentCoupling(\boldsymbol{q})\Bigr)^{1/2}
    \\
    &=\int_{\reals^d\times\reals^d\times\reals^d}\innerProduct{\bar\varTangentReals}{x_2-\bar x}\d\varTangentCoupling_2(\bar x,\bar\varTangentReals,x_2)
    -\varepsilon\Bigl(\int_{\reals^d\times\reals^d\times\reals^d}\norm{x_2-\bar x}^2\d\varTangentCoupling_2(\bar x,\bar\varTangentReals,x_2)\Bigr)^{1/2},
\end{aligned}
\end{equation}
where the second line uses $\pushforward{\projection{1}{}}{\boldsymbol\varTangentCoupling}=\varTangentCoupling_2\times\delta_{\beta_2}$ and is precisely the bound on $\beta$ in the definition of $\Lambda_2$ at $\varTangentCoupling_2$.
Hence, $\varTangentCoupling_2\times\delta_{\beta_2}\in\Lambda_2$ implies $\beta_2\leq\beta_0'$.
%
Consider the displacement $(0,0,\varTangentReals',\Delta\beta)$ with $\Delta\beta\coloneqq\beta'-\beta_0'$, which moves the $x$-marginal to $\varGeneric'\in\Omega_2$ and sets the epigraphical variable to $\beta_2+\Delta\beta=\beta_2+\beta'-\beta_0'\leq\beta'$ (as $\beta_2\leq\beta_0'$), so the moved configuration lies in $\Lambda_2$.
The triangle inequality for the seminorm $w\mapsto(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{w}^2\d\boldsymbol\varTangentCoupling(\boldsymbol{q}))^{1/2}$ applied to $x_2+\varTangentReals'-\bar x=(x_2-\bar x)+\varTangentReals'$, together with the Cauchy--Schwarz bound $\abs{\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\bar\varTangentReals}{\varTangentReals'}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})}\leq\norm{\varTangentFixed}_{\varFixed}\norm{\varTangent'}_{\varGeneric_2}$, gives
\begin{equation*}
    \Delta\beta
    \geq
    \int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\bar\varTangentReals}{\varTangentReals'}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})
    -\varepsilon\Bigl(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals'}^2\d\boldsymbol\varTangentCoupling(\boldsymbol{q})\Bigr)^{1/2},
    \qquad
    \abs{\Delta\beta}\leq(\norm{\varTangentFixed}_{\varFixed}+\varepsilon)\,\norm{\varTangent'}_{\varGeneric_2}.
\end{equation*}
Substituting into~\eqref{eq:lemma-fuzzy:regular_cone_lambda_2}, whose right-hand side is $\onotation{\norm{\varTangent'}_{\varGeneric_2}}$ (since $(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals'}^2\d\boldsymbol\varTangentCoupling(\boldsymbol{q})+\abs{\Delta\beta}^2)^{1/2}\leq\sqrt{1+(\norm{\varTangentFixed}_{\varFixed}+\varepsilon)^2}\,\norm{\varTangent'}_{\varGeneric_2}$ by the bound on $\abs{\Delta\beta}$), and using $\lambda_2\geq0$,
\begin{equation}\label{eq:lemma-fuzzy:omega2_normal}
    \int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\innerProduct{\varTangentReals_2+\lambda_2\bar\varTangentReals}{\varTangentReals'}\d\boldsymbol\varTangentCoupling(\boldsymbol{q})
    \leq
    \lambda_2\varepsilon\Bigl(\int_{\epigraphSpace\times\epigraphSpace\times\epigraphSpace}\norm{\varTangentReals'}^2\d\boldsymbol\varTangentCoupling(\boldsymbol{q})\Bigr)^{1/2}
    +\onotation{\norm{\varTangent'}_{\varGeneric_2}}.
\end{equation}
As $\varGeneric'\in\Omega_2$ and the coupling $\boldsymbol\varTangentCoupling$ realizing $\varTangent'$ were arbitrary,~\eqref{eq:lemma-fuzzy:omega2_normal} yields $\innerProduct{\eta_2^{\parallel}}{\varTangent'}_{\varGeneric_2}\leq\lambda_2\varepsilon\norm{\varTangent'}_{\varGeneric_2}+\onotation{\norm{\varTangent'}_{\varGeneric_2}}$ for every $\varGeneric'\in\Omega_2$, where $\eta_2^{\parallel}\coloneqq\pushforward{(\projection{x_2}{},\,\projection{\varTangentReals_2}{}+\lambda_2\projection{\bar\varTangentReals}{})}{\boldsymbol{\varTangent}_2^{\parallel}}$.
Since $\pushforward{\projection{1}{}}{\eta_2^{\parallel}}=\varGeneric_2$, the variation $\eta_2^{\parallel}$ satisfies the hypothesis of~\cref{lemma:eps_to_exact_normal} at $\varGeneric_2$ with $\lambda_2\varepsilon$ in place of $\varepsilon$.
Thus, by~\cref{lemma:eps_to_exact_normal}, with accuracies $\lambda_2\varepsilon$ and $\sigma$, there are $\tilde\varGeneric_2\in\Omega_2$ with $\wassersteinDistance{\varGeneric_2}{\tilde\varGeneric_2}{2}\leq\sigma$ and a strong regular normal $\bar\eta_2\in\normalConeRegularStrong{\Omega_2}{\tilde\varGeneric_2}$ with $\wassersteinDistance{\eta_2^{\parallel}}{\bar\eta_2}{2}\leq\lambda_2\varepsilon+\sigma$.

\emph{Step 6 (Cancellation and the multiplier identity).}
By~\eqref{eq:lemma-fuzzy:cancellation}, $\boldsymbol{\varTangentReals}_1=-\boldsymbol{\varTangentReals}_2$ $\almostEverywhere{\varPlanGeneric_{\boldsymbol\varTangent}}$. Let
\begin{equation*}
    \eta_1\coloneqq\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1},
    \qquad
    \eta_2\coloneqq\pushforward{(\projection{x_2}{},\,\projection{\varTangentReals_2}{}+\lambda_2\projection{\bar\varTangentReals}{})}{\boldsymbol{\varTangent}_2},
    \qquad
    \lambda\coloneqq\lambda_2\geq 0.
\end{equation*}
Pushing $\varPlanGeneric_{\boldsymbol\varTangent}$ forward under the map that extracts the pair $(\bar x,\bar\varTangentReals)$ from the $\Lambda_2$-factor, the pair $(x_1,\varTangentReals_1)$ from $\boldsymbol{\varTangent}_1$, and the pair $(x_2,\varTangentReals_2+\lambda\bar\varTangentReals)$ from $\boldsymbol{\varTangent}_2$ yields a transport plan $\varPlanGeneric\in\setPlans{\varTangentFixed}{\eta_1,\eta_2}$. Along $\varPlanGeneric$ the arrow of $\eta_1$ is $\varTangentReals_1$, that of $\eta_2$ is $\varTangentReals_2+\lambda\bar\varTangentReals$, and $\varTangentReals_1=-\varTangentReals_2$, so $\lambda\bar\varTangentReals-(\varTangentReals_1+(\varTangentReals_2+\lambda\bar\varTangentReals))=0$ holds $\almostEverywhere{\varPlanGeneric}$.

\emph{Step 7 (Closeness to the strong regular normal cones).}
The extracted normals are close to the strong regular normal cones. First, $\eta_1$ is $\sigma$-close to $\normalConeRegularStrong{\Omega_1}{\varGeneric_1}$: by Step~4, $\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1^{\parallel}}\in\normalConeRegularStrong{\Omega_1}{\varGeneric_1}$, the projection $(\projection{x_1}{},\projection{\varTangentReals_1}{})$ is $1$-Lipschitz, and $\wassersteinDistance{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_1^{\parallel}}{2}\leq\sigma$, so $\wassersteinDistance{\eta_1}{\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1^{\parallel}}}{2}\leq\sigma$. Second, the same Lipschitz bound gives $\wassersteinDistance{\eta_2}{\eta_2^{\parallel}}{2}\leq\sigma$, so by Step~5 $\eta_2$ is $(\lambda_2\varepsilon+2\sigma)$-close to $\normalConeRegularStrong{\Omega_2}{\tilde\varGeneric_2}$.

\emph{Step 8 (Nontriviality).}
We show that $m\coloneqq\max\{\lambda,\norm{\eta_1}_{\varGeneric_1}\}$ is bounded away from $0$ for $\sigma$ small. We proceed in three steps.
%
First, we bound the projected normal $\eta_1^{\parallel}\coloneqq\pushforward{(\projection{x_1}{},\projection{\varTangentReals_1}{})}{\boldsymbol{\varTangent}_1^{\parallel}}$. From $\norm{\boldsymbol{\varTangent}_1}=1$ and $\wassersteinDistance{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_1^{\parallel}}{2}\leq\sigma$ we get $(1-\sigma)^2\leq\norm{\boldsymbol{\varTangent}_1^{\parallel}}^2\leq(1+\sigma)^2$. Since $\boldsymbol{w}_1=0$ (Fact~2) and $0\leq\rho_1\leq\sigma^2$, the decomposition~\eqref{eq:lemma-fuzzy:norm_decomposition} reads $\norm{\boldsymbol{\varTangent}_1^{\parallel}}^2=\norm{\eta_1^{\parallel}}_{\varGeneric_1}^2+\lambda_1^2+\rho_1$, whence $\norm{\eta_1^{\parallel}}_{\varGeneric_1}^2+\lambda_1^2\geq(1-\sigma)^2-\sigma^2=1-2\sigma$.
%
Second, we transfer this bound from $\eta_1^{\parallel}$ to $\eta_1$. The projection $(\projection{x_1}{},\projection{\varTangentReals_1}{})$ is $1$-Lipschitz, so $\wassersteinDistance{\eta_1}{\eta_1^{\parallel}}{2}\leq\sigma$ by Step~7, and hence $\bigl|\norm{\eta_1}_{\varGeneric_1}-\norm{\eta_1^{\parallel}}_{\varGeneric_1}\bigr|\leq\sigma$ by the reverse triangle inequality. With $\norm{\eta_1^{\parallel}}_{\varGeneric_1}\leq1+\sigma$ this also gives $\norm{\eta_1}_{\varGeneric_1}\leq\norm{\eta_1^{\parallel}}_{\varGeneric_1}+\sigma\leq1+2\sigma$. The identity $a^2-b^2=(a-b)(a+b)$ then yields $\bigl|\norm{\eta_1}_{\varGeneric_1}^2-\norm{\eta_1^{\parallel}}_{\varGeneric_1}^2\bigr|\leq\bigl|\norm{\eta_1}_{\varGeneric_1}-\norm{\eta_1^{\parallel}}_{\varGeneric_1}\bigr|\bigl(\norm{\eta_1}_{\varGeneric_1}+\norm{\eta_1^{\parallel}}_{\varGeneric_1}\bigr)\leq\sigma(2+3\sigma)=2\sigma+3\sigma^2$, and hence $\norm{\eta_1}_{\varGeneric_1}^2+\lambda_1^2\geq(1-2\sigma)-(2\sigma+3\sigma^2)=1-4\sigma-3\sigma^2$.
%
Third, we compare the two multipliers, as the bound just obtained involves $\lambda_1$ and not $\lambda=\lambda_2$. By Fact~1, $c_1=-c_2$ and $\abs{\lambda_i-c_i}\leq\sigma$, so $\abs{\lambda_1+\lambda_2}\leq2\sigma$. Since $\lambda_1\leq0$ (Step~4) and $\lambda_2\geq0$ (Step~5), we have $\abs{\lambda_1}=-\lambda_1$, hence $\bigl|\lambda-\abs{\lambda_1}\bigr|=\abs{\lambda_2+\lambda_1}\leq2\sigma$ and in particular $\lambda\geq\abs{\lambda_1}-2\sigma$.
%
Combining the three estimates, $m\geq\max\{\abs{\lambda_1},\norm{\eta_1}_{\varGeneric_1}\}-2\sigma\geq\tfrac{1}{\sqrt2}\sqrt{\lambda_1^2+\norm{\eta_1}_{\varGeneric_1}^2}-2\sigma\geq\tfrac{1}{\sqrt2}\sqrt{1-4\sigma-3\sigma^2}-2\sigma$, which is bounded away from $0$ for $\sigma$ small.

\emph{Step 9 (Conclusion).}
Renormalizing by the positive factor $m^{-1}$, which preserves the cones and scales the multiplier identity of Step~6, we set $\varTangent_1\coloneqq\tfrac1m\eta_1$ and $\varTangent_2\coloneqq\tfrac1m\eta_2$ and replace $\lambda$ by $\lambda/m$. Then $\max\{\lambda,\norm{\varTangent_1}_{\varGeneric_1}\}=1$, which is~\eqref{eq:lemma-fuzzy:nontriviality}, and the rescaled transport plan $\varPlanGeneric\in\setPlans{\varTangentFixed}{\varTangent_1,\varTangent_2}$ still satisfies $\lambda\bar\varTangentReals-(\varTangentReals_1+\varTangentReals_2)=0$ $\almostEverywhere{\varPlanGeneric}$, which gives~\eqref{eq:lemma-fuzzy:the-statement}.

Let $\varGeneric_2'\coloneqq\tilde\varGeneric_2\in\Omega_2$ be the base of the exact $\Omega_2$-normal of Step~5. By Step~7, $\varTangent_1$ is $\tfrac{\sigma}{m}$-close to $\normalConeRegularStrong{\Omega_1}{\varGeneric_1}$ and $\varTangent_2$ is $\tfrac1m(\lambda_2\varepsilon+2\sigma)$-close to $\normalConeRegularStrong{\Omega_2}{\varGeneric_2'}$. Since $\projection{3}{}$ is $1$-Lipschitz and $\pushforward{\projection{3}{}}{\bar\varTangentCoupling}=\varFixed$, estimate~\eqref{eq:lemma-fuzzy:close_points} gives $\wassersteinDistance{\varFixed}{\varGeneric_i}{2}<\sigma$ for $i\in\{1,2\}$; with $\wassersteinDistance{\varGeneric_2}{\varGeneric_2'}{2}\leq\sigma$ (Step~5) this also gives $\wassersteinDistance{\varFixed}{\varGeneric_2'}{2}<2\sigma$.

We bound the base displacements of $\varPlanGeneric$. Under $\varPlanGeneric$, $\bar x$ and $x_2$ are the base point and the moved point of $\varTangentCoupling_2$ (Step~6), so their joint law is the $(\projection{1}{},\projection{3}{})$-marginal of $\varTangentCoupling_2$. Since $(\bar x,\bar\varTangentReals,x)\mapsto\bar x-x$ is $\sqrt2$-Lipschitz, $\bar x=x$ on the support of $\bar\varTangentCoupling$, and $\wassersteinDistance{\bar\varTangentCoupling}{\varTangentCoupling_2}{2}<\sigma$ by~\eqref{eq:lemma-fuzzy:close_points}, we get $\int_{(\reals^d\times\reals^d)^3}\norm{\bar x-x_2}^2\d\varPlanGeneric(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)\leq2\sigma^2$. Next, $x_1$ and $x_2$ are coupled under $\varPlanGeneric$ by the optimal transport plan $\pushforward{(\projection{1}{},\projection{3}{})}{\varPlanGeneric_{\boldsymbol\varTangent}}\in\setPlansOptimal{\varTangentCoupling_1\times\delta_{\beta_1}}{\varTangentCoupling_2\times\delta_{\beta_2}}$; since $\varTangentCoupling_1\times\delta_{\beta_1}$ and $\varTangentCoupling_2\times\delta_{\beta_2}$ are each within $\sigma$ of $\bar\varTangentCoupling\times\delta_0$ by~\eqref{eq:lemma-fuzzy:close_points}, this gives $\int_{(\reals^d\times\reals^d)^3}\norm{x_1-x_2}^2\d\varPlanGeneric(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)\leq\wassersteinDistance{\varTangentCoupling_1\times\delta_{\beta_1}}{\varTangentCoupling_2\times\delta_{\beta_2}}{2}^2\leq(2\sigma)^2$. The triangle inequality then gives $\int_{(\reals^d\times\reals^d)^3}\norm{\bar x-x_1}^2\d\varPlanGeneric(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)\leq(\sqrt2+2)^2\sigma^2$.
%
Finally, all error terms are bounded by an absolute constant $C\geq1$ times $\varepsilon+\sigma$ or $\sigma^2$.
The construction with $\varepsilon/(2C)$ in place of $\varepsilon$ and $\sigma=\varepsilon/(2C)$ thus proves the lemma.


==> elements/fuzzy-intersection_title.tex <==
A fuzzy intersection rule%


==> elements/intersection_rule_strong_body.tex <==
    Let $\Omega_1$ and $\Omega_2$ be locally closed sets around $\varFixed\in\Omega_1\cap\Omega_2$.
    Suppose that (i)
        $\normalConeStrong{\Omega_1}{\varFixed}\cap \left(-\normalConeStrong{\Omega_2}{\varFixed}\right)= \{\localZero{\varFixed}\}$
    and that (ii) either $\Omega_1$ or $\Omega_2$ is \gls*{acr:snc} at $\varFixed$. Then,
        $\normalConeStrong{\Omega_1\cap\Omega_2}{\varFixed} \subseteq \normalConeStrong{\Omega_1}{\varFixed}
        +
        \normalConeStrong{\Omega_2}{\varFixed}$.


==> elements/intersection_rule_strong_proof.tex <==
We divide the proof into steps.
Without loss of generality,  we assume that $\Omega_1$ is \gls*{acr:snc} at $\varFixed$.

\emph{Step 1 (Approximation and per-step fuzzy rule).}
Let $\varTangentFixed\in\normalConeStrong{\Omega_1\cap\Omega_2}{\varFixed}$. By~\cref{definition:def_fuzzy_normal_cone}, there are $\varGeneric_k\convergenceWasserstein\varFixed$ in $\Omega_1\cap\Omega_2$ and strong regular normals $\varTangent_k\in\normalConeRegularStrong{\Omega_1\cap\Omega_2}{\varGeneric_k}$ such that $\varTangent_k\convergenceWasserstein\varTangentFixed$. As $\varTangent_k$ is a strong regular normal, for a sequence $\varepsilon_k\fromAbove0$,~\cref{lemma:fuzzy-intersection} applies to it at $\varGeneric_k$ (in particular, since $\Omega_1$ and $\Omega_2$ are locally closed around $\varFixed$, they are locally closed around $\varGeneric_k$ for $k$ large enough) with accuracy $\varepsilon_k$, providing a multiplier $\lambda_k\geq0$, base points $\varGeneric_{i,k}\in\Omega_i\cap\wassersteinBall{\varGeneric_k}{\varepsilon_k}{2}$, a point $\varGeneric_{2,k}'\in\Omega_2\cap\wassersteinBall{\varGeneric_k}{2\varepsilon_k}{2}$, variations $\varTangent_{1,k},\varTangent_{2,k}$ that are $\varepsilon_k$-close with respect to $\wassersteinDistance{}{}{2}$ to $\normalConeRegularStrong{\Omega_1}{\varGeneric_{1,k}}$ and $\normalConeRegularStrong{\Omega_2}{\varGeneric_{2,k}'}$ respectively, and a transport plan $\varPlanGeneric_k\in\setPlans{\varTangent_k}{\varTangent_{1,k},\varTangent_{2,k}}$ with $\int_{(\reals^d\times\reals^d)^3}\norm{\bar x-x_1}^2\d\varPlanGeneric_k(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)\leq\varepsilon_k^2$ and $\int_{(\reals^d\times\reals^d)^3}\norm{\bar x-x_2}^2\d\varPlanGeneric_k(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)\leq\varepsilon_k^2$, such that
\begin{align}\label{eq:intersection-strong:cancellation}
    \int_{(\reals^d\times\reals^d)^3}\norm{\lambda_k\bar\varTangentReals-(\varTangentReals_1+\varTangentReals_2)}^2\d\varPlanGeneric_k(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)&=0
    \\
    \max\{\lambda_k,\norm{\varTangent_{1,k}}_{\varGeneric_{1,k}}\}&=1.
    \label{eq:intersection-strong:nontriviality}
\end{align}
Since $\wassersteinDistance{\varGeneric_{i,k}}{\varFixed}{2}\leq\varepsilon_k+\wassersteinDistance{\varGeneric_k}{\varFixed}{2}$, we have $\varGeneric_{i,k}\convergenceWasserstein\varFixed$.

\emph{Step 2 (Boundedness and compactness).}
We first record uniform bounds on the multipliers $\lambda_k$ and on the variation norms. Since $\varTangent_k\convergenceWasserstein\varTangentFixed$, the norms $\norm{\varTangent_k}_{\varGeneric_k}$ converge to $\norm{\varTangentFixed}_{\varFixed}$ and are in particular bounded, while~\eqref{eq:intersection-strong:nontriviality} gives $\lambda_k\leq1$ and $\norm{\varTangent_{1,k}}_{\varGeneric_{1,k}}\leq1$. For the remaining norm,~\eqref{eq:intersection-strong:cancellation} gives $\varTangentReals_2=\lambda_k\bar\varTangentReals-\varTangentReals_1$ $\almostEverywhere{\varPlanGeneric_k}$. The triangle inequality then yields $\norm{\varTangent_{2,k}}_{\varGeneric_{2,k}}\leq\lambda_k\norm{\varTangent_k}_{\varGeneric_k}+\norm{\varTangent_{1,k}}_{\varGeneric_{1,k}}$, which is bounded as well.
%
The marginals $\varGeneric_k,\varGeneric_{1,k},\varGeneric_{2,k}$ converge to $\varFixed$ and are hence tight.
Moreover, $\norm{\varTangent_k}_{\varGeneric_k}^2$, $\norm{\varTangent_{i,k}}_{\varGeneric_{i,k}}^2$ are uniformly bounded, hence the second marginals are tight. By Prokhorov's theorem~\cite[Theorem~5.1.3]{ambrosio2005gradient} and~\cite[Lemma~4.4]{villani2009optimal}, along a subsequence we have $\lambda_k\to\lambda\geq0$, $\varTangent_{i,k}\convergenceNarrow\varTangent_i$ for some $\varTangent_i\in\Pp{2}{\reals^d\times\reals^d}$, and $\varPlanGeneric_k\convergenceNarrow\varPlanGeneric\in\setPlans{\varTangentFixed}{\varTangent_1,\varTangent_2}$.
The first marginal of $\varTangent_i$ is $\varFixed$. Indeed $\pushforward{\projection{1}{}}{\varTangent_{i,k}}=\varGeneric_{i,k}\convergenceWasserstein\varFixed$, and the first marginal is narrowly continuous.
%
It remains to show that $\bar x=x_1=x_2$ $\almostEverywhere{\varPlanGeneric}$.
Narrow convergence of $\varPlanGeneric_k\convergenceNarrow\varPlanGeneric$ together with lower semicontinuity gives
\begin{align*}
    \!
    \int_{(\reals^d\times\reals^d)^3}\norm{\bar x-x_i}^2\d\varPlanGeneric(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)
    &\leq\liminf_{k\to\infty}\int_{(\reals^d\times\reals^d)^3}\norm{\bar x-x_i}^2\d\varPlanGeneric_k(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)
    \\
    &\leq\limsup_{k\to\infty}\varepsilon_k^2=0 .
\end{align*}
Therefore, $\bar x=x_1=x_2$ $\almostEverywhere{\varPlanGeneric}$.

\emph{Step 3 (Normal to $\Omega_1$ via sequential normal compactness).}
Pick $\hat\varTangent_{1,k}\in\normalConeRegularStrong{\Omega_1}{\varGeneric_{1,k}}$ with $\wassersteinDistance{\varTangent_{1,k}}{\hat\varTangent_{1,k}}{2}\leq\varepsilon_k$; then $\hat\varTangent_{1,k}\convergenceNarrow\varTangent_1$. Since $\Omega_1$ is \gls*{acr:snc} and $\varGeneric_{1,k}\convergenceWasserstein\varFixed$,~\cref{definition:def_snc} gives $\hat\varTangent_{1,k}\convergenceWasserstein\varTangent_1$, whence $\varTangent_{1,k}\convergenceWasserstein\varTangent_1$ and, in particular, $\norm{\varTangent_{1,k}}_{\varGeneric_{1,k}}\to\norm{\varTangent_1}_{\varFixed}$. As $\hat\varTangent_{1,k}\in\normalConeRegularStrong{\Omega_1}{\varGeneric_{1,k}}$, $\varGeneric_{1,k}\convergenceWasserstein\varFixed$, and $\hat\varTangent_{1,k}\convergenceWasserstein\varTangent_1$,~\cref{definition:def_fuzzy_normal_cone} gives $\varTangent_1\in\normalConeStrong{\Omega_1}{\varFixed}$.

\emph{Step 4 (Multiplier identity in the limit).}
Eq.~\eqref{eq:intersection-strong:cancellation} states that $\varTangentReals_1+\varTangentReals_2=\lambda_k\bar\varTangentReals$ holds $\almostEverywhere{\varPlanGeneric_k}$. Thus, $\varTangentReals_2-(\lambda\bar\varTangentReals-\varTangentReals_1)=(\lambda_k-\lambda)\bar\varTangentReals$ $\almostEverywhere{\varPlanGeneric_k}$.
Since the $(\bar x,\bar\varTangentReals)$-marginal of $\varPlanGeneric_k$ is $\varTangent_k$ we have
\begin{equation*}
    \int_{(\reals^d\times\reals^d)^3}\norm{\varTangentReals_2-(\lambda\bar\varTangentReals-\varTangentReals_1)}^2\d\varPlanGeneric_k(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)
    =(\lambda_k-\lambda)^2\norm{\varTangent_k}_{\varGeneric_k}^2\to0,
\end{equation*}
where we used that $\lambda_k\to\lambda$ and $\norm{\varTangent_k}_{\varGeneric_k}$ is bounded.
Again by narrow lower semicontinuity we have
\begin{equation*}
    \int_{(\reals^d\times\reals^d)^3}\norm{\varTangentReals_2-(\lambda\bar\varTangentReals-\varTangentReals_1)}^2\d\varPlanGeneric(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)
    =0.
\end{equation*}
Hence, $\varTangentReals_1+\varTangentReals_2=\lambda\bar\varTangentReals$ holds $\almostEverywhere{\varPlanGeneric}$. Moreover, $\bar x=x_1=x_2$ $\almostEverywhere{\varPlanGeneric}$ (Step~2), so $\varPlanGeneric$ couples $\varTangent_1$ and $\varTangent_2$ over a common first marginal. By definition, $\varTangent_1\localSum{\varPlanGeneric}\varTangent_2$ is the law of $(x_1,\varTangentReals_1+\varTangentReals_2)$ under $\varPlanGeneric$.
Since $\varTangentReals_1+\varTangentReals_2=\lambda\bar\varTangentReals$ and $x_1=\bar x$ $\almostEverywhere{\varPlanGeneric}$, this is the law of $(\bar x,\lambda\bar\varTangentReals)$, that is $\lambda\varTangentFixed$. Thus,
\begin{equation}\label{eq:intersection-strong:limit-identity}
    \lambda\varTangentFixed=\varTangent_1\localSum{\varPlanGeneric}\varTangent_2.
\end{equation}

\emph{Step 5 (Normal to $\Omega_2$ via the cancellation).}
Expanding the square and using $\varTangentReals_2=\lambda_k\bar\varTangentReals-\varTangentReals_1$,
\begin{equation*}
    \norm{\varTangent_{2,k}}_{\varGeneric_{2,k}}^2
    =\lambda_k^2\norm{\varTangent_k}_{\varGeneric_k}^2
    -2\lambda_k\int_{(\reals^d\times\reals^d)^3}\innerProduct{\bar\varTangentReals}{\varTangentReals_1}\d\varPlanGeneric_k(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)
    +\norm{\varTangent_{1,k}}_{\varGeneric_{1,k}}^2.
\end{equation*}
We show that the cross term converges. We work with the $(\bar\varTangentReals,\varTangentReals_1)$-marginal $m_k\coloneqq\pushforward{(\projection{2}{},\projection{4}{})}{\varPlanGeneric_k}$ of $\varPlanGeneric_k$.
Clearly, $m_k$ converges narrowly to the corresponding marginal $m$ of $\varPlanGeneric$ (as $\varPlanGeneric_k\convergenceNarrow\varPlanGeneric$), and its second moment $\norm{\varTangent_k}_{\varGeneric_k}^2+\norm{\varTangent_{1,k}}_{\varGeneric_{1,k}}^2$ converges to $\norm{\varTangentFixed}_{\varFixed}^2+\norm{\varTangent_1}_{\varFixed}^2$ (as $\varTangent_k\convergenceWasserstein\varTangentFixed$ and $\varTangent_{1,k}\convergenceWasserstein\varTangent_1$), which equals the second moment of $m$. By~\cite[Theorem~6.9]{villani2009optimal}, narrow convergence of $m_k$ together with convergence of its second moment is equivalent to $m_k\convergenceWasserstein m$.
Thus, $\int_{(\reals^d\times\reals^d)^3}\innerProduct{\bar\varTangentReals}{\varTangentReals_1}\d\varPlanGeneric_k(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)\to\int_{(\reals^d\times\reals^d)^3}\innerProduct{\bar\varTangentReals}{\varTangentReals_1}\d\varPlanGeneric(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)$.
%
Passing to the limit and using $\lambda_k\to\lambda$, $\norm{\varTangent_k}_{\varGeneric_k}\to\norm{\varTangentFixed}_{\varFixed}$, $\norm{\varTangent_{1,k}}_{\varGeneric_{1,k}}\to\norm{\varTangent_1}_{\varFixed}$, and the convergence of the cross term established above, we obtain
\begin{align*}
    \lim_{k\to\infty}\norm{\varTangent_{2,k}}_{\varGeneric_{2,k}}^2
    &=\lambda^2\norm{\varTangentFixed}_{\varFixed}^2
    -2\lambda\int_{(\reals^d\times\reals^d)^3}\innerProduct{\bar\varTangentReals}{\varTangentReals_1}\d\varPlanGeneric(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)
    +\norm{\varTangent_1}_{\varFixed}^2
    \\
    &=\int_{(\reals^d\times\reals^d)^3}\norm{\lambda\bar\varTangentReals-\varTangentReals_1}^2\d\varPlanGeneric(\bar x,\bar\varTangentReals,x_1,\varTangentReals_1,x_2,\varTangentReals_2)
    =\norm{\varTangent_2}_{\varFixed}^2 ,
\end{align*}
where the second line recombines the square (the $(\bar x,\bar\varTangentReals)$- and $(x_1,\varTangentReals_1)$-marginals of $\varPlanGeneric$ being $\varTangentFixed$ and $\varTangent_1$, respectively) and applies~\eqref{eq:intersection-strong:limit-identity} (i.e., $\varTangentReals_2=\lambda\bar\varTangentReals-\varTangentReals_1$ $\almostEverywhere{\varPlanGeneric}$).
Thus, $\norm{\varTangent_{2,k}}_{\varGeneric_{2,k}}\to\norm{\varTangent_2}_{\varFixed}$.
With $\varTangent_{2,k}\convergenceNarrow\varTangent_2$ and $\varGeneric_{2,k}\convergenceWasserstein\varFixed$, the convergence of second moments yields convergence in Wasserstein $\varTangent_{2,k}\convergenceWasserstein\varTangent_2$. Choosing $\hat\varTangent_{2,k}\in\normalConeRegularStrong{\Omega_2}{\varGeneric_{2,k}'}$ within $\varepsilon_k$ of $\varTangent_{2,k}$ (where $\varGeneric_{2,k}'\convergenceWasserstein\varFixed$ since $\varGeneric_{2,k}'\in\wassersteinBall{\varGeneric_k}{2\varepsilon_k}{2}$ and $\varGeneric_k\convergenceWasserstein\varFixed$), also $\hat\varTangent_{2,k}\convergenceWasserstein\varTangent_2$, and~\cref{definition:def_fuzzy_normal_cone} gives $\varTangent_2\in\normalConeStrong{\Omega_2}{\varFixed}$.

\emph{Step 6 (Ruling out $\lambda=0$).}
Passing~\eqref{eq:intersection-strong:nontriviality} to the limit via $\lambda_k\to\lambda$ and $\norm{\varTangent_{1,k}}_{\varGeneric_{1,k}}\to\norm{\varTangent_1}_{\varFixed}$ gives $\max\{\lambda,\norm{\varTangent_1}_{\varFixed}\}=1$. Suppose $\lambda=0$.
Then $\norm{\varTangent_1}_{\varFixed}=1$, so $\varTangent_1\neq\localZero{\varFixed}$. With $\lambda=0$,~\eqref{eq:intersection-strong:limit-identity} reads $\varTangentReals_1+\varTangentReals_2=0$ $\almostEverywhere{\varPlanGeneric}$. Since $\bar x=x_1=x_2$ $\almostEverywhere{\varPlanGeneric}$ and $\varTangent_1,\varTangent_2$ are recovered as the $(x_1,\varTangentReals_1)$- and $(x_2,\varTangentReals_2)$-marginals of $\varPlanGeneric$, we conclude that $\varTangent_2=\pushforward{(\projection{1}{},-\projection{2}{})}{\varTangent_1}=-\varTangent_1$.
Hence, $\localZero{\varFixed}\neq\varTangent_1\in\normalConeStrong{\Omega_1}{\varFixed}\cap\left(-\normalConeStrong{\Omega_2}{\varFixed}\right)$, contradicting assumption~(i). Therefore, $\lambda>0$.

\emph{Step 7 (Conclusion).}
As the normal cones are cones and $\lambda>0$, dividing~\eqref{eq:intersection-strong:limit-identity} by $\lambda$ gives
\begin{equation*}
    \varTangentFixed=\tfrac1\lambda\varTangent_1\localSum{\varPlanGeneric}\tfrac1\lambda\varTangent_2\in\normalConeStrong{\Omega_1}{\varFixed}+\normalConeStrong{\Omega_2}{\varFixed}.
\end{equation*}
As $\varTangentFixed\in\normalConeStrong{\Omega_1\cap\Omega_2}{\varFixed}$ was arbitrary, we conclude $\normalConeStrong{\Omega_1\cap\Omega_2}{\varFixed}\subseteq\normalConeStrong{\Omega_1}{\varFixed}+\normalConeStrong{\Omega_2}{\varFixed}$.


==> elements/intersection_rule_strong_title.tex <==
Intersection rule for strong normal cones%


==> elements/lemma_deterministic_coordinate_body.tex <==
{%
Let $\varFixed \in \Pp{2}{\reals^d}$, $b \in \reals$, and let $T$ be as in
\eqref{equation:extraction-map-epigraph}, so that $\pushforward{T}{\cdot}$
maps transport plans (resp., variations) on $\reals^{d+1}$ to transport plans
(resp., variations) on $\reals^d$; we write $\boldsymbol{x}=(x,\beta)$ with
$x\in\reals^d$ and $\beta\in\reals$. Then:
\begin{enumerate}[leftmargin=*]
\item\label{item:deterministic_coordinate:transport}
\emph{Optimal transport.} For every
$\boldsymbol{\varGeneric}\in\Pp{2}{\reals^{d+1}}$, with
$\varGeneric\coloneqq\pushforward{(\projection{1}{},\ldots,\projection{d}{})}{\boldsymbol{\varGeneric}}\in\Pp{2}{\reals^d}$,
every
$\boldsymbol{\varPlanGeneric}\in\setPlans{\varFixed\times\delta_b}{\boldsymbol{\varGeneric}}$
satisfies
$\pushforward{T}{\boldsymbol{\varPlanGeneric}}\in\setPlans{\varFixed}{\varGeneric}$
and
\begin{equation*}
\int_{\reals^{d+1}\times\reals^{d+1}}\norm{\boldsymbol{x}'-\boldsymbol{x}}^2\d\boldsymbol{\varPlanGeneric}(\boldsymbol{x},\boldsymbol{x}')
=
\int_{\reals^{d}\times\reals^{d}}\norm{x'-x}^2\d(\pushforward{T}{\boldsymbol{\varPlanGeneric}})(x,x')
+
\int_{\reals^{d+1}}\abs{\beta'-b}^2\d\boldsymbol{\varGeneric}(x',\beta'),
\end{equation*}
where the last term does not depend on $\boldsymbol{\varPlanGeneric}$. In
particular,
$\wassersteinDistance{\varFixed\times\delta_b}{\boldsymbol{\varGeneric}}{2}^2=\wassersteinDistance{\varFixed}{\varGeneric}{2}^2+\int_{\reals^{d+1}}\abs{\beta'-b}^2\d\boldsymbol{\varGeneric}(x',\beta')$;
$\boldsymbol{\varPlanGeneric}\in\setPlansOptimal{\varFixed\times\delta_b}{\boldsymbol{\varGeneric}}$
if and only if
$\pushforward{T}{\boldsymbol{\varPlanGeneric}}\in\setPlansOptimal{\varFixed}{\varGeneric}$;
and every $\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varGeneric}$ is of
the form $\pushforward{T}{\boldsymbol{\varPlanGeneric}}$ for some
$\boldsymbol{\varPlanGeneric}\in\setPlansOptimal{\varFixed\times\delta_b}{\boldsymbol{\varGeneric}}$.
If, additionally, $\boldsymbol{\varGeneric}=\varGeneric\times\delta_\beta$
for some $\beta\in\reals$, then
\begin{equation*}
\setPlansOptimal{\varFixed\times\delta_b}{\varGeneric\times\delta_\beta}
=
\left\{
\pushforward{(\projection{1}{},b,\projection{2}{},\beta)}{\varPlanGeneric}
\st
\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varGeneric}
\right\},
\end{equation*}
and every variation in
$\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varFixed\times\delta_b}{\varGeneric\times\delta_\beta}}$
has last velocity component almost everywhere equal to $\beta-b$.
\item\label{item:deterministic_coordinate:tangency}
\emph{Tangency.} A variation $\boldsymbol{\varTangent}$ at
$\varFixed\times\delta_b$ satisfies
$\boldsymbol{\varTangent}\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varFixed\times\delta_b}$
if and only if
$\pushforward{T}{\boldsymbol{\varTangent}}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.
Moreover, $\pushforward{T}{\cdot}$ is $1$-Lipschitz: for all variations
$\boldsymbol{\varTangent}_1,\boldsymbol{\varTangent}_2$ at
$\varFixed\times\delta_b$,
$\wassersteinDistance{\pushforward{T}{\boldsymbol{\varTangent}_1}}{\pushforward{T}{\boldsymbol{\varTangent}_2}}{\varFixed}\leq\wassersteinDistance{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_2}{\varFixed\times\delta_b}$
and, for all
$\boldsymbol{\varTangent}_1,\boldsymbol{\varTangent}_2\in\Pp{2}{\reals^{d+1}\times\reals^{d+1}}$,
$\wassersteinDistance{\pushforward{T}{\boldsymbol{\varTangent}_1}}{\pushforward{T}{\boldsymbol{\varTangent}_2}}{2}\leq\wassersteinDistance{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_2}{2}$.
\item\label{item:deterministic_coordinate:splitting}
\emph{Norm and inner product.} Let $\boldsymbol{\varTangentOther}$ be a
variation at $\varFixed\times\delta_b$ whose last velocity component is
almost everywhere equal to some $c\in\reals$. Then,
$\norm{\boldsymbol{\varTangentOther}}_{\varFixed\times\delta_b}^2=\norm{\pushforward{T}{\boldsymbol{\varTangentOther}}}_{\varFixed}^2+c^2$
and, for every variation $\boldsymbol{\varTangent}$ at
$\varFixed\times\delta_b$,
\begin{equation}
\label{eq:deterministic_coordinate:splitting}
\innerProduct{\boldsymbol{\varTangent}}{\boldsymbol{\varTangentOther}}_{\varFixed\times\delta_b}
=
\innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\pushforward{T}{\boldsymbol{\varTangentOther}}}_{\varFixed}
+
c\,\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}.
\end{equation}
\end{enumerate}
}


==> elements/lemma_deterministic_coordinate_proof.tex <==
{%
Throughout, we use that the last coordinate of the first marginal of any
transport plan out of, and of any variation at, $\varFixed\times\delta_b$ is
almost everywhere equal to $b$. We prove the three statements separately.

\emph{Proof of \ref{item:deterministic_coordinate:transport}.} The marginals
of $\pushforward{T}{\boldsymbol{\varPlanGeneric}}$ are
$\pushforward{(\projection{1}{},\ldots,\projection{d}{})}{(\varFixed\times\delta_b)}=\varFixed$
and $\varGeneric$, so
$\pushforward{T}{\boldsymbol{\varPlanGeneric}}\in\setPlans{\varFixed}{\varGeneric}$.
Since $\beta=b$ for $\boldsymbol{\varPlanGeneric}$-almost every
$((x,\beta),(x',\beta'))$, we have
$\norm{\boldsymbol{x}'-\boldsymbol{x}}^2=\norm{x'-x}^2+\abs{\beta'-b}^2$
$\almostEverywhere{\boldsymbol{\varPlanGeneric}}$, and integrating yields the
displayed identity, where the last term equals
$\int_{\reals^{d+1}}\abs{\beta'-b}^2\d\boldsymbol{\varGeneric}(x',\beta')$ by
the marginal constraint and, in particular, does not depend on
$\boldsymbol{\varPlanGeneric}$. Hence, the cost of every
$\boldsymbol{\varPlanGeneric}\in\setPlans{\varFixed\times\delta_b}{\boldsymbol{\varGeneric}}$
is at least
$\wassersteinDistance{\varFixed}{\varGeneric}{2}^2+\int_{\reals^{d+1}}\abs{\beta'-b}^2\d\boldsymbol{\varGeneric}(x',\beta')$.
The bound is attained: let
$\{\boldsymbol{\varGeneric}_{x'}\}_{x'\in\reals^d}\subseteq\Pp{2}{\reals}$ be
the disintegration of $\boldsymbol{\varGeneric}$ with respect to $\varGeneric$
(cf. \cite[Theorem 5.3.1]{ambrosio2005gradient}) and, for
$\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varGeneric}$, let
$\boldsymbol{\varPlanGeneric}$ be the law of $((x,b),(x',\beta'))$ under
$\d\boldsymbol{\varGeneric}_{x'}(\beta')\d\varPlanGeneric(x,x')$. Then,
$\boldsymbol{\varPlanGeneric}\in\setPlans{\varFixed\times\delta_b}{\boldsymbol{\varGeneric}}$
with $\pushforward{T}{\boldsymbol{\varPlanGeneric}}=\varPlanGeneric$, and its
cost attains the lower bound. This proves the expression for
$\wassersteinDistance{\varFixed\times\delta_b}{\boldsymbol{\varGeneric}}{2}^2$,
and, with it, both the optimality equivalence (the cost of
$\boldsymbol{\varPlanGeneric}$ is minimal if and only if the cost of
$\pushforward{T}{\boldsymbol{\varPlanGeneric}}$ is) and the attainment of
every $\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varGeneric}$ as a
projection. If $\boldsymbol{\varGeneric}=\varGeneric\times\delta_\beta$, the
only transport plan of $\delta_b$ and $\delta_\beta$ is $\delta_{(b,\beta)}$, so
every
$\boldsymbol{\varPlanGeneric}\in\setPlans{\varFixed\times\delta_b}{\varGeneric\times\delta_\beta}$
equals
$\pushforward{(\projection{1}{},b,\projection{2}{},\beta)}{(\pushforward{T}{\boldsymbol{\varPlanGeneric}})}$;
combined with the optimality equivalence, this yields the characterization of
$\setPlansOptimal{\varFixed\times\delta_b}{\varGeneric\times\delta_\beta}$.
Finally, the variation induced by such a
$\boldsymbol{\varPlanGeneric}$ has last velocity component $\beta-b$ almost
surely, since the last coordinates of the two marginals are almost everywhere $b$
and $\beta$, respectively.

\emph{Proof of \ref{item:deterministic_coordinate:tangency}.} We start with
the $1$-Lipschitz bounds. For the first, let
$\boldsymbol{\varTangentCoupling}\in\setPlansCommonMarginal{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_2}{1}$:
dropping the last component of the anchor and of the two velocities maps
$\boldsymbol{\varTangentCoupling}$ to an element of
$\setPlansCommonMarginal{\pushforward{T}{\boldsymbol{\varTangent}_1}}{\pushforward{T}{\boldsymbol{\varTangent}_2}}{1}$
whose cost is no larger, since
$\norm{\varTangentReals_1-\varTangentReals_2}^2\leq\norm{\boldsymbol{\varTangentReals}_1-\boldsymbol{\varTangentReals}_2}^2$;
minimizing over $\boldsymbol{\varTangentCoupling}$ yields the bound. The
second bound is analogous, using that $T$ is a coordinate projection and,
thus, $1$-Lipschitz, so any coupling of $\boldsymbol{\varTangent}_1$ and
$\boldsymbol{\varTangent}_2$ pushes forward, via $T$ applied to both
components, to a coupling of the images with no larger cost.

Next, observe that, since $T$ drops the last component of positions and
velocities alike, for every variation $\boldsymbol{\varTangent}$ at
$\varFixed\times\delta_b$ and every $\varepsilon\geq0$, dropping the last
coordinate of both marginals of
$\pushforward{(\projection{1}{},\projection{1}{}+\varepsilon\projection{2}{})}{\boldsymbol{\varTangent}}$
yields
$\pushforward{(\projection{1}{},\projection{1}{}+\varepsilon\projection{2}{})}{(\pushforward{T}{\boldsymbol{\varTangent}})}$.
By the optimality equivalence in
\ref{item:deterministic_coordinate:transport},
$\pushforward{(\projection{1}{},\projection{1}{}+\varepsilon\projection{2}{})}{\boldsymbol{\varTangent}}$
is optimal if and only if
$\pushforward{(\projection{1}{},\projection{1}{}+\varepsilon\projection{2}{})}{(\pushforward{T}{\boldsymbol{\varTangent}})}$
is. Hence, $\boldsymbol{\varTangent}$ belongs to the set in
\eqref{definition:tangent_space} (with base point $\varFixed\times\delta_b$)
if and only if $\pushforward{T}{\boldsymbol{\varTangent}}$ belongs to the set
in \eqref{definition:tangent_space} (with base point $\varFixed$).

For the ``only if'' direction of the tangency claim, let
$\boldsymbol{\varTangent}\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varFixed\times\delta_b}$
and let $(\boldsymbol{\varTangent}_k)_{k\in\naturals}$ in the set in
\eqref{definition:tangent_space} with
$\wassersteinDistance{\boldsymbol{\varTangent}_k}{\boldsymbol{\varTangent}}{\varFixed\times\delta_b}\to0$.
Then, $\pushforward{T}{\boldsymbol{\varTangent}_k}$ belongs to the set in
\eqref{definition:tangent_space} by the previous paragraph, and
$\wassersteinDistance{\pushforward{T}{\boldsymbol{\varTangent}_k}}{\pushforward{T}{\boldsymbol{\varTangent}}}{\varFixed}\to0$
by the first $1$-Lipschitz bound, so
$\pushforward{T}{\boldsymbol{\varTangent}}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.

For the ``if'' direction, let
$\varTangent\coloneqq\pushforward{T}{\boldsymbol{\varTangent}}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$
and let
$(\varTangent_k)_{k\in\naturals}\subseteq\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed}$
with $\wassersteinDistance{\varTangent_k}{\varTangent}{\varFixed}\to0$; such a
sequence exists because the tangent space is the
$\wassersteinDistance{}{}{\varFixed}$-closure of the set in
\eqref{definition:tangent_space}. Since the last position component of
$\boldsymbol{\varTangent}$ is deterministic, $\boldsymbol{\varTangent}$ is
characterized by the law of $((x,\varTangentReals),u)$, where
$(x,\varTangentReals)\sim\varTangent$ and $u\in\reals$ denotes the last
velocity component; let
$\{\boldsymbol{\varTangent}_{(x,\varTangentReals)}\}_{(x,\varTangentReals)\in\reals^d\times\reals^d}\subseteq\Pp{2}{\reals}$
be the disintegration of this law with respect to $(x,\varTangentReals)$ (cf.
\cite[Theorem 5.3.1]{ambrosio2005gradient}). For each $k$, let
$\varTangentCoupling_k\in\setPlansCommonMarginal{\varTangent}{\varTangent_k}{1}$
attain $\wassersteinDistance{\varTangent}{\varTangent_k}{\varFixed}$, define
$\hat{\varTangentCoupling}_k$ via
$\d\hat{\varTangentCoupling}_k(x,\varTangentReals,\varTangentReals_k,u)\coloneqq\d\boldsymbol{\varTangent}_{(x,\varTangentReals)}(u)\d\varTangentCoupling_k(x,\varTangentReals,\varTangentReals_k)$,
and let $\boldsymbol{\varTangent}_k$ be the law of
$((x,b),(\varTangentReals_k,u))$ under $\hat{\varTangentCoupling}_k$. Then,
$\boldsymbol{\varTangent}_k$ is a variation at $\varFixed\times\delta_b$ with
$\pushforward{T}{\boldsymbol{\varTangent}_k}=\varTangent_k$ in the set in
\eqref{definition:tangent_space} and, thus, $\boldsymbol{\varTangent}_k$
belongs to the set in \eqref{definition:tangent_space} by the equivalence
above.
{Moreover, let $\boldsymbol{\varTangentCoupling}_k$ be the law
of $((x,b),(\varTangentReals_k,u),(\varTangentReals,u))$ under
$\hat{\varTangentCoupling}_k$, i.e., the pushforward of
$\hat{\varTangentCoupling}_k$ under the map
$(x,\varTangentReals,\varTangentReals_k,u)\mapsto((x,b),(\varTangentReals_k,u),(\varTangentReals,u))$
from $\reals^d\times\reals^d\times\reals^d\times\reals$ to
$\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}$. Writing
$\boldsymbol{\varTangentReals}_k\coloneqq(\varTangentReals_k,u)$ and
$\boldsymbol{\varTangentReals}\coloneqq(\varTangentReals,u)$ for the two
velocity slots, which share the last coordinate $u$, the
$((x,b),\boldsymbol{\varTangentReals}_k)$-marginal of
$\boldsymbol{\varTangentCoupling}_k$ is $\boldsymbol{\varTangent}_k$ by the
definition of $\boldsymbol{\varTangent}_k$, and its
$((x,b),\boldsymbol{\varTangentReals})$-marginal is
$\boldsymbol{\varTangent}$, since the $(x,\varTangentReals)$-marginal of
$\varTangentCoupling_k$ is $\varTangent$ and the kernel
$\boldsymbol{\varTangent}_{(x,\varTangentReals)}$ does not depend on
$\varTangentReals_k$. Hence,
$\boldsymbol{\varTangentCoupling}_k\in\setPlansCommonMarginal{\boldsymbol{\varTangent}_k}{\boldsymbol{\varTangent}}{1}$
and
\begin{equation*}
\begin{aligned}
\wassersteinDistance{\boldsymbol{\varTangent}_k}{\boldsymbol{\varTangent}}{\varFixed\times\delta_b}^2
&\leq
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}\norm{\boldsymbol{\varTangentReals}_k-\boldsymbol{\varTangentReals}}^2\d\boldsymbol{\varTangentCoupling}_k(\boldsymbol{x},\boldsymbol{\varTangentReals}_k,\boldsymbol{\varTangentReals})
\\&=
\int_{\reals^d\times\reals^d\times\reals^d\times\reals}\norm{\varTangentReals_k-\varTangentReals}^2\d\hat{\varTangentCoupling}_k(x,\varTangentReals,\varTangentReals_k,u)
=
\wassersteinDistance{\varTangent_k}{\varTangent}{\varFixed}^2
\to0,
\end{aligned}
\end{equation*}
where the first equality is the change of variables defining
$\boldsymbol{\varTangentCoupling}_k$ together with
$\norm{\boldsymbol{\varTangentReals}_k-\boldsymbol{\varTangentReals}}^2=\norm{\varTangentReals_k-\varTangentReals}^2$
(the shared $u$ cancels), and the second holds because the
$(x,\varTangentReals,\varTangentReals_k)$-marginal of
$\hat{\varTangentCoupling}_k$ is $\varTangentCoupling_k$, which attains
$\wassersteinDistance{\varTangent}{\varTangent_k}{\varFixed}$.}
Since the tangent space is
$\wassersteinDistance{}{}{\varFixed\times\delta_b}$-closed, we conclude
$\boldsymbol{\varTangent}\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varFixed\times\delta_b}$.

\emph{Proof of \ref{item:deterministic_coordinate:splitting}.} Since the last
position and velocity components of $\boldsymbol{\varTangentOther}$ are
deterministic, $\boldsymbol{\varTangentOther}$ is the law of $((x,b),(\varTangentReals,c))$ for
$(x,\varTangentReals)\sim\pushforward{T}{\boldsymbol{\varTangentOther}}$; in
particular,
$\norm{\boldsymbol{\varTangentOther}}_{\varFixed\times\delta_b}^2=\norm{\pushforward{T}{\boldsymbol{\varTangentOther}}}_{\varFixed}^2+c^2$.
For the inner product, let
$\boldsymbol{\varTangentCoupling}\in\setPlansCommonMarginal{\boldsymbol{\varTangent}}{\boldsymbol{\varTangentOther}}{1}$
and write the two velocities as $(\varTangentReals_1,u_1)$ and
$(\varTangentReals_2,u_2)$. Then, $u_2=c$ almost everywhere, so
\begin{align*}
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}&\innerProduct{\boldsymbol{\varTangentReals}_1}{\boldsymbol{\varTangentReals}_2}\d\boldsymbol{\varTangentCoupling}(\boldsymbol{x},\boldsymbol{\varTangentReals}_1,\boldsymbol{\varTangentReals}_2)
\\&=
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}\innerProduct{\varTangentReals_1}{\varTangentReals_2}\d\boldsymbol{\varTangentCoupling}(\boldsymbol{x},\boldsymbol{\varTangentReals}_1,\boldsymbol{\varTangentReals}_2)
+
c\,\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}},
\end{align*}
where the second term does not depend on
$\boldsymbol{\varTangentCoupling}$. Dropping the last component of the anchor
and of the two velocities maps $\boldsymbol{\varTangentCoupling}$ to an
element of
$\setPlansCommonMarginal{\pushforward{T}{\boldsymbol{\varTangent}}}{\pushforward{T}{\boldsymbol{\varTangentOther}}}{1}$
with the same value of the first term; conversely, every
$\varTangentCoupling\in\setPlansCommonMarginal{\pushforward{T}{\boldsymbol{\varTangent}}}{\pushforward{T}{\boldsymbol{\varTangentOther}}}{1}$
lifts to an admissible $\boldsymbol{\varTangentCoupling}$ with the same value
of the first term: with
$\{\boldsymbol{\varTangent}_{(x,\varTangentReals_1)}\}_{(x,\varTangentReals_1)\in\reals^d\times\reals^d}\subseteq\Pp{2}{\reals}$
the disintegration, with respect to $(x,\varTangentReals_1)$, of the law of
$((x,\varTangentReals_1),u_1)$ under $\boldsymbol{\varTangent}$, take the law
of $((x,b),(\varTangentReals_1,u_1),(\varTangentReals_2,c))$ under
$\d\boldsymbol{\varTangent}_{(x,\varTangentReals_1)}(u_1)\d\varTangentCoupling(x,\varTangentReals_1,\varTangentReals_2)$.
Taking the maximum over the couplings yields
\eqref{eq:deterministic_coordinate:splitting}.
}


==> elements/lemma_deterministic_coordinate_title.tex <==
Splitting off a deterministic coordinate%


==> elements/lemma_fuzzy_optimality_condition_body.tex <==
Let $\Omega_1,\Omega_2\subseteq\Pp{2}{\reals^d}$ be nonempty sets and let $(\varFixed_1,\varFixed_2)\in\Omega_1\times\Omega_2$, $\varepsilon>0$, and $a\in\reals^d$ with $\pushforward{(\identity{}+a)}{\varFixed_1}\neq\varFixed_2$, so that $c\coloneqq\wassersteinDistance{\pushforward{(\identity{}+a)}{\varFixed_1}}{\varFixed_2}{2}>0$.
%
Consider sequences $((\tilde\varGeneric_{1,j},\tilde\varGeneric_{2,j}))_{j\in\naturals}\subseteq\Omega_1\times\Omega_2$ so that 
    $\wassersteinDistance{\varFixed_i}{\tilde\varGeneric_{i,j}}{2}^2\leq\frac{2^{-j}}{4}\varepsilon^2$.
Suppose that $(\varFixed_1,\varFixed_2)$ is a local minimizer of 
\begin{equation*}
    \psi(\varGeneric_1,\varGeneric_2)
    \coloneqq
    \wassersteinDistance{\pushforward{(\identity{}+a)}\varGeneric_1}{\varGeneric_2}{2}
    +
    \frac{1}{2}
    \sum_{j=0}^\infty
    2^{-j}
    \left(\wassersteinDistance{\varGeneric_1}{\tilde\varGeneric_{1,j}}{2}^2
    +\wassersteinDistance{\varGeneric_2}{\tilde\varGeneric_{2,j}}{2}^2\right)
\end{equation*}
relative to the set $\Omega_1\times\Omega_2$.
%
{Then, there is an optimal transport plan $\varPlanGeneric\in\setPlansOptimal{\varFixed_1}{\varFixed_2}$ so that
$
    \varTangent_1\coloneqq\tfrac1c\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{}-a)}{\varPlanGeneric}\in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed_1}
$
and
$
    \varTangent_2\coloneqq\tfrac1c\pushforward{(\projection{2}{},\projection{1}{}-\projection{2}{}+a)}{\varPlanGeneric}\in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed_2},
$
with $\norm{\varTangent_1}_{\varFixed_1}=\norm{\varTangent_2}_{\varFixed_2}=1$, are $\varepsilon$-close with respect to $\wassersteinDistance{}{}{\varFixed_i}$ to the strong regular normal cones $\normalConeRegularStrong{\Omega_1}{\varFixed_1}$ and $\normalConeRegularStrong{\Omega_2}{\varFixed_2}$, respectively.
In particular, there is $\varPlanGeneric_{\varTangent}\in\setPlans{\varTangent_1}{\varTangent_2}$ with $\pushforward{(\projection{1}{},\projection{3}{})}{\varPlanGeneric_{\varTangent}}=\varPlanGeneric$ such that
$\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d}\norm{\varTangentReals_1+\varTangentReals_2}^2\d\varPlanGeneric_{\varTangent}(x_1,\varTangentReals_1,x_2,\varTangentReals_2)=0$.}


==> elements/lemma_fuzzy_optimality_condition_proof.tex <==
Fix $\varPlanGeneric\in\setPlansOptimal{\varFixed_1}{\varFixed_2}$ and let $c$, $\varTangent_1$, and $\varTangent_2$ be as in the statement; we show they enjoy the asserted properties (so, in particular, such a transport plan and such variations exist). Write $W_2^a(\varGeneric_1,\varGeneric_2)\coloneqq\wassersteinDistance{\pushforward{(\identity{}+a)}{\varGeneric_1}}{\varGeneric_2}{2}$ for the separation, so that $c=W_2^a(\varFixed_1,\varFixed_2)$. We proceed in six steps.

{\emph{Step 1 (Unit norm and tangent-cone membership).}
We start with the norm.
Since the shift by the constant $a$ preserves cyclical monotonicity of the support, $\pushforward{(\projection{1}{}+a,\projection{2}{})}{\varPlanGeneric}$ is optimal between $\pushforward{(\identity{}+a)}{\varFixed_1}$ and $\varFixed_2$, whence $\norm{c\varTangent_1}_{\varFixed_1}=\norm{c\varTangent_2}_{\varFixed_2}=W_2^a(\varFixed_1,\varFixed_2)=c$; that is, $\norm{\varTangent_1}_{\varFixed_1}=\norm{\varTangent_2}_{\varFixed_2}=1$.}
%
{We now show that $\varTangent_1\in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed_1}$;
the proof for $\varTangent_2$ is analogous.
Since $\varPlanGeneric$ is optimal, it is supported on the subdifferential of a convex function $\phi$.
Then, the transport plan $\pushforward{(\projection{1}{},\projection{1}{}+\tau\projection{2}{})}{\varTangent_1}
=
\pushforward{(\projection{1}{}, (1-\tfrac{\tau}{c})\projection{1}{}+\tfrac{\tau}{c}\projection{2}{}-\tfrac{\tau}{c}a)}{\varPlanGeneric}
$
is supported on the subdifferential of the function $x\mapsto \frac{1-\tau/c}{2}\norm{x}^2 + \tfrac{\tau}{c}\phi(x) - \tfrac{\tau}{c}\innerProduct{a}{x}$, which is clearly convex for all $\tau\in[0,c)$, which proves optimality of $\pushforward{(\projection{1}{},\projection{1}{}+\tau\projection{2}{})}{\varTangent_1}$ between its marginals for all $\tau$ sufficiently small and, with it, that $\varTangent_1\in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed_1}$.}

\emph{Step 2 (Cancellation).}
Let
$
    \varPlanGeneric_{\varTangent}
    \coloneqq
    \pushforward{(\projection{1}{},\tfrac1c(\projection{2}{}-\projection{1}{}-a),\projection{2}{},\tfrac1c(\projection{1}{}-\projection{2}{}+a))}{\varPlanGeneric}.
$
By construction, $\varPlanGeneric_{\varTangent}\in\setPlans{\varTangent_1}{\varTangent_2}$ and $\pushforward{(\projection{1}{},\projection{3}{})}{\varPlanGeneric_{\varTangent}}=\varPlanGeneric\in\setPlansOptimal{\varFixed_1}{\varFixed_2}$. Moreover,
    $\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d} \norm{\varTangentReals_1+\varTangentReals_2}^2\d\varPlanGeneric_{\varTangent}(x_1,\varTangentReals_1,x_2,\varTangentReals_2)
    =
    \tfrac{1}{c^2}\int_{\reals^d\times\reals^d}
    \norm{-(x_1-x_2+a)-(x_2-x_1-a)}^2\d\varPlanGeneric(x_1,x_2)
    =0$.

\emph{Step 3 (The candidate normal $\varTangentFixed$).}
Let $\varTangent_{i,j} \in -\pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\setPlansOptimal{\varFixed_i}{\tilde\varGeneric_{i,j}}}$ for $i \in \{1,  2\}, j \in \naturals$.
%
By~\cref{proposition:prop_wassersteindistance_regular_subgradient_must_be_plan}, we have that $\varTangent_{i,j}\in\subgradientRegular{\left(-\frac{1}{2}\wassersteinDistance{\cdot}{\tilde\varGeneric_{i,j}}{2}^2\right)}(\varFixed_i)$. {Define
    $\varTangentFixed \coloneqq (\varTangent_1+\sum_{j=0}^\infty2^{-j}\varTangent_{1,j},\varTangent_2+\sum_{j=0}^\infty2^{-j}\varTangent_{2,j})$}
where, for simplicity of notation, we omit the sum couplings in {$\setPlansCommonMarginal{\varTangent_i}{\varTangent_{i,0},\varTangent_{i,1},\varTangent_{i,2},\ldots}{1}$, $i\in\{1, 2\}$.
Since $\norm{\varTangent_{i,j}}_{\varFixed_i}=\wassersteinDistance{\varFixed_i}{\tilde\varGeneric_{i,j}}{2}\leq\tfrac{\varepsilon}{2}2^{-j/2}$, $\varTangentFixed$ is well defined, as detailed below.}

{\emph{Step~4} ($\varTangentFixed$ belongs to the tangent space).
We show that the first component $\varTangentFixed_1=\varTangent_1+\sum_{j=0}^\infty 2^{-j}\varTangent_{1,j}$ lies in $\tangentCone{\Pp{2}{\reals^d}}{\varFixed_1}$; the argument for $\varTangentFixed_2$ is identical.
By Step~1, it suffices to exhibit, for all sufficiently small $\tau\geq0$, a convex function whose subdifferential supports the transport plan $\pushforward{(\projection{1}{},\projection{1}{}+\tau\projection{2}{})}{\varTangentFixed_1}$, as this renders the transport plan optimal.
Each constituent variation is induced by an optimal transport plan: $\varTangent_1=\tfrac1c\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{}-a)}{\varPlanGeneric}$ with $\varPlanGeneric\in\setPlansOptimal{\varFixed_1}{\varFixed_2}$ supported on $\partial\phi$, and $\varTangent_{1,j}=\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\varPlanGeneric_j}$ with $\varPlanGeneric_j\in\setPlansOptimal{\varFixed_1}{\tilde\varGeneric_{1,j}}$ supported on $\partial\phi_j$, where $\phi$ and the $\phi_j$ are convex.
Gluing $\varPlanGeneric$ and the $\varPlanGeneric_j$ along $\varFixed_1$ yields the sum coupling $\varTangentCoupling_1^\star\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_{1,0},\varTangent_{1,1},\ldots}{1}$ of Step~3, a law of tuples $(x,x_2,y_0,y_1,\ldots)\in\reals^d\times\reals^d\times(\times_{j=0}^\infty\reals^d)$ with first marginal $\varFixed_1$, $(x,x_2)\in\supp\varPlanGeneric$, and $(x,y_j)\in\supp\varPlanGeneric_j$ for every $j$. Thus, $x_2\in\partial\phi(x)$ and $y_j\in\partial\phi_j(x)$, and the arrows of $\varTangent_1$ and $\varTangent_{1,j}$ over $x$ are $\tfrac1c(x_2-x-a)$ and $y_j-x$.
%
We now proceed in two steps.
First, we show that the series $\sum_{j=0}^\infty 2^{-j}\phi_j$ is a proper convex function.
Normalize each $\phi_j$ by $\phi_j(x_0)=0$ at a base point $x_0\in\supp\varFixed_1$ carrying support points $(x_0,y_{j,0})\in\supp\varPlanGeneric_j$ with $\sum_{j=0}^\infty 2^{-j}\norm{y_{j,0}}<\infty$; such an $x_0$ exists because $\int_{\reals^d\times\reals^d\times(\times_{j=0}^\infty\reals^d)}\sum_{j=0}^\infty 2^{-j}\norm{y_j-x}\d\varTangentCoupling_1^\star(x,x_2,y_0,y_1,\ldots)=\sum_{j=0}^\infty 2^{-j}\int_{\reals^d\times\reals^d}\norm{v}\d\varTangent_{1,j}(x,v)\leq\sum_{j=0}^\infty 2^{-j}\norm{\varTangent_{1,j}}_{\varFixed_1}<\infty$, where the equality marginalizes $\varTangentCoupling_1^\star$ onto each $\varTangent_{1,j}$ and the inequality is Jensen's ($L^1\leq L^2$). Hence, $\sum_{j=0}^\infty 2^{-j}\norm{y_j-x}<\infty$ $\almostEverywhere{\varTangentCoupling_1^\star}$, and so $\sum_{j=0}^\infty 2^{-j}\norm{y_{j,0}}\leq\sum_{j=0}^\infty 2^{-j}\norm{y_{j,0}-x_0}+2\norm{x_0}<\infty$ for $\varTangentCoupling_1^\star$-almost every $(x_0,y_{0,0},y_{1,0},\ldots)$.
The subgradient inequality then gives $\phi_j(z)\geq\phi_j(x_0)+\innerProduct{y_{j,0}}{z-x_0}\geq-\norm{y_{j,0}}\norm{z-x_0}$ for all $z\in\reals^d$, whence $\sum_{j=0}^\infty 2^{-j}\phi_j(z)\geq-\bigl(\sum_{j=0}^\infty 2^{-j}\norm{y_{j,0}}\bigr)\norm{z-x_0}>-\infty$. As the series vanishes at $x_0$, it is a proper convex function.
%
Second, we construct the desired convex function.
The arrow of $\varTangentFixed_1$ is $w=\tfrac1c(x_2-x-a)+\sum_{j=0}^\infty 2^{-j}(y_j-x)$ $\almostEverywhere{\varTangentCoupling_1^\star}$, and for $\tau\in[0,\tfrac{c}{1+2c}]$ we set $h_\tau\coloneqq\tfrac{1-\tau(\tfrac1c+2)}{2}\norm{\cdot}^2+\tfrac{\tau}{c}\phi+\tau\sum_{j=0}^\infty 2^{-j}\phi_j-\tfrac{\tau}{c}\innerProduct{a}{\cdot}$.
Since $\sum_{j=0}^\infty 2^{-j}\norm{y_j-x}<\infty$, summing the subgradient inequalities of the $\phi_j$ weighted by $2^{-j}$ gives $\sum_{j=0}^\infty 2^{-j}y_j\in\partial(\sum_{j=0}^\infty 2^{-j}\phi_j)(x)$.
With $x_2\in\partial\phi(x)$ this yields $x+\tau w=\bigl(1-\tau(\tfrac1c+2)\bigr)x+\tfrac{\tau}{c}x_2+\tau\sum_{j=0}^\infty 2^{-j}y_j-\tfrac{\tau}{c}a\in\partial h_\tau(x)$.
Moreover, $h_\tau$ is proper and convex, its quadratic coefficient $1-\tau(\tfrac1c+2)$ being nonnegative for $\tau\leq\tfrac{c}{1+2c}$ (note $\tfrac1c+\sum_{j=0}^\infty 2^{-j}=\tfrac1c+2$) and $\phi,\sum_{j=0}^\infty 2^{-j}\phi_j$ proper convex.
Hence $\pushforward{(\projection{1}{},\projection{1}{}+\tau\projection{2}{})}{\varTangentFixed_1}$ is supported on $\partial h_\tau$ and thus optimal for every $\tau\in[0,\tfrac{c}{1+2c}]$, so $\varTangentFixed_1\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed_1}$.
The same argument gives $\varTangentFixed_2\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed_2}$.}

\emph{Step 5 ($\varTangentFixed$ is a strong regular normal to $\Omega_1\times\Omega_2$).}
By Step~4, $\varTangentFixed\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed_1}\times\tangentCone{\Pp{2}{\reals^d}}{\varFixed_2}$, so by the definition of strong regular normal cone (cf. \cref{definition:def_fuzzy_normal_cone}) it remains to verify that $\varTangentFixed$ satisfies the defining inequality of $\normalConeRegularStrong{\Omega_1\times\Omega_2}{(\varFixed_1,\varFixed_2)}$.
{For $\Omega_1\times\Omega_2\subseteq\Pp{2}{\reals^d}\times\Pp{2}{\reals^d}$, the strong regular normal cone of \cref{definition:def_fuzzy_normal_cone} is understood componentwise, with $\innerProduct{\varTangentFixed}{\varTangentFixed'}_{(\varFixed_1,\varFixed_2)}\coloneqq\innerProduct{\varTangentFixed_1}{\varTangentFixed_1'}_{\varFixed_1}+\innerProduct{\varTangentFixed_2}{\varTangentFixed_2'}_{\varFixed_2}$ and $\norm{\varTangentFixed'}_{(\varFixed_1,\varFixed_2)}^2\coloneqq\norm{\varTangentFixed_1'}_{\varFixed_1}^2+\norm{\varTangentFixed_2'}_{\varFixed_2}^2$, where $\varTangentFixed=(\varTangentFixed_1,\varTangentFixed_2)$ denotes the two components of $\varTangentFixed$.
For this, consider any $\varTangentCoupling \in \Pp{2}{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}$, $\pushforward{(\projection{1}{}, \projection{3}{})}{\varTangentCoupling} = \varTangentFixed_1$, $\pushforward{(\projection{2}{}, \projection{4}{})}{\varTangentCoupling} = \varTangentFixed_2$, $\pushforward{(\projection{1}{} + \projection{5}{})}{\varTangentCoupling}\eqqcolon\varGeneric_1 \in \Omega_1$, $\pushforward{(\projection{2}{} + \projection{6}{})}{\varTangentCoupling}\eqqcolon\varGeneric_2\in \Omega_2$.
%
We want to show that
\begin{align*}
\heartsuit
\coloneqq
&\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\innerProduct{\bar{\varTangentReals}_1}{\varTangentReals_1'}
+
\innerProduct{\bar{\varTangentReals}_2}{\varTangentReals_2'}
\d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2')
\\
&\qquad\leq
\left(\tfrac1c+2\right)
\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\norm{\varTangentReals_1'}^2 + \norm{\varTangentReals_2'}^2
\d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2'),
\end{align*}%
whenever the right-hand side is sufficiently small.
We now define $\varTangentCoupling_{\infty} \in \Pp{2}{\reals^d\times\reals^d\times\reals^d\times(\times_{j=0}^\infty\reals^d)\times\reals^d\times(\times_{j=0}^\infty\reals^d)\times\reals^d\times\reals^d}$ with marginals $\varTangent_i, \varTangent_{i,j}, i\in\{1, 2\}, j \in\naturals$.
For this, we extend each sum coupling in $\setPlansCommonMarginal{\varTangent_i}{\varTangent_{i,0},\varTangent_{i,1},\ldots}{1}$ by the coordinate $\bar\varTangentReals_i\coloneqq\varTangentReals_i+\sum_{j=0}^\infty 2^{-j}\varTangentReals_{i,j}$ and glue it to $\varTangentCoupling$ along the common marginal given by the $i$-th component of $\varTangentFixed$, i.e., the joint law of $(\bar x_i,\bar\varTangentReals_i)$; the countably many coordinates are handled via the Kolmogorov extension theorem as in \cref{remark:rem_lemma_pushforward_and_optimal_transport}.
This coupling satisfies
\begin{align*}
\heartsuit
&=
\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\innerProduct{\bar{\varTangentReals}_1}{\varTangentReals_1'}
+
\innerProduct{\bar{\varTangentReals}_2}{\varTangentReals_2'}
\d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2')
\\&=
\int_{\reals^d\times\reals^d\times(\times_{j=0}^\infty\reals^d)\times(\times_{j=0}^\infty\reals^d)\times\reals^d\times\reals^d}
\Biggl(
\innerProduct{\varTangentReals_1 + \sum_{j = 0}^\infty2^{-j}\varTangentReals_{1,j}}{\varTangentReals_1'}
\\&\qquad\qquad\qquad+
\innerProduct{\varTangentReals_2 + \sum_{j = 0}^\infty2^{-j}\varTangentReals_{2,j}}{\varTangentReals_2'}
\Biggr)
\d\varTangentCoupling_\infty(
\bar{x}_1, \bar{x}_2, \varTangentReals_1, \varTangentReals_{1,0}, \ldots, {\varTangentReals}_2, {\varTangentReals}_{2,0}, \ldots, {\varTangentReals}_1', {\varTangentReals}_2')
\\&=
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_1}{\varTangentReals_1'}
\d\varTangentCoupling_{1}(\bar{x}_1, \varTangentReals_1, \varTangentReals_1')
+
\sum_{j = 0}^\infty
2^{-j}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_{1,j}}{\varTangentReals_1'}
\d\varTangentCoupling_{1,j}(\bar{x}_1, \varTangentReals_{1,j}, \varTangentReals_1')
\\&+
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_2}{\varTangentReals_2'}
\d\varTangentCoupling_{2}(\bar{x}_2, \varTangentReals_2, \varTangentReals_2')
+
\sum_{j = 0}^\infty
2^{-j}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_{2,j}}{\varTangentReals_2'}
\d\varTangentCoupling_{2,j}(\bar{x}_2, \varTangentReals_{2,j}, \varTangentReals_2'),
\end{align*}
with $\varTangentCoupling_{i}, \varTangentCoupling_{i,j}, i\in\{1, 2\}$ marginalizations of $\varTangentCoupling_\infty$ so that $\pushforward{(\projection{1}{}, \projection{2}{})}{\varTangentCoupling_i} = \varTangent_i, \pushforward{(\projection{1}{} + \projection{3}{})}{\varTangentCoupling_i}=\varGeneric_i \in \Omega_i, \pushforward{(\projection{1}{}, \projection{2}{})}{\varTangentCoupling_{i,j}} = \varTangent_{i,j}, \pushforward{(\projection{1}{} + \projection{3}{})}{\varTangentCoupling_{i,j}}=\varGeneric_i\in\Omega_i$.
%
We start by upper bounding the terms in the infinite sum.
By~\cite[Theorem 10.2.2]{ambrosio2005gradient}, we have
\begin{align*}
    \frac{1}{2}\wassersteinDistance{\varGeneric}{\varReference}{2}^2
    &-
    \frac{1}{2}\wassersteinDistance{\varFixed}{\varReference}{2}^2
    +
    \int_{\reals^d\times\reals^d\times\reals^d}\innerProduct{x_2-x_1}{x_3-x_1}\d\theta(x_1,x_2,x_3)
    \\
    &\leq
    \int_{\reals^d\times\reals^d\times\reals^d} \norm{x_1-x_3}^2\d\theta(x_1,x_2,x_3)
\end{align*}
for all $\theta\in\setPlans{\varPlanGeneric}{\mu}$ and for every $\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varReference}$. With $\varReference=\tilde\varGeneric_{i,j}$, $\varFixed=\varFixed_i$, and $\varGeneric=\varGeneric_i$, we conclude
\begin{equation}\label{eq:proof_fuzzy_optimality_conditions:bound_ij}
\begin{aligned}
    \int_{\reals^d\times\reals^d\times\reals^d} &\innerProduct{\varTangentReals_{i,j}}{\varTangentReals_i'}
    \d\varTangentCoupling_{i,j}(\bar{x}_i, \varTangentReals_{i,j}, \varTangentReals_i')
    \\
    &\leq
    \frac{1}{2}\wassersteinDistance{\varFixed_i}{\tilde\varGeneric_{i,j}}{2}^2 -
    \frac{1}{2}\wassersteinDistance{\varGeneric_i}{\tilde\varGeneric_{i,j}}{2}^2
    +
    \int_{\reals^d\times\reals^d\times\reals^d}
    \norm{\varTangentReals_i'}^2
    \d\varTangentCoupling_{i,j}(\bar{x}_i, \varTangentReals_{i,j}, \varTangentReals_i').
\end{aligned}
\end{equation}
For the other two terms, we now prove
\begin{equation}\label{eq:proof_fuzzy_optimality_conditions:bound_joint_12}
\begin{aligned}
    \int_{\reals^d\times\reals^d\times\reals^d} &\innerProduct{\varTangentReals_{1}}{\varTangentReals_1'}
    \d\varTangentCoupling_{1}(\bar{x}_1, \varTangentReals_{1}, \varTangentReals_1')
    +
    \int_{\reals^d\times\reals^d\times\reals^d} \innerProduct{\varTangentReals_{2}}{\varTangentReals_2'}
    \d\varTangentCoupling_{2}(\bar{x}_2, \varTangentReals_{2}, \varTangentReals_2')
    \\
    &\leq
    \frac{1}{c}\left(\frac{1}{2}\wassersteinDistance{\pushforward{(\identity{}+a)}\varFixed_1}{\varFixed_2}{2}^2
    -
    \frac{1}{2}\wassersteinDistance{\pushforward{(\identity{}+a)}\varGeneric_1}{\varGeneric_2}{2}^2\right)
    \\
    &+
    \frac{1}{c}\int_{\reals^d\times\reals^d\times\reals^d}
    \norm{\varTangentReals_1'}^2
    \d\varTangentCoupling_{1}(\bar{x}_1, \varTangentReals_{1}, \varTangentReals_1')
    +
    \frac{1}{c}\int_{\reals^d\times\reals^d\times\reals^d}
    \norm{\varTangentReals_2'}^2
    \d\varTangentCoupling_{2}(\bar{x}_2, \varTangentReals_{2}, \varTangentReals_2').
\end{aligned}
\end{equation}
By definition of $\varTangent_i$, on the support of $\varTangent_i$, and so also on that of $\varTangentCoupling_i$, it holds $\varTangentReals_1 = \tfrac1c(\bar{x}_2 - \bar{x}_1 - a)$ and $\varTangentReals_2 = \tfrac1c(\bar{x}_1 - \bar{x}_2 + a)$ for $(\bar{x}_1,\bar{x}_2)$ in the support of $\varPlanGeneric \in \setPlansOptimal{\varFixed_1}{\varFixed_2}$.
In particular $\varTangentReals_2 = -\varTangentReals_1$ and $\bar{x}_1+a-\bar{x}_2=-c\varTangentReals_1=c\varTangentReals_2$, and the transport plan $\pushforward{(\projection{1}{}+a,\projection{2}{})}{\varPlanGeneric}$ is optimal between $\pushforward{(\identity{}+a)}{\varFixed_1}$ and $\varFixed_2$.
%
On $\supp\varTangent_1$ we have $\pushforward{(\projection{1}{},\projection{1}{}+a+c\projection{2}{})}{\varTangent_1}=\varPlanGeneric$, so augmenting $\varTangentCoupling_1$ with the deterministic coordinate $\bar{x}_2\coloneqq\bar{x}_1+a+c\varTangentReals_1$ and $\varTangentCoupling_2$ with $\bar{x}_1\coloneqq\bar{x}_2-a+c\varTangentReals_2$ produces two transport plans with common $(\bar{x}_1,\bar{x}_2)$-marginal $\varPlanGeneric$.
Gluing them along this joint marginal yields $\tilde\varTangentCoupling \in \Pp{2}{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}$, on which $\bar{x}_1+a-\bar{x}_2=-c\varTangentReals_1=c\varTangentReals_2$ holds almost everywhere by construction, such that
$\pushforward{(\projection{1}{},\projection{3}{},\projection{5}{})}{\tilde\varTangentCoupling} = \varTangentCoupling_1$,
$\pushforward{(\projection{2}{},\projection{4}{},\projection{6}{})}{\tilde\varTangentCoupling} = \varTangentCoupling_2$, and
$\pushforward{(\projection{1}{},\projection{2}{})}{\tilde\varTangentCoupling} = \varPlanGeneric$.
The marginals of $\tilde\varTangentCoupling$ corresponding to the displacement variables satisfy $\pushforward{(\projection{1}{}+\projection{5}{})}{\tilde\varTangentCoupling} = \varGeneric_1$ and $\pushforward{(\projection{2}{}+\projection{6}{})}{\tilde\varTangentCoupling} = \varGeneric_2$ by construction of $\varTangentCoupling_i$.
%
Then $\pushforward{(\projection{1}{}+a+\projection{5}{},\, \projection{2}{}+\projection{6}{})}{\tilde\varTangentCoupling} \in \setPlans{\pushforward{(\identity{}+a)}{\varGeneric_1}}{\varGeneric_2}$, which yields
\begin{align*}
&\frac{1}{2}\wassersteinDistance{\pushforward{(\identity{}+a)}{\varGeneric_1}}{\varGeneric_2}{2}^2
\\
&\quad\leq
\frac{1}{2}
\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\norm{\bar{x}_1 + a + \varTangentReals_1' - \bar{x}_2 - \varTangentReals_2'}^2
\d\tilde\varTangentCoupling(\bar{x}_1, \bar{x}_2, \varTangentReals_1, \varTangentReals_2, \varTangentReals_1', \varTangentReals_2')
\\
&\quad=
\frac{1}{2}\wassersteinDistance{\pushforward{(\identity{}+a)}{\varFixed_1}}{\varFixed_2}{2}^2
+
\frac{1}{2}
\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\norm{\varTangentReals_1' -\varTangentReals_2'}^2
\d\tilde\varTangentCoupling(\bar{x}_1, \bar{x}_2, \varTangentReals_1, \varTangentReals_2, \varTangentReals_1', \varTangentReals_2')
\\
&\quad-
\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\innerProduct{\bar{x}_1 + a-\bar{x}_2}{\varTangentReals_2'}
-
\innerProduct{\bar{x}_1 + a-\bar{x}_2}{\varTangentReals_1'}
\d\tilde\varTangentCoupling(\bar{x}_1, \bar{x}_2, \varTangentReals_1, \varTangentReals_2, \varTangentReals_1', \varTangentReals_2')
\\
&\quad=
\frac{1}{2}\wassersteinDistance{\pushforward{(\identity{}+a)}{\varFixed_1}}{\varFixed_2}{2}^2
+
\frac{1}{2}
\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\norm{\varTangentReals_1' -\varTangentReals_2'}^2
\d\tilde\varTangentCoupling(\bar{x}_1, \bar{x}_2, \varTangentReals_1, \varTangentReals_2, \varTangentReals_1', \varTangentReals_2')
\\
&\quad-
c\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_1}{\varTangentReals_1'}
+
\innerProduct{\varTangentReals_2}{\varTangentReals_2'}
\d\tilde\varTangentCoupling(\bar{x}_1, \bar{x}_2, \varTangentReals_1, \varTangentReals_2, \varTangentReals_1', \varTangentReals_2')
\\
&\quad\leq
\frac{1}{2}\wassersteinDistance{\pushforward{(\identity{}+a)}{\varFixed_1}}{\varFixed_2}{2}^2
+
\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\norm{\varTangentReals_1'}^2 +\norm{\varTangentReals_2'}^2
\d\tilde\varTangentCoupling(\bar{x}_1, \bar{x}_2, \varTangentReals_1, \varTangentReals_2, \varTangentReals_1', \varTangentReals_2')
\\
&\quad-
c\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_1}{\varTangentReals_1'}
+
\innerProduct{\varTangentReals_2}{\varTangentReals_2'}
\d\tilde\varTangentCoupling(\bar{x}_1, \bar{x}_2, \varTangentReals_1, \varTangentReals_2, \varTangentReals_1', \varTangentReals_2').
\end{align*}
where, for the second equality, we realize that, on the support of $\varTangentCoupling_i$ and so also on that of $\tilde\varTangentCoupling$,  $\bar{x}_1 + a - \bar{x}_2 = -c\varTangentReals_1 = c\varTangentReals_2$.
Rearranging the terms, marginalizing, and dividing by $c>0$ yields~\eqref{eq:proof_fuzzy_optimality_conditions:bound_joint_12}.
Combining~\eqref{eq:proof_fuzzy_optimality_conditions:bound_joint_12} and~\eqref{eq:proof_fuzzy_optimality_conditions:bound_ij}, we obtain
\begin{align*}
    \heartsuit
    &\overset{\mathrm{(a)}}{\leq}
    \frac{1}{c}\left(\frac{1}{2}W_2^a(\varFixed_1,\varFixed_2)^2-\frac{1}{2}W_2^a(\varGeneric_1,\varGeneric_2)^2\right)
    \\
    &\qquad+
    \frac{1}{2}
    \sum_{j=0}^\infty 2^{-j}\left(\wassersteinDistance{\varFixed_1}{\tilde\varGeneric_{1,j}}{2}^2+\wassersteinDistance{\varFixed_2}{\tilde\varGeneric_{2,j}}{2}^2-\wassersteinDistance{\varGeneric_1}{\tilde\varGeneric_{1,j}}{2}^2-\wassersteinDistance{\varGeneric_2}{\tilde\varGeneric_{2,j}}{2}^2\right)
    \\
    &\qquad+
    \left(\frac{1}{c}+\sum_{j=0}^\infty 2^{-j}\right)
    \int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
    \norm{\varTangentReals_{1}'}^2+\norm{\varTangentReals_{2}'}^2
    \d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2')
    \\
    &\overset{\mathrm{(b)}}{\leq}
    W_2^a(\varFixed_1,\varFixed_2)-W_2^a(\varGeneric_1,\varGeneric_2)
    \\
    &\qquad+
    \frac{1}{2}
    \sum_{j=0}^\infty 2^{-j}\left(\wassersteinDistance{\varFixed_1}{\tilde\varGeneric_{1,j}}{2}^2+\wassersteinDistance{\varFixed_2}{\tilde\varGeneric_{2,j}}{2}^2-\wassersteinDistance{\varGeneric_1}{\tilde\varGeneric_{1,j}}{2}^2-\wassersteinDistance{\varGeneric_2}{\tilde\varGeneric_{2,j}}{2}^2\right)
    \\
    &\qquad
    +
    \left(\frac{1}{c}+2\right)
    \int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
    \norm{\varTangentReals_{1}'}^2+\norm{\varTangentReals_{2}'}^2
    \d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2')
    \\
    &\overset{\mathrm{(c)}}{=}
    \psi(\varFixed_1,\varFixed_2)
    -
    \psi(\varGeneric_1,\varGeneric_2)
    \\&\qquad+
    \left(\frac{1}{c}+2\right)
    \int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
    \norm{\varTangentReals_{1}'}^2+\norm{\varTangentReals_{2}'}^2
    \d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2')
    \\
    &\overset{\mathrm{(d)}}{\leq}
    \left(\frac{1}{c}+2\right)
    \int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}
    \norm{\varTangentReals_{1}'}^2+\norm{\varTangentReals_{2}'}^2
    \d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2'),
\end{align*}
where (a) combines~\eqref{eq:proof_fuzzy_optimality_conditions:bound_ij} and~\eqref{eq:proof_fuzzy_optimality_conditions:bound_joint_12}; (b) uses the elementary bound $\tfrac1c\bigl(\tfrac12 s^2-\tfrac12 t^2\bigr)\leq s-t$, valid for $s=c=W_2^a(\varFixed_1,\varFixed_2)$ and all $t=W_2^a(\varGeneric_1,\varGeneric_2)\geq0$ (the bound follows from $-\tfrac{(s-t)^2}{2c}\leq0$), together with $\tfrac1c+\sum_{j=0}^\infty 2^{-j}=\tfrac1c+2$; (c) is the definition of $\psi$; and (d) is the local optimality of $(\varFixed_1,\varFixed_2)$ for $\psi$, applicable because the transport plan $(\bar x_i,\bar x_i+\varTangentReals_i')$ gives $\wassersteinDistance{\varFixed_i}{\varGeneric_i}{2}^2\leq\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}\norm{\varTangentReals_i'}^2\d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2')$, so that a small right-hand side keeps $(\varGeneric_1,\varGeneric_2)$ within the neighborhood where $\psi$ is minimized at $(\varFixed_1,\varFixed_2)$.
Maximizing $\heartsuit$ over the couplings $\varTangentCoupling$ realizing a given variation $\varTangentFixed'\coloneqq\pushforward{(\projection{1}{},\projection{2}{},\projection{5}{},\projection{6}{})}{\varTangentCoupling}$ of $\Omega_1\times\Omega_2$ at $(\varFixed_1,\varFixed_2)$, with $\norm{\varTangentFixed'}_{(\varFixed_1,\varFixed_2)}^2=\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d\times\reals^d}\norm{\varTangentReals_1'}^2+\norm{\varTangentReals_2'}^2\d\varTangentCoupling(\bar{x}_1, \bar{x}_2, \bar{\varTangentReals}_1, \bar{\varTangentReals}_2, {\varTangentReals}_1', {\varTangentReals}_2')$, gives $\innerProduct{\varTangentFixed}{\varTangentFixed'}_{(\varFixed_1,\varFixed_2)}\leq\bigl(\tfrac1c+2\bigr)\norm{\varTangentFixed'}_{(\varFixed_1,\varFixed_2)}^2=\onotation{\norm{\varTangentFixed'}_{(\varFixed_1,\varFixed_2)}}$ for $\norm{\varTangentFixed'}_{(\varFixed_1,\varFixed_2)}$ small.
Since $(\varGeneric_1,\varGeneric_2)\in\Omega_1\times\Omega_2$ and $\varTangentFixed'$ were arbitrary, $\varTangentFixed$ belongs to the strong regular normal cone $\normalConeRegularStrong{\Omega_1\times\Omega_2}{(\varFixed_1,\varFixed_2)}$.}

{\emph{Step 6 ($\varTangent_1$ and $\varTangent_2$ are $\varepsilon$-close to the strong regular normal cones).}
We show that $\varTangent_i$ is $\varepsilon$-close to the strong regular normal cone $\normalConeRegularStrong{\Omega_i}{\varFixed_i}$. Clearly, by Step 5 above, $\varTangent_i+\sum_{j=0}^\infty2^{-j}\varTangent_{i,j}$ lies in $\normalConeRegularStrong{\Omega_i}{\varFixed_i}$.
Fix the sum coupling $\varTangentCoupling_1^\star\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_{1,0},\varTangent_{1,1},\ldots}{1}$ used to build the first component of $\varTangentFixed$ in Step~3. By definition, $\varTangentCoupling_1^\star$ is a measure on $\reals^d\times\reals^d\times\left(\times_{j=0}^\infty\reals^d\right)$ with coordinates $(\bar x_1,\varTangentReals_1,\varTangentReals_{1,0},\varTangentReals_{1,1},\ldots)$ and $\pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling_1^\star}=\varTangent_1$ and $\pushforward{(\projection{1}{},\projection{j+3}{})}{\varTangentCoupling_1^\star}=\varTangent_{1,j}$ for every $j\in\naturals$. Writing $\bar\varTangentReals_1\coloneqq\varTangentReals_1+\sum_{j=0}^\infty2^{-j}\varTangentReals_{1,j}$ for the induced arrow (as in Step~5), the first component of $\varTangentFixed$ can be expressed as $\varTangentFixed_1=\pushforward{(\projection{1}{},\bar\varTangentReals_1)}{\varTangentCoupling_1^\star}$.
Consider the pushforward
$
\tilde\gamma
\coloneqq
\pushforward{(\projection{1}{},\projection{2}{},\bar\varTangentReals_1)}{\varTangentCoupling_1^\star}\in\Pp{2}{\reals^d\times\reals^d\times\reals^d}.
$
Its marginals are $\pushforward{(\projection{1}{},\projection{2}{})}{\tilde\gamma}=\varTangent_1$ and $\pushforward{(\projection{1}{},\projection{3}{})}{\tilde\gamma}=\varTangentFixed_1$, and so $\tilde\gamma\in\setPlansCommonMarginal{\varTangent_1}{\varTangentFixed_1}{1}$.
Thus,
\begin{align*}
    \wassersteinDistance{\varTangent_1}{\varTangentFixed_1}{\varFixed_1}^2
    &\leq
    \int_{\reals^d\times\reals^d\times\left(\times_{j=0}^\infty\reals^d\right)}
    \norm{\sum_{j=0}^\infty2^{-j}\varTangentReals_{1,j}}^2
    \d\varTangentCoupling_1^\star(\bar x_1,\varTangentReals_1,\varTangentReals_{1,0},\varTangentReals_{1,1},\ldots).
\end{align*}
Taking the square root and using the triangle inequality} in the space $\Lp{2}{\reals^d\times\reals^d\times(\times_{j=0}^\infty\reals^d)}{\varTangentCoupling_1^\star}$ upper bounds the above by
{
    $\sum_{j=0}^\infty 2^{-j}\norm{\varTangent_{1,j}}_{\varFixed_{1}}
    =
    \sum_{j=0}^\infty2^{-j}\wassersteinDistance{\varFixed_1}{\tilde\varGeneric_{1,j}}{2}
    \leq
    \frac{\varepsilon}{2}
    \sum_{j=0}^\infty 2^{-j}2^{-j/2}
    <
    \varepsilon$.}
Analogously, $\wassersteinDistance{\varTangent_2}{\varTangent_2+\sum_{j=0}^\infty2^{-j}\varTangent_{2,j}}{\varFixed_2}< \varepsilon$, proving that $\varTangent_i$ is $\varepsilon$-close to the strong regular normal cone $\normalConeRegularStrong{\Omega_i}{\varFixed_i}$.
Together with the preceding steps, this establishes all assertions of the lemma.



==> elements/lemma_fuzzy_optimality_condition_title.tex <==
Fuzzy optimality condition%

==> elements/lemma_pushforward_and_optimal_transport_body.tex <==
Assume that, for $i \in \{1, 2\}$,
$\mathcal{X}, \mathcal{X}_i, \mathcal{X}_{i'}$ are separable completely metrizable topological spaces,
$c: \mathcal{X}_{1'}\times\mathcal{X}_{2'} \to \realsBar$ is a transportation cost,
$l_i: \mathcal{X}_i \to \mathcal{X}_{i'}$ are maps, and
$\varTangent_i \in \Pp{2}{\mathcal{X}\times\mathcal{X}_{i}}$ are probability measures
such that $\pushforward{\projection{1}{}}{\varTangent_1} = \pushforward{\projection{1}{}}{\varTangent_2}$.
Then, for every
$\varTangentCoupling \in \setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}$,
there exists
$\varTangentCoupling' \in \setPlansCommonMarginal{\pushforward{(\projection{1}{}, \comp{\projection{2}{}}{l_1})}{\varTangent_1}}{\pushforward{(\projection{1}{}, \comp{\projection{2}{}}{l_2})}{\varTangent_2}}{1}$
{such that:
\begin{equation*}
\int_{\mathcal{X}\times\mathcal{X}_1\times\mathcal{X}_2}
c(l_1(x_1), l_2(x_2))
\d\varTangentCoupling(x, x_1, x_2)
= 
\int_{\mathcal{X}\times\mathcal{X}_{1'}\times\mathcal{X}_{2'}}
c(x_1', x_2') \d\varTangentCoupling'(x, x_1', x_2')
.
\end{equation*}
In particular, it holds:}
\begin{equation*}
\begin{aligned}
&{\inf_{
\varTangentCoupling
\in \setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}
}
\int_{\mathcal{X}\times\mathcal{X}_1\times\mathcal{X}_2}
c(l_1(x_1), l_2(x_2))
\d\varTangentCoupling(x, x_1, x_2)}
\\&\qquad\qquad\qquad= 
{\inf_{
\varTangentCoupling' \in \setPlansCommonMarginal{\pushforward{(\projection{1}{}, \comp{\projection{2}{}}{l_1})}{\varTangent_1}}{\pushforward{(\projection{1}{}, \comp{\projection{2}{}}{l_2})}{\varTangent_2}}{1}
}
\int_{\mathcal{X}\times\mathcal{X}_{1'}\times\mathcal{X}_{2'}}
c(x_1', x_2') \d\varTangentCoupling'(x, x_1', x_2')
.}
\end{aligned}
\end{equation*}

==> elements/lemma_pushforward_and_optimal_transport_title.tex <==
Pushforward and optimal transport%

==> elements/linear_strongly_differentiable_body.tex <==
Let $c\in\reals^d$ and let $l:\Pp{2}{\reals^d}\to\reals$ be the expected value $l(\varGeneric)\coloneqq\expectedValue{x\sim\varGeneric}{\innerProduct{c}{x}}$. Then, $l$ is strongly differentiable at every $\varFixed\in\Pp{2}{\reals^d}$, with strong gradient $\gradientStrong{}{l}(\varFixed)=\gradient{}{l}(\varFixed)=\varFixed\times\delta_c$.


==> elements/linear_strongly_differentiable_proof.tex <==
To start, membership of $\pm(\varFixed\times\delta_c)$ to the tangent space follows from \cref{proposition:prop_functional_expected_value} applied to $\pm l$.
%
Then, fix $\varFixed\in\Pp{2}{\reals^d}$.
For every $\varGeneric\in\Pp{2}{\reals^d}$ and $\varPlanGeneric\in\setPlans{\varFixed}{\varGeneric}$, the variation $\varTangent=\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\varPlanGeneric}$ satisfies
\begin{equation*}
    l(\varGeneric)-l(\varFixed)
    =
    \int_{\reals^d}\innerProduct{c}{x}\d\varGeneric(x)-\int_{\reals^d}\innerProduct{c}{x}\d\varFixed(x)
    =
    \int_{\reals^d\times\reals^d}\innerProduct{c}{\varTangentReals}\d\varTangent(x,\varTangentReals)
    =
    \innerProduct{\varFixed\times\delta_c}{\varTangent}_{\varFixed},
\end{equation*}
where the last equality holds because the arrow of $\varFixed\times\delta_c$ equals $c$ almost everywhere, so the integral in \eqref{definition:geometry:inner_product} takes the value $\int_{\reals^d\times\reals^d}\innerProduct{c}{\varTangentReals}\d\varTangent(x,\varTangentReals)$ for every coupling $\varTangentCoupling\in\setPlansCommonMarginal{\varFixed\times\delta_c}{\varTangent}{1}$, and the maximum trivializes.
As this identity holds with no remainder, applying it to $l$ and to $-l$ gives $\varFixed\times\delta_c\in\subgradientRegularStrong{l}(\varFixed)$ and $-\varFixed\times\delta_c\in\subgradientRegularStrong{(-l)}(\varFixed)$, respectively. Hence, $\varFixed\times\delta_c\in-\subgradientRegularStrong{(-l)}(\varFixed)\cap\subgradientRegularStrong{l}(\varFixed)$, and $l$ is strongly differentiable with $\gradientStrong{}{l}(\varFixed)=\gradient{}{l}(\varFixed)=\varFixed\times\delta_c$.


==> elements/linear_strongly_differentiable_title.tex <==
Strong differentiability of linear functionals%

==> elements/normal_cone_linear_constraint_body.tex <==
{%
Let $c \in \reals^d \setminus \{0\}$, let $\gamma \in \reals$, and let
$l : \Pp{2}{\reals^d} \to \reals$ be the linear functional
$l(\varGeneric) \coloneqq \expectedValue{x \sim \varGeneric}{\innerProduct{c}{x}}$. Consider
$
\feasibleSet
\coloneqq
\left\{
\varGeneric \in \Pp{2}{\reals^d}
\st
l(\varGeneric) \leq \gamma
\right\}.
$
Then, $\feasibleSet$ is closed and \gls*{acr:snc} at every
$\varFixed \in \feasibleSet$, and
\begin{equation*}
\normalConeRegularStrong{\feasibleSet}{\varFixed}
=
\normalConeStrong{\feasibleSet}{\varFixed}
=
\begin{cases}
\left\{
\lambda \, (\varFixed \times \delta_c)
\st
\lambda \geq 0
\right\}
&
\text{if } l(\varFixed) = \gamma,
\\[2pt]
\{\localZero{\varFixed}\}
&
\text{if } l(\varFixed) < \gamma.
\end{cases}
\end{equation*}
}


==> elements/normal_cone_linear_constraint_proof.tex <==
{%
We divide the proof into steps.

\emph{Step 1 (two preliminaries).} For a variation $\boldsymbol{a}$ at a point
$\varReference$ whose arrow equals a constant $a \in \reals^d$ almost everywhere, the
maximization in \eqref{definition:geometry:inner_product} is vacuous, as in the proof of \cref{lemma:linear_strongly_differentiable}. Thus,
\begin{equation}
\label{eq:linear_constraint:pairing}
\innerProduct{\boldsymbol{a}}{\varTangent}_{\varReference}
=
\int_{\reals^d \times \reals^d} \innerProduct{a}{\varTangentReals} \d\varTangent(x, \varTangentReals)
\qquad
\text{for every variation } \varTangent \text{ at } \varReference.
\end{equation}
This applies in
particular to $\varReference \times \delta_a$, which lies in
$\tangentCone{\Pp{2}{\reals^d}}{\varReference}$ by
\cref{lemma:linear_strongly_differentiable}.
Moreover, $l$ is $\norm{c}$-Lipschitz
with respect to $\wassersteinDistance{}{}{2}$ (its integrand
$x \mapsto \innerProduct{c}{x}$ is $\norm{c}$-Lipschitz), hence continuous, so
$\feasibleSet = l^{-1}((-\infty, \gamma])$ is closed.

\emph{Step 2 (interior points).} If $l(\varFixed) < \gamma$, then, by continuity of
$l$, $\varFixed$ lies in the interior of $\feasibleSet$, and
\cref{lemma:strong_vs_regular_normal_cone} with
\cref{proposition:prop_normal_cones_trivial}\ref{item:normal_cone:interior_point}
give
$\normalConeRegularStrong{\feasibleSet}{\varFixed} \subseteq \normalConeRegular{\feasibleSet}{\varFixed} = \{\localZero{\varFixed}\}$.
We assume $l(\varFixed) = \gamma$ throughout Steps~3 and~4.

\emph{Step 3 (the ray consists of normals).} Let $\lambda \geq 0$. For every
$\varGeneric \in \feasibleSet$ and every
$\varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlans{\varFixed}{\varGeneric}}$,
the arrow of $\lambda \, (\varFixed \times \delta_c)$ is the constant $\lambda c$, so
\eqref{eq:linear_constraint:pairing} gives
\begin{equation*}
\innerProduct{\lambda \, (\varFixed \times \delta_c)}{\varTangent}_{\varFixed}
=
\lambda \int_{\reals^d \times \reals^d} \innerProduct{c}{\varTangentReals} \d\varTangent(x, \varTangentReals)
=
\lambda \bigl( l(\varGeneric) - l(\varFixed) \bigr)
=
\lambda \bigl( l(\varGeneric) - \gamma \bigr)
\leq 0,
\end{equation*}
where the second equality holds for any transport plan because
$\int_{\reals^d \times \reals^d} \innerProduct{c}{\varTangentReals} \d\varTangent(x, \varTangentReals)
= \int_{\reals^d} \innerProduct{c}{x'} \d\varGeneric(x')
- \int_{\reals^d} \innerProduct{c}{x} \d\varFixed(x) = l(\varGeneric) - l(\varFixed)$.
As $\lambda \, (\varFixed \times \delta_c) \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$
by Step~1, this shows
$\lambda \, (\varFixed \times \delta_c) \in \normalConeRegularStrong{\feasibleSet}{\varFixed}$.

\emph{Step 4 (every strong regular normal lies on the ray).} Let
$\varTangentFixed \in \normalConeRegularStrong{\feasibleSet}{\varFixed}$ and
set $m \coloneqq \int_{\reals^d \times \reals^d} \innerProduct{c}{\varTangentReals} \d\varTangentFixed(x, \varTangentReals)$. We first
record which variations point into $\feasibleSet$: the endpoint
$\varGeneric_{\varTangent} \coloneqq \pushforward{(\projection{1}{} + \projection{2}{})}{\varTangent}$
of a variation $\varTangent$ at $\varFixed$ satisfies
$l(\varGeneric_{\varTangent}) = \gamma + \int_{\reals^d \times \reals^d} \innerProduct{c}{\varTangentReals} \d\varTangent(x, \varTangentReals)$,
so $\varGeneric_{\varTangent} \in \feasibleSet$ if and only if
$\int_{\reals^d \times \reals^d} \innerProduct{c}{\varTangentReals} \d\varTangent(x, \varTangentReals) \leq 0$, and then
$\varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlans{\varFixed}{\varGeneric_{\varTangent}}}$.

\emph{(i)~The multiplier is nonnegative.} For $s > 0$, the variation
$\varTangent_s \coloneqq \varFixed \times \delta_{-s c}$ has constant arrow $-sc$, so
$\int_{\reals^d \times \reals^d} \innerProduct{c}{\varTangentReals} \d\varTangent_s(x, \varTangentReals) = -s \norm{c}^2 \leq 0$; hence
$\varTangent_s$ points into $\feasibleSet$, with
$\norm{\varTangent_s}_{\varFixed} = s \norm{c}$. By
\eqref{eq:linear_constraint:pairing},
$\innerProduct{\varTangentFixed}{\varTangent_s}_{\varFixed} = -s \, m$, and the defining
inequality of $\varTangentFixed$ (with $\varGeneric_{\varTangent_s} \convergenceWasserstein \varFixed$ as
$s \fromAbove 0$) yields
$-s \, m \leq \onotation{\norm{\varTangent_s}_{\varFixed}} = \onotation{s}$; dividing by
$s$ gives $m \geq 0$.

\emph{(ii)~The normal is deterministic and aligned with $c$.} Write
$\hat c \coloneqq c / \norm{c}$ and let
$\varTangentFixed_0 \coloneqq \pushforward{(\projection{1}{}, \projection{2}{} - \tfrac{m}{\norm{c}^2} c)}{\varTangentFixed}$
be the variation with the same base as $\varTangentFixed$ and arrow
$\varTangentReals_0 \coloneqq \varTangentReals - \tfrac{m}{\norm{c}^2} c$. Its mean
$c$-component vanishes,
$\int_{\reals^d \times \reals^d} \innerProduct{c}{\varTangentReals_0} \d\varTangentFixed_0(x, \varTangentReals_0) = m - m = 0$, so
$s \varTangentFixed_0$ points into $\feasibleSet$ for every $s \geq 0$.
Since
$\pushforward{(\projection{1}{}, \projection{2}{}, \projection{2}{} - \tfrac{m}{\norm{c}^2} c)}{\varTangentFixed} \in \setPlansCommonMarginal{\varTangentFixed}{\varTangentFixed_0}{1}$,
\eqref{definition:geometry:inner_product} and the split
$\varTangentReals = \innerProduct{\hat c}{\varTangentReals} \hat c + \varTangentReals^{\perp}$
into components parallel and orthogonal to $c$ give, using
$m = \norm{c} \int_{\reals^d \times \reals^d} \innerProduct{\hat c}{\varTangentReals} \d\varTangentFixed(x, \varTangentReals)$,
\begin{align*}
\innerProduct{\varTangentFixed}{\varTangentFixed_0}_{\varFixed}
&\geq
\int_{\reals^d \times \reals^d} \innerProduct{\varTangentReals}{\varTangentReals - \tfrac{m}{\norm{c}^2} c} \d\varTangentFixed(x, \varTangentReals)
\\
&=
\int_{\reals^d \times \reals^d} \norm{\varTangentReals}^2 \d\varTangentFixed(x, \varTangentReals) - \frac{m^2}{\norm{c}^2}
\\
&=
\left( \int_{\reals^d \times \reals^d} \innerProduct{\hat c}{\varTangentReals}^2 \d\varTangentFixed(x, \varTangentReals) - \left( \int_{\reals^d \times \reals^d} \innerProduct{\hat c}{\varTangentReals} \d\varTangentFixed(x, \varTangentReals) \right)^{2} \right)
\\
&\quad
+ \int_{\reals^d \times \reals^d} \norm{\varTangentReals^{\perp}}^2 \d\varTangentFixed(x, \varTangentReals).
\end{align*}
Both terms are nonnegative (the first by Jensen's inequality).
On the other hand, the defining inequality of $\varTangentFixed$ along
$s \varTangentFixed_0$ ($s \fromAbove 0$), with homogeneity
(\cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:homogeneity}), gives
$\innerProduct{\varTangentFixed}{\varTangentFixed_0}_{\varFixed} \leq 0$. Hence both
nonnegative terms vanish: $\varTangentReals^{\perp} = 0$ almost everywhere, and
$\innerProduct{\hat c}{\varTangentReals}$ is $\almostEverywhere{\varTangentFixed}$ equal to its
mean $\tfrac{m}{\norm{c}}$. Therefore $\varTangentReals = \tfrac{m}{\norm{c}^2} c$
almost everywhere, i.e., $\varTangentFixed = \tfrac{m}{\norm{c}^2} (\varFixed \times \delta_c)$
with $\tfrac{m}{\norm{c}^2} \geq 0$ by~(i). With Step~3, this proves
$\normalConeRegularStrong{\feasibleSet}{\varFixed} = \{ \lambda \, (\varFixed \times \delta_c) \st \lambda \geq 0 \}$.

\emph{Step 5 (\gls*{acr:snc} and the strong normal cone).} Fix
$\varFixed \in \feasibleSet$ and take
$\varGeneric_n \convergenceWasserstein \varFixed$ in $\feasibleSet$ and
$\varTangent_n \in \normalConeRegularStrong{\feasibleSet}{\varGeneric_n}$
with $\varTangent_n \convergenceNarrow \varTangent$. By Steps~2--4,
$\varTangent_n = \varGeneric_n \times \delta_{\lambda_n c}$ for some $\lambda_n \geq 0$.
Narrow convergence makes $(\varTangent_n)_{n \in \naturals}$ tight (Prokhorov,
\cite[Theorem 5.1.3]{ambrosio2005gradient}); as the arrow marginal of $\varTangent_n$
is $\delta_{\lambda_n c}$ and $c \neq 0$, this forces $(\lambda_n)_{n \in \naturals}$ to
be bounded. Along any subsequence with $\lambda_n \to \lambda$, coupling
$\varTangent_n = \varGeneric_n \times \delta_{\lambda_n c}$ and
$\varFixed \times \delta_{\lambda c}$ through an optimal transport plan of
$(\varGeneric_n, \varFixed)$ and the (deterministic) arrows gives
$
\wassersteinDistance{\varTangent_n}{\varFixed \times \delta_{\lambda c}}{2}^2
\leq
\wassersteinDistance{\varGeneric_n}{\varFixed}{2}^2 + \norm{\lambda_n c - \lambda c}^2
\to 0,
$
so $\varTangent_n \convergenceWasserstein \varFixed \times \delta_{\lambda c}$; as
convergence in Wasserstein implies narrow convergence and the narrow limit is unique,
$\varFixed \times \delta_{\lambda c} = \varTangent$, which determines $\lambda$ uniquely
($c \neq 0$). Thus every subsequence of the bounded $(\lambda_n)_{n \in \naturals}$ has a
further subsequence converging to this same $\lambda$, whence $\lambda_n \to \lambda$ and
$\varTangent_n \convergenceWasserstein \varTangent = \lambda \, (\varFixed \times \delta_c)$.
This is the \gls*{acr:snc} property. Finally,
$\normalConeRegularStrong{\feasibleSet}{\varFixed} \subseteq \normalConeStrong{\feasibleSet}{\varFixed}$
always, while the argument just made shows every element of
$\normalConeStrong{\feasibleSet}{\varFixed}$ lies on the ray. At boundary points ($l(\varFixed) = \gamma$) this
yields $\normalConeStrong{\feasibleSet}{\varFixed} = \normalConeRegularStrong{\feasibleSet}{\varFixed}$;
at interior points ($l(\varFixed) < \gamma$), continuity of $l$ gives
$l(\varGeneric_n) < \gamma$ for $n$ large, so $\lambda_n = 0$ by Step~2 and
$\varTangent = \localZero{\varFixed}$, whence
$\normalConeStrong{\feasibleSet}{\varFixed} = \{\localZero{\varFixed}\}$,
in agreement with Step~2.
}


==> elements/normal_cone_linear_constraint_title.tex <==
Normal cone of a linear constraint%


==> elements/prop_calculus_body.tex <==
Consider the proper functionals $\objective_1,\objective_2: \Pp{2}{\reals^d} \to \realsBar$, $g: \realsBar \to \realsBar$ with $g(+\infty) = +\infty$, and $\varFixed \in \Pp{2}{\reals^d}$ so that $\objective_i(\varFixed) \in \reals$, $g$ is continuously differentiable at $\objective_1(\varFixed) \in \reals$ with $g(\objective_1(\varFixed)) \in \reals$, and $\objective_1$ continuous in Wasserstein at $\varFixed$. Then, the following rules hold:
\begin{enumerate}
\item\label{prop_calculus_sum_rule} Sum rule:
$
    \subgradientRegular{(\objective_1+\objective_2)}(\varFixed)
    \supseteq
    \subgradientRegular{(\objective_1)}(\varFixed)
    +
    \subgradientRegular{(\objective_2)}(\varFixed)
    \coloneqq
    \left\{
    \varTangent_1\localSum{\varTangentCoupling} \varTangent_2 \st \varTangent_i \in \subgradientRegular{\objective_i}(\varFixed), \varTangentCoupling \in \setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}
    \right\}.
$
In particular, if $\objective_2$ is differentiable {on a Wasserstein
neighborhood of} $\varFixed$ {with $\varGeneric \mapsto \gradient{}{\objective_2}(\varGeneric)$
continuous at $\varFixed$ (convergence in Wasserstein in the argument and in the value)}, then
$
    \subgradientRegular{(\objective_1+\objective_2)}(\varFixed)
    =
    \subgradientRegular{(\objective_1)}(\varFixed)
    +
    \{\gradient{}\objective_2(\varFixed)\}
$
and, thus,
$
    \subgradient{(\objective_1 + \objective_2)}(\varFixed)
    = \subgradient{\objective_1}(\varFixed) + \left\{\gradient{}{\objective_2}(\varFixed)\right\}.
$

\item\label{prop_calculus_chain_rule}
Chain rule: If $g'(\objective_1(\varFixed)) > 0$, then
    $\subgradientRegular{(\comp{\objective_1}{g})}(\varFixed)=
    g'(\objective_1(\varFixed)){\subgradientRegular{\objective_1}(\varFixed)}
    \coloneqq
    \{ g'(\objective_1(\varFixed))\varTangent\st\varTangent\in\subgradientRegular{\objective_1}(\varFixed)\}$ and{, if
    in addition $\objective_1$ is continuous in Wasserstein on a neighborhood of
    $\varFixed$,}
    $\subgradient{(\comp{\objective_1}{g})}(\varFixed)=
    g'(\objective_1(\varFixed)){\subgradient{\objective_1}(\varFixed)}.$

\item\label{prop_calculus_chain_rule:differentiable}
{Chain rule (the differentiable case): If $\objective_1$ is differentiable at $\varFixed$, then $\comp{\objective_1}{g}$ is differentiable at $\varFixed$ and
$
\gradient{}(\comp{\objective_1}{g})(\varFixed) = g'(\objective_1(\varFixed))\gradient{}\objective_1(\varFixed).
$}
\end{enumerate}


==> elements/prop_calculus_proof.tex <==
We prove the statements separately.
\begin{enumerate}
    \item Let $\varTangent_1 \in \subgradientRegular{\objective_1}(\varFixed), \varTangent_2 \in \subgradientRegular{\objective_2}(\varFixed)$. Then, for all $\varTangentCoupling \in \setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}$, and all $\varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$,
    \begin{align*}
        &
        \frac{1}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}\Bigl(
        \left(\objective_1(\varGeneric) + \objective_2(\varGeneric)\right) - \left(\objective_1(\varFixed) + \objective_2(\varFixed)\right)
        \\&\qquad
        - \innerProduct{\varTangent_1 \localSum{\varTangentCoupling} \varTangent_2}{\varTangent}_{\varFixed}\Bigr)
        \\&\qquad\geq
        \frac{1}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}\Bigl(
        \left(\objective_1(\varGeneric) + \objective_2(\varGeneric)\right) - \left(\objective_1(\varFixed) + \objective_2(\varFixed)\right)
        \\&\qquad\qquad
        - \innerProduct{\varTangent_1}{\varTangent}_{\varFixed} - \innerProduct{\varTangent_2}{\varTangent}_{\varFixed}\Bigr),
    \end{align*}
    where the inequality follows from \cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:sublinear}. Then,
    \begin{align*}
    &\liminf_{\substack{
        \varGeneric \convergenceWasserstein \varFixed
        \\
        \varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}}}
        \frac{1}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}\Bigl(
        \left(\objective_1(\varGeneric) + \objective_2(\varGeneric)\right) - \left(\objective_1(\varFixed) + \objective_2(\varFixed)\right)
        \\&\qquad\qquad
        - \innerProduct{\varTangent_1 \localSum{\varTangentCoupling} \varTangent_2}{\varTangent}_{\varFixed}\Bigr)
        \\&\geq
        \liminf_{\substack{
        \varGeneric \convergenceWasserstein \varFixed
        \\
        \varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}}}
        \frac{\objective_1(\varGeneric) - \objective_1(\varFixed) - \innerProduct{\varTangent_1}{\varTangent}_{\varFixed}}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
        \\&\qquad+\liminf_{\substack{
        \varGeneric \convergenceWasserstein \varFixed
        \\
        \varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}}}
        \frac{\objective_2(\varGeneric) - \objective_2(\varFixed) - \innerProduct{\varTangent_2}{\varTangent}_{\varFixed}}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
        \geq 0.
    \end{align*}
    This shows that $\varTangent_1 \localSum{\varTangentCoupling} \varTangent_2\in\subgradientRegular{(\objective_1+\objective_2)}(\varFixed)$, proving the desired inclusion.
    %
    When $\objective_2$ is differentiable at $\varFixed$, {we can show the other direction:
    {Since $\objective_2$ is differentiable at $\varFixed$, it is finite on a
    Wasserstein neighborhood of $\varFixed$; because regular subgradients at $\varFixed$
    depend only on the values of the functional near $\varFixed$, we may assume without
    loss of generality that $\objective_2$ is real-valued, so that $-\objective_2$ is
    proper and $\objective_1 = \objective_1 + \objective_2 - \objective_2$.}
    In view of the above inclusion, we have}
    $\subgradientRegular{\objective_1}(\varFixed)
        = \subgradientRegular{(\objective_1 + \objective_2 - \objective_2)}(\varFixed)
        \supseteq
        \subgradientRegular{(\objective_1 + \objective_2)}(\varFixed)
        +
        \subgradientRegular{(-\objective_2)}(\varFixed)
        =
        \subgradientRegular{(\objective_1 + \objective_2)}(\varFixed)
        +
        \{-\gradient{}{\objective_2}(\varFixed)\}$
        and, thus,
        {
        $
        \subgradientRegular{\objective_1}(\varFixed)
        +\{\gradient{}{\objective_2}(\varFixed)\}\supseteq \subgradientRegular{(\objective_1 + \objective_2)}(\varFixed)
        +
        \{-\gradient{}{\objective_2}(\varFixed)\}+\{\gradient{}{\objective_2}(\varFixed)\}.
        $}
        {For every
        $\varTangent\in\subgradientRegular{(\objective_1 + \objective_2)}(\varFixed)$
        and every
        $\varTangentCoupling\in\setPlansCommonMarginal{\varTangent}{-\gradient{}{\objective_2}(\varFixed)}{1}$,
        the coupling
        $\varTangentCoupling'\coloneqq\pushforward{(\projection{1}{},\projection{2}{}+\projection{3}{},-\projection{3}{})}{\varTangentCoupling}$
        belongs to
        $\setPlansCommonMarginal{\varTangent\localSum{\varTangentCoupling}(-\gradient{}{\objective_2}(\varFixed))}{\gradient{}{\objective_2}(\varFixed)}{1}$
        and satisfies
        $(\varTangent\localSum{\varTangentCoupling}(-\gradient{}{\objective_2}(\varFixed)))\localSum{\varTangentCoupling'}\gradient{}{\objective_2}(\varFixed)=\pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling}=\varTangent$,
        so that $\subgradientRegular{(\objective_1 +
        \objective_2)}(\varFixed)+\{-\gradient{}{\objective_2}(\varFixed)\}+\{\gradient{}{\objective_2}(\varFixed)\}\supseteq\subgradientRegular{(\objective_1
        + \objective_2)}(\varFixed)$, which gives the desired inclusion.}
        %
        {It remains to establish the equality for the general
        subgradients, i.e.,
        $\subgradient{(\objective_1 + \objective_2)}(\varFixed) =
        \subgradient{\objective_1}(\varFixed) +
        \{\gradient{}{\objective_2}(\varFixed)\}$. We first record three facts.
        (i) continuity at $\varFixed$ (convergence in Wasserstein in the argument and in the value) of the map
        $\varGeneric \mapsto \gradient{}{\objective_2}(\varGeneric)$ presupposes
        that this map is defined on a Wasserstein neighborhood of $\varFixed$,
        i.e., that $\objective_2$ is differentiable there. In particular, the
        equality for the regular subgradients established above holds at every
        $\varOther$ in this neighborhood with $\objective_1(\varOther) \in \reals$:
        its proof uses only that
        $\objective_1(\varOther), \objective_2(\varOther) \in \reals$ and that
        $\objective_2$ is differentiable at $\varOther$.
        (ii) By
        \cref{proposition:prop_differentiability_properties}\ref{item:gradient_induced_by_map},
        $\varTangentFixed \coloneqq \gradient{}{\objective_2}(\varFixed)$ is
        induced by a map, for every variation $\varTangent$ at $\varFixed$ the
        set $\setPlansCommonMarginal{\varTangent}{\varTangentFixed}{1}$ is a
        singleton (so the sums in $\subgradient{\objective_1}(\varFixed) +
        \{\gradient{}{\objective_2}(\varFixed)\}$ do not depend on the choice of
        the coupling, and we write $\varTangent \localSum{} \varTangentFixed$),
        and $\objective_2$ is continuous in Wasserstein at $\varFixed$.
        (iii) Let $\varGeneric_n \convergenceWasserstein \varFixed$, let
        $\varTangent_n, \varTangentOther_n$ be variations at $\varGeneric_n$ with
        $\varTangent_n \convergenceWasserstein \varTangent$ and
        $\varTangentOther_n \convergenceWasserstein \varTangentOther$, and suppose
        that $\varTangentOther$ is induced by a map. Then, for any choice of
        $\varTangentCoupling_n \in
        \setPlansCommonMarginal{\varTangent_n}{\varTangentOther_n}{1}$, the
        sequence $(\varTangentCoupling_n)_{n\in\naturals}$ converges in
        Wasserstein to the unique element $\varTangentCoupling$ of
        $\setPlansCommonMarginal{\varTangent}{\varTangentOther}{1}$, and
        $\varTangent_n \localSum{\varTangentCoupling_n} \varTangentOther_n
        \convergenceWasserstein
        \varTangent \localSum{\varTangentCoupling} \varTangentOther$. Indeed,
        $(\varTangentCoupling_n)_{n\in\naturals}$ is tight, because its
        $(\projection{1}{},\projection{2}{})$- and
        $(\projection{1}{},\projection{3}{})$-marginals converge in
        Wasserstein and are therefore tight; every narrow limit point has marginals
        $\varTangent$ and $\varTangentOther$ (pushforwards through projections
        commute with narrow limits) and thus equals $\varTangentCoupling$, which
        is unique because $\varTangentOther$ is induced by a map, say by $\psi$:
        every element of
        $\setPlansCommonMarginal{\varTangent}{\varTangentOther}{1}$ is
        concentrated on $\{\varTangentReals_2 = \psi(\bar x)\}$ and is therefore
        the pushforward of $\varTangent$ under $(\bar x, \varTangentReals_1)
        \mapsto (\bar x, \varTangentReals_1, \psi(\bar x))$ (cf.\ the proof of
        \cref{proposition:prop_differentiability_properties}\ref{item:gradient_induced_by_map}).
        Hence,
        $\varTangentCoupling_n \convergenceNarrow \varTangentCoupling$, and the
        second moments converge, since they split along the marginals:
        \begin{align*}
        \int_{\reals^d\times\reals^d\times\reals^d}
        &\norm{\bar x}^2 + \norm{\varTangentReals_1}^2 + \norm{\varTangentReals_2}^2
        \d\varTangentCoupling_n(\bar x,\varTangentReals_1,\varTangentReals_2)
        \\&=
        \int_{\reals^d\times\reals^d} \norm{\bar x}^2 + \norm{\varTangentReals_1}^2 \d\varTangent_n(\bar x,\varTangentReals_1)
        \\&\qquad
        +
        \int_{\reals^d\times\reals^d} \norm{\varTangentReals_2}^2 \d\varTangentOther_n(\bar x,\varTangentReals_2)
        \\
        &\to
        \int_{\reals^d\times\reals^d} \norm{\bar x}^2 + \norm{\varTangentReals_1}^2 \d\varTangent(\bar x,\varTangentReals_1)
        \\&\qquad
        +
        \int_{\reals^d\times\reals^d} \norm{\varTangentReals_2}^2 \d\varTangentOther(\bar x,\varTangentReals_2)
        \\&=
        \int_{\reals^d\times\reals^d\times\reals^d}
        \norm{\bar x}^2 + \norm{\varTangentReals_1}^2 + \norm{\varTangentReals_2}^2
        \d\varTangentCoupling(\bar x,\varTangentReals_1,\varTangentReals_2),
        \end{align*}
        so $\varTangentCoupling_n \convergenceWasserstein \varTangentCoupling$
        (cf. \cite[Proposition 7.1.5]{ambrosio2005gradient}); the sums converge
        because the map $(\bar x, \varTangentReals_1, \varTangentReals_2) \mapsto
        (\bar x, \varTangentReals_1 + \varTangentReals_2)$ is Lipschitz.}

        {We now prove the inclusion $\supseteq$. Let
        $\varTangent \in \subgradient{\objective_1}(\varFixed)$ and take sequences
        $\varGeneric_n \convergenceWasserstein \varFixed$ with
        $\objective_1(\varGeneric_n) \to \objective_1(\varFixed)$ and
        $\subgradientRegular{\objective_1}(\varGeneric_n) \ni \varTangent_n
        \convergenceWasserstein \varTangent$ (cf.
        \cref{definition:def_sub_sup_differentiability}\ref{item:subgradient}).
        For $n$ sufficiently large, $\objective_1(\varGeneric_n) \in \reals$ and
        $\objective_2$ is differentiable at $\varGeneric_n$ with
        $\varTangentFixed_n \coloneqq \gradient{}{\objective_2}(\varGeneric_n) \in
        \subgradientRegular{\objective_2}(\varGeneric_n)$ (cf.
        \cref{proposition:prop_differentiability_properties}\ref{item:gradient_uniqueness});
        moreover, $\varTangentFixed_n \convergenceWasserstein \varTangentFixed$ by
        hypothesis. Fix any $\varTangentCoupling_n \in
        \setPlansCommonMarginal{\varTangent_n}{\varTangentFixed_n}{1}$ (nonempty,
        e.g., by the gluing lemma \cite[Gluing Lemma]{villani2009optimal}). By the
        sum rule proved above, applied at $\varGeneric_n$,
        $\varTangent_n \localSum{\varTangentCoupling_n} \varTangentFixed_n \in
        \subgradientRegular{(\objective_1 + \objective_2)}(\varGeneric_n)$, and, by
        (iii), $\varTangent_n \localSum{\varTangentCoupling_n} \varTangentFixed_n
        \convergenceWasserstein \varTangent \localSum{} \varTangentFixed$. Since,
        by (ii), $(\objective_1 + \objective_2)(\varGeneric_n) \to
        (\objective_1 + \objective_2)(\varFixed)$, we conclude
        $\varTangent \localSum{} \varTangentFixed \in
        \subgradient{(\objective_1 + \objective_2)}(\varFixed)$, which proves
        $\supseteq$ (recall from (ii) that the sum does not depend on the
        coupling).}

        {For the inclusion $\subseteq$, let $\varTangentOther \in
        \subgradient{(\objective_1 + \objective_2)}(\varFixed)$ and take sequences
        $\varGeneric_n \convergenceWasserstein \varFixed$ with
        $(\objective_1 + \objective_2)(\varGeneric_n) \to
        (\objective_1 + \objective_2)(\varFixed)$ and
        $\subgradientRegular{(\objective_1 + \objective_2)}(\varGeneric_n) \ni
        \varTangentOther_n \convergenceWasserstein \varTangentOther$. For $n$
        sufficiently large, $\objective_2(\varGeneric_n) \in \reals$ (by
        differentiability) and $\objective_1(\varGeneric_n) =
        (\objective_1 + \objective_2)(\varGeneric_n) -
        \objective_2(\varGeneric_n) \in \reals$, so, by (i), there are
        $\varTangent_n \in \subgradientRegular{\objective_1}(\varGeneric_n)$ and
        $\varTangentCoupling_n \in
        \setPlansCommonMarginal{\varTangent_n}{\varTangentFixed_n}{1}$, with
        $\varTangentFixed_n \coloneqq \gradient{}{\objective_2}(\varGeneric_n)$,
        so that
        $\varTangentOther_n = \varTangent_n \localSum{\varTangentCoupling_n}
        \varTangentFixed_n$. The couplings
        $\tilde\varTangentCoupling_n \coloneqq \pushforward{(\projection{1}{},
        \projection{2}{} + \projection{3}{},
        \projection{3}{})}{\varTangentCoupling_n} \in
        \setPlansCommonMarginal{\varTangentOther_n}{\varTangentFixed_n}{1}$ satisfy
        the assumptions of (iii), since
        $\varTangentOther_n \convergenceWasserstein \varTangentOther$ and
        $\varTangentFixed_n \convergenceWasserstein \varTangentFixed$ by
        hypothesis; hence,
        $\tilde\varTangentCoupling_n \convergenceWasserstein
        \tilde\varTangentCoupling$, the unique element of
        $\setPlansCommonMarginal{\varTangentOther}{\varTangentFixed}{1}$. Since the
        map $(\bar x, \varTangentReals_1, \varTangentReals_2) \mapsto
        (\bar x, \varTangentReals_1 - \varTangentReals_2)$ is Lipschitz,
        $\varTangent_n = \pushforward{(\projection{1}{}, \projection{2}{} -
        \projection{3}{})}{\tilde\varTangentCoupling_n} \convergenceWasserstein
        \varTangent \coloneqq \pushforward{(\projection{1}{}, \projection{2}{} -
        \projection{3}{})}{\tilde\varTangentCoupling}$. Moreover, by (ii),
        $\objective_1(\varGeneric_n) = (\objective_1 + \objective_2)(\varGeneric_n)
        - \objective_2(\varGeneric_n) \to \objective_1(\varFixed)$, so
        $\varTangent \in \subgradient{\objective_1}(\varFixed)$. Finally,
        $\varTangentCoupling \coloneqq \pushforward{(\projection{1}{},
        \projection{2}{} - \projection{3}{},
        \projection{3}{})}{\tilde\varTangentCoupling} \in
        \setPlansCommonMarginal{\varTangent}{\varTangentFixed}{1}$ and
        $\varTangent \localSum{\varTangentCoupling} \varTangentFixed =
        \pushforward{(\projection{1}{},
        \projection{2}{})}{\tilde\varTangentCoupling} = \varTangentOther$, so
        $\varTangentOther \in \subgradient{\objective_1}(\varFixed) +
        \{\gradient{}{\objective_2}(\varFixed)\}$. This establishes the desired
        equality.}
    \item
{
We first prove the statement for the regular subgradient.
To ease notation, let $\alpha \coloneqq \objective_1(\varFixed)<+\infty$ and $c \coloneqq g'(\alpha)>0$.}

{
To start, we show that
$
c\,\subgradientRegular{\objective_1}(\varFixed)
\subseteq
\subgradientRegular{(\comp{\objective_1}{g})}(\varFixed).
$
To this end, let $\varTangent\in \subgradientRegular{\objective_1}(\varFixed)$ and define, for $\varGeneric$ near $\varFixed$,
\[
q(\varGeneric)\coloneqq
\begin{cases}
\dfrac{g(\objective_1(\varGeneric))-g(\objective_1(\varFixed))}
{\objective_1(\varGeneric)-\objective_1(\varFixed)},
& \text{if }\objective_1(\varGeneric)\neq \objective_1(\varFixed),\\[1.2ex]
c,
& \text{if }\objective_1(\varGeneric)=\objective_1(\varFixed).
\end{cases}
\]
Since $\objective_1$ is continuous in Wasserstein at $\varFixed$ and $g$ is differentiable at $\alpha$, we have
$
q(\varGeneric)\to c
$
as
$
\varGeneric\convergenceWasserstein\varFixed.
$
Now let
$
\varTangentOther\in
\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}
{\setPlansOptimal{\varFixed}{\varGeneric}}.
$
Then,
\begin{align*}
&
\frac{
g(\objective_1(\varGeneric))-g(\objective_1(\varFixed))
-\innerProduct{c\varTangent}{\varTangentOther}_{\varFixed}
}{
\wassersteinDistance{\varFixed}{\varGeneric}{2}
}
\\
&=
q(\varGeneric)\,
\frac{
\objective_1(\varGeneric)-\objective_1(\varFixed)
-\innerProduct{\varTangent}{\varTangentOther}_{\varFixed}
}{
\wassersteinDistance{\varFixed}{\varGeneric}{2}
}
+
\bigl(q(\varGeneric)-c\bigr)
\frac{
\innerProduct{\varTangent}{\varTangentOther}_{\varFixed}
}{
\wassersteinDistance{\varFixed}{\varGeneric}{2}
}.
\end{align*}
By Cauchy--Schwarz,
$
\abs{\innerProduct{\varTangent}{\varTangentOther}_{\varFixed}}
\le
\norm{\varTangent}_{\varFixed}\,
\norm{\varTangentOther}_{\varFixed}
=
\norm{\varTangent}_{\varFixed}\,
\wassersteinDistance{\varFixed}{\varGeneric}{2},
$
so that
\[
\bigl(q(\varGeneric)-c\bigr)
\frac{
\innerProduct{\varTangent}{\varTangentOther}_{\varFixed}
}{
\wassersteinDistance{\varFixed}{\varGeneric}{2}
}
\to 0
\qquad\text{as }\varGeneric\convergenceWasserstein\varFixed.
\]
Since $q(\varGeneric)\to c>0$ and $\varTangent\in \subgradientRegular{\objective_1}(\varFixed)$, we conclude that
\begin{align*}
\liminf_{\substack{
\varGeneric \convergenceWasserstein \varFixed
\\
\varTangentOther\in
\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}
{\setPlansOptimal{\varFixed}{\varGeneric}}
}}
&
\frac{1}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}\Bigl(
g(\objective_1(\varGeneric))-g(\objective_1(\varFixed))
\\&\qquad
-\innerProduct{c\varTangent}{\varTangentOther}_{\varFixed}
\Bigr)
\ge 0.
\end{align*}
Hence,
$
c\,\varTangent\in \subgradientRegular{(\comp{\objective_1}{g})}(\varFixed),
$
which proves the desired inclusion.}

{
We now prove the reverse inclusion. Since $g'(\alpha)>0$ and $g$ is continuously differentiable, there exists an open interval $I\subseteq\reals$ containing $\alpha$ such that $g$ is strictly increasing on $I$. Therefore, $g_{|I}$ admits an inverse
$
h:g(I)\to I,
$
which is continuously differentiable at $g(\alpha)$ and satisfies
$
h'(g(\alpha))=\frac{1}{g'(\alpha)}=\frac{1}{c}.
$
{We extend $h$ to a map $\realsBar \to \realsBar$ that is
continuously differentiable near $g(\alpha)$, strictly increasing, and satisfies
$h(+\infty) = +\infty$; since $\comp{\comp{\objective_1}{g}}{h}$ then coincides
with $\objective_1$ on a Wasserstein neighborhood of $\varFixed$, and regular
subgradients at $\varFixed$ depend only on the values of the functional near
$\varFixed$, the equality below holds.}
Because $\objective_1$ is continuous at $\varFixed$, after possibly restricting to a Wasserstein neighborhood of $\varFixed$ we may assume that $\objective_1(\varGeneric)\in I$, so that
$
\objective_1(\varGeneric)=h(g(\objective_1(\varGeneric)))
$
for all $\varGeneric \text{ close enough to }\varFixed$.
Applying the inclusion already proved to the functional $\comp{\objective_1}{g}$ and the map $h$, we obtain
\[
\frac{1}{c}\,
\subgradientRegular{(\comp{\objective_1}{g})}(\varFixed)
\subseteq
\subgradientRegular{(\comp{\comp{\objective_1}{g}}{h})}(\varFixed)
=
\subgradientRegular{\objective_1}(\varFixed).
\]
Therefore,
$
\subgradientRegular{(\comp{\objective_1}{g})}(\varFixed)
\subseteq
c\,\subgradientRegular{\objective_1}(\varFixed).
$
This proves the reverse inclusion and thus
$
\subgradientRegular{(\comp{\objective_1}{g})}(\varFixed)
=
g'(\objective_1(\varFixed))\,
\subgradientRegular{\objective_1}(\varFixed).
$}

{We now establish the statement for the general subgradient, under
the additional hypothesis that $\objective_1$ is continuous in Wasserstein on a
neighborhood of $\varFixed$ (cf.\ the statement).
To start, we collect the ingredients. Since $\objective_1$ is continuous at
$\varFixed$, for every sequence $\varGeneric_n \convergenceWasserstein \varFixed$ we
have $\alpha_n \coloneqq \objective_1(\varGeneric_n) \to \alpha \in \reals$; after
possibly shrinking the interval $I$ introduced above so that $g' > 0$ on $I$
(possible, since $g'$ is continuous at $\alpha$ with $g'(\alpha) = c > 0$), for $n$
sufficiently large we have $\alpha_n \in I$,
$c_n \coloneqq g'(\alpha_n) > 0$ with $c_n \to c$, and
$g(\alpha_n) \to g(\alpha) \in \reals$. Since, moreover, $\objective_1$ is
continuous at $\varGeneric_n$ for $n$ sufficiently large, the argument used above for the regular subgradients applies verbatim
at $\varGeneric_n$ (with the same interval $I$ and the same extension of
$h = (g_{|I})^{-1}$, which is continuously differentiable near $g(\alpha_n)$ for
$n$ sufficiently large) and yields
\[
\subgradientRegular{(\comp{\objective_1}{g})}(\varGeneric_n)
=
c_n\,\subgradientRegular{\objective_1}(\varGeneric_n).
\]
We also record that scaled variations converge: if $\lambda_n \to \lambda$ in
$\reals$ and $\varTangent_n \convergenceWasserstein \varTangent$, then
$\lambda_n \varTangent_n \convergenceWasserstein \lambda\varTangent$, since
$\wassersteinDistance{\lambda_n\varTangent_n}{\lambda_n\varTangent}{2} \leq
\max(1, \abs{\lambda_n})\wassersteinDistance{\varTangent_n}{\varTangent}{2}$ (the
map $(\bar x, \varTangentReals) \mapsto (\bar x, \lambda_n \varTangentReals)$ is
$\max(1, \abs{\lambda_n})$-Lipschitz) and
$\wassersteinDistance{\lambda_n\varTangent}{\lambda\varTangent}{2}^2 \leq
(\lambda_n - \lambda)^2 \int_{\reals^d\times\reals^d}
\norm{\varTangentReals}^2 \d\varTangent(\bar x, \varTangentReals)$.}

{Let now $\varTangentOther \in
\subgradient{(\comp{\objective_1}{g})}(\varFixed)$ and take sequences
$\varGeneric_n \convergenceWasserstein \varFixed$ with
$g(\objective_1(\varGeneric_n)) \to g(\objective_1(\varFixed))$ and
$\subgradientRegular{(\comp{\objective_1}{g})}(\varGeneric_n) \ni \varTangentOther_n
\convergenceWasserstein \varTangentOther$ (cf.
\cref{definition:def_sub_sup_differentiability}\ref{item:subgradient}). For $n$
sufficiently large, $\varTangent_n \coloneqq c_n^{-1} \varTangentOther_n \in
\subgradientRegular{\objective_1}(\varGeneric_n)$ by the display above, and
$\varTangent_n \convergenceWasserstein c^{-1}\varTangentOther$ since
$c_n^{-1} \to c^{-1} > 0$. As $\objective_1(\varGeneric_n) \to
\objective_1(\varFixed)$ by continuity of $\objective_1$ at $\varFixed$, we
conclude $c^{-1}\varTangentOther \in \subgradient{\objective_1}(\varFixed)$, i.e.,
$\varTangentOther = c\left(c^{-1}\varTangentOther\right) \in
g'(\objective_1(\varFixed))\,\subgradient{\objective_1}(\varFixed)$.
Conversely, let $\varTangent \in \subgradient{\objective_1}(\varFixed)$ and take
sequences $\varGeneric_n \convergenceWasserstein \varFixed$ with
$\objective_1(\varGeneric_n) \to \objective_1(\varFixed)$ and
$\subgradientRegular{\objective_1}(\varGeneric_n) \ni \varTangent_n
\convergenceWasserstein \varTangent$. For $n$ sufficiently large,
$c_n \varTangent_n \in
\subgradientRegular{(\comp{\objective_1}{g})}(\varGeneric_n)$ by the display above,
$c_n\varTangent_n \convergenceWasserstein c\varTangent$, and
$g(\objective_1(\varGeneric_n)) \to g(\objective_1(\varFixed))$ by continuity of
$g$ on $I$, so $c\varTangent \in
\subgradient{(\comp{\objective_1}{g})}(\varFixed)$. The two inclusions prove the
claim.}


    \item
{Let $\alpha \coloneqq \objective_1(\varFixed) \in \reals$,
$c \coloneqq g'(\alpha) \in \reals$ (possibly nonpositive), and
$\varTangentFixed \coloneqq \gradient{}{\objective_1}(\varFixed)$, which is induced
by a map by
\cref{proposition:prop_differentiability_properties}\ref{item:gradient_induced_by_map};
in particular,
$\innerProduct{\tau\varTangentFixed}{\varTangent}_{\varFixed} =
\tau\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}$ for all
$\tau \in \reals$ and all variations $\varTangent$ at $\varFixed$. Define $q$ as in
the proof of \ref{prop_calculus_chain_rule}; the argument there shows that
$q(\varGeneric) \to c$ as $\varGeneric \convergenceWasserstein \varFixed$ (it uses
only continuity of $\objective_1$ at $\varFixed$ and differentiability of $g$ at
$\alpha$, not the sign of $c$), so $q$ is bounded on a Wasserstein neighborhood of
$\varFixed$. By
\cref{proposition:prop_differentiability_properties}\ref{item:gradient_characterization},
for all $\varGeneric$ in a Wasserstein neighborhood of $\varFixed$ on which
$\objective_1$ is real-valued and $q$ is defined (which suffices, as the
$\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$ statements below only
constrain the behavior as $\varGeneric \convergenceWasserstein \varFixed$) and all
$\varTangent \in \pushforward{(\projection{1}{}, \projection{2}{} -
\projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$,
\begin{align*}
(\comp{\objective_1}{g})(\varGeneric) - (\comp{\objective_1}{g})(\varFixed)
&=
q(\varGeneric)\left(\objective_1(\varGeneric) - \objective_1(\varFixed)\right)
\\
&=
q(\varGeneric)\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
\\
&=
c\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
+
\left(q(\varGeneric) - c\right)
\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
\\&\qquad
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
\\
&=
\innerProduct{c\varTangentFixed}{\varTangent}_{\varFixed}
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}},
\end{align*}
where the second equality holds because $q$ is bounded near $\varFixed$, and the
last one because
$\left(q(\varGeneric) - c\right)\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
= \onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$ (by
$q(\varGeneric) \to c$ together with
$\abs{\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}} \leq
\norm{\varTangentFixed}_{\varFixed}\norm{\varTangent}_{\varFixed} =
\norm{\varTangentFixed}_{\varFixed}\wassersteinDistance{\varFixed}{\varGeneric}{2}$,
where the two-sided bound holds since $\varTangentFixed$ is induced by a map, so
the inner product is a single integral to which the Cauchy--Schwarz inequality
applies)
and because $c\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed} =
\innerProduct{c\varTangentFixed}{\varTangent}_{\varFixed}$ for any sign of $c$, as
$\varTangentFixed$ is induced by a map. Next, both $c\varTangentFixed$ and
$-c\varTangentFixed$ belong to $\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$: by
\cref{definition:def_differentiability} and
\cref{definition:def_sub_sup_differentiability}\ref{item:subgradient:regular}, both
$\varTangentFixed \in \subgradientRegular{\objective_1}(\varFixed)$ and
$-\varTangentFixed \in \subgradientRegular{(-\objective_1)}(\varFixed)$ lie in the
tangent space, and $\pm c\varTangentFixed \in \{\abs{c}\varTangentFixed,
\abs{c}(-\varTangentFixed)\}$, so
\cref{proposition:prop_sum_scale_well_defined} applies. Therefore, the display
above shows $c\varTangentFixed \in
\subgradientRegular{(\comp{\objective_1}{g})}(\varFixed)$ and, after negating it
and using $\innerProduct{-c\varTangentFixed}{\varTangent}_{\varFixed} =
-\innerProduct{c\varTangentFixed}{\varTangent}_{\varFixed}$,
$-c\varTangentFixed \in
\subgradientRegular{(-(\comp{\objective_1}{g}))}(\varFixed)$. By
\cref{definition:def_differentiability} and
\cref{proposition:prop_differentiability_properties}\ref{item:gradient_uniqueness},
$\comp{\objective_1}{g}$ is differentiable at $\varFixed$ with
$\gradient{}{(\comp{\objective_1}{g})}(\varFixed) \localEquiv{\varFixed}
c\varTangentFixed =
g'(\objective_1(\varFixed))\,\gradient{}{\objective_1}(\varFixed)$.}
\end{enumerate}


==> elements/prop_calculus_title.tex <==
Subdifferential calculus%

==> elements/prop_differentiability_properties_body.tex <==
Consider a functional $\objective: \Pp{2}{\reals^d} \to \realsBar$ and a probability measure $\varFixed \in \Pp{2}{\reals^d}$, where $\objective(\varFixed) \in \reals$. Then,
\begin{enumerate}[leftmargin=*]
\item
\label{item:subdifferential-cap-superdifferential}
For all $\varTangent_l \in \subgradientRegular{\objective}(\varFixed)$ and $\varTangent_u \in -\subgradientRegular{(-\objective)}(\varFixed)$, it holds $\varTangent_l \localEquiv{\varFixed} \varTangent_u$; in particular, either $\subgradientRegular{\objective}(\varFixed)$ or $\subgradientRegular{(-\objective)}(\varFixed)$ is empty, or $\objective$ is differentiable at $\varFixed$.
\item
\label{item:lowerbound:subdifferential}
If $G: \Pp{2}{\reals^d} \to \realsBar$ is a lower bound on $\objective$, i.e., $G(\varGeneric) \leq \objective(\varGeneric)$ for all $\varGeneric \in \Pp{2}{\reals^d}$ and $G(\varFixed) = \objective(\varFixed)$, then $\subgradientRegular{G}(\varFixed) \subseteq \subgradientRegular{\objective}(\varFixed)$.
\end{enumerate}
If $\objective$ is differentiable at $\varFixed$, the following statements hold:
\begin{enumerate}[leftmargin=*,start=3]
\item
\label{item:gradient_uniqueness}
For all $\varTangent_1,\varTangent_2 \in -\subgradientRegular{(-\objective)}(\varFixed) \cap \subgradientRegular{\objective}(\varFixed)$, $\varTangent_1 \localEquiv{\varFixed} \varTangent_2$. Thus, we call this unique element the {gradient} of $\objective$ at $\varFixed$, written $\gradient{{}}{\objective}(\varFixed)$.
In particular, it satisfies $\subgradientRegular{\objective}(\varFixed) \localEquiv{\varFixed} \{\gradient{{}}{\objective}(\varFixed)\} \subseteq \subgradient{\objective}(\varFixed)$.
\item
\label{item:gradient_characterization}
A tangent element $\varTangent \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ is the {gradient} of $\objective$ at $\varFixed$ if and only if for all $\varGeneric \in \Pp{2}{\reals^d}$ and $\varTangent' \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$ we have
\begin{equation}
\label{item:gradient_characterization:2}
\begin{aligned}
\objective(\varGeneric) - \objective(\varFixed)
&=
{\innerProduct{\varTangent}{\varTangent'}_{\varFixed}
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}}
\\
&=
{\underset{{\varTangentCoupling \in \setPlansCommonMarginal{\varTangent}{\varTangent'}{1}}}{\min}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_1}{\varTangentReals_2}
\d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}.}
\end{aligned}
\end{equation}
\item

\label{item:gradient_induced_by_map}
{The gradient is induced by a map: there exists a Borel
$\phi \in \Lp{2}{\reals^d}{\varFixed}$ so that
$\gradient{{}}{\objective}(\varFixed) =
\pushforward{(\identity{}, \phi)}{\varFixed}$. In particular, (1) for every
variation $\varTangent \in \PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$, the set
$\setPlansCommonMarginal{\varTangent}{\gradient{{}}{\objective}(\varFixed)}{1}$ is
a singleton, so sums with $\gradient{{}}{\objective}(\varFixed)$ do not depend on
the choice of the coupling; (2)
$\innerProduct{\tau\gradient{{}}{\objective}(\varFixed)}{\varTangent}_{\varFixed} =
\tau\innerProduct{\gradient{{}}{\objective}(\varFixed)}{\varTangent}_{\varFixed}$
for all $\tau \in \reals$ and all variations $\varTangent$ at $\varFixed$; and
(3) $\objective$ is continuous in Wasserstein at $\varFixed$.}
\end{enumerate}


==> elements/prop_differentiability_properties_proof.tex <==
We prove the statements separately:
\begin{enumerate}[leftmargin=*]
    \item
Let $\varTangent_l \in \subgradientRegular{\objective}(\varFixed)$ and $-\varTangent_u \in \subgradientRegular{(-\objective)}(\varFixed)$. We prove that $\varTangent_l=\varTangent_u$; i.e., if both $\objective$ and $-\objective$ admit a regular subgradient, then these coincide (up to the direction of the arrows) and $\objective$ is differentiable at $\varFixed$.
%
{We prove the claim in three
steps: we show that
\begin{equation}
\label{item:subgradient-characterization:nonpositive-all}
\innerProduct{\varTangent_l}{\varTangent}_{\varFixed}
+ \innerProduct{-\varTangent_u}{\varTangent}_{\varFixed}
\leq 0
\qquad \text{for all } \varTangent \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed},
\end{equation}
first for $\varTangent \in \tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed}$
(Step 1) and then, by density, on the whole tangent space (Step 2); we
conclude by evaluating
\eqref{item:subgradient-characterization:nonpositive-all} at
$\varTangent = \varTangent_l$ and $\varTangent = -\varTangent_u$ (Step 3).}

{\emph{Step 1
(\eqref{item:subgradient-characterization:nonpositive-all} in $\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed}$).}
Let $\varTangent \in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed}$.
If $\norm{\varTangent}_{\varFixed} = 0$, both inner products in \eqref{item:subgradient-characterization:nonpositive-all} are nonpositive by the Cauchy--Schwarz inequality (\cref{proposition:prop_wasserstein_geom}\ref{item:wass_geom:cauchy_schwarz}) and there is nothing to prove. Let then $\norm{\varTangent}_{\varFixed} > 0$.
By \eqref{definition:tangent_space}, there is $\bar\varepsilon > 0$ so that,
for all $\varepsilon \in (0, \bar\varepsilon)$,
$\pushforward{(\projection{1}{}, \projection{1}{} +
\varepsilon\projection{2}{})}{\varTangent} \in
\setPlansOptimal{\varFixed}{\varGeneric_\varepsilon}$ for
$\varGeneric_\varepsilon \coloneqq
\pushforward{(\projection{1}{} + \varepsilon\projection{2}{})}{\varTangent}$.
In particular, $\varepsilon\varTangent \in \pushforward{(\projection{1}{},
\projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric_\varepsilon}}$,
$\wassersteinDistance{\varFixed}{\varGeneric_\varepsilon}{2} =
\varepsilon\norm{\varTangent}_{\varFixed}$, and
$\varGeneric_\varepsilon \convergenceWasserstein \varFixed$ as
$\varepsilon \fromAbove 0$. Thus, both regular subgradient inequalities (for
$\varTangent_l \in \subgradientRegular{\objective}(\varFixed)$ and
$-\varTangent_u \in \subgradientRegular{(-\objective)}(\varFixed)$) apply
along $(\varGeneric_\varepsilon, \varepsilon\varTangent)$. In particular, we
may assume without loss of generality $\objective(\varGeneric_\varepsilon) \in \reals$ for all
$\varepsilon$ sufficiently small; otherwise, were $\objective(\varGeneric_\varepsilon) = +\infty$ (resp.,\ $-\infty$) along a
subsequence $\varepsilon \fromAbove 0$, the difference quotient in the regular subgradient inequality for
$-\varTangent_u \in \subgradientRegular{(-\objective)}(\varFixed)$
(resp.,\ $\varTangent_l \in \subgradientRegular{\objective}(\varFixed)$) would
tend to $-\infty$, contradicting that inequality.
Thus, with \cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:homogeneity}, we get
\begin{align*}
0
&\leq
\liminf_{\varepsilon \fromAbove 0}
\frac{\objective(\varGeneric_\varepsilon) - \objective(\varFixed)
- \innerProduct{\varTangent_l}{\varepsilon\varTangent}_{\varFixed}}
{\wassersteinDistance{\varFixed}{\varGeneric_\varepsilon}{2}}
\\
&\hphantom{{}\leq{}} +
\liminf_{\varepsilon \fromAbove 0}
\frac{-\objective(\varGeneric_\varepsilon) + \objective(\varFixed)
- \innerProduct{-\varTangent_u}{\varepsilon\varTangent}_{\varFixed}}
{\wassersteinDistance{\varFixed}{\varGeneric_\varepsilon}{2}}
\\
&\leq
\liminf_{\varepsilon \fromAbove 0}
\left(
-
\frac{\varepsilon\innerProduct{\varTangent_l}{\varTangent}_{\varFixed}
+ \varepsilon\innerProduct{-\varTangent_u}{\varTangent}_{\varFixed}}
{\varepsilon\norm{\varTangent}_{\varFixed}}
\right)
\\
&=
-\frac{\innerProduct{\varTangent_l}{\varTangent}_{\varFixed}
+ \innerProduct{-\varTangent_u}{\varTangent}_{\varFixed}}
{\norm{\varTangent}_{\varFixed}};
\end{align*}
i.e., \eqref{item:subgradient-characterization:nonpositive-all} holds on $\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed}$}.

{\emph{Step 2 (extension to the tangent space).}
Both $\varTangent \mapsto \innerProduct{\varTangent_l}{\varTangent}_{\varFixed}$
and
$\varTangent \mapsto \innerProduct{-\varTangent_u}{\varTangent}_{\varFixed}$
are continuous with respect to $\wassersteinDistance{}{}{\varFixed}$
(\cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:continuity_wass}).
Since $\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ is the closure with respect
to $\wassersteinDistance{}{}{\varFixed}$ of the set in
\eqref{definition:tangent_space}, Step 1 extends by continuity and
\eqref{item:subgradient-characterization:nonpositive-all} holds on all of
$\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.}

{\emph{Step 3 (conclusion).}
As regular subgradients, both $\varTangent_l$ and $-\varTangent_u$ belong to
$\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ (cf.
\cref{definition:def_sub_sup_differentiability}\ref{item:subgradient:regular}),
so \eqref{item:subgradient-characterization:nonpositive-all} applies to both.
Using
$\innerProduct{\varTangent}{\varTangent}_{\varFixed} =
\norm{\varTangent}_{\varFixed}^2$
(\cref{proposition:prop_wasserstein_geom}\ref{item:wass_geom:cauchy_schwarz})
and $\norm{-\varTangent_u}_{\varFixed} = \norm{\varTangent_u}_{\varFixed}$, we obtain
$
\norm{\varTangent_l}_{\varFixed}^2
+ \innerProduct{-\varTangent_u}{\varTangent_l}_{\varFixed}
\leq 0
$
and
$
\innerProduct{\varTangent_l}{-\varTangent_u}_{\varFixed}
+ \norm{\varTangent_u}_{\varFixed}^2
\leq 0
$, and so, by the symmetry of the inner product,
\[
\norm{\varTangent_l}_{\varFixed}^2
+ \norm{\varTangent_u}_{\varFixed}^2
+ 2\innerProduct{-\varTangent_u}{\varTangent_l}_{\varFixed}
\leq 0.
\]
By \cref{lemma:lemma_pushforward_and_optimal_transport},
$\innerProduct{-\varTangent_u}{\varTangent_l}_{\varFixed} =
-\min_{\varTangentCoupling \in
\setPlansCommonMarginal{\varTangent_u}{\varTangent_l}{1}}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_u}{\varTangentReals_l}
\d\varTangentCoupling(\bar x, \varTangentReals_u, \varTangentReals_l)
\geq -\innerProduct{\varTangent_u}{\varTangent_l}_{\varFixed}$, the minimum
never exceeding the maximum in \eqref{definition:geometry:inner_product} over
the same set of couplings, and so
\[
0
\geq
\norm{\varTangent_l}_{\varFixed}^2
+ \norm{\varTangent_u}_{\varFixed}^2
- 2\innerProduct{\varTangent_u}{\varTangent_l}_{\varFixed}
=
\wassersteinDistance{\varTangent_u}{\varTangent_l}{\varFixed}^2,
\]
where the last equality follows from \cref{proposition:prop_wasserstein_geom}\ref{item:distance_norm_innerproduct}.
Therefore, $\wassersteinDistance{\varTangent_u}{\varTangent_l}{\varFixed} = 0$
and, thus, $\varTangent_u = \varTangent_l$; see
\cite[Proposition 12.4.6]{ambrosio2005gradient}.}

\item
For any $\varTangent \in \subgradientRegular{G}(\varFixed)$ and any $\varGeneric \in \Pp{2}{\reals^d}$ we have
$\objective(\varGeneric) - \objective(\varFixed)
\geq
G(\varGeneric) - G(\varFixed)
\geq
\sup_{\varTangentOther \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}}\innerProduct{\varTangent}{\varTangentOther}_{\varFixed} + \onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$
and so $\varTangent \in \subgradientRegular{\objective}(\varFixed)$.

\item This statement follows from \ref{item:subdifferential-cap-superdifferential}.

\item
We prove the two directions separately.

We start by showing that if $\varTangent \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ satisfies \eqref{item:gradient_characterization:2}, then $\objective$ is differentiable with $\varTangent \localEquiv{\varFixed} \gradient{{}}{\objective}(\varFixed)$. Indeed, if $\varTangent$ satisfies \eqref{item:gradient_characterization:2}, $\varTangent \in \subgradientRegular{\objective}(\varFixed)$.
Since $\objective$ is differentiable at $\varFixed$ by assumption, \ref{item:gradient_uniqueness} gives $\subgradientRegular{\objective}(\varFixed) \localEquiv{\varFixed} \{\gradient{{}}{\objective}(\varFixed)\}$, and therefore $\varTangent \localEquiv{\varFixed} \gradient{{}}{\objective}(\varFixed)$.

On the other hand, {let $\varTangent \localEquiv{\varFixed} \gradient{{}}{\objective}(\varFixed)$.
Then,} $\varTangent \in \subgradientRegular{\objective}(\varFixed)$ and, for all $\varGeneric \in \Pp{2}{\reals^d}$ and $\varTangent' \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$, we have
$\objective(\varGeneric) - \objective(\varFixed)
\geq
{\max_{
\varTangentCoupling
\in
\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}
}}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$.
Moreover, since also $-\varTangent \in \subgradientRegular{(-\objective)}(\varFixed)$, using \cref{lemma:lemma_pushforward_and_optimal_transport} we get
\begin{align*}
    -\objective(\varGeneric) -
    (-\objective(\varFixed))
    &\geq
    {\max_{
    \varTangentCoupling
    \in
\setPlansCommonMarginal{-\varTangent}{\varTangent'}{1}
    }}
    \int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
    \\&\qquad
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
    +
    \onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
    \\&=
    {\max_{
    \varTangentCoupling
    \in
\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}
    }}
    \int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{-\varTangentReals}{\varTangentReals'}
    \\&\qquad
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
    +
    \onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
    \\&=
    -\inf_{
    \varTangentCoupling
    \in
\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}
    }
    \int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
    \\&\qquad
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
    +
    \onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
    \\
    \Leftrightarrow
    \objective(\varGeneric) - \objective(\varFixed)
    &\leq
    \inf_{
    \varTangentCoupling
    \in
\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}
    }
    \int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
    \\&\qquad
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
    +
    \onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}.
\end{align*}
As a result, we have
${\max_{
\varTangentCoupling
\in
\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}
}}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
\leq
\inf_{
\varTangentCoupling
\in
\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}
}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$, which is equivalent to
${\max_{
\varTangentCoupling
\in
\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}
}}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
=
\inf_{
\varTangentCoupling
\in
\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}
}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals')
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$.
{To conclude, we show that the infimum is attained. The set $\setPlansCommonMarginal{\varTangent}{\varTangent'}{1}$ is narrowly compact, since it is a set of couplings with fixed marginals \cite[Remark 5.2.3]{ambrosio2005gradient}. Moreover, the map
$
\varTangentCoupling \mapsto
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals}{\varTangentReals'}
\d\varTangentCoupling(\bar x,\varTangentReals,\varTangentReals')
$
is continuous on this set \cite[Lemma 5.2.4]{ambrosio2005gradient}. Thus, the infimum is attained and the statement follows.}


\item
{Abbreviate
$\varTangentFixed \coloneqq \gradient{{}}{\objective}(\varFixed)$. We first prove
the map structure, in four steps, and then (1)--(3).}

{\emph{Step 1 (a max--min identity along tangent directions).}
For every variation $\varTangent$ at $\varFixed$,
\cref{lemma:lemma_pushforward_and_optimal_transport} yields
\begin{equation}
\label{item:gradient_induced_by_map:minus_is_min}
\innerProduct{-\varTangentFixed}{\varTangent}_{\varFixed}
=
-
\min_{\varTangentCoupling \in
\setPlansCommonMarginal{\varTangentFixed}{\varTangent}{1}}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_1}{\varTangentReals_2}
\d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2).
\end{equation}
In particular, since the minimum in
\eqref{item:gradient_induced_by_map:minus_is_min} never exceeds the maximum in
\eqref{definition:geometry:inner_product} over the same set of couplings,
$\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed} +
\innerProduct{-\varTangentFixed}{\varTangent}_{\varFixed} \geq 0$ for every
variation $\varTangent$ at $\varFixed$.}
{We claim that, conversely,
\begin{equation}
\label{item:gradient_induced_by_map:max_equals_min}
\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
+
\innerProduct{-\varTangentFixed}{\varTangent}_{\varFixed}
=
0
\qquad
\text{for all }
\varTangent \in
\tangentCone{\Pp{2}{\reals^d}}{\varFixed}.
\end{equation}
Indeed, since $\objective$ is differentiable at
$\varFixed$, \cref{definition:def_differentiability} gives
$\varTangentFixed \in \subgradientRegular{\objective}(\varFixed)$ and
$-\varTangentFixed \in \subgradientRegular{(-\objective)}(\varFixed)$, so
\eqref{item:subgradient-characterization:nonpositive-all}, established in the
proof of \ref{item:subdifferential-cap-superdifferential}, applies with
$\varTangent_l = \varTangent_u = \varTangentFixed$ and gives
$\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed} +
\innerProduct{-\varTangentFixed}{\varTangent}_{\varFixed} \leq 0$ for all
$\varTangent \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$. This proves
\eqref{item:gradient_induced_by_map:max_equals_min}.}

{\emph{Step 2 (the minimum over the self-couplings of the gradient
equals its squared norm).} We claim that
\begin{equation}
\label{item:gradient_induced_by_map:min_self}
\min_{\varTangentCoupling \in
\setPlansCommonMarginal{\varTangentFixed}{\varTangentFixed}{1}}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_1}{\varTangentReals_2}
\d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
=
\norm{\varTangentFixed}_{\varFixed}^2.
\end{equation}
As a regular subgradient, $\varTangentFixed$ belongs to
$\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ (cf.
\cref{definition:def_sub_sup_differentiability}\ref{item:subgradient:regular}),
so evaluating \eqref{item:gradient_induced_by_map:max_equals_min} at
$\varTangent = \varTangentFixed$ gives
$\innerProduct{\varTangentFixed}{\varTangentFixed}_{\varFixed} +
\innerProduct{-\varTangentFixed}{\varTangentFixed}_{\varFixed} = 0$. Since
$\innerProduct{\varTangentFixed}{\varTangentFixed}_{\varFixed} =
\norm{\varTangentFixed}_{\varFixed}^2$
(\cref{proposition:prop_wasserstein_geom}\ref{item:wass_geom:cauchy_schwarz}),
this reads
$\innerProduct{-\varTangentFixed}{\varTangentFixed}_{\varFixed} =
-\norm{\varTangentFixed}_{\varFixed}^2$, which is
\eqref{item:gradient_induced_by_map:min_self} in view of
\eqref{item:gradient_induced_by_map:minus_is_min} with
$\varTangent = \varTangentFixed$.}

{\emph{Step 3 (every self-coupling of the gradient is concentrated
on the diagonal).} Let $\varTangentCoupling \in
\setPlansCommonMarginal{\varTangentFixed}{\varTangentFixed}{1}$ be arbitrary.
By~\eqref{item:gradient_induced_by_map:min_self}, we have
$\int_{\reals^d\times\reals^d\times\reals^d} \innerProduct{\varTangentReals_1}{\varTangentReals_2} \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
\geq \norm{\varTangentFixed}_{\varFixed}^2$. For the reverse bound, we integrate
with respect to $\varTangentCoupling$ the pointwise Young inequality
$\innerProduct{\varTangentReals_1}{\varTangentReals_2} \leq
\frac{1}{2}\norm{\varTangentReals_1}^2 + \frac{1}{2}\norm{\varTangentReals_2}^2$
(which amounts to
$0 \leq \frac{1}{2}\norm{\varTangentReals_1 - \varTangentReals_2}^2$).
Since
$\pushforward{\projection{12}{}}{\varTangentCoupling} =
\pushforward{\projection{13}{}}{\varTangentCoupling} = \varTangentFixed$, both
$\int_{\reals^d\times\reals^d\times\reals^d} \norm{\varTangentReals_1}^2 \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)$ and
$\int_{\reals^d\times\reals^d\times\reals^d} \norm{\varTangentReals_2}^2 \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)$ equal
$\int_{\reals^d\times\reals^d} \norm{\varTangentReals}^2
\d\varTangentFixed(\bar x, \varTangentReals) =
\norm{\varTangentFixed}_{\varFixed}^2$ (cf. \eqref{definition:geometry:norm}), so
that
$\int_{\reals^d\times\reals^d\times\reals^d} \innerProduct{\varTangentReals_1}{\varTangentReals_2} \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
\leq \norm{\varTangentFixed}_{\varFixed}^2$. Hence, equality holds, and,
expanding the square,
\[
\int_{\reals^d\times\reals^d\times\reals^d}
\norm{\varTangentReals_1 - \varTangentReals_2}^2 \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
=
2\norm{\varTangentFixed}_{\varFixed}^2
-
2\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_1}{\varTangentReals_2} \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
=
0;
\]
i.e., $\varTangentReals_1 = \varTangentReals_2$ holds
$\almostEverywhere{\varTangentCoupling}$.}

{\emph{Step 4 (the gradient is induced by a map).} Disintegrate
$\varTangentFixed$ with respect to its first marginal $\varFixed$ (cf.
\cite[Theorem 5.3.1]{ambrosio2005gradient}): there is a Borel family
$\{(\varTangentFixed)_{\bar x}\}_{\bar x \in \reals^d} \subseteq \Pp{}{\reals^d}$,
with $\int_{\reals^d} \norm{\varTangentReals}^2
\d(\varTangentFixed)_{\bar x}(\varTangentReals) < \infty$ for $\varFixed$-almost
every $\bar x$, so that $\varTangentFixed = \int_{\reals^d} \delta_{\bar x}
\times (\varTangentFixed)_{\bar x} \d\varFixed(\bar x)$. Consider
\[
\varTangentCoupling^\ast
\coloneqq
\int_{\reals^d}
\delta_{\bar x}
\times (\varTangentFixed)_{\bar x}
\times (\varTangentFixed)_{\bar x}
\d\varFixed(\bar x),
\]
i.e., the coupling of two copies of $\varTangentFixed$ under which the two arrows
are drawn independently from $(\varTangentFixed)_{\bar x}$, conditionally on the
base point $\bar x$. Since
$\pushforward{\projection{12}{}}{\varTangentCoupling^\ast}=\pushforward{\projection{13}{}}{\varTangentCoupling^\ast}=\varTangentFixed$, we have $\varTangentCoupling^\ast \in
\setPlansCommonMarginal{\varTangentFixed}{\varTangentFixed}{1}$, and Step 3 gives
\[
1
=
\varTangentCoupling^\ast\left(\left\{\varTangentReals_1 =
\varTangentReals_2\right\}\right)
=
\int_{\reals^d}
\left((\varTangentFixed)_{\bar x} \times (\varTangentFixed)_{\bar x}\right)
\left(\left\{(\varTangentReals_1, \varTangentReals_2)
\st \varTangentReals_1 = \varTangentReals_2\right\}\right)
\d\varFixed(\bar x),
\]
so that $(\varTangentFixed)_{\bar x} \times (\varTangentFixed)_{\bar x}$ is
concentrated on the diagonal for $\varFixed$-almost every $\bar x$. For a
probability measure $\theta \in \Pp{}{\reals^d}$, the Fubini--Tonelli theorem
gives
$(\theta \times \theta)\left(\left\{\varTangentReals_1 =
\varTangentReals_2\right\}\right) = \int_{\reals^d}
\theta(\{\varTangentReals\}) \d\theta(\varTangentReals)$, which equals $1$ if and
only if $\theta(\{\varTangentReals\}) = 1$ for $\theta$-almost every
$\varTangentReals$, i.e., if and only if $\theta$ is a Dirac measure. Therefore,
for $\varFixed$-almost every $\bar x$,
$(\varTangentFixed)_{\bar x} = \delta_{\phi(\bar x)}$, where
$\phi(\bar x) \coloneqq \int_{\reals^d} \varTangentReals
\d(\varTangentFixed)_{\bar x}(\varTangentReals)$ is Borel (by measurability of
the disintegration) and belongs to $\Lp{2}{\reals^d}{\varFixed}$, since
$\int_{\reals^d} \norm{\phi(\bar x)}^2 \d\varFixed(\bar x) =
\int_{\reals^d\times\reals^d} \norm{\varTangentReals}^2 \d\varTangentFixed(\bar x, \varTangentReals) =
\norm{\varTangentFixed}_{\varFixed}^2 < \infty$. Hence,
$\varTangentFixed = \int_{\reals^d} \delta_{\bar x} \times \delta_{\phi(\bar x)}
\d\varFixed(\bar x) = \pushforward{(\identity{}, \phi)}{\varFixed}$, as claimed.}

{\emph{Step 5 (consequences).} For (1), let $\varTangent$ be a
variation at $\varFixed$ and $\varTangentCoupling \in
\setPlansCommonMarginal{\varTangent}{\varTangentFixed}{1}$. Its marginal
$\pushforward{\projection{13}{}}{\varTangentCoupling} = \varTangentFixed$ is
concentrated on the graph $\{(\bar x, \phi(\bar x)) \st \bar x \in \reals^d\}$,
so $\varTangentReals_2 = \phi(\bar x)$ holds $\almostEverywhere{\varTangentCoupling}$ and, consequently, $\varTangentCoupling$ is the pushforward of
$\varTangent$ under $(\bar x, \varTangentReals) \mapsto
(\bar x, \varTangentReals, \phi(\bar x))$.
Conversely, this pushforward always
belongs to $\setPlansCommonMarginal{\varTangent}{\varTangentFixed}{1}$, which is
therefore a singleton. For (2), observe that, for $\tau \in \reals$,
$\tau\varTangentFixed = \pushforward{(\identity{}, \tau\phi)}{\varFixed}$ (cf.
\cref{definition:def_almost_linear_structure_wass}\ref{item:local-scale}) is again
induced by a map, so, by the argument of (1), the unique element of
$\setPlansCommonMarginal{\tau\varTangentFixed}{\varTangent}{1}$ is the pushforward
of $\varTangent$ under $(\bar x, \varTangentReals) \mapsto
(\bar x, \tau\phi(\bar x), \varTangentReals)$, whence
\[
\innerProduct{\tau\varTangentFixed}{\varTangent}_{\varFixed}
=
\int_{\reals^d\times\reals^d}
\innerProduct{\tau\phi(\bar x)}{\varTangentReals}
\d\varTangent(\bar x, \varTangentReals)
=
\tau
\int_{\reals^d\times\reals^d}
\innerProduct{\phi(\bar x)}{\varTangentReals}
\d\varTangent(\bar x, \varTangentReals)
=
\tau\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed},
\]
where the last equality is the case $\tau = 1$ of the first two equalities.
For (3), let
$\varGeneric_k \convergenceWasserstein \varFixed$ (without loss of generality,
$\varGeneric_k \neq \varFixed$ for all $k$) and pick any
$\varTangent_k \in \pushforward{(\projection{1}{}, \projection{2}{} -
\projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric_k}}$, so that
$\norm{\varTangent_k}_{\varFixed} =
\wassersteinDistance{\varFixed}{\varGeneric_k}{2}$. Since
$\pushforward{\projection{1}{}}{\varTangent_k} = \varFixed$, the Cauchy--Schwarz
inequality in $\Lp{2}{\reals^d\times\reals^d}{\varTangent_k}$ gives
$\abs{\int_{\reals^d\times\reals^d} \innerProduct{\phi(\bar x)}{\varTangentReals}\d\varTangent_k(\bar x, \varTangentReals)} \leq
(\int_{\reals^d\times\reals^d} \norm{\phi(\bar x)}^2 \d\varTangent_k(\bar x, \varTangentReals))^{1/2}
(\int_{\reals^d\times\reals^d} \norm{\varTangentReals}^2 \d\varTangent_k(\bar x, \varTangentReals))^{1/2} =
\norm{\varTangentFixed}_{\varFixed}
\wassersteinDistance{\varFixed}{\varGeneric_k}{2}$ and, thus, by (2) with
$\tau = \pm1$,
$\abs{\innerProduct{\pm\varTangentFixed}{\varTangent_k}_{\varFixed}} \leq
\norm{\varTangentFixed}_{\varFixed}
\wassersteinDistance{\varFixed}{\varGeneric_k}{2}$. The subgradient inequalities
for $\varTangentFixed \in \subgradientRegular{\objective}(\varFixed)$ and
$-\varTangentFixed \in \subgradientRegular{(-\objective)}(\varFixed)$ along
$(\varGeneric_k, \varTangent_k)$ then give
\[
-\norm{\varTangentFixed}_{\varFixed}
\leq
\liminf_{k \to \infty}
\frac{\objective(\varGeneric_k) - \objective(\varFixed)}
{\wassersteinDistance{\varFixed}{\varGeneric_k}{2}}
\leq
\limsup_{k \to \infty}
\frac{\objective(\varGeneric_k) - \objective(\varFixed)}
{\wassersteinDistance{\varFixed}{\varGeneric_k}{2}}
\leq
\norm{\varTangentFixed}_{\varFixed};
\]
in particular, $\objective(\varGeneric_k) \in \reals$ for $k$ sufficiently large
and $\objective(\varGeneric_k) \to \objective(\varFixed)$. Since the sequence was
arbitrary, $\objective$ is continuous in Wasserstein at $\varFixed$.}
\end{enumerate}


==> elements/prop_differentiability_properties_title.tex <==
Characterization of the (sub)gradients%

==> elements/prop_epigraph_normal_tangent_body.tex <==
For $\objective: \Pp{2}{\reals^d} \to \realsBar$, consider $\varFixed \in \Pp{2}{\reals^d}$ at which $\objective$ is finite. For all
 $\boldsymbol{\varTangent} \in \normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ (i.e., at the boundary of $\epigraph{\objective}$) we have $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}} \leq 0$.

==> elements/prop_epigraph_normal_tangent_proof.tex <==
We prove the result for the regular normal cone, and then argue by continuity for the general normal cone.
%
Let $\boldsymbol{\varTangent}\in \normalConeRegular{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ and suppose, for the sake of contradiction, that
$\beta\coloneqq\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}} > 0$.
%
In this case, $(\varFixed\times\delta_{\objective(\varFixed)})\times(\delta_0\times\delta_\beta)$ belongs to the tangent cone $\tangentCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$.
%
Indeed, {note first that
$(\varFixed\times\delta_{\objective(\varFixed)})\times(\delta_0\times\delta_\beta)\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varFixed\times\delta_{\objective(\varFixed)}}$:}
{with $T$ as in \eqref{equation:extraction-map-epigraph},
$\pushforward{T}{(\varFixed\times\delta_{\objective(\varFixed)})\times(\delta_0\times\delta_\beta)}=\localZero{\varFixed}$
is tangent at $\varFixed$, so the claim follows from
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}.} Consider the sequences $\varGeneric_n = \varFixed \convergenceWasserstein \varFixed$ and $\lambda_n \coloneqq \objective(\varFixed) + \beta\tau_n\geq \objective(\varFixed)$ for some $\tau_n\fromAbove0$.
Then,
$\varFixed\times\delta_{\lambda_n}\in\epigraph{\objective}$ for all $n$ and
$\varFixed\times\delta_{\lambda_n}\convergenceWasserstein\varFixed\times \delta_{\objective(\varFixed)}$.
{Moreover, by
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport}
(product-target case, with $b=\objective(\varFixed)$, $\varGeneric=\varFixed$, and
$\beta=\lambda_n$) and since $\setPlansOptimal{\varFixed}{\varFixed}$ is the identity
transport plan,
$\boldsymbol{\varTangent}_n\coloneqq(\varFixed\times\delta_{\objective(\varFixed)})\times(\delta_0\times\delta_{\lambda_n-\objective(\varFixed)})$
is the variation induced by the unique optimal transport plan between
$\varFixed\times\delta_{\objective(\varFixed)}$ and $\varFixed\times\delta_{\lambda_n}$,
with last velocity component almost everywhere $\lambda_n-\objective(\varFixed)$.}
Then, $\frac{1}{\tau_n}\boldsymbol{\varTangent}_n=(\varFixed\times\delta_{\objective(\varFixed)})
\times
(\delta_0\times\delta_{\frac{\lambda_n-\objective(\varFixed)}{\tau_n}})=(\varFixed\times\delta_{\objective(\varFixed)})
\times
(\delta_0\times\delta_{\beta})$.
In particular, $\frac{1}{\tau_n}\boldsymbol{\varTangent}_n\convergenceWasserstein(\varFixed\times\delta_{\objective(\varFixed)})
\times
(\delta_0\times\delta_{\beta})$, which therefore belongs to $\tangentCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$.
%
We can now show that the inner product between $\boldsymbol{\varTangent}$ and this tangent vector is strictly positive, which contradicts~\cref{proposition:prop_normal_tangent_cones}.
Specifically,
    {by
    \cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting}
    (with $c=\beta$ and the variation
    $(\varFixed\times\delta_{\objective(\varFixed)})\times(\delta_0\times\delta_\beta)$,
    whose last velocity component is almost everywhere $\beta$) and
    $\pushforward{T}{(\varFixed\times\delta_{\objective(\varFixed)})\times(\delta_0\times\delta_\beta)}=\localZero{\varFixed}$,
    $\innerProduct{\boldsymbol{\varTangent}}{(\varFixed\times\delta_{\objective(\varFixed)})\times(\delta_0\times\delta_\beta)}_{\varFixed\times\delta_{\objective(\varFixed)}}
    =
    \beta\,\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}
    =
    \beta^2>0$,
    where the last equality is the definition of $\beta$.}
This contradicts~\cref{proposition:prop_normal_tangent_cones}, and concludes the proof for the regular normal cone.
%
{The argument above applies verbatim at any
$\varGeneric\times\delta_b\in\epigraph{\objective}$, replacing
$\objective(\varFixed)$ by $b$ and setting $\lambda_n\coloneqq b+\beta\tau_n\geq
b\geq\objective(\varGeneric)$, so every regular normal at every point of
$\epigraph{\objective}$ satisfies the claimed bound. Since any
$\boldsymbol{\varTangent}\in\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$
is the Wasserstein limit of such regular normals and the map
$\boldsymbol{\varTangent}\mapsto\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}$
is continuous in Wasserstein, the bound passes to the
limit.}


==> elements/prop_epigraph_normal_tangent_title.tex <==
Characterization of the epigraphical normals%

==> elements/prop_functional_expected_value_body.tex <==
Let $V: \reals^d \to (-\infty, +\infty]$ be a proper, lower semicontinuous, and $\lambda$-convex (i.e., $x\mapsto V(x)-\frac{\lambda}{2}\norm{x}^2$ is convex, with $\lambda\in\reals$) function.
Consider the functional $\objective: \Pp{2}{\reals^d} \to \realsBar$,
$
\objective(\varGeneric)
\coloneqq
\expectedValue{x \sim \varGeneric}{V(x)}.
$
Then,
\begin{enumerate}
\item $\objective$ is proper and lower semicontinuous.
\item At every $\varFixed \in \Pp{2}{\reals^d}$ at which $\objective$ is finite, $\varTangent \in \subgradientRegular{\objective}(\varFixed)$ (resp. $\varTangent \in \subgradient{\objective}(\varFixed)$)
if and only if for all $(x, y) \in \supp{(\varTangent)}$, $y \in \subgradientRegular{V}(x)$ (resp. $y \in \subgradient{V}(x)$).
%
\item\label{prop_functional_expected_value_differentiable} If $V$ is differentiable and $V(x) \leq C(1+ \norm{x}^2)$ for some $C>0$, $\objective$ is differentiable at any $\varFixed \in \Pp{2}{\reals^d}$ and
$
\gradient{}{\objective}(\varFixed)
\localEquiv{\varFixed}
\pushforward{(\identity{}, \gradient{}{V})}{\varFixed}.
$
\end{enumerate}


==> elements/prop_functional_expected_value_proof.tex <==
We prove the statements separately.
\begin{enumerate}
\item See \cite[Proposition 10.4.2]{ambrosio2005gradient}.
\item The proposed subgradients are in our definition of tangent space in virtue of $\lambda$-convexity of $V$ by an argument analogous to \cite[Lemma 2.6]{Lanzetti2022}. Then the result follows from approximation (cf. \cite[Proposition 5.1.8]{ambrosio2005gradient}) and by definition of the general subgradient (cf. \cref{definition:def_sub_sup_differentiability}), in view of \cref{proposition:prop_subgradient_convex}.
\item
{Set $\varTangentFixed\coloneqq\pushforward{(\identity{},\gradient{}{V})}{\varFixed}$.
We show that $\objective$ is differentiable at every $\varFixed\in\Pp{2}{\reals^d}$
with $\gradient{}{\objective}(\varFixed)\localEquiv{\varFixed}\varTangentFixed$; when
$V\in\C{2}{\reals^d}{}$ has uniformly bounded Hessian, this is
\cite[Proposition 2.20]{Lanzetti2022}.}

{\emph{Step 1 (linear growth of $\gradient{}{V}$).}
Since $V$ is differentiable, it is real-valued, and
$W\coloneqq V-\frac{\lambda}{2}\norm{\cdot}^2$ is a finite, differentiable, convex
function with $\gradient{}{W}=\gradient{}{V}-\lambda\identity{}$. The hypothesis $V(x)\leq C(1+\norm{x}^2)$ is one half of a two-sided quadratic
bound; the other half is an explicit quadratic minorant of the $\lambda$-convex
$V$. With $g\coloneqq\gradient{}{W}(0)$, the subgradient inequality for the convex
$W$ at $0$, namely $W(x)\geq W(0)+\innerProduct{g}{x}$, reads
$
V(x)\geq V(0)+\innerProduct{g}{x}+\tfrac{\lambda}{2}\norm{x}^2
$ for all $x\in\reals^d$.
Since $\innerProduct{g}{x}\geq-\tfrac{1}{2}\norm{g}^2-\tfrac{1}{2}\norm{x}^2$ and
$\tfrac{\lambda}{2}\norm{x}^2\geq-\tfrac{\abs{\lambda}}{2}\norm{x}^2$, this yields
$V(x)\geq-C_0(1+\norm{x}^2)$ for some $C_0>0$; combined with the upper bound
(enlarging $C_0$ so that $C_0\geq C$), $\abs{V(x)}\leq C_0(1+\norm{x}^2)$, and hence
$\abs{W(x)}\leq C_0'(1+\norm{x}^2)$ for some $C_0'>0$. In particular,
$\objective(\varGeneric)=\expectedValue{x\sim\varGeneric}{V(x)}\in\reals$ for all
$\varGeneric\in\Pp{2}{\reals^d}$. Convexity of $W$ together with this bound forces
the linear growth $\norm{\gradient{}{V}(x)}\leq C_1(1+\norm{x})$ for some $C_1>0$.
Indeed, the gradient inequality for the convex function $W$ gives
$\innerProduct{\gradient{}{W}(x)}{h}\leq W(x+h)-W(x)$ for all $h$. Fix $x$ with
$\gradient{}{W}(x)\neq0$ (otherwise the bound below is trivial) and evaluate this
at $h=(1+\norm{x})\gradient{}{W}(x)/\norm{\gradient{}{W}(x)}$, so that
$\norm{h}=1+\norm{x}$ and hence $\norm{x+h}\leq 1+2\norm{x}$; then
\begin{align*}
(1+\norm{x})\norm{\gradient{}{W}(x)}
&=\innerProduct{\gradient{}{W}(x)}{h}\leq W(x+h)-W(x)\\
&\leq C_0'(1+\norm{x+h}^2)+C_0'(1+\norm{x}^2)\\
&\leq C_0'\big(2+(1+2\norm{x})^2+\norm{x}^2\big)\leq 5C_0'(1+\norm{x})^2,
\end{align*}
where we used $\abs{W}\leq C_0'(1+\norm{\cdot}^2)$ in the second line and
$\norm{x+h}\leq 1+2\norm{x}$ in the third. Dividing by $1+\norm{x}>0$ yields
$\norm{\gradient{}{W}(x)}\leq 5C_0'(1+\norm{x})$, which also holds trivially when
$\gradient{}{W}(x)=0$. Since $\gradient{}{V}=\gradient{}{W}+\lambda\identity{}$, we
conclude $\norm{\gradient{}{V}(x)}\leq 5C_0'(1+\norm{x})+\abs{\lambda}\norm{x}\leq
C_1(1+\norm{x})$ with $C_1\coloneqq 5C_0'+\abs{\lambda}$. Consequently $\gradient{}{V}\in\Lp{2}{\reals^d}{\varFixed}$, and
$\varTangentFixed\in\PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$.}

{\emph{Step 2 (first-order estimate).}
Fix $\varGeneric\in\Pp{2}{\reals^d}$, an optimal transport plan
$\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varGeneric}$, and the induced variation
$\varTangent\coloneqq\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\varPlanGeneric}$,
so that $\pushforward{\projection{1}{}}{\varTangent}=\varFixed$ and
$\norm{\varTangent}_{\varFixed}=\wassersteinDistance{\varFixed}{\varGeneric}{2}$. Writing
$R(x,\varTangentReals)\coloneqq V(x+\varTangentReals)-V(x)-\innerProduct{\gradient{}{V}(x)}{\varTangentReals}$
and using $\pushforward{\projection{1}{}}{\varTangent}=\varFixed$ and
$\varGeneric=\pushforward{(\projection{1}{}+\projection{2}{})}{\varTangent}$,
\begin{equation}\label{eq:expected_value:remainder}
\objective(\varGeneric)-\objective(\varFixed)
-\int_{\reals^d\times\reals^d}\innerProduct{\gradient{}{V}(x)}{\varTangentReals}\d\varTangent(x,\varTangentReals)
=\int_{\reals^d\times\reals^d}R(x,\varTangentReals)\d\varTangent(x,\varTangentReals).
\end{equation}
Since $\varTangentFixed$ is induced by the map $\gradient{}{V}$, every
$\varTangentCoupling\in\setPlansCommonMarginal{\varTangentFixed}{\varTangent}{1}$ has
first variation $\gradient{}{V}(\bar x)$ for $\varFixed$-almost every $\bar x$, so
$\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
=\int_{\reals^d\times\reals^d}\innerProduct{\gradient{}{V}(x)}{\varTangentReals}\d\varTangent(x,\varTangentReals)$
(cf. \cref{lemma:lemma_pushforward_and_optimal_transport}). We claim that the
right-hand side of \eqref{eq:expected_value:remainder} is
$\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$ as
$\varGeneric\to\varFixed$, uniformly over the choice of optimal transport plan. For $s>0$, let
\[
\omega(x,s)\coloneqq\sup_{0<\norm{\varTangentReals}\leq s}\frac{\abs{R(x,\varTangentReals)}}{\norm{\varTangentReals}}.
\]
Differentiability of $V$ at $x$ gives $\omega(x,s)\fromAbove 0$ as $s\fromAbove 0$.
Moreover, since $V=W+\frac{\lambda}{2}\norm{\cdot}^2$ with $W$ convex, the map
$t\mapsto V(x+t\varTangentReals)$ is absolutely continuous with derivative
$\innerProduct{\gradient{}{V}(x+t\varTangentReals)}{\varTangentReals}$, so the
fundamental theorem of calculus gives
$V(x+\varTangentReals)-V(x)=\int_0^1\innerProduct{\gradient{}{V}(x+t\varTangentReals)}{\varTangentReals}\d t$;
subtracting the constant $\innerProduct{\gradient{}{V}(x)}{\varTangentReals}$ yields
$R(x,\varTangentReals)=\int_0^1\innerProduct{\gradient{}{V}(x+t\varTangentReals)-\gradient{}{V}(x)}{\varTangentReals}\d t$.
Together with the linear growth of $\gradient{}{V}$, this gives
$\omega(x,s)\leq C_2(1+\norm{x}+s)$. By the Cauchy--Schwarz inequality and
$\abs{R(x,\varTangentReals)}\leq\omega(x,\norm{\varTangentReals})\norm{\varTangentReals}$,
\[
\frac{\abs{\int_{\reals^d\times\reals^d}R(x,\varTangentReals)\d\varTangent(x,\varTangentReals)}}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
\leq\left(\int_{\reals^d\times\reals^d}\omega(x,\norm{\varTangentReals})^2\d\varTangent(x,\varTangentReals)\right)^{1/2}.
\]
Fix $\delta>0$ and split the last integral along $\{\norm{\varTangentReals}\leq\delta\}$
and $\{\norm{\varTangentReals}>\delta\}$. On the first set, monotonicity of $\omega$ in
$s$ and $\pushforward{\projection{1}{}}{\varTangent}=\varFixed$ give
$\int_{\{\norm{\varTangentReals}\leq\delta\}}\omega(x,\norm{\varTangentReals})^2\d\varTangent(x,\varTangentReals)
\leq\int_{\reals^d}\omega(x,\delta)^2\d\varFixed(x)$, which does not depend on
$\varGeneric$. On the second set, $\omega(x,s)\leq C_2(1+\norm{x}+s)$ and $(a+b)^2\leq2a^2+2b^2$
give $\omega(x,\norm{\varTangentReals})^2\leq C_3\big((1+\norm{x})^2+\norm{\varTangentReals}^2\big)$
with $C_3\coloneqq2C_2^2$, whence
\begin{align*}
&\int_{\{\norm{\varTangentReals}>\delta\}}\omega(x,\norm{\varTangentReals})^2\d\varTangent(x,\varTangentReals)\\
&\qquad\leq C_3\int_{\{\norm{\varTangentReals}>\delta\}}(1+\norm{x})^2\d\varTangent(x,\varTangentReals)\\
&\qquad\qquad+C_3\int_{\{\norm{\varTangentReals}>\delta\}}\norm{\varTangentReals}^2\d\varTangent(x,\varTangentReals).
\end{align*}
The last integral is at most $\int_{\reals^d\times\reals^d}\norm{\varTangentReals}^2\d\varTangent(x,\varTangentReals)=\wassersteinDistance{\varFixed}{\varGeneric}{2}^2$,
which vanishes as $\varGeneric\to\varFixed$. For the first, fix $R>0$ and split
$\{\norm{\varTangentReals}>\delta\}$ according to whether $\norm{x}\leq R$ or $\norm{x}>R$. We first bound the $\varTangent$-measure of the set
$\{\norm{\varTangentReals}>\delta\}$. At every point $(x,\varTangentReals)$,
$
\indicator{\{\norm{\varTangentReals}>\delta\}}(x,\varTangentReals)\leq\frac{\norm{\varTangentReals}^2}{\delta^2},
$
since the left-hand side is $1$ when $\norm{\varTangentReals}>\delta$, and then
$\norm{\varTangentReals}^2/\delta^2>1$, and $0$ otherwise, while the right-hand side is
nonnegative. Integrating this pointwise inequality against $\varTangent$ and recalling
$\int_{\reals^d\times\reals^d}\norm{\varTangentReals}^2\d\varTangent(x,\varTangentReals)=\wassersteinDistance{\varFixed}{\varGeneric}{2}^2$,
\begin{align*}
\varTangent(\{\norm{\varTangentReals}>\delta\})
&=\int_{\reals^d\times\reals^d}\indicator{\{\norm{\varTangentReals}>\delta\}}(x,\varTangentReals)\d\varTangent(x,\varTangentReals)\\
&\leq\frac{1}{\delta^2}\int_{\reals^d\times\reals^d}\norm{\varTangentReals}^2\d\varTangent(x,\varTangentReals)
=\frac{\wassersteinDistance{\varFixed}{\varGeneric}{2}^2}{\delta^2}.
\end{align*}
Using this and $\pushforward{\projection{1}{}}{\varTangent}=\varFixed$,
\begin{align*}
\int_{\{\norm{\varTangentReals}>\delta\}}(1+\norm{x})^2\d\varTangent(x,\varTangentReals)
&\leq(1+R)^2\,\varTangent(\{\norm{\varTangentReals}>\delta\})+\int_{\{\norm{x}>R\}}(1+\norm{x})^2\d\varFixed(x)\\
&\leq\frac{(1+R)^2}{\delta^2}\wassersteinDistance{\varFixed}{\varGeneric}{2}^2+\int_{\{\norm{x}>R\}}(1+\norm{x})^2\d\varFixed(x).
\end{align*}
For each fixed $R$ the first term vanishes as $\varGeneric\to\varFixed$, so
\[
\limsup_{\varGeneric\to\varFixed}\int_{\{\norm{\varTangentReals}>\delta\}}(1+\norm{x})^2\d\varTangent(x,\varTangentReals)
\leq\int_{\{\norm{x}>R\}}(1+\norm{x})^2\d\varFixed(x).
\]
Since $(1+\norm{x})^2\in\Lp{1}{\reals^d}{\varFixed}$ (as $\varFixed\in\Pp{2}{\reals^d}$),
letting $R\to\infty$ sends the right-hand side to $0$; consequently
$\int_{\{\norm{\varTangentReals}>\delta\}}\omega(x,\norm{\varTangentReals})^2\d\varTangent(x,\varTangentReals)\to0$
as $\varGeneric\to\varFixed$. Hence, for every $\delta>0$,
\[
\limsup_{\varGeneric\to\varFixed}\int_{\reals^d\times\reals^d}\omega(x,\norm{\varTangentReals})^2\d\varTangent(x,\varTangentReals)
\leq\int_{\reals^d}\omega(x,\delta)^2\d\varFixed(x),
\]
and letting $\delta\fromAbove 0$ (dominated convergence, with dominating function
$C_2^2(2+\norm{x})^2\in\Lp{1}{\reals^d}{\varFixed}$) shows this $\limsup$ is $0$.
With \eqref{eq:expected_value:remainder}, we conclude
\begin{equation}\label{eq:expected_value:expansion}
\objective(\varGeneric)-\objective(\varFixed)
=\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}
+\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}.
\end{equation}}

{\emph{Step 3 (tangency of $\varTangentFixed$ and $-\varTangentFixed$).}
For $\varepsilon>0$ with $1+\varepsilon\lambda>0$, the function
$\frac{1}{2}\norm{\cdot}^2+\varepsilon V
=\varepsilon W+\frac{1+\varepsilon\lambda}{2}\norm{\cdot}^2$ is convex, so its gradient
$\identity{}+\varepsilon\gradient{}{V}$ is an optimal transport map
\cite[Theorem 1.48]{santambrogio2015optimal}; that is,
$\pushforward{(\projection{1}{},\projection{1}{}+\varepsilon\projection{2}{})}{\varTangentFixed}
=\pushforward{(\identity{},\identity{}+\varepsilon\gradient{}{V})}{\varFixed}$ is optimal
for all such $\varepsilon$, and \eqref{definition:tangent_space} yields
$\varTangentFixed\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$. For $-\varTangentFixed$ we
argue by approximation, since $\frac{1}{2}\norm{\cdot}^2-\varepsilon V$ need not be
convex when $\gradient{}{V}$ is not Lipschitz. For $\tau>0$, let
$W_\tau\coloneqq\moreau{W}{\tau}$ be the Moreau envelope of the convex function $W$
and set $V_\tau\coloneqq W_\tau+\frac{\lambda}{2}\norm{\cdot}^2$. Then $W_\tau$ is convex
and continuously differentiable, with $\tfrac{1}{\tau}$-Lipschitz gradient
$\gradient{}{W_\tau}=\tfrac{1}{\tau}(\identity{}-\proximalMapping{W}{\tau})$
\cite[Proposition 12.30]{bauschke2011convex}, so $V_\tau$ is differentiable with
$L_\tau$-Lipschitz gradient $\gradient{}{V_\tau}=\gradient{}{W_\tau}+\lambda\identity{}$,
where $L_\tau\coloneqq\tfrac{1}{\tau}+\abs{\lambda}$. As above,
$\frac{1}{2}\norm{\cdot}^2-\varepsilon V_\tau$ is convex for $\varepsilon\leq 1/L_\tau$, so
$\identity{}-\varepsilon\gradient{}{V_\tau}$ is an optimal transport map and
$\pushforward{(\identity{},-\gradient{}{V_\tau})}{\varFixed}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.
Finally, as $\tau\fromAbove 0$, $\gradient{}{W_\tau}(x)\to\gradient{}{W}(x)$ for every
$x$, with $\norm{\gradient{}{W_\tau}(x)}\leq\norm{\gradient{}{W}(x)}$
\cite[Proposition 12.30]{bauschke2011convex}; hence
$\gradient{}{V_\tau}\to\gradient{}{V}$ pointwise and, by dominated convergence (using
the linear growth of $\gradient{}{V}$ and $\varFixed\in\Pp{2}{\reals^d}$), in
$\Lp{2}{\reals^d}{\varFixed}$. Since
$\wassersteinDistance{\pushforward{(\identity{},-\gradient{}{V_\tau})}{\varFixed}}{-\varTangentFixed}{\varFixed}
\leq\norm{\gradient{}{V_\tau}-\gradient{}{V}}_{\Lp{2}{\reals^d}{\varFixed}}\to0$ and the
tangent space is closed with respect to $\wassersteinDistance{}{}{\varFixed}$, we obtain
$-\varTangentFixed\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.}

{\emph{Conclusion.}
By \eqref{eq:expected_value:expansion} and
$\varTangentFixed\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$, for all
$\varGeneric\in\Pp{2}{\reals^d}$ and all
$\varTangent\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$
we have $\objective(\varGeneric)-\objective(\varFixed)\geq
\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}+\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$,
i.e., $\varTangentFixed\in\subgradientRegular{\objective}(\varFixed)$. Since
$\varTangentFixed$ is induced by a map,
$\innerProduct{-\varTangentFixed}{\varTangent}_{\varFixed}=-\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed}$,
so negating \eqref{eq:expected_value:expansion} and using
$-\varTangentFixed\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ gives
$-\objective(\varGeneric)-(-\objective(\varFixed))\geq
\innerProduct{-\varTangentFixed}{\varTangent}_{\varFixed}+\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$,
i.e., $-\varTangentFixed\in\subgradientRegular{(-\objective)}(\varFixed)$. Therefore
$\varTangentFixed\in-\subgradientRegular{(-\objective)}(\varFixed)\cap\subgradientRegular{\objective}(\varFixed)$,
and by \cref{definition:def_differentiability} the functional $\objective$ is
differentiable at $\varFixed$ with
$\gradient{}{\objective}(\varFixed)\localEquiv{\varFixed}\varTangentFixed
=\pushforward{(\identity{},\gradient{}{V})}{\varFixed}$.}
\end{enumerate}


==> elements/prop_functional_expected_value_title.tex <==
Expected value%

==> elements/prop_functional_interaction_body.tex <==
Let $U:\reals^d\to\reals$ be a twice continuously differentiable
function with bounded Hessian
and consider the functional $\objective: \Pp{2}{\reals^d} \to \realsBar$,
$
\objective(\varGeneric)
\coloneqq
\frac{1}{2}
\expectedValue{(x, y) \sim \varGeneric\times\varGeneric}{U(x-y)}.
$
Then,
\begin{enumerate}[leftmargin=*]
\item
\uniqueLabel{item:interaction:properness}
$\objective$ is proper and continuous.

\item
\uniqueLabel{item:interaction:differentiability}
$\objective$ is differentiable and its gradient at
$\varFixed \in \Pp{2}{\reals^d}$ is
\[
\gradient{}{\objective}(\varFixed)
\localEquiv{\varFixed}
\pushforward{(\identity{}, T_{\varFixed})}{\varFixed},
\quad\text{where}\quad
{
T_{\varFixed}(x)
\coloneqq
\frac{1}{2}\int_{\reals^d}
\bigl(\gradient{}{U}(x-y)-\gradient{}{U}(y-x)\bigr)\,\d\varFixed(y).
}
\]
\item
{If, in addition, $U$ is even, then $\gradient{}{U}$ is odd and
\[
{
T_{\varFixed}(x)
=
\int_{\reals^d} \gradient{}{U}(x-y)\,\d\varFixed(y)
=
(\gradient{}{U} \conv \varFixed)(x),
}
\]
where $\conv$ denotes the
\WikipediaLink{https://en.wikipedia.org/wiki/Convolution}{convolution}
operation. Consequently,
$
{
\gradient{}{\objective}(\varFixed)
\localEquiv{\varFixed}
\pushforward{(\identity{}, (\gradient{}{U} \conv \varFixed))}{\varFixed}.
}
$}
\end{enumerate}

==> elements/prop_functional_interaction_proof.tex <==
We prove the statements separately.
\begin{enumerate}[leftmargin=*]
\item See \cite[Proposition 2.21(i)-(ii)]{Lanzetti2022}.

\item
The proof is analogous to \cite[Proposition 2.21(v)]{Lanzetti2022}. However, the last step there uses that $\gradient{}{U}$ is odd, which requires $U$ to be even. We therefore repeat the same argument for completeness and keep the antisymmetrized expression.
{Let $\varGeneric \in \Pp{2}{\reals^d}$ and let $\varPlanGeneric \in \setPlansOptimal{\varFixed}{\varGeneric}$.
Define $\varTangent
\coloneqq
\pushforward{(\projection{1}{}, \projection{2}{}-\projection{1}{})}{\varPlanGeneric}$.
Then,
\begin{align*}
\objective(\varGeneric)-\objective(\varFixed)
&=
\frac{1}{2}
\int_{\reals^d\times\reals^d}
U(x-y)\d(\varGeneric\times\varGeneric)(x,y)
-
\frac{1}{2}
\int_{\reals^d\times\reals^d}
U(\bar x- \bar y)\d(\varFixed\times\varFixed)(\bar x, \bar y)
\\
&=
\frac{1}{2}
\int_{\reals^d\times\reals^d}\int_{\reals^d\times\reals^d}
\left(U(x-y)-U(\bar x-\bar y)\right)
\d\varPlanGeneric(\bar x, x)\d\varPlanGeneric(\bar y, y).
\end{align*}
Since $U\in C^2(\reals^d)$ with bounded Hessian, there exists $M>0$ such that
$\norm{\nabla^2 U(z)}\le M$ for all $z\in\reals^d$.
Thus, by Taylor expansion,
\begin{align*}
U(x-y)-U(\bar x-\bar y)
&=
\innerProduct{\gradient{}{U}(\bar x-\bar y)}{(x-y)-(\bar x-\bar y)}
+
R(x,y,\bar x,\bar y),
\end{align*}
with
$
|R(x,y,\bar x,\bar y)|
\le
\frac{M}{2}\norm{(\bar x -x)-(\bar y -y)}^2$.
Since
\begin{align*}
&\int_{\reals^d\times\reals^d}\int_{\reals^d\times\reals^d}
\norm{(\bar x-x)-(\bar y-y)}^2
\d\varPlanGeneric(\bar x, x)\d\varPlanGeneric(\bar y, y)
\\
&\le
2\int_{\reals^d\times\reals^d}\int_{\reals^d\times\reals^d}
\left(\norm{\bar x-x}^2+\norm{\bar y-y}^2\right)
\d\varPlanGeneric(\bar x, x)\d\varPlanGeneric(\bar y,y)
\\
&=
4\int_{\reals^d\times\reals^d}\norm{\bar x-x}^2\d\varPlanGeneric(\bar x,x)
=
4\wassersteinDistance{\varFixed}{\varGeneric}{2}^2,
\end{align*}
we have that
\begin{align*}
\objective(\varGeneric)-\objective(\varFixed)
&=
\frac{1}{2}
\int_{\reals^d\times\reals^d}\int_{\reals^d\times\reals^d}
\innerProduct{\gradient{}{U}(\bar x-\bar y)}{(x-\bar x)-(y-\bar y)}
\d\varPlanGeneric(\bar x, x)\d\varPlanGeneric(\bar y,y)
\\
&
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}.
\end{align*}
Next, we split the first-order term to obtain
\begin{align*}
&\frac{1}{2}
\int_{\reals^d\times\reals^d}\int_{\reals^d\times\reals^d}
\innerProduct{\gradient{}{U}(\bar x-\bar y)}{(x-\bar x)-(y-\bar y)}
\d\varPlanGeneric(\bar x,x)\d\varPlanGeneric(\bar y,y)
\\
&=
\frac{1}{2}
\int_{\reals^d\times\reals^d}
\innerProduct{
\int_{\reals^d}\gradient{}{U}(\bar x-\bar y)\d\varFixed(\bar y)
}{x-\bar x}
\d\varPlanGeneric(\bar x,x)
\\
&
-
\frac{1}{2}
\int_{\reals^d\times\reals^d}
\innerProduct{
\int_{\reals^d}\gradient{}{U}(\bar x-\bar y)\d\varFixed(\bar x)
}{y-\bar y}
\d\varPlanGeneric(\bar y,y)
\\
&=
\frac{1}{2}
\int_{\reals^d\times\reals^d}
\innerProduct{
\int_{\reals^d}\gradient{}{U}(\bar x-\bar y)\d\varFixed(\bar y)
}{x-\bar x}
\d\varPlanGeneric(\bar x,x)
\\
&
-
\frac{1}{2}
\int_{\reals^d\times\reals^d}
\innerProduct{
\int_{\reals^d}\gradient{}{U}(\bar y-\bar x)\d\varFixed(\bar y)
}{x-\bar x}
\d\varPlanGeneric(\bar x,x)
\\
&=
\int_{\reals^d\times\reals^d}
\innerProduct{T_{\varFixed}(\bar x)}{x-\bar x}
\d\varPlanGeneric(\bar x,x),
\end{align*}
where $T_{\varFixed}(\bar x)
\coloneqq
\frac{1}{2}\int_{\reals^d}
\left(\gradient{}{U}(\bar x-\bar y)-\gradient{}{U}(\bar y-\bar x)\right)\d\varFixed(\bar y)$.
Thus,
\begin{align*}
\objective(\varGeneric)-\objective(\varFixed)
&=
\int_{\reals^d\times\reals^d}
\innerProduct{T_{\varFixed}(\bar x)}{x-\bar x}
\d\varPlanGeneric(\bar x,x)
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
\\
&=
\int_{\reals^d\times\reals^d}
\innerProduct{T_{\varFixed}(\bar x)}{\varTangentReals}
\d\varTangent(\bar x,\varTangentReals)
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}.
\end{align*}
Moreover, since $U$ has bounded Hessian, $\gradient{}{U}$ has at most linear growth, and therefore there exists $C>0$ such that
$
\norm{T_{\varFixed}(x)}
\le
C\left(1+\norm{x}+\int_{\reals^d}\norm{y}\d\varFixed(y)\right),
$
which implies $T_{\varFixed}\in \Lp{2}{\reals^d}{\varFixed}$.
{Moreover, $T_{\varFixed}=\gradient{}{W}$ with
$W(x)\coloneqq\frac{1}{2}\int_{\reals^d}\left(U(x-y)+U(y-x)\right)\d\varFixed(y)$,
where differentiation under the integral sign is justified by the linear growth of
$\gradient{}{U}$; $W$ is twice continuously differentiable with
$\norm{\nabla^2 W(x)}\leq M$ for all $x\in\reals^d$, so for $0<\varepsilon<1/M$ the
map $\identity{}+\varepsilon T_{\varFixed}$ is the gradient of a convex function and
hence an optimal transport map \cite[Theorem 1.48]{santambrogio2015optimal}. Thus,
$\pushforward{(\identity{},T_{\varFixed})}{\varFixed}$ belongs to the set in
\eqref{definition:tangent_space} and, in particular, to
$\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$; the same argument applied to
$-T_{\varFixed}$ gives
$\pushforward{(\identity{},-T_{\varFixed})}{\varFixed}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.}
For any
$\varTangentCoupling
\in
\setPlansCommonMarginal
{\pushforward{(\identity{},T_{\varFixed})}{\varFixed}}
{\varTangent}{1}$,
\begin{align*}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals'}{\varTangentReals}
&\d\varTangentCoupling(\bar x,\varTangentReals',\varTangentReals)
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
\\&=
\int_{\reals^d\times\reals^d}
\innerProduct{T_{\varFixed}(\bar x)}{\varTangentReals}
\d\varTangent(\bar x,\varTangentReals)
+
\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
\\&=
\objective(\varGeneric)-\objective(\varFixed),
\end{align*}
{where the first equality uses that
$\pushforward{\projection{12}{}}{\varTangentCoupling}$ is induced by the map
$T_{\varFixed}$, so that $\varTangentReals'=T_{\varFixed}(\bar x)$ for
$\varTangentCoupling$-almost every $(\bar x, \varTangentReals', \varTangentReals)$.}
Since the above holds for every $\varGeneric \in \Pp{2}{\reals^d}$ and every
$\varPlanGeneric \in \setPlansOptimal{\varFixed}{\varGeneric}$, we conclude that
$\pushforward{(\identity{},T_{\varFixed})}{\varFixed}
\in
\subgradientRegular{\objective}(\varFixed)
\cap
-\subgradientRegular{(-\objective)}(\varFixed)$
and, thus, $\gradient{}{\objective}(\varFixed)
\localEquiv{\varFixed}
\pushforward{(\identity{},T_{\varFixed})}{\varFixed}$.
}

\item
{
If $U$ is even, then $\nabla U$ is odd. Then, $\nabla U(y-x)=-\nabla U(x-y)$ and, thus,
$
T_{\varFixed}(\bar x)
=
\int_{\reals^d}\nabla U(\bar x-\bar y)\d\varFixed(\bar y)
=
(\nabla U\conv\varFixed)(\bar x).
$
It follows that $\gradient{}{\objective}(\varFixed)
\localEquiv{\varFixed}
\pushforward{(\identity{},(\nabla U\conv\varFixed))}{\varFixed}$.
}
\end{enumerate}


==> elements/prop_functional_interaction_title.tex <==
Interaction energy%

==> elements/prop_functional_optimal_transport_body.tex <==
Let $\varReference \in \Pp{2}{\reals^d}$ and consider $c: \reals^d\times\reals^d \to \nonnegativeReals$ twice continuously differentiable with bounded \WikipediaLink{https://en.wikipedia.org/wiki/Hessian_matrix}{Hessian} on $\reals^d\times\reals^d$ and satisfying the twist condition, i.e., $y\mapsto\gradient{x}{c}(x,y)$ is injective for all $x\in\reals^d$.
Consider the functional $\objective: \Pp{2}{\reals^d} \to \realsBar$,
$
\objective(\varGeneric)
\coloneqq
\wassersteinDistance{\varGeneric}{\varReference}{c}
$ as defined in \eqref{definition:optimaltransport}.
Then,
\begin{enumerate}[leftmargin=*]
\item
\label{item:optimal_transport:properness}
$\objective$ is proper, nonnegative, and continuous.
\item
\label{item:optimal_transport:differentiable}
At any $\varFixed \in \Pp{2}{\reals^d}$,
$\objective$ is subdifferentiable with
$
\emptyset\neq
\subgradient{\objective}(\varFixed)
\localSubseteq{\varFixed}
\pushforward{(\projection{1}{}, \gradient{x}{c})}{\setPlansOptimalCost{\varFixed}{\varReference}{c}}
$, where $\setPlansOptimalCost{\varFixed}{\varReference}{c}$ is the set of transport plans between $\varFixed$ and $\varReference$ that yield the minimum in the definition of $\wassersteinDistance{\varFixed}{\varReference}{c}$.
\item If $\setPlansOptimalCost{\varFixed}{\varReference}{c}$ is a singleton and induced by an optimal transport map (e.g., $\varFixed$ is absolutely continuous), then
$\objective$ is differentiable with
$
\gradient{}{\objective}(\varFixed)
\localEquiv{\varFixed}
\pushforward{(\projection{1}{}, \gradient{x}{c})}{\varPlanGeneric},
$ where
$\varPlanGeneric$ is the unique element in $\setPlansOptimalCost{\varFixed}{\varReference}{c}$.
\end{enumerate}


==> elements/prop_functional_optimal_transport_proof.tex <==
In virtue of \cite[Theorem 4.1]{villani2009optimal}, $\objective$ is well defined. We now prove the statements separately.
\begin{enumerate}[leftmargin=*]
\item
From the nonnegativity of $c$ it directly follows that $\objective$ is nonnegative.
Let $\varGeneric\in\Pp{2}{\reals^d}$.
To show that $\objective(\varGeneric)<+\infty$, consider the Taylor expansion of $c$ at $(x,y)=(0,0)$:
    \begin{equation}
    \label{eq:expansion}
        c(x, y) - c(0, 0)
    \leq
    \innerProduct{\gradient{x}{c}(0, 0)}{x} + \innerProduct{\gradient{y}{c}(0, 0)}{y}
    +
    \frac{M}{2}(\norm{x}^2+\norm{y}^2),
    \end{equation}
where $M<+\infty$ since the Hessian of $c$ is bounded. Thus, using Cauchy--Schwarz's and Young's inequalities, there exists $C>0$ so that
$
c(x, y)
\leq
C(1+\norm{x}^2+\norm{y}^2)
$. Thus, for any $\gamma\in\setPlans{\varGeneric}{\varReference}$ we have
    $\int_{\reals^d\times\reals^d}c(x,y)\d\gamma(x,y)
    \leq
    C\int_{\reals^d\times\reals^d}1+\norm{x}^2+\norm{y}^2\d\gamma(x,y)
    =
    C\left(1+\int_{\reals^d}\norm{x}^2\d\varGeneric(x)+\int_{\reals^d}\norm{y}^2\d\varReference(y)\right)
    <
    +\infty$
since both $\varGeneric$ and $\varReference$ have finite second moment. Thus, $\wassersteinDistance{\varGeneric}{\varReference}{c}<+\infty$ for all $\varGeneric\in\Pp{2}{\reals^d}$, and $\objective$ is proper.
%
To show continuity, first observe that optimal transport discrepancies are narrowly lower semicontinuous~\cite[Remark 6.12]{villani2009optimal}. Since convergence in Wasserstein implies narrow convergence, they are also lower semicontinuous in Wasserstein.
Thus, it suffices to establish upper semicontinuity.
For this, consider the function ${\varPlanGeneric\mapsto\int_{\reals^d\times\reals^d}c(x,y)\d\varPlanGeneric(x,y)}$. Since $c$ is continuous with bounded Hessian (and thus at most quadratic growth), this function is continuous in Wasserstein.
Moreover, by~\cref{lemma:set_plans}, the set-valued map $\varGeneric\mapsto\setPlans{\varGeneric}{\varReference}$ is nonempty and lower hemicontinuous.
Thus, $\varGeneric\mapsto\objective(\varGeneric)=\min_{\varPlanGeneric\in\setPlans{\varGeneric}{\varReference}}\int_{\reals^d\times\reals^d}c(x,y)\d\varPlanGeneric(x,y)$ is upper semicontinuous~\cite[Lemma 17.29]{guide2006infinite}. Overall, $\objective$ is therefore continuous.


\item
We divide the proof into six steps.

\emph{Step 1 ($\varTangent^{+}$ and $\varTangent^{-}$ belong to $\Pp{2}{\reals^d\times\reals^d}$).}
Fix $\varPlanGeneric \in \setPlansOptimalCost{\varFixed}{\varReference}{c}$ and define the variations
$\varTangent^{+} \coloneqq \pushforward{(\projection{1}{}, \gradient{x}{c})}{\varPlanGeneric}$
and
$\varTangent^{-} \coloneqq \pushforward{(\projection{1}{}, -\gradient{x}{c})}{\varPlanGeneric}$.
Boundedness of the Hessian implies that $\gradient{x}{c}$ is Lipschitz (with some constant $L$). Thus,
\begin{align*}
    \norm{\varTangent^{+}}_{\varFixed}^2
    &=
    \int_{\reals^d\times\reals^d}
    \norm{\gradient{x}{c}(\bar x, \hat x)}^2
    \d\varPlanGeneric(\bar x, \hat x)
    \\
    &\leq
    2\norm{\gradient{x}{c}(0, 0)}^2
    \\&\qquad
    +
    2\int_{\reals^d\times\reals^d}
    \norm{\gradient{x}{c}(\bar x, \hat x)-\gradient{x}{c}(0, 0)}^2
    \d\varPlanGeneric(\bar x, \hat x)
    \\
    &\leq
    2\norm{\gradient{x}{c}(0, 0)}^2
    \\&\qquad
    +
    2L^2\left(\int_{\reals^d}
    \norm{\bar x}^2\d\varFixed(\bar x)+\int_{\reals^d}\norm{\hat x}^2\d\varReference(\hat x)\right)
    < +\infty,
\end{align*}
since $\varFixed, \varReference \in \Pp{2}{\reals^d}$; the same bound holds for $\varTangent^{-}$. Thus, both $\varTangent^{+}$ and $\varTangent^{-}$ have finite second moment and, having first marginal $\varFixed$, belong to $\Pp{2}{\reals^d\times\reals^d}$.

\emph{Step 2 ($\varTangent^{+}$ and $\varTangent^{-}$ belong to the tangent space).}
We show that $\varTangent^{-} \in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed}$, which is what \emph{Step 3} requires.
Let $M$ bound the Hessian of $c$ as in \eqref{eq:expansion} and fix $\varepsilon \in [0, \frac{1}{M})$. We claim that the transport plan
$
    \varPlanGeneric_\varepsilon
    \coloneqq
    \pushforward{(\projection{1}{}, \projection{1}{} - \varepsilon\gradient{x}{c})}{\varPlanGeneric}
$
is optimal for the quadratic cost, i.e., $\varPlanGeneric_\varepsilon \in \setPlansOptimal{\varFixed}{\pushforward{(\projection{1}{} - \varepsilon\gradient{x}{c})}{\varPlanGeneric}}$. In virtue of \cite[Theorem 5.10]{villani2009optimal}, it suffices to show that the support of $\varPlanGeneric_\varepsilon$ is cyclically monotone (its transport cost is finite by the moment bound above). Since $\varPlanGeneric$ is $c$-optimal, $\supp{\varPlanGeneric}$ is $c$-cyclically monotone \cite[Theorem 5.10]{villani2009optimal}. Thus, for every finite family $(\bar x_1,\hat x_1),\dots,(\bar x_n,\hat x_n)\in\supp{\varPlanGeneric}$ (indices modulo $n$),
\begin{equation}
\label{eq:ccm}
    \sum_{i=1}^n c(\bar x_i, \hat x_i) \leq \sum_{i=1}^n c(\bar x_{i+1}, \hat x_i).
\end{equation}
With $p_i \coloneqq \bar x_i - \varepsilon\gradient{x}{c}(\bar x_i, \hat x_i)$ and $Q \coloneqq \sum_i \norm{\bar x_{i+1}-\bar x_i}^2$, the identity $\sum_i \innerProduct{\bar x_i}{\bar x_{i+1}-\bar x_i} = -\frac{1}{2}Q$ gives
\begin{equation*}
    \sum_{i=1}^n \innerProduct{p_i}{\bar x_{i+1}-\bar x_i}
    =
    -\tfrac{1}{2}Q
    -\varepsilon\sum_{i=1}^n \innerProduct{\gradient{x}{c}(\bar x_i,\hat x_i)}{\bar x_{i+1}-\bar x_i}.
\end{equation*}
The Taylor expansion of $c(\cdot,\hat x_i)$ (with $M$-bounded Hessian) yields $c(\bar x_{i+1},\hat x_i)-c(\bar x_i,\hat x_i) \leq \innerProduct{\gradient{x}{c}(\bar x_i,\hat x_i)}{\bar x_{i+1}-\bar x_i}+\frac{M}{2}\norm{\bar x_{i+1}-\bar x_i}^2$; summing and using \eqref{eq:ccm},
\begin{equation*}
    \sum_{i=1}^n \innerProduct{\gradient{x}{c}(\bar x_i,\hat x_i)}{\bar x_{i+1}-\bar x_i}
    \geq
    \sum_{i=1}^n\left(c(\bar x_{i+1},\hat x_i)-c(\bar x_i,\hat x_i)\right)-\tfrac{M}{2}Q
    \geq
    -\tfrac{M}{2}Q.
\end{equation*}
Therefore $\sum_i \innerProduct{p_i}{\bar x_{i+1}-\bar x_i} \leq -\frac{1}{2}Q + \varepsilon\frac{M}{2}Q = -(1-\varepsilon M)\frac{Q}{2}\leq 0$ for $\varepsilon\leq\frac{1}{M}$. As cyclical monotonicity is a closed condition and the map $(\bar x, \hat x)\mapsto(\bar x, \bar x - \varepsilon\gradient{x}{c}(\bar x, \hat x))$ is continuous, it passes to $\supp{\varPlanGeneric_\varepsilon}$, proving the claim.

For every $\varepsilon\in[0,\frac{1}{M})$, $\pushforward{(\projection{1}{}, \projection{1}{}+\varepsilon\projection{2}{})}{\varTangent^{-}}=\varPlanGeneric_\varepsilon$ is quadratically optimal; hence, by \eqref{definition:tangent_space} (with $\bar\varepsilon=\frac{1}{M}$), $\varTangent^{-} \in \tangentSpaceInterior{\Pp{2}{\reals^d}}{\varFixed}\subseteq\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.
Since the tangent space is closed under negation~(\cref{proposition:prop_sum_scale_well_defined} with $\tau=-1$), also $\varTangent^{+}=-\varTangent^{-}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.

\emph{Step 3 (Superdifferentiability).}
We generalize~\cite[Proposition 2.17(vi)]{Lanzetti2022} to any measure.
Via Taylor's expansion we have, for any $x_1, x_2, x_3 \in \reals^d$,
$
c(x_3, x_2) - c(x_1, x_2)
\leq
\innerProduct{\gradient{x}{c}(x_1, x_2)}{x_3 - x_1}
+
\frac{M}{2}\norm{x_3 - x_1}^2.
$
Fix $\varGeneric\in\Pp{2}{\reals^d}$, $\varTangent \in \setPlansOptimalCost{\varFixed}{\varReference}{c}$, an optimal transport plan $\varTangent' \in \setPlansOptimal{\varFixed}{\varGeneric}$, and $\varTangentCoupling \in \setPlansCommonMarginal{\varTangent}{\varTangent'}{1}$. Then,
\begin{align*}
    \objective(\varGeneric) - \objective(\varFixed)
    &\leq
    \int_{\reals^d\times\reals^d\times\reals^d}
    c(x, \hat x) - c(\bar x, \hat x)
    \d\varTangentCoupling(\bar x, \hat x, x)
    \\&\leq
    \int_{\reals^d\times\reals^d\times\reals^d}
    \innerProduct{\gradient{x}{c}(\bar x, \hat x)}{x - \bar x}
    \d\varTangentCoupling(\bar x, \hat x, x)
    \\&\qquad
    +
    \frac{M}{2}\wassersteinDistance{\varFixed}{\varGeneric}{2}^2.
\end{align*}
The integrand pairs the arrow of $\pushforward{(\projection{1}{}, \gradient{x}{c})}{\varTangent}$ with the arrow of the displacement variation $\pushforward{(\projection{1}{}, \projection{2}{}-\projection{1}{})}{\varTangent'}$. 
We can minimize over couplings to obtain 
\begin{align*}
    \objective(\varGeneric) &- \objective(\varFixed)
    +\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
    \\&\leq
    \min_{\varTangentCoupling \in \setPlansCommonMarginal{\pushforward{(\projection{1}{}, \gradient{x}{c})}{\varTangent}}{\pushforward{(\projection{1}{}, \projection{2}{}-\projection{1}{})}{\varTangent'}}{1}}
    \\&\qquad
    \int_{\reals^d\times\reals^d\times\reals^d}
    \innerProduct{\varTangentReals_1}{\varTangentReals_2}
    \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2),
\end{align*}
where we used $\frac{M}{2}\wassersteinDistance{\varFixed}{\varGeneric}{2}^2 = \onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$ and~\cref{lemma:lemma_pushforward_and_optimal_transport} (applied with $l_1=\gradient{x}{c}$, $l_2(\bar x,x)=x-\bar x$, and cost $\innerProduct{\cdot}{\cdot}$ to the variations augmented with their base point).
Thus, 
\begin{align*}
    -\objective(\varGeneric) &- (-\objective(\varFixed))
    +\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
    \\&\geq
    -
    \min_{\varTangentCoupling \in \setPlansCommonMarginal{\pushforward{(\projection{1}{}, \gradient{x}{c})}{\varTangent}}{\pushforward{(\projection{1}{}, \projection{2}{}-\projection{1}{})}{\varTangent'}}{1}}
    \\&\qquad
    \int_{\reals^d\times\reals^d\times\reals^d}
    \innerProduct{\varTangentReals_1}{\varTangentReals_2}
    \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
    \\&=
    \innerProduct{\pushforward{(\projection{1}{}, -\gradient{x}{c})}{\varTangent}}{\pushforward{(\projection{1}{}, \projection{2}{}-\projection{1}{})}{\varTangent'}}_{\varFixed},
\end{align*}
where the last equality follows from $-\min_{\varTangentCoupling} f = \max_{\varTangentCoupling}(-f)$ and~\cref{lemma:lemma_pushforward_and_optimal_transport} (with the map $\varTangentReals\mapsto-\varTangentReals$), together with the definition~\eqref{definition:geometry:inner_product} of the inner product. Since $\pushforward{(\projection{1}{}, -\gradient{x}{c})}{\varTangent}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ by \emph{Step 2} and $\varGeneric$, $\varTangent'$ were arbitrary, this shows $\pushforward{(\projection{1}{}, -\gradient{x}{c})}{\varTangent}\in\subgradientRegular{(-\objective)}(\varFixed)$ and, thus, $\pushforward{(\projection{1}{}, \gradient{x}{c})}{\varTangent} \in -\subgradientRegular{(-\objective)}(\varFixed)$.

\emph{Step 4 (Subdifferentiability when $\setPlansOptimalCost{\varFixed}{\varReference}{c}$ is a singleton and induced by an optimal transport map $\optMap{\varFixed}{\varReference}$).}
The proof is identical to the proof of~\cite[Proposition 2.17(vi)]{Lanzetti2022}. Indeed, let
$\bar\varTangent=\pushforward{(\identity{},\comp{(\identity{},\optMap{\varFixed}{\varReference})}{\gradient{x}{c}})}{\varFixed}$
be the candidate subgradient. For $\varGeneric\in\Pp{2}{\reals^d}$, let
$\varTangent=\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\varPlanGeneric}$ with $\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varGeneric}$.
Then, since the second coordinate of $\bar\varTangent$ is a deterministic function of the first, $\varTangentCoupling\coloneqq\pushforward{(\projection{1}{},\comp{(\projection{1}{},\comp{\projection{1}{}}{\optMap{\varFixed}{\varReference}})}{\gradient{x}{c}},\projection{2}{}-\projection{1}{})}{\varPlanGeneric}$
is the unique element in
$\setPlansCommonMarginal{\bar\varTangent}{\varTangent}{1}$.
This trivializes the inner product to $\innerProduct{\bar\varTangent}{\varTangent}_{\varFixed}=\int_{\reals^d\times\reals^d}\innerProduct{\gradient{x}{}c(\bar x,\optMap{\varFixed}{\varReference}(\bar x))}{\hat x-\bar x}\d\varPlanGeneric(\bar x,\hat x)$, so that we can directly use the argument in~\cite[Proposition 2.17(vi)]{Lanzetti2022} (in particular, no modifications are needed to deal with the inner product).
Finally, $\bar\varTangent$ is the variation $\varTangent^{+}$ of \emph{Step 2} for the $c$-optimal transport plan $\pushforward{(\identity{},\optMap{\varFixed}{\varReference})}{\varFixed}$, so $\bar\varTangent\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ by \emph{Step 2}.
Hence, $\bar\varTangent\in\subgradientRegular{\objective}(\varFixed)$.

\emph{Step 5 (Differentiability at absolutely continuous measures).}
When $c$ has bounded Hessian and $y\mapsto\gradient{x}c(x,y)$ is injective, absolute continuity is sufficient for existence and uniqueness of an optimal transport map between $\varFixed$ and $\varReference$~\cite[Theorem 10.28]{villani2009optimal}. Thus, at all absolutely continuous measures, both the regular sub- and superdifferentials are nonempty. Thus,~\cref{proposition:prop_differentiability_properties} implies that $\objective$ is differentiable at all absolutely continuous probability measures.

\emph{Step 6 (Generalized subgradient).}
Let $(\varGeneric_n)_{n \in \naturals} \subseteq \Pp{2}{\reals^d}$ be a sequence such that $\varGeneric_n \convergenceWasserstein \varFixed$ and $\objective$ is differentiable at every $\varGeneric_n$, so that $\subgradientRegular{\objective}(\varGeneric_n) \neq \emptyset$ (cf. \cref{proposition:prop_differentiability_properties}). Such a sequence always exists since $\Ppabs{2}{\reals^d}$ is dense in $\Pp{2}{\reals^d}$.
Since $\objective$ is continuous, we also have that $\objective(\varGeneric_n)\to\objective(\varFixed)$.
We can then proceed as in the proof of~\cref{proposition:prop_wassersteindistance_general_subgradient} (together with Lipschitz continuity of $\gradient{x}c$), to conclude that $\subgradient{\objective}$ is nonempty and contained (as a result of the same arguments as in \cref{proposition:prop_wassersteindistance_regular_subgradient_must_be_plan}\ref{item:prop_wassersteindistance_regular_subgradient_must_be_plan:regular_necessary}) in $\pushforward{(\projection{1}{},\gradient{x}c)}{\setPlansOptimalCost{\varFixed}{\varReference}{c}}$.

\item By \emph{Step 3}, $\pushforward{(\projection{1}{}, \gradient{x}{c})}{\varPlanGeneric}\in-\subgradientRegular{(-\objective)}(\varFixed)$, and by \emph{Step 4}, $\pushforward{(\projection{1}{}, \gradient{x}{c})}{\varPlanGeneric}\in\subgradientRegular{\objective}(\varFixed)$; hence $\objective$ is differentiable at $\varFixed$ with $\gradient{}{\objective}(\varFixed)\localEquiv{\varFixed}\pushforward{(\projection{1}{}, \gradient{x}{c})}{\varPlanGeneric}$ by~\cref{proposition:prop_differentiability_properties}.
\end{enumerate}


==> elements/prop_functional_optimal_transport_title.tex <==
Optimal transport discrepancy%

==> elements/prop_normal_cone_product_body.tex <==
\,
\begin{enumerate}[leftmargin=*]
\item
{%
\label{item:product:cylinder} For $\Omega_1\subseteq\Pp{2}{\reals^{m}}$ and $\Omega_2\subseteq\Pp{2}{\reals^{d}}$, let $\feasibleSet=\{\varGeneric\in\Pp{2}{\reals^{m}\times\reals^{d}}\st\pushforward{\projection{1}{}}{\varGeneric}\in\Omega_1,\ \pushforward{\projection{2}{}}{\varGeneric}\in\Omega_2\}$ and $\varFixed\in\feasibleSet$. Then, we have
\begin{align*}
  \normalConeRegularStrong{\feasibleSet}{\varFixed}
  &=
  \{
      \varTangent\in\Pp{2}{\reals^m\times\reals^d\times\reals^m\times\reals^d}, \pushforward{\projection{12}{}}{\varTangent}=\varFixed
      \st
      \\
      &\qquad\qquad\qquad
      \pushforward{\projection{13}{}}{\varTangent}\in\normalConeRegularStrong{\Omega_1}{\pushforward{\projection{1}{}}{\varFixed}},
      \pushforward{\projection{24}{}}{\varTangent}\in\normalConeRegularStrong{\Omega_2}{\pushforward{\projection{2}{}}{\varFixed}}
  \}
  \\
  \normalConeStrong{\feasibleSet}{\varFixed}
  &=
  \{
      \varTangent\in\Pp{2}{\reals^m\times\reals^d\times\reals^m\times\reals^d}, \pushforward{\projection{12}{}}{\varTangent}=\varFixed
      \st
      \\
      &\qquad\qquad\qquad
      \pushforward{\projection{13}{}}{\varTangent}\in\normalConeStrong{\Omega_1}{\pushforward{\projection{1}{}}{\varFixed}},
      \pushforward{\projection{24}{}}{\varTangent}\in\normalConeStrong{\Omega_2}{\pushforward{\projection{2}{}}{\varFixed}}
  \}.
\end{align*}
In particular, membership of $\pushforward{\projection{13}{}}{\varTangent}$ and $\pushforward{\projection{24}{}}{\varTangent}$ in the strong regular normal cones implies $\varTangent\in\tangentSpace{(\varFixed)}{\Pp{2}{\reals^m\times\reals^d}}$.
If $\Omega_1$ is \gls*{acr:snc} at $\pushforward{\projection{1}{}}{\varFixed}$ and $\Omega_2$ is \gls*{acr:snc} at $\pushforward{\projection{2}{}}{\varFixed}$, then $\feasibleSet$ is \gls*{acr:snc} at $\varFixed$.
Finally, if $\Omega_1=\Pp{2}{\reals^m}$, i.e., $\feasibleSet=\{\varGeneric\in\Pp{2}{\reals^{m}\times\reals^{d}}\st\pushforward{\projection{2}{}}{\varGeneric}\in\Omega_2\}$, then
\begin{align*}
  \normalConeRegularStrong{\feasibleSet}{\varFixed}
  &=
  \{
      \varTangent\in\Pp{2}{\reals^m\times\reals^d\times\reals^m\times\reals^d}, \pushforward{\projection{12}{}}{\varTangent}=\varFixed
      \st
      \\
      &\qquad\qquad\qquad
      \pushforward{\projection{13}{}}{\varTangent}=\localZero{\pushforward{\projection{1}{}}{\varFixed}},
      \pushforward{\projection{24}{}}{\varTangent}\in\normalConeRegularStrong{\Omega_2}{\pushforward{\projection{2}{}}{\varFixed}}
  \}
  \\
  \normalConeStrong{\feasibleSet}{\varFixed}
  &=
  \{
      \varTangent\in\Pp{2}{\reals^m\times\reals^d\times\reals^m\times\reals^d}, \pushforward{\projection{12}{}}{\varTangent}=\varFixed
      \st
      \\
      &\qquad\qquad\qquad
      \pushforward{\projection{13}{}}{\varTangent}=\localZero{\pushforward{\projection{1}{}}{\varFixed}},
      \pushforward{\projection{24}{}}{\varTangent}\in\normalConeStrong{\Omega_2}{\pushforward{\projection{2}{}}{\varFixed}}
  \},
\end{align*}
and $\feasibleSet$ is \gls*{acr:snc} at $\varFixed$ whenever $\Omega_2$ is \gls*{acr:snc} at $\pushforward{\projection{2}{}}{\varFixed}$.
}

\item\label{item:product:delta}
{%
For $\feasibleSet=\{\varGeneric_1\times\delta_{b}\in\Pp{2}{\reals^{d}\times\reals}\st\varGeneric_1\in\Omega, b \in B\}$ and $\varFixed = \varFixed_1 \times\delta_{\bar b}\in\feasibleSet$, with $\Omega\subseteq\Pp{2}{\reals^{d}}$ and $B \subseteq \reals$, we have
\begin{align*}
  \normalConeRegular{\feasibleSet}{\varFixed}
  &=
  \{
      \varTangent\in\tangentSpace{(\varFixed)}{\Pp{2}{\reals^d\times\reals}}
      \st
      \\
      &\qquad\qquad\qquad
      \pushforward{\projection{13}{}}{\varTangent}\in\normalConeRegular{\Omega}{\varFixed_1},
      \pushforward{\projection{24}{}}{\varTangent}=\delta_{\bar b}\times\nu, \expectedValue{\varTangentReals\sim\nu}{\varTangentReals}\in\normalConeRegular{B}{\bar b}
  \}
  \\
  \normalCone{\feasibleSet}{\varFixed}
  &=
  \{
      \varTangent\in\Pp{2}{\reals^d\times\reals\times\reals^d\times\reals}, \pushforward{\projection{12}{}}{\varTangent}=\varFixed
      \st
      \\
      &\qquad\qquad\qquad
      \pushforward{\projection{13}{}}{\varTangent}\in\normalCone{\Omega}{\varFixed_1},
      \pushforward{\projection{24}{}}{\varTangent}=\delta_{\bar b}\times\nu, \expectedValue{\varTangentReals\sim\nu}{\varTangentReals}\in\normalCone{B}{\bar b}
  \}
  \\
  \normalConeRegularStrong{\feasibleSet}{\varFixed}
  &=
  \{
      \varTangent\in\tangentSpace{(\varFixed)}{\Pp{2}{\reals^d\times\reals}}
      \st
      \\
      &\qquad\qquad\qquad
      \pushforward{\projection{13}{}}{\varTangent}\in\normalConeRegularStrong{\Omega}{\varFixed_1},
      \pushforward{\projection{24}{}}{\varTangent}=\delta_{\bar b}\times\nu, \expectedValue{\varTangentReals\sim\nu}{\varTangentReals}\in\normalConeRegular{B}{\bar b}
  \}
  \\
  \normalConeStrong{\feasibleSet}{\varFixed}
  &=
  \{
      \varTangent\in\Pp{2}{\reals^d\times\reals\times\reals^d\times\reals}, \pushforward{\projection{12}{}}{\varTangent}=\varFixed
      \st
      \\
      &\qquad\qquad\qquad
      \pushforward{\projection{13}{}}{\varTangent}\in\normalConeStrong{\Omega}{\varFixed_1},
      \pushforward{\projection{24}{}}{\varTangent}=\delta_{\bar b}\times\nu, \expectedValue{\varTangentReals\sim\nu}{\varTangentReals}\in\normalCone{B}{\bar b}
  \}.
  \end{align*}
In particular, if $B = \nonnegativeReals$, $\expectedValue{\varTangentReals\sim\nu}{\varTangentReals} = 0$ for $\bar b > 0$ and $\expectedValue{\varTangentReals\sim\nu}{\varTangentReals} \leq 0$ for $\bar b = 0$.
}
\end{enumerate}


==> elements/prop_normal_cone_product_proof.tex <==
We prove the two parts separately.


\begin{enumerate}[leftmargin=*]
\item
{%
Throughout, $\varFixed_1\coloneqq\pushforward{\projection{1}{}}{\varFixed}\in\Omega_1$ and $\varFixed_2\coloneqq\pushforward{\projection{2}{}}{\varFixed}\in\Omega_2$ denote the two marginals of $\varFixed$ on $\reals^m$ and $\reals^d$, and $(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2)$ the coordinates of a variation at $\varFixed$.
As a preliminary, notice that $\norm{\varTangent}_{\varFixed}^2=\norm{\pushforward{\projection{13}{}}{\varTangent}}_{\varFixed_1}^2+\norm{\pushforward{\projection{24}{}}{\varTangent}}_{\varFixed_2}^2$ for every variation $\varTangent$ at $\varFixed$.
}

{%
\emph{Step 1 (normal-cone inequalities for the marginals).}
Let $\bar\varTangent\in\normalConeRegularStrong{\feasibleSet}{\varFixed}$; we show that $\innerProduct{\pushforward{\projection{24}{}}{\bar\varTangent}}{\varTangent_2}_{\varFixed_2}\leq\onotation{\norm{\varTangent_2}_{\varFixed_2}}$ for all $\varGeneric_2\in\Omega_2$ and $\varTangent_2\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varFixed_2}{\varGeneric_2}}$.
Let $\varTangentCoupling_2\in\setPlansCommonMarginal{\pushforward{\projection{24}{}}{\bar\varTangent}}{\varTangent_2}{1}$ attain $\innerProduct{\pushforward{\projection{24}{}}{\bar\varTangent}}{\varTangent_2}_{\varFixed_2}$.
Glue $\bar\varTangent$ and $\varTangentCoupling_2$ along their common marginal $\pushforward{\projection{24}{}}{\bar\varTangent}$, setting the $\reals^m$-velocity to $0$, to obtain a coupling $\varTangentCoupling$, and let $\varTangent$ be the variation at $\varFixed$ it induces (its $(\bar x_1,\bar x_2,\varTangentReals_1,\varTangentReals_2)$-marginal).
Then $\varTangentReals_1=0$ on the support of $\varTangent$, $\pushforward{\projection{24}{}}{\varTangent}=\varTangent_2$, $\norm{\varTangent}_{\varFixed}=\norm{\varTangent_2}_{\varFixed_2}$, and $\varTangentCoupling\in\setPlansCommonMarginal{\bar\varTangent}{\varTangent}{1}$ has $(\bar x_2,\bar\varTangentReals_2,\varTangentReals_2)$-marginal $\varTangentCoupling_2$.
The transport plan generating $\varTangent$ sends $\varFixed$ to a target $\varGeneric$ with $\reals^m$-marginal $\varFixed_1\in\Omega_1$ and $\reals^d$-marginal $\varGeneric_2\in\Omega_2$, so $\varGeneric\in\feasibleSet$, $\varTangent$ is an admissible test in \cref{definition:def_fuzzy_normal_cone}, and
\begin{align*}
    \onotation{\norm{\varTangent_2}_{\varFixed_2}}
    =
    \onotation{\norm{\varTangent}_{\varFixed}}
    \geq
    \innerProduct{\bar\varTangent}{\varTangent}_{\varFixed}
    &\geq
    \int_{(\reals^m\times\reals^d)^3} \innerProduct{\bar\varTangentReals_1}{\varTangentReals_1}+\innerProduct{\bar\varTangentReals_2}{\varTangentReals_2}
    \\
    &\hphantom{{}\geq{}}
    \d\varTangentCoupling(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,\varTangentReals_1,\varTangentReals_2)
    \\
    &=
    \int_{\reals^d\times\reals^d\times\reals^d} \innerProduct{\bar\varTangentReals_2}{\varTangentReals_2}
    \\
    &\hphantom{{}={}}
    \d\varTangentCoupling_2(\bar x_2,\bar\varTangentReals_2,\varTangentReals_2)
    =
    \innerProduct{\pushforward{\projection{24}{}}{\bar\varTangent}}{\varTangent_2}_{\varFixed_2},
\end{align*}
where the second equality uses $\varTangentReals_1=0$ on the support of $\varTangent$.
Analogously, $\innerProduct{\pushforward{\projection{13}{}}{\bar\varTangent}}{\varTangent_1}_{\varFixed_1}\leq\onotation{\norm{\varTangent_1}_{\varFixed_1}}$ for all $\varGeneric_1\in\Omega_1$ and $\varTangent_1\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varFixed_1}{\varGeneric_1}}$.
}

{%
\emph{Step 2 (the marginals are tangent).}
Let $\eta\coloneqq\pushforward{\projection{24}{}}{\bar\varTangent}$ and $\nu_t\coloneqq\pushforward{(\projection{2}{}+t\projection{4}{})}{\bar\varTangent}$ for $t>0$.
We claim that
\begin{equation}\label{equation:normal_cone_product:marginal_derivative}
\lim_{t\fromAbove0}\ \frac{\wassersteinDistance{\varFixed_2}{\nu_t}{2}}{t}\;=\;\norm{\eta}_{\varFixed_2}.
\end{equation}
The inequality ``$\leq$'' always holds, since the transport plan $\pushforward{(\projection{2}{},\projection{2}{}+t\projection{4}{})}{\bar\varTangent}$ couples $\varFixed_2$ and $\nu_t$ with cost $t^2\norm{\eta}_{\varFixed_2}^2$; if $\norm{\eta}_{\varFixed_2}=0$ \eqref{equation:normal_cone_product:marginal_derivative} is trivial.
Otherwise, suppose towards a contradiction that $\wassersteinDistance{\varFixed_2}{\nu_{t_n}}{2}\leq(1-\delta)\,t_n\norm{\eta}_{\varFixed_2}$ for some $\delta>0$ and $t_n\fromAbove0$.
Pick $\bar\alpha_n\in\setPlansOptimal{\nu_{t_n}}{\varFixed_2}$ and glue it to $\bar\varTangent$ along $\nu_{t_n}=\pushforward{(\projection{2}{}+t_n\projection{4}{})}{\bar\varTangent}$.
This yields $\Theta_n\in\Pp{2}{(\reals^m\times\reals^d)\times(\reals^m\times\reals^d)\times\reals^d}$, with coordinates $(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,z)$, such that
$
\pushforward{(\projection{\bar x_1}{},\projection{\bar x_2}{},\projection{\bar\varTangentReals_1}{},\projection{\bar\varTangentReals_2}{})}{\Theta_n}=\bar\varTangent
$
and
$
\pushforward{(\projection{\bar x_2}{}+t_n\projection{\bar\varTangentReals_2}{},\,\projection{z}{})}{\Theta_n}=\bar\alpha_n.
$
In particular, $\int_{(\reals^m\times\reals^d)^2\times\reals^d}\norm{z-\bar x_2-t_n\bar\varTangentReals_2}^2\d\Theta_n(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,z)=\wassersteinDistance{\nu_{t_n}}{\varFixed_2}{2}^2$.
Define
$
\varTangent_n\coloneqq\pushforward{\bigl(\projection{\bar x_1}{},\projection{\bar x_2}{},\,0,\,\projection{z}{}-\projection{\bar x_2}{}\bigr)}{\Theta_n},
$
induced by the transport plan $\pushforward{(\projection{\bar x_1}{},\projection{\bar x_2}{},\projection{\bar x_1}{},\projection{z}{})}{\Theta_n}\in\setPlans{\varFixed}{\varGeneric_n}$ with $\varGeneric_n\coloneqq\pushforward{(\projection{\bar x_1}{},\projection{z}{})}{\Theta_n}$.
Since $\pushforward{\projection{1}{}}{\varGeneric_n}=\varFixed_1\in\Omega_1$ and $\pushforward{\projection{2}{}}{\varGeneric_n}=\pushforward{\projection{z}{}}{\Theta_n}=\varFixed_2\in\Omega_2$, we have $\varGeneric_n\in\feasibleSet$, and $\varTangent_n$ is an admissible test in \cref{definition:def_fuzzy_normal_cone}.
Moreover, $\pushforward{\bigl(\projection{\bar x_1}{},\projection{\bar x_2}{},\projection{\bar\varTangentReals_1}{},\projection{\bar\varTangentReals_2}{},\,0,\,\projection{z}{}-\projection{\bar x_2}{}\bigr)}{\Theta_n}\in\setPlansCommonMarginal{\bar\varTangent}{\varTangent_n}{1}$, so, writing $\projection{z}{}-\projection{\bar x_2}{}=t_n\projection{\bar\varTangentReals_2}{}+(\projection{z}{}-\projection{\bar x_2}{}-t_n\projection{\bar\varTangentReals_2}{})$ and applying Cauchy--Schwarz,
\begin{align*}
\innerProduct{\bar\varTangent}{\varTangent_n}_{\varFixed}
&\geq{}\int_{(\reals^m\times\reals^d)^2\times\reals^d}\innerProduct{\bar\varTangentReals_2}{z-\bar x_2}\d\Theta_n(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,z)
\\
&=t_n\norm{\eta}_{\varFixed_2}^2+\int_{(\reals^m\times\reals^d)^2\times\reals^d}\innerProduct{\bar\varTangentReals_2}{z-\bar x_2-t_n\bar\varTangentReals_2}
\\
&\hphantom{{}={}}\d\Theta_n(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,z)
\\
&\geq t_n\norm{\eta}_{\varFixed_2}^2-\norm{\eta}_{\varFixed_2}\wassersteinDistance{\nu_{t_n}}{\varFixed_2}{2}
\\
&\geq\delta\,t_n\norm{\eta}_{\varFixed_2}^2.
\end{align*}
Similarly, triangle inequality in $\Lp{2}{\reals^d}{\Theta_n}$ gives $\norm{\varTangent_n}_{\varFixed}\leq t_n\norm{\eta}_{\varFixed_2}+\wassersteinDistance{\nu_{t_n}}{\varFixed_2}{2}\leq2t_n\norm{\eta}_{\varFixed_2}\to0$.
In particular, observe that $\norm{\varTangent_n}_{\varFixed}>0$; otherwise, $z=\bar x_2$ $\almostEverywhere{\Theta_n}$, and we would get $0\geq\delta t_n\norm{\eta}_{\varFixed_2}^2>0$.
Hence $\innerProduct{\bar\varTangent}{\varTangent_n}_{\varFixed}\geq\tfrac{\delta}{2}\norm{\eta}_{\varFixed_2}\norm{\varTangent_n}_{\varFixed}$ along a sequence with vanishing norms, contradicting $\innerProduct{\bar\varTangent}{\varTangent_n}_{\varFixed}\leq\onotation{\norm{\varTangent_n}_{\varFixed}}$ and yielding \eqref{equation:normal_cone_product:marginal_derivative}.
By \cite[Theorem~4.19]{gigli2008geometry}, a transport plan with first marginal $\varFixed_2$ is tangent if and only if it satisfies \eqref{equation:normal_cone_product:marginal_derivative}.
Hence $\eta\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed_2}$ and, with Step~1, $\eta\in\normalConeRegularStrong{\Omega_2}{\varFixed_2}$.
The same argument shows $\pushforward{\projection{13}{}}{\bar\varTangent}\in\tangentCone{\Pp{2}{\reals^m}}{\varFixed_1}$ and thus $\pushforward{\projection{13}{}}{\bar\varTangent}\in\normalConeRegularStrong{\Omega_1}{\varFixed_1}$.
Since $\pushforward{\projection{12}{}}{\bar\varTangent}=\varFixed$ by \cref{definition:def_fuzzy_normal_cone}, Steps~1--2 prove the inclusion ``$\subseteq$'' of the first equality.
}

{%
\emph{Step 3 (a lifting lemma).}
We show that, if $\varGeneric\in\Pp{2}{\reals^m\times\reals^d}$ and $\hat\varTangent\in\PpLocal{2}{(\reals^m\times\reals^d)\times(\reals^m\times\reals^d)}{\varGeneric}$ with $\pushforward{\projection{13}{}}{\hat\varTangent}\in\tangentCone{\Pp{2}{\reals^m}}{\pushforward{\projection{1}{}}{\varGeneric}}$ and $\pushforward{\projection{24}{}}{\hat\varTangent}\in\tangentCone{\Pp{2}{\reals^d}}{\pushforward{\projection{2}{}}{\varGeneric}}$, then $\hat\varTangent\in\tangentCone{\Pp{2}{\reals^m\times\reals^d}}{\varGeneric}$.
Suppose first that both marginals lie in the respective sets \eqref{definition:tangent_space} with $\bar\varepsilon_1,\bar\varepsilon_2$.
For $\varepsilon\in[0,\min\{\bar\varepsilon_1,\bar\varepsilon_2\})$ their $\varepsilon$-transport plans are optimal, so their supports are cyclically monotone and there are convex $\psi_\varepsilon$, $\phi_\varepsilon$ with $y_1+\varepsilon w_1\in\partial\psi_\varepsilon(y_1)$ and $y_2+\varepsilon w_2\in\partial\phi_\varepsilon(y_2)$ for all $(y_1,w_1)$, $(y_2,w_2)$ in the supports of $\pushforward{\projection{13}{}}{\hat\varTangent}$, $\pushforward{\projection{24}{}}{\hat\varTangent}$ (cf.\ \cite[Theorem 5.10]{villani2009optimal}).
The support of the joint $\varepsilon$-transport plan of $\hat\varTangent$ consists of pairs $\bigl((y_1,y_2),(y_1+\varepsilon w_1,y_2+\varepsilon w_2)\bigr)$ with $(y_1,w_1)$ and $(y_2,w_2)$ in those supports, hence is contained in the graph of $\partial\Phi_\varepsilon$ for the convex, separable $\Phi_\varepsilon(z_1,z_2)\coloneqq\psi_\varepsilon(z_1)+\phi_\varepsilon(z_2)$; the joint $\varepsilon$-transport plan is therefore optimal, and $\hat\varTangent$ lies in the joint set \eqref{definition:tangent_space} with $\bar\varepsilon\coloneqq\min\{\bar\varepsilon_1,\bar\varepsilon_2\}$.
Note that only the \emph{supports} of the marginals enter: the correlations between $w_1$, $w_2$, and the base are arbitrary.
In general, pick $\zeta^1_k$, $\zeta^2_k$ in the sets \eqref{definition:tangent_space} at $\pushforward{\projection{1}{}}{\varGeneric}$, $\pushforward{\projection{2}{}}{\varGeneric}$ converging to $\pushforward{\projection{13}{}}{\hat\varTangent}$, $\pushforward{\projection{24}{}}{\hat\varTangent}$ in the respective distances, and let $\theta^1_k\in\setPlansCommonMarginal{\pushforward{\projection{13}{}}{\hat\varTangent}}{\zeta^1_k}{1}$ and $\theta^2_k\in\setPlansCommonMarginal{\pushforward{\projection{24}{}}{\hat\varTangent}}{\zeta^2_k}{1}$ attain the two distances.
Glue $\theta^1_k$ and $\theta^2_k$ to $\hat\varTangent$, along $\pushforward{\projection{13}{}}{\hat\varTangent}$ and $\pushforward{\projection{24}{}}{\hat\varTangent}$, respectively.
This yields $\Lambda_k\in\Pp{2}{(\reals^m\times\reals^d)^3}$, with coordinates $(y_1,y_2,w_1,w_2,u_1,u_2)$, such that
$
\pushforward{(\projection{y_1}{},\projection{y_2}{},\projection{w_1}{},\projection{w_2}{})}{\Lambda_k}=\hat\varTangent,
$
$
\pushforward{(\projection{y_1}{},\projection{w_1}{},\projection{u_1}{})}{\Lambda_k}=\theta^1_k,
$
and
$
\pushforward{(\projection{y_2}{},\projection{w_2}{},\projection{u_2}{})}{\Lambda_k}=\theta^2_k .
$
Set $\hat\zeta_k\coloneqq\pushforward{(\projection{y_1}{},\projection{y_2}{},\projection{u_1}{},\projection{u_2}{})}{\Lambda_k}$.
Its marginals are $\pushforward{(\projection{y_1}{},\projection{u_1}{})}{\Lambda_k}=\pushforward{(\projection{1}{},\projection{3}{})}{\theta^1_k}=\zeta^1_k$ and, likewise, $\zeta^2_k$, so $\hat\zeta_k$ lies in the joint set \eqref{definition:tangent_space} by the first part.
Moreover, $\Lambda_k\in\setPlansCommonMarginal{\hat\varTangent}{\hat\zeta_k}{1}$, so
\begin{align*}
\wassersteinDistance{\hat\varTangent}{\hat\zeta_k}{\varGeneric}^2
&\leq\int_{(\reals^m\times\reals^d)^3}\norm{(w_1,w_2)-(u_1,u_2)}^2
\\
&\hphantom{{}\leq{}}\d\Lambda_k(y_1,y_2,w_1,w_2,u_1,u_2)
\\
&=\wassersteinDistance{\pushforward{\projection{13}{}}{\hat\varTangent}}{\zeta^1_k}{\pushforward{\projection{1}{}}{\varGeneric}}^2
+\wassersteinDistance{\pushforward{\projection{24}{}}{\hat\varTangent}}{\zeta^2_k}{\pushforward{\projection{2}{}}{\varGeneric}}^2
\to0 .
\end{align*}
}

{%
\emph{Step 4 (converse inclusion for the strong regular normal cone).}
Conversely, let $\bar\varTangent\in\Pp{2}{\reals^m\times\reals^d\times\reals^m\times\reals^d}$ with $\pushforward{\projection{12}{}}{\bar\varTangent}=\varFixed$, $\pushforward{\projection{13}{}}{\bar\varTangent}\in\normalConeRegularStrong{\Omega_1}{\varFixed_1}$ and $\pushforward{\projection{24}{}}{\bar\varTangent}\in\normalConeRegularStrong{\Omega_2}{\varFixed_2}$.
By \cref{definition:def_fuzzy_normal_cone}, the two marginals belong to $\tangentCone{\Pp{2}{\reals^m}}{\varFixed_1}$ and $\tangentCone{\Pp{2}{\reals^d}}{\varFixed_2}$, so Step~3 gives $\bar\varTangent\in\tangentCone{\Pp{2}{\reals^m\times\reals^d}}{\varFixed}$.
Then, for all $\varTangent\in\pushforward{(\projection{1}{},\projection{2}{},\projection{3}{}-\projection{1}{},\projection{4}{}-\projection{2}{})}{\setPlans{\varFixed}{\varGeneric}}$ with $\varGeneric\in\feasibleSet$,
\begin{align*}
    \innerProduct{\bar\varTangent}{\varTangent}_{\varFixed}
    &=
    \max_{\varTangentCoupling\in\setPlansCommonMarginal{\bar\varTangent}{\varTangent}{1}}
    \int_{(\reals^m\times\reals^d)^3} \innerProduct{\bar\varTangentReals_1}{\varTangentReals_1}+\innerProduct{\bar\varTangentReals_2}{\varTangentReals_2}
    \\
    &\hphantom{{}={}}
    \d\varTangentCoupling(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,\varTangentReals_1,\varTangentReals_2)
    \\
    &\leq
    \innerProduct{\pushforward{\projection{13}{}}{\bar\varTangent}}{\pushforward{\projection{13}{}}{\varTangent}}_{\varFixed_1}
    +
    \innerProduct{\pushforward{\projection{24}{}}{\bar\varTangent}}{\pushforward{\projection{24}{}}{\varTangent}}_{\varFixed_2}
    \\
    &\leq
    \onotation{\norm{\pushforward{\projection{13}{}}{\varTangent}}_{\varFixed_1}}
    +
    \onotation{\norm{\pushforward{\projection{24}{}}{\varTangent}}_{\varFixed_2}}
    \leq\onotation{\norm{\varTangent}_{\varFixed}}
\end{align*}
where the first inequality uses that the joint maximum is upper bounded by the sum of the independent maxima, and the second inequality uses $\pushforward{\projection{13}{}}{\varTangent}\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varFixed_1}{\pushforward{\projection{1}{}}{\varGeneric}}}$ with $\pushforward{\projection{1}{}}{\varGeneric}\in\Omega_1$ together with $\pushforward{\projection{13}{}}{\bar\varTangent}\in\normalConeRegularStrong{\Omega_1}{\varFixed_1}$, and the symmetric memberships for the second factor; the last inequality holds because $\norm{\pushforward{\projection{13}{}}{\varTangent}}_{\varFixed_1},\norm{\pushforward{\projection{24}{}}{\varTangent}}_{\varFixed_2}\leq\norm{\varTangent}_{\varFixed}$, so both error terms are $\onotation{\norm{\varTangent}_{\varFixed}}$ along any admissible family with $\norm{\varTangent}_{\varFixed}\to0$.
Hence $\bar\varTangent\in\normalConeRegularStrong{\feasibleSet}{\varFixed}$.
Together with Steps~1--2, this proves the first equality.
}

{%
\emph{Step 5 (the strong normal cone).}
For ``$\subseteq$'', let $\boldsymbol\varGeneric_n\in\feasibleSet$, $\boldsymbol\varGeneric_n\convergenceWasserstein\varFixed$, and $\hat\varTangent_n\in\normalConeRegularStrong{\feasibleSet}{\boldsymbol\varGeneric_n}$ with $\hat\varTangent_n\convergenceWasserstein\bar\varTangent$, as in \cref{definition:def_fuzzy_normal_cone}; in particular $\pushforward{\projection{12}{}}{\bar\varTangent}=\varFixed$.
The projections $\pushforward{\projection{13}{}}{}$, $\pushforward{\projection{24}{}}{}$, $\pushforward{\projection{1}{}}{}$, and $\pushforward{\projection{2}{}}{}$ are $1$-Lipschitz with respect to $\wassersteinDistance{}{}{2}$.
By the first equality, $\pushforward{\projection{13}{}}{\hat\varTangent_n}\in\normalConeRegularStrong{\Omega_1}{\pushforward{\projection{1}{}}{\boldsymbol\varGeneric_n}}$ with $\pushforward{\projection{1}{}}{\boldsymbol\varGeneric_n}\convergenceWasserstein\varFixed_1$ and $\pushforward{\projection{13}{}}{\hat\varTangent_n}\convergenceWasserstein\pushforward{\projection{13}{}}{\bar\varTangent}$, whence $\pushforward{\projection{13}{}}{\bar\varTangent}\in\normalConeStrong{\Omega_1}{\varFixed_1}$; symmetrically, $\pushforward{\projection{24}{}}{\bar\varTangent}\in\normalConeStrong{\Omega_2}{\varFixed_2}$.
For ``$\supseteq$'', let $\bar\varTangent$ satisfy $\pushforward{\projection{12}{}}{\bar\varTangent}=\varFixed$, $\pushforward{\projection{13}{}}{\bar\varTangent}\in\normalConeStrong{\Omega_1}{\varFixed_1}$, and $\pushforward{\projection{24}{}}{\bar\varTangent}\in\normalConeStrong{\Omega_2}{\varFixed_2}$. Then, there are $\varGeneric_{1,n}\in\Omega_1$, $\varGeneric_{1,n}\convergenceWasserstein\varFixed_1$, $\varTangent^1_n\in\normalConeRegularStrong{\Omega_1}{\varGeneric_{1,n}}$, $\varTangent^1_n\convergenceWasserstein\pushforward{\projection{13}{}}{\bar\varTangent}$, and $\varGeneric_{2,n}\in\Omega_2$, $\varGeneric_{2,n}\convergenceWasserstein\varFixed_2$, $\varTangent^2_n\in\normalConeRegularStrong{\Omega_2}{\varGeneric_{2,n}}$, $\varTangent^2_n\convergenceWasserstein\pushforward{\projection{24}{}}{\bar\varTangent}$.
Choose $\beta^1_n\in\setPlans{\pushforward{\projection{13}{}}{\bar\varTangent}}{\varTangent^1_n}$, with coordinates $(\bar x_1,\bar\varTangentReals_1,y_1,w_1)$, and $\beta^2_n\in\setPlans{\pushforward{\projection{24}{}}{\bar\varTangent}}{\varTangent^2_n}$, with coordinates $(\bar x_2,\bar\varTangentReals_2,y_2,w_2)$, such that $\int_{(\reals^m\times\reals^m)^2}\norm{y_1-\bar x_1}^2+\norm{w_1-\bar\varTangentReals_1}^2\d\beta^1_n(\bar x_1,\bar\varTangentReals_1,y_1,w_1)\to0$ and $\int_{(\reals^d\times\reals^d)^2}\norm{y_2-\bar x_2}^2+\norm{w_2-\bar\varTangentReals_2}^2\d\beta^2_n(\bar x_2,\bar\varTangentReals_2,y_2,w_2)\to0$, and glue them to $\bar\varTangent$, along $\pushforward{\projection{13}{}}{\bar\varTangent}$ and $\pushforward{\projection{24}{}}{\bar\varTangent}$ respectively.
This yields $\Lambda_n\in\Pp{2}{(\reals^m\times\reals^d)^4}$, with coordinates $(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,y_1,w_1,y_2,w_2)$, such that
$
\pushforward{(\projection{\bar x_1}{},\projection{\bar x_2}{},\projection{\bar\varTangentReals_1}{},\projection{\bar\varTangentReals_2}{})}{\Lambda_n}=\bar\varTangent,
\pushforward{(\projection{\bar x_1}{},\projection{\bar\varTangentReals_1}{},\projection{y_1}{},\projection{w_1}{})}{\Lambda_n}=\beta^1_n,
$
and
$
\pushforward{(\projection{\bar x_2}{},\projection{\bar\varTangentReals_2}{},\projection{y_2}{},\projection{w_2}{})}{\Lambda_n}=\beta^2_n .
$
Set
$
\varFixed_n\coloneqq\pushforward{(\projection{y_1}{},\projection{y_2}{})}{\Lambda_n}
$
and
$
\hat\varTangent_n\coloneqq\pushforward{(\projection{y_1}{},\projection{y_2}{},\projection{w_1}{},\projection{w_2}{})}{\Lambda_n} .
$
Then: (i) $\pushforward{\projection{1}{}}{\varFixed_n}=\pushforward{\projection{1}{}}{\varTangent^1_n}=\varGeneric_{1,n}\in\Omega_1$ and $\pushforward{\projection{2}{}}{\varFixed_n}=\varGeneric_{2,n}\in\Omega_2$, so $\varFixed_n\in\feasibleSet$, and $\wassersteinDistance{\varFixed_n}{\varFixed}{2}^2\leq\int_{(\reals^m\times\reals^d)^4}\norm{y_1-\bar x_1}^2+\norm{y_2-\bar x_2}^2\d\Lambda_n(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,y_1,w_1,y_2,w_2)\to0$; (ii) $\pushforward{\bigl((\projection{\bar x_1}{},\projection{\bar x_2}{},\projection{\bar\varTangentReals_1}{},\projection{\bar\varTangentReals_2}{}),(\projection{y_1}{},\projection{y_2}{},\projection{w_1}{},\projection{w_2}{})\bigr)}{\Lambda_n}$ couples $\bar\varTangent$ and $\hat\varTangent_n$ with cost $\int_{(\reals^m\times\reals^d)^4}\norm{y_1-\bar x_1}^2+\norm{y_2-\bar x_2}^2+\norm{w_1-\bar\varTangentReals_1}^2+\norm{w_2-\bar\varTangentReals_2}^2\d\Lambda_n(\bar x_1,\bar x_2,\bar\varTangentReals_1,\bar\varTangentReals_2,y_1,w_1,y_2,w_2)\to0$, so $\hat\varTangent_n\convergenceWasserstein\bar\varTangent$; (iii) $\pushforward{\projection{13}{}}{\hat\varTangent_n}=\pushforward{(\projection{3}{},\projection{4}{})}{\beta^1_n}=\varTangent^1_n\in\normalConeRegularStrong{\Omega_1}{\varGeneric_{1,n}}$ and $\pushforward{\projection{24}{}}{\hat\varTangent_n}=\varTangent^2_n\in\normalConeRegularStrong{\Omega_2}{\varGeneric_{2,n}}$, with $\varGeneric_{1,n}$ and $\varGeneric_{2,n}$ the marginals of $\varFixed_n$, so Step~4, applied at $\varFixed_n$, gives $\hat\varTangent_n\in\normalConeRegularStrong{\feasibleSet}{\varFixed_n}$.
By \cref{definition:def_fuzzy_normal_cone}, $\bar\varTangent\in\normalConeStrong{\feasibleSet}{\varFixed}$.
}

{%
\emph{Step 6 (\gls*{acr:snc}).}
Let $\boldsymbol\varGeneric_n\in\feasibleSet$, $\boldsymbol\varGeneric_n\convergenceWasserstein\varFixed$, and $\hat\varTangent_n\in\normalConeRegularStrong{\feasibleSet}{\boldsymbol\varGeneric_n}$ with $\hat\varTangent_n\convergenceNarrow\hat\varTangent$.
We show $\hat\varTangent_n\convergenceWasserstein\hat\varTangent$.
By the first equality at $\boldsymbol\varGeneric_n$, $\pushforward{\projection{13}{}}{\hat\varTangent_n}\in\normalConeRegularStrong{\Omega_1}{\pushforward{\projection{1}{}}{\boldsymbol\varGeneric_n}}$ and $\pushforward{\projection{24}{}}{\hat\varTangent_n}\in\normalConeRegularStrong{\Omega_2}{\pushforward{\projection{2}{}}{\boldsymbol\varGeneric_n}}$.
Both sequences of marginals converge narrowly (continuous projections), with bases converging in Wasserstein, so, since $\Omega_1$ and $\Omega_2$ are \gls*{acr:snc}, $\pushforward{\projection{13}{}}{\hat\varTangent_n}\convergenceWasserstein\pushforward{\projection{13}{}}{\hat\varTangent}$ and $\pushforward{\projection{24}{}}{\hat\varTangent_n}\convergenceWasserstein\pushforward{\projection{24}{}}{\hat\varTangent}$.
Hence, the second moment of $\hat\varTangent_n$ converges to that of $\hat\varTangent$, and narrow convergence together with convergence of the second moments is equivalent to convergence in Wasserstein \cite[Theorem 6.9]{villani2009optimal}.
}

{%
\emph{Step 7 (the cylinder case $\Omega_1=\Pp{2}{\reals^m}$).}
By \cref{lemma:strong_vs_regular_normal_cone} and \cref{proposition:prop_normal_cones_trivial}\ref{item:normal_cone:no_constraints}, the strong (regular) normal cones of $\Pp{2}{\reals^m}$ reduce to $\{\localZero{\varFixed_1}\}$, and $\Pp{2}{\reals^m}$ is \gls*{acr:snc}; substituting $\Omega_1=\Pp{2}{\reals^m}$ into the general statement gives the final part.
}

\item {Write $\varFixed_1\coloneqq\pushforward{\projection{1}{}}{\varFixed}$, so that $\varFixed=\varFixed_1\times\delta_{\bar b}$, and let $\delta_{\bar b}\times\nu\coloneqq\pushforward{\projection{24}{}}{\bar\varTangent}$.
We first record two structural facts and then prove the two inclusions in the regular case. \gls*{acr:snc} and the statements for the normal cone follow directly from the expressions for the (strong) regular normal cone, on which its proof below focuses.
}

{%
Here $\feasibleSet\subseteq\Pp{2}{\reals^d\times\reals}$, variations at
$\varFixed$ live in $\Pp{2}{(\reals^d\times\reals)\times(\reals^d\times\reals)}$,
and the block projections $\projection{13}{}$ and $\projection{24}{}$ retain,
respectively, the $\reals^d$-position with its $\reals^d$-velocity and the
$\reals$-position with its $\reals$-velocity. Under the identification
$\reals^d\times\reals=\reals^{d+1}$, the map $\projection{13}{}$ coincides with
$T$ of \eqref{equation:extraction-map-epigraph}; we therefore apply
\cref{lemma:lemma_deterministic_coordinate} with
$\pushforward{\projection{13}{}}{\cdot}$ in place of $\pushforward{T}{\cdot}$
and with the last velocity component given by the second component of the
$\projection{24}{}$-block.
}

{%
\emph{Fact 1 (set of optimal transport plans).}
Fix $\varGeneric=\varGeneric_1\times\delta_b\in\feasibleSet$. By
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport},
with the lemma's base and target deterministic coordinates instantiated as
$\bar b$ and $b$, a transport plan of $\varFixed=\varFixed_1\times\delta_{\bar b}$ and
$\varGeneric=\varGeneric_1\times\delta_b$ has the form
$\pushforward{(\projection{1}{},\projection{3}{},\projection{2}{},\projection{4}{})}{(\gamma\times\delta_{(\bar b,b)})}$
with $\gamma$ a transport plan of $\varFixed_1$ and $\varGeneric_1$, and its cost is
$\int_{\reals^d\times\reals^d}\norm{x'-x}^2\d\gamma(x,x')+\abs{b-\bar b}^2$;
consequently,
$
    \setPlansOptimal{\varFixed}{\varGeneric}=\bigl\{
        \pushforward{(\projection{1}{},\projection{3}{},\projection{2}{},\projection{4}{})}{(\gamma\times\delta_{(\bar b,b)})}
        \st\gamma\in\setPlansOptimal{\varFixed_1}{\varGeneric_1}\bigr\}.
$
}

{%
\emph{Fact 2 ($\pushforward{\projection{13}{}}{\bar\varTangent}$ is tangent).}
By \cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}
(under the identification above),
$\pushforward{\projection{13}{}}{\bar\varTangent}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed_1}$
if and only if $\bar\varTangent\in\tangentCone{\Pp{2}{\reals^d\times\reals}}{\varFixed}$.
}

{
By Fact~1, every variation $\varTangent\in\pushforward{(\projection{1}{},\projection{2}{},\projection{3}{}-\projection{1}{},\projection{4}{}-\projection{2}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$ with $\varGeneric=\varGeneric_1\times\delta_b\in\feasibleSet$ satisfies $\pushforward{\projection{13}{}}{\varTangent}=\varTangent_1\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlansOptimal{\varFixed_1}{\varGeneric_1}}$ and $\pushforward{\projection{24}{}}{\varTangent}=\delta_{(\bar b,\,b-\bar b)}$.
}

{%
Since $\varTangent$ has last velocity component almost everywhere equal to
$b-\bar b$ (Fact~1), $\pushforward{\projection{13}{}}{\varTangent}=\varTangent_1$,
and $\pushforward{\projection{24}{}}{\bar\varTangent}=\delta_{\bar b}\times\nu$
(so that the last velocity component of $\bar\varTangent$ is distributed as
$\nu$), \eqref{eq:deterministic_coordinate:splitting} (cf.
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting}),
with $c=b-\bar b$, gives
$
    \innerProduct{\bar\varTangent}{\varTangent}_{\varFixed}
    =
    \innerProduct{\pushforward{\projection{13}{}}{\bar\varTangent}}{\varTangent_1}_{\varFixed_1}
    +
    (b-\bar b)\expectedValue{\varTangentReals\sim\nu}{\varTangentReals}.
$
Moreover, $\norm{\varTangent}_{\varFixed}^2=\wassersteinDistance{\varFixed_1}{\varGeneric_1}{2}^2+\abs{b-\bar b}^2=\wassersteinDistance{\varFixed}{\varGeneric}{2}^2$:
the first equality is
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting}
with $c=b-\bar b$, using that $\varTangent_1=\pushforward{\projection{13}{}}{\varTangent}$
is induced by an optimal transport plan, whence
$\norm{\varTangent_1}_{\varFixed_1}=\wassersteinDistance{\varFixed_1}{\varGeneric_1}{2}$;
the second is the distance split of
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport}.
}

{
For the ``$\subseteq$'' inclusion, let $\bar\varTangent\in\normalConeRegular{\feasibleSet}{\varFixed}$.
Taking $b=\bar b$ yields $\innerProduct{\pushforward{\projection{13}{}}{\bar\varTangent}}{\varTangent_1}_{\varFixed_1}\leq\onotation{\wassersteinDistance{\varFixed_1}{\varGeneric_1}{2}}$ for all $\varGeneric_1\in\Omega$, i.e., $\pushforward{\projection{13}{}}{\bar\varTangent}\in\normalConeRegular{\Omega}{\varFixed_1}$ (since it is tangent by Fact~2).
Taking $\varGeneric_1=\varFixed_1$, so that $\varTangent_1=\localZero{\varFixed_1}$, yields $(b-\bar b)\expectedValue{\varTangentReals\sim\nu}{\varTangentReals}\leq\onotation{\abs{b-\bar b}}$ for all $b\in B$, i.e., $\expectedValue{\varTangentReals\sim\nu}{\varTangentReals}\in\normalConeRegular{B}{\bar b}$ (cf. \cite[Definition 6.3]{rockafellar2009variational}).
}

{
For the ``$\supseteq$'' inclusion, if $\pushforward{\projection{13}{}}{\bar\varTangent}\in\normalConeRegular{\Omega}{\varFixed_1}$ and $\expectedValue{\varTangentReals\sim\nu}{\varTangentReals}\in\normalConeRegular{B}{\bar b}$, then $\innerProduct{\pushforward{\projection{13}{}}{\bar\varTangent}}{\varTangent_1}_{\varFixed_1}\leq\onotation{\wassersteinDistance{\varFixed_1}{\varGeneric_1}{2}}$ and $(b-\bar b)\expectedValue{\varTangentReals\sim\nu}{\varTangentReals}\leq\onotation{\abs{b-\bar b}}$.
Thus, $\innerProduct{\bar\varTangent}{\varTangent}_{\varFixed}\leq\onotation{\wassersteinDistance{\varFixed_1}{\varGeneric_1}{2}}+\onotation{\abs{b-\bar b}}\leq\onotation{\wassersteinDistance{\varFixed}{\varGeneric}{2}}$.
The statement for the strong regular normal cone is analogous.
Finally, for $B=\nonnegativeReals$ one has $\normalConeRegular{B}{\bar b}=\{0\}$ if $\bar b>0$ and $\normalConeRegular{B}{\bar b}=(-\infty,0]$ if $\bar b=0$, giving the stated sign conditions on $\expectedValue{\varTangentReals\sim\nu}{\varTangentReals}$.
}

\end{enumerate}


==> elements/prop_normal_cone_product_title.tex <==
Product rule%

==> elements/prop_normal_cone_wasserstein_ball_body.tex <==
{For $\varepsilon>0$  and $\varReference \in \Pp{2}{\reals^d}$, consider the closed Wasserstein ball $\feasibleSet=\closedWassersteinBall{\varReference}{\varepsilon}{2}=\{\varGeneric\in\Pp{2}{\reals^d}\st\wassersteinDistance{\varGeneric}{\varReference}{2}\leq\varepsilon\}$. Let $\varFixed\in\feasibleSet$. Then,
\begin{enumerate}
    \item if $\varFixed$ lies in the interior of $\feasibleSet$ (i.e., $\wassersteinDistance{\varFixed}{\varReference}{2}<\varepsilon$), then $\normalCone{\feasibleSet}{\varFixed}=\normalConeStrong{\feasibleSet}{\varFixed}=\{\localZero{\varFixed}\}$;
%
    \item if $\varFixed$ is at the boundary of $\feasibleSet$ (i.e., $\wassersteinDistance{\varFixed}{\varReference}{2}=\varepsilon$), then
    $\normalConeStrong{\feasibleSet}{\varFixed}
    \subseteq
    \{
    \varTangent\st
    \varTangent\in
    \pushforward{(\projection{1}{}, 2\lambda(\projection{1}{} - \projection{2}{}))}{\setPlansOptimal{\varFixed}{\varReference}},
    \lambda\geq 0
    \}$.
    In particular, if $\varFixed$ is absolutely continuous, then
    $\normalConeStrong{\feasibleSet}{\varFixed}
    \subseteq
    \{
    \pushforward{(\identity{}, 2\lambda(\identity{} - T))}{\varFixed}
    \st
    \lambda\geq 0
    \}$, where $T$ is the unique optimal transport map between $\varFixed$ and $\varReference$;
    and
%
    \item the closed Wasserstein ball $\feasibleSet$ is \gls*{acr:snc} at $\varFixed$ (\cref{definition:def_snc}).
\end{enumerate}}


==> elements/prop_normal_cone_wasserstein_ball_proof.tex <==
We prove the statements separately.

\begin{enumerate}
\item The statement follows directly from~\cref{proposition:prop_normal_cones_trivial}.
{For the strong normal cone, since the interior of
$\feasibleSet$ is open, every $\varGeneric\in\feasibleSet$ close to
$\varFixed$ is an interior point as well, so
$\normalConeRegularStrong{\feasibleSet}{\varGeneric}\subseteq\normalConeRegular{\feasibleSet}{\varGeneric}=\{\localZero{\varGeneric}\}$
by \cref{lemma:strong_vs_regular_normal_cone} and
\cref{proposition:prop_normal_cones_trivial}\ref{item:normal_cone:interior_point}; hence the witnesses in
\cref{definition:def_fuzzy_normal_cone} satisfy
$\varTangent_n=\localZero{\varGeneric_n}\convergenceWasserstein\localZero{\varFixed}$,
and $\normalConeStrong{\feasibleSet}{\varFixed}=\{\localZero{\varFixed}\}$.}

\item We use~\cref{proposition:prop_normal_cones_constraints_simple}.
%
{We write $\feasibleSet=\{\varGeneric\in\Pp{2}{\reals^d}\st\objective(\varGeneric)\leq 0\}$
with $\objective(\varGeneric)\coloneqq\wassersteinDistance{\varGeneric}{\varReference}{2}^2-\varepsilon^2$,
which is proper and continuous and satisfies $\objective(\varFixed)=0$ since $\varFixed$
lies at the boundary.}
By~\cref{proposition:prop_wassersteindistance_general_subgradient}, $\subgradient{\objective}(\varFixed)$ is not empty and is contained in
$
\pushforward{(\projection{1}{}, 2\projection{1}{} - 2\projection{2}{})}{\setPlansOptimal{\varFixed}{\varReference}}
${,
where the factor 2 arises since there is no $\frac{1}{2}$ in front of the Wasserstein distance, and the additive constant $-\varepsilon^2$ does not affect the subgradient} (\cref{corollary:cor_chain_rule_linear}).
Since $\varFixed$ lies at the boundary, we have $\varFixed\neq\varReference$ and so $\setPlansOptimal{\varFixed}{\varReference}$ does not contain the ``identity transport plan'' $\pushforward{(\identity{},\identity{})}{\varFixed}$.
%
If $\localZero{\varFixed}=\pushforward{(\projection{1}{},2(\projection{1}{}-\projection{2}{}))}{\gamma}$ for some $\gamma\in\setPlansOptimal{\varFixed}{\varReference}$, then $x=\hat x$ holds $\almostEverywhere{\gamma}$, i.e., $\gamma$ is the identity transport plan.
Thus, $\localZero{\varFixed}$ does not belong to the subgradient of $\objective$, and the constraint qualification in~\cref{proposition:prop_normal_cones_constraints_simple} holds true.
Moreover, by~\cref{proposition:cor_subgradients_horizon}, $\objective$ has trivial horizon subgradient.
{Here, \cref{proposition:cor_subgradients_horizon} covers
$\frac{1}{2}\wassersteinDistance{\varGeneric}{\varReference}{2}^2$, and the property transfers
to $\objective$ since positive scaling and additive constants do not affect the horizon
subgradient. Indeed, $\epigraph{\objective}$ is the image of
$\epigraph{\left(\frac{1}{2}\wassersteinDistance{\cdot}{\varReference}{2}^2\right)}$ under the
map $\varGeneric\times\delta_\beta\mapsto\varGeneric\times\delta_{2\beta-\varepsilon^2}$;
correspondingly, the (regular) epigraphical normals of the two epigraphs are in bijection,
via rescaling of the last velocity component by $\frac{1}{2}$, which preserves convergence
and the zero-expectation condition in
\cref{definition:def_sub_sup_differentiability_horizon}; since the extraction map
\eqref{equation:extraction-map-epigraph} discards that component, the two horizon
subdifferentials coincide.
With this, \cref{proposition:prop_normal_cones_constraints_simple}
bounds the strong normal cone by the cone generated by the subdifferential of
$\objective$ at $\varFixed$, together with its horizon subdifferential; the
latter is trivial by the above, so
$
\normalConeStrong{\feasibleSet}{\varFixed}
\subseteq
\{\lambda\varTangent\st\lambda\geq 0,\ \varTangent\in\subgradient{\objective}(\varFixed)\}
$
and hence}
$
\normalConeStrong{\feasibleSet}{\varFixed}
\subseteq
\{
\varTangent\st
\varTangent\in
\pushforward{(\projection{1}{}, 2\lambda(\projection{1}{} - \projection{2}{}))}{\setPlansOptimal{\varFixed}{\varReference}},
\lambda\geq 0
\}.
$
In particular, if $\varFixed$ is absolutely continuous, then $\setPlansOptimal{\varFixed}{\varReference}=\{\pushforward{(\identity{},T)}{\varFixed}\}$, where $T$ is the unique optimal transport map~\cite{brenier1991polar}, and
$\normalConeStrong{\feasibleSet}{\varFixed}
\subseteq
\{
\pushforward{(\identity{}, 2\lambda(\identity{} - T))}{\varFixed}
\st
\lambda\geq 0
\}.
$
{Note that the argument of this item applies verbatim at every
boundary point of $\feasibleSet$; i.e., for every $\varGeneric\in\feasibleSet$
with $\wassersteinDistance{\varGeneric}{\varReference}{2}=\varepsilon$ we have
$\normalConeStrong{\feasibleSet}{\varGeneric}\subseteq\{\varTangent\st\varTangent\in\pushforward{(\projection{1}{},2\lambda(\projection{1}{}-\projection{2}{}))}{\setPlansOptimal{\varGeneric}{\varReference}},\lambda\geq0\}$.}





\item
Without loss of generality, we assume that $\varFixed$ lies at the boundary of the Wasserstein ball; otherwise, the result follows directly from~(i).
%
Consider any sequence $(\varGeneric_n)_{n \in \naturals} \subseteq \feasibleSet$, $\varGeneric_n\convergenceWasserstein\varFixed$ and $\varTangent_n\in\normalConeRegularStrong{\feasibleSet}{\varGeneric_n}$ so that $\varTangent_n\convergenceNarrow\varTangent$. By the above, since $\varTangent_n$ belongs to the strong regular normal cone, we necessarily have $\varTangent_n=2\lambda_n\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\gamma_n}$ for some $\gamma_n\in\setPlansOptimal{\varGeneric_n}{\varReference}$ and $\lambda_n\geq 0$.
{Indeed,
$\normalConeRegularStrong{\feasibleSet}{\varGeneric_n}\subseteq\normalConeStrong{\feasibleSet}{\varGeneric_n}$, so if
$\varGeneric_n$ lies at the boundary the representation follows from the
previous item applied at $\varGeneric_n$; if instead $\varGeneric_n$ lies in
the interior, then
$\normalConeRegularStrong{\feasibleSet}{\varGeneric_n}\subseteq\normalConeRegular{\feasibleSet}{\varGeneric_n}=\{\localZero{\varGeneric_n}\}$
by \cref{lemma:strong_vs_regular_normal_cone} and
\cref{proposition:prop_normal_cones_trivial}\ref{item:normal_cone:interior_point}, so the representation holds with
$\lambda_n=0$ and any
$\gamma_n\in\setPlansOptimal{\varGeneric_n}{\varReference}$.}
By stability of optimal transport plans~\cite[Theorem 5.20]{villani2009optimal}, we have that, up to passing to a subsequence, $\gamma_n\convergenceNarrow\gamma$ for some $\gamma\in\setPlansOptimal{\varFixed}{\varReference}$.
%
We now consider two cases separately.
\begin{enumerate}
\item {Suppose that, up to subsequences, $\lambda_n$ converges to $\lambda\coloneqq\lim_{n\to\infty}\lambda_n\geq 0$.
%
Since $\lambda_n\to\lambda$, the maps $(x,\hat x)\mapsto(x,2\lambda_n(x-\hat x))$
converge to $(x,\hat x)\mapsto(x,2\lambda(x-\hat x))$ uniformly on compact sets;
as $\gamma_n\convergenceNarrow\gamma$,~\cite[Lemma 5.2.1]{ambrosio2005gradient}
yields
$\varTangent_n\convergenceNarrow 2\lambda\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\gamma}$.
Since, by assumption, $\varTangent_n\convergenceNarrow\varTangent$, uniqueness of
the narrow limit gives
$\varTangent=2\lambda\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\gamma}$, with $\gamma$ as above.
%
Then, since narrow convergence together with convergence of the
second moment is equivalent to convergence in
Wasserstein~\cite[Theorem~6.9]{villani2009optimal}, it suffices to establish}
convergence of the second moment to conclude $\varTangent_n\convergenceWasserstein\varTangent$:
\begin{align*}
    \int_{\reals^d\times\reals^d}\norm{x_n}^2+\norm{\varTangentReals}^2\d\varTangent_n(x_n,\varTangentReals)
    ={}&
    \int_{\reals^d\times\reals^d}
    \norm{x_n}^2+4\lambda_n^2\norm{x_n-\hat x}^2\d\gamma_n(x_n,\hat x)
    \\
    ={}&
    \int_{\reals^d}
    \norm{x_n}^2\d\varGeneric_n(x_n) + 4\lambda_n^2\wassersteinDistance{\varGeneric_n}{\varReference}{2}^2
    \\
    \to{}&
    \int_{\reals^d}
    \norm{\bar x}^2\d\varFixed(\bar x) + 4\lambda^2\wassersteinDistance{\varFixed}{\varReference}{2}^2
    \\
    ={}&
    \int_{\reals^d\times\reals^d}\norm{\bar x}^2+\norm{\varTangentReals}^2\d\varTangent(\bar x,\varTangentReals),
\end{align*}
where we used convergence in Wasserstein of $\varGeneric_n$ to $\varFixed$.
%
Thus, $\varTangent_n\convergenceWasserstein\varTangent$.

\item {We consider the case $\lim_{n\to\infty}\lambda_n=+\infty$, and show that this contradicts narrow convergence of $\varTangent_n$.
Since the radius of the ball is strictly positive (i.e., $\varepsilon>0$) and $\varFixed$ lies at the boundary, we necessarily have $\varFixed\neq\varReference$. Thus, there are $\eta_1, \eta_2>0$ so that $\gamma(\{\norm{\bar x-\hat x}>\eta_1\})\geq \eta_2$.
%
By Portmanteau theorem, we have $\liminf_{n\to\infty}\gamma_n(\{\norm{x_n-\hat x}>\eta_1\})\geq \gamma(\{\norm{\bar x-\hat x}>\eta_1\})\geq \eta_2$, so that $\gamma_n(\{\norm{x_n-\hat x}>\eta_1\})\geq \frac{\eta_2}{2}$ for $n$ large enough. The definition of $\varTangent_n$ then yields, for $n$ large enough (in particular, $\lambda_n>0$),
\begin{equation*}
    (\pushforward{\projection{2}{}}{\varTangent_n})(\{\norm{\varTangentReals}>2\lambda_n\eta_1\})
    =
    \gamma_n(\{2\lambda_n\norm{x_n-\hat x}>2\lambda_n\eta_1\})
    \geq
    \frac{\eta_2}{2}.
\end{equation*}
However, since it converges narrowly, $\varTangent_n$ is tight by Prokhorov theorem~\cite[Theorem 5.1.3]{ambrosio2005gradient}, and hence so is $\pushforward{\projection{2}{}}{\varTangent_n}$.
Thus, there is $R>0$ large enough so that $(\pushforward{\projection{2}{}}{\varTangent_n})(\{\norm{\varTangentReals}>R\})<\frac{\eta_2}{2}$. For $n$ large enough, $2\eta_1\lambda_n>R$ and we conclude
\begin{equation*}
    \frac{\eta_2}{2}
    \leq
    (\pushforward{\projection{2}{}}{\varTangent_n})(\{\norm{\varTangentReals}>2\lambda_n\eta_1\})
    \leq
    (\pushforward{\projection{2}{}}{\varTangent_n})(\{\norm{\varTangentReals}>R\})
    <
    \frac{\eta_2}{2}.
\end{equation*}
This is a contradiction. The same argument applies along any subsequence with
$\lambda_n\to+\infty$: extracting, as above, a further subsequence with
$\gamma_n\convergenceNarrow\gamma\in\setPlansOptimal{\varFixed}{\varReference}$
\cite[Theorem~5.20]{villani2009optimal}, the contradiction persists, since
$(\varTangent_n)_{n\in\naturals}$ is tight. Hence,
$(\lambda_n)_{n\in\naturals}$ is bounded.}
\end{enumerate}
{Every subsequence of
$(\varTangent_n)_{n\in\naturals}$ then admits a further subsequence along which
$\lambda_n$ and $\gamma_n$ converge, and by case (a) it converges to
$\varTangent$ in Wasserstein. Since this limit does not depend on the
subsequence, the whole sequence satisfies
$\varTangent_n\convergenceWasserstein\varTangent$.
Overall, we can therefore conclude that the closed Wasserstein
ball is \gls*{acr:snc} at $\varFixed$.}

\end{enumerate}


==> elements/prop_normal_cone_wasserstein_ball_title.tex <==
Normal cone to closed Wasserstein balls%

==> elements/prop_normal_cones_constraints_simple_body.tex <==
Suppose $
\feasibleSet \coloneqq \left\{
\varGeneric \in \Pp{2}{\reals^d}
\st
\objective(\varGeneric) \leq 0
\right\}
$ for a proper, continuous functional $\objective: \Pp{2}{\reals^d} \to \realsBar$.
Then, at any $\varFixed \in \feasibleSet$ so that $\objective(\varFixed) = 0$, we have
$\normalConeRegular{\feasibleSet}{\varFixed}
\supseteq
\left\{\lambda\varTangent \st \lambda \geq 0, \varTangent \in \subgradientRegular{\objective}(\varFixed)\right\}$
{and 
$\normalConeRegularStrong{\feasibleSet}{\varFixed}
\supseteq
\left\{\lambda\varTangent \st \lambda \geq 0, \varTangent \in \subgradientRegularStrong{\objective}(\varFixed)\right\}$,}
and, if $\localZero{\varFixed} \not\in \subgradient{\objective}(\varFixed)$, then
$\normalConeStrong{\feasibleSet}{\varFixed}
\subseteq\left\{\lambda\varTangent \st \lambda \geq 0, \varTangent \in \subgradient{\objective}(\varFixed)\right\} \cup \subgradientHzn{\objective}(\varFixed)$.
If $\objective(\varFixed) < 0$, then $\normalConeRegular{\feasibleSet}{\varFixed} = \normalCone{\feasibleSet}{\varFixed} = \normalConeRegularStrong{\feasibleSet}{\varFixed} = \normalConeStrong{\feasibleSet}{\varFixed} = \{\localZero{\varFixed}\}$.


==> elements/prop_normal_cones_constraints_simple_proof.tex <==
The statement for $\varFixed\in\feasibleSet$ so that
$\objective(\varFixed) < 0$ follows by continuity of $\objective$ and
\cref{proposition:prop_normal_cones_trivial}.
{For the strong cones in the case $\objective(\varFixed)<0$: since
$\objective$ is continuous, $\{\varGeneric\in\Pp{2}{\reals^d}\st\objective(\varGeneric)<0\}$ is open, so every
$\varGeneric\in\feasibleSet$ close to $\varFixed$ lies in the interior of
$\feasibleSet$ and
$\normalConeRegularStrong{\feasibleSet}{\varGeneric}\subseteq\normalConeRegular{\feasibleSet}{\varGeneric}=\{\localZero{\varGeneric}\}$
by \cref{lemma:strong_vs_regular_normal_cone} and
\cref{proposition:prop_normal_cones_trivial}\ref{item:normal_cone:interior_point};
hence the witnesses in \cref{definition:def_fuzzy_normal_cone} satisfy
$\varTangent_n=\localZero{\varGeneric_n}\convergenceWasserstein\localZero{\varFixed}$,
and $\normalConeStrong{\feasibleSet}{\varFixed}=\{\localZero{\varFixed}\}$
as well.}
Thus, we focus on the case $\objective(\varFixed) = 0$.

We start by proving the statement for the regular normal cone. If $\subgradientRegular{\objective}(\varFixed) = \emptyset$, the statement trivially holds so we suppose $\subgradientRegular{\objective}(\varFixed) \neq \emptyset$. Fix $\varTangent \in \subgradientRegular{\objective}(\varFixed)$ and $\lambda \geq 0$. If $\lambda = 0$, the statement holds in virtue of \cref{proposition:prop_normal_tangent_cones}; i.e., $\localZero{\varFixed} \in \normalConeRegular{\feasibleSet}{\varFixed}$. Thus, suppose $\lambda > 0$. We have that
\begin{align*}
    \limsup_{\substack{
    {\varGeneric \in\feasibleSet, \varGeneric \convergenceWasserstein \varFixed}
    \\
    \varPlanGeneric \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}
    }}
    \frac{\innerProduct{\lambda\varTangent}{\varPlanGeneric}_{\varFixed}}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
    =
    \limsup_{\substack{
    {\varGeneric \in\feasibleSet, \varGeneric \convergenceWasserstein \varFixed}
    \\
    \varPlanGeneric \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}
    }}
    \frac{\lambda\innerProduct{\varTangent}{\varPlanGeneric}_{\varFixed}}{\wassersteinDistance{\varFixed}{\varGeneric}{2}},
\end{align*}
which is upper bounded by
\begin{equation*}
    \limsup_{\substack{
    {\varGeneric \in\feasibleSet, \varGeneric \convergenceWasserstein \varFixed}
    \\
    \varPlanGeneric \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}
    }}\hspace{-.5cm}
    \frac{\lambda\left(\innerProduct{\varTangent}{\varPlanGeneric}_{\varFixed} - \objective(\varGeneric) + \objective(\varFixed)\right)}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
    \leq
    \limsup_{\substack{
    {\varGeneric \convergenceWasserstein \varFixed}
    \\
    \varPlanGeneric \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}
    }}\hspace{-.5cm}
    \frac{\lambda\left(\innerProduct{\varTangent}{\varPlanGeneric}_{\varFixed} - \objective(\varGeneric) + \objective(\varFixed)\right)}{\wassersteinDistance{\varFixed}{\varGeneric}{2}}
\end{equation*}
and, thus, is nonpositive.
 This concludes that $\lambda \varTangent \in \normalConeRegular{\feasibleSet}{\varFixed}$.
{The same argument establishes the strong statement. For
$\lambda=0$,
$\localZero{\varFixed}\in\normalConeRegularStrong{\feasibleSet}{\varFixed}$,
since
$\innerProduct{\localZero{\varFixed}}{\varPlanGeneric}_{\varFixed}=0$ for
every variation $\varPlanGeneric$ (cf.
\cref{proposition:prop_wasserstein_geom}\ref{item:negate_zero_is_zero}) and
$\localZero{\varFixed}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$. For
$\lambda>0$ and $\varTangent\in\subgradientRegularStrong{\objective}(\varFixed)$,
it suffices to repeat the display above with
$\setPlans{\varFixed}{\varGeneric}$ in place of
$\setPlansOptimal{\varFixed}{\varGeneric}$ and
$\norm{\varPlanGeneric}_{\varFixed}$ in place of
$\wassersteinDistance{\varFixed}{\varGeneric}{2}$, using the defining
inequality of
\cref{definition:def_strong_sub_sup_differentiability}\ref{item:strong_subgradient:regular}
in the last step; this yields
$\lambda\varTangent\in\normalConeRegularStrong{\feasibleSet}{\varFixed}$ by
\cref{definition:def_fuzzy_normal_cone}.}

{For the second inclusion, we observe that the set
$\feasibleSet$ can equivalently be expressed as
$\feasibleSet=\pushforward{(\projection{1}{},\ldots,\projection{d}{})}{(\epigraph{\objective}\cap D)}$,
with
$
D
\coloneqq
\left\{
\boldsymbol{\varGeneric} \in \Pp{2}{\reals^{d+1}}
\st
\expectedValue{\boldsymbol{x} \sim \boldsymbol{\varGeneric}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{x}}}
\leq
\objective(\varFixed)
\right\}
$;
i.e., $D$ collects the probability measures whose last coordinate has
expected value at most $\objective(\varFixed)$, a sublevel set of the
linear functional $l$ of \cref{section:variational-geometry:epigraphs}.
Write $E\coloneqq\epigraph{\objective}\cap D$ and recall that $T$, as in
\eqref{equation:extraction-map-epigraph}, drops the last component of
positions and velocities. Since the elements of $\epigraph{\objective}$
have deterministic last coordinate, we have
$E=\left\{\varGeneric'\times\delta_{\beta'}\in\Pp{2}{\reals^{d+1}}\st\objective(\varGeneric')\leq\beta'\leq\objective(\varFixed)\right\}$.
In particular, $\varGeneric'\in\feasibleSet$ for every
$\varGeneric'\times\delta_{\beta'}\in E$, and
$\varGeneric\times\delta_{\objective(\varFixed)}\in E$ for every
$\varGeneric\in\feasibleSet$, which together yield the expression for
$\feasibleSet$ above. We collect three auxiliary facts.}

{\emph{Fact 1 (normals of $\feasibleSet$ lift to normals of
$E$).} Let $\varGeneric\in\feasibleSet$ and
$\varTangent\in\normalConeRegularStrong{\feasibleSet}{\varGeneric}$. Then,
$\boldsymbol{\varTangent}\coloneqq\pushforward{(\projection{1}{},\objective(\varFixed),\projection{2}{},0)}{\varTangent}$,
i.e., the lift of $\varTangent$ with vanishing last velocity component,
belongs to
$\normalConeRegularStrong{E}{\varGeneric\times\delta_{\objective(\varFixed)}}$.
To see this, fix $\varGeneric'\times\delta_{\beta'}\in E$ and
$\boldsymbol{\varTangentOther}\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varGeneric\times\delta_{\objective(\varFixed)}}{\varGeneric'\times\delta_{\beta'}}}$.
Since the last coordinates of both endpoints are deterministic, the last
velocity component of $\boldsymbol{\varTangentOther}$ is almost everywhere
constant, equal to $\beta'-\objective(\varFixed)$,
$\varTangentOther\coloneqq\pushforward{T}{\boldsymbol{\varTangentOther}}\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlans{\varGeneric}{\varGeneric'}}$
with $\varGeneric'\in\feasibleSet$, and
$\norm{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_{\objective(\varFixed)}}^2=\norm{\varTangentOther}_{\varGeneric}^2+\abs{\beta'-\objective(\varFixed)}^2\geq\norm{\varTangentOther}_{\varGeneric}^2$
(cf.
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport}
and \ref{item:deterministic_coordinate:splitting}).
By \eqref{eq:deterministic_coordinate:splitting} (cf.
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting}),
applicable since the last velocity component of
$\boldsymbol{\varTangentOther}$ is almost everywhere constant, and since the
last velocity component of $\boldsymbol{\varTangent}$ vanishes almost
surely (so that, in particular, its expectation is zero),
\begin{align*}
\innerProduct{\boldsymbol{\varTangent}}{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_{\objective(\varFixed)}}
&=
\innerProduct{\varTangent}{\varTangentOther}_{\varGeneric}
+
(\beta'-\objective(\varFixed))
\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}
\\
&=
\innerProduct{\varTangent}{\varTangentOther}_{\varGeneric}
\leq
\onotation{\norm{\varTangentOther}_{\varGeneric}}
\leq
\onotation{\norm{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_{\objective(\varFixed)}}},
\end{align*}
where the first inequality is the defining property of
$\varTangent\in\normalConeRegularStrong{\feasibleSet}{\varGeneric}$ in
\cref{definition:def_fuzzy_normal_cone} (applicable since
$\varGeneric'\in\feasibleSet$), and the second holds because
$\norm{\varTangentOther}_{\varGeneric}\leq\norm{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_{\objective(\varFixed)}}$. Moreover, $\boldsymbol{\varTangent}$
is a variation at $\varGeneric\times\delta_{\objective(\varFixed)}$ with
$\pushforward{T}{\boldsymbol{\varTangent}}=\varTangent\in\tangentCone{\Pp{2}{\reals^d}}{\varGeneric}$,
so
$\boldsymbol{\varTangent}\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varGeneric\times\delta_{\objective(\varFixed)}}$
by \cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}.
Hence,
$\boldsymbol{\varTangent}\in\normalConeRegularStrong{E}{\varGeneric\times\delta_{\objective(\varFixed)}}$.
Consequently, if $\varTangent\in\normalConeStrong{\feasibleSet}{\varFixed}$,
witnessed by $\varGeneric_n\convergenceWasserstein\varFixed$ in
$\feasibleSet$ and
$\varTangent_n\in\normalConeRegularStrong{\feasibleSet}{\varGeneric_n}$ with
$\varTangent_n\convergenceWasserstein\varTangent$, then the lifts
$\boldsymbol{\varTangent}_n\coloneqq\pushforward{(\projection{1}{},\objective(\varFixed),\projection{2}{},0)}{\varTangent_n}$
are strong regular normals of $E$ at
$\varGeneric_n\times\delta_{\objective(\varFixed)}\convergenceWasserstein\varFixed\times\delta_{\objective(\varFixed)}$,
and appending the deterministic coordinates to near-optimal transport plans
between $\varTangent_n$ and $\varTangent$ shows
$\boldsymbol{\varTangent}_n\convergenceWasserstein\boldsymbol{\varTangent}$;
thus, the lift
$\boldsymbol{\varTangent}=\pushforward{(\projection{1}{},\objective(\varFixed),\projection{2}{},0)}{\varTangent}$
of $\varTangent$ belongs to
$\normalConeStrong{E}{\varFixed\times\delta_{\objective(\varFixed)}}$.}

{\emph{Fact 2 (variational geometry of $D$).} The set $D$ is
the sublevel set, at level $\objective(\varFixed)\in\reals$, of the linear
functional on $\Pp{2}{\reals^{d+1}}$ induced by
$c=(0,\ldots,0,1)\in\reals^{d+1}\setminus\{0\}$. Thus,
\cref{lemma:normal_cone_linear_constraint} (applied in
$\Pp{2}{\reals^{d+1}}$) shows that $D$ is closed and \gls*{acr:snc} at
every point and, since
$l(\varFixed\times\delta_{\objective(\varFixed)})=\objective(\varFixed)$
(i.e., $\varFixed\times\delta_{\objective(\varFixed)}$ lies at the
boundary of $D$),
\begin{equation*}
\normalConeStrong{D}{\varFixed\times\delta_{\objective(\varFixed)}}
=
\normalConeRegularStrong{D}{\varFixed\times\delta_{\objective(\varFixed)}}
=
\left\{
(\varFixed\times\delta_{\objective(\varFixed)})\times\delta_{(0,\ldots,0,\lambda)}
\st
\lambda\geq 0
\right\}.
\end{equation*}
In particular, every
$\boldsymbol{\varTangent}_2\in\normalConeStrong{D}{\varFixed\times\delta_{\objective(\varFixed)}}$
satisfies
$\pushforward{T}{\boldsymbol{\varTangent}_2}=\localZero{\varFixed}$.}

{\emph{Fact 3 (intersection rule for the pair
$(\epigraph{\objective},D)$).} If
$\localZero{\varFixed}\notin\subgradient{\objective}(\varFixed)$, then
$\normalConeStrong{E}{\varFixed\times\delta_{\objective(\varFixed)}}
\subseteq
\normalConeStrong{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}
+
\normalConeStrong{D}{\varFixed\times\delta_{\objective(\varFixed)}}$;
i.e., for every
$\boldsymbol{\varTangent}\in\normalConeStrong{E}{\varFixed\times\delta_{\objective(\varFixed)}}$
there are
$\boldsymbol{\varTangent}_1\in\normalConeStrong{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$,
$\boldsymbol{\varTangent}_2\in\normalConeStrong{D}{\varFixed\times\delta_{\objective(\varFixed)}}$,
and
$\boldsymbol{\varTangentCoupling}\in\setPlansCommonMarginal{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_2}{1}$
with
$\boldsymbol{\varTangent}=\boldsymbol{\varTangent}_1\localSum{\boldsymbol{\varTangentCoupling}}\boldsymbol{\varTangent}_2$.
This is \cref{theorem:intersection_rule_strong} applied to
$\Omega_1=\epigraph{\objective}$ and $\Omega_2=D$ at
$\varFixed\times\delta_{\objective(\varFixed)}\in\Omega_1\cap\Omega_2$,
whose assumptions we now verify. First, both sets are closed, hence
locally closed around $\varFixed\times\delta_{\objective(\varFixed)}$:
the set $D$ by Fact 2, and $\epigraph{\objective}$ since $\objective$ is
continuous, the maps
$\boldsymbol{\varGeneric}\mapsto\pushforward{(\projection{1}{},\ldots,\projection{d}{})}{\boldsymbol{\varGeneric}}$
and
$\boldsymbol{\varGeneric}\mapsto\pushforward{\projection{d+1}{}}{\boldsymbol{\varGeneric}}$
are $1$-Lipschitz with respect to $\wassersteinDistance{}{}{2}$, and a
Wasserstein limit of Dirac deltas is a Dirac delta.
Second, $D$ is \gls*{acr:snc} at
$\varFixed\times\delta_{\objective(\varFixed)}$ by Fact 2, so
assumption (ii) of \cref{theorem:intersection_rule_strong} holds.
Third, for assumption (i), let
$\boldsymbol{\varTangent}\in\normalConeStrong{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}\cap\left(-\normalConeStrong{D}{\varFixed\times\delta_{\objective(\varFixed)}}\right)$.
By Fact 2,
$\boldsymbol{\varTangent}=(\varFixed\times\delta_{\objective(\varFixed)})\times\delta_{(0,\ldots,0,-\lambda)}$
for some $\lambda\geq 0$; in particular,
$\pushforward{\projection{1}{}}{\boldsymbol{\varTangent}}=\varFixed\times\delta_{\objective(\varFixed)}$,
the last velocity component of $\boldsymbol{\varTangent}$ has expectation
$-\lambda$, and
$\pushforward{T}{\boldsymbol{\varTangent}}=\localZero{\varFixed}$.
Suppose, for the sake of contradiction, that $\lambda>0$. Since
$\boldsymbol{\varTangent}\in\normalConeStrong{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}\subseteq\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$
by \cref{lemma:strong_vs_regular_normal_cone},
\cref{proposition:th_subgradients_epigraphical_normals} applies (recall
$\objective(\varFixed)=0\in\reals$) and, the expectation of the last
velocity component being $-\lambda<0$, it yields
$\localZero{\varFixed}=\frac{1}{\lambda}\pushforward{T}{\boldsymbol{\varTangent}}\in\subgradient{\objective}(\varFixed)$,
contradicting
$\localZero{\varFixed}\notin\subgradient{\objective}(\varFixed)$. Thus,
$\lambda=0$ and
$\boldsymbol{\varTangent}=\localZero{\varFixed\times\delta_{\objective(\varFixed)}}$,
so that assumption (i) of \cref{theorem:intersection_rule_strong} holds as
well.}

{%
We are now ready to prove the desired inclusion. Let
$\varTangent\in\normalConeStrong{\feasibleSet}{\varFixed}$ and let
$\boldsymbol{\varTangent}\coloneqq\pushforward{(\projection{1}{},\objective(\varFixed),\projection{2}{},0)}{\varTangent}$
be its lift with vanishing last velocity component, so that
$\boldsymbol{\varTangent}\in\normalConeStrong{E}{\varFixed\times\delta_{\objective(\varFixed)}}$
and $\pushforward{T}{\boldsymbol{\varTangent}}=\varTangent$ by Fact 1. By
Fact 3, there are
$\boldsymbol{\varTangent}_1\in\normalConeStrong{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$,
$\boldsymbol{\varTangent}_2\in\normalConeStrong{D}{\varFixed\times\delta_{\objective(\varFixed)}}$,
and
$\boldsymbol{\varTangentCoupling}\in\setPlansCommonMarginal{\boldsymbol{\varTangent}_1}{\boldsymbol{\varTangent}_2}{1}$
with
$\boldsymbol{\varTangent}=\boldsymbol{\varTangent}_1\localSum{\boldsymbol{\varTangentCoupling}}\boldsymbol{\varTangent}_2$.
Pushing this identity forward by $T$ (the computation with test functions in
the proof of \cref{theorem:th_first_order_optimality_conditions} below applies
verbatim, with $\hat{T}$ as defined there) yields
$\varTangent=\pushforward{T}{\boldsymbol{\varTangent}}=\pushforward{T}{\boldsymbol{\varTangent}_1}\localSum{\pushforward{\hat{T}}{\boldsymbol{\varTangentCoupling}}}\pushforward{T}{\boldsymbol{\varTangent}_2}$.
By Fact 2, $\pushforward{T}{\boldsymbol{\varTangent}_2}=\localZero{\varFixed}$,
so $\varTangent=\pushforward{T}{\boldsymbol{\varTangent}_1}$ by
\cref{proposition:prop_wasserstein_geom}\ref{item:wass_geom:sum:zero}. By
\cref{lemma:strong_vs_regular_normal_cone},
$\boldsymbol{\varTangent}_1\in\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$,
so \cref{proposition:th_subgradients_epigraphical_normals} applies (recall
$\objective(\varFixed)=0\in\reals$): either the last velocity component of
$\boldsymbol{\varTangent}_1$ has expectation $-\lambda$ with $\lambda>0$ and
$\frac{1}{\lambda}\varTangent=\frac{1}{\lambda}\pushforward{T}{\boldsymbol{\varTangent}_1}\in\subgradient{\objective}(\varFixed)$,
so that
$\varTangent\in\left\{\lambda\varTangent'\st\lambda\geq0,\varTangent'\in\subgradient{\objective}(\varFixed)\right\}$,
or it has zero expectation and
$\varTangent=\pushforward{T}{\boldsymbol{\varTangent}_1}\in\subgradientHzn{\objective}(\varFixed)$.
In both cases,
$\varTangent\in\left\{\lambda\varTangent'\st\lambda\geq0,\varTangent'\in\subgradient{\objective}(\varFixed)\right\}\cup\subgradientHzn{\objective}(\varFixed)$,
which establishes the second inclusion.}


==> elements/prop_normal_cones_constraints_simple_title.tex <==
Level sets%

==> elements/prop_normal_cones_trivial_body.tex <==
Let $\feasibleSet \subseteq \Pp{2}{\reals^d}$ and $\varFixed \in \feasibleSet$. Then,
\begin{enumerate}[leftmargin=*]
\item
\uniqueLabel{item:normal_cone:no_constraints}
if $\feasibleSet = \Pp{2}{\reals^d}$, then
$
    \normalConeRegular{\feasibleSet}{\varFixed} = \normalCone{\feasibleSet}{\varFixed} = \normalCone{\Pp{2}{\reals^d}}{\varFixed} = \{\localZero{\varFixed}\}
$;
\item
\uniqueLabel{item:normal_cone:interior_point}
if $\varFixed$ is in the interior (with respect to the Wasserstein distance) of $\feasibleSet$, i.e., $\varFixed\in \interior{\feasibleSet}{\wassersteinDistance{}{}{2}}$, then
$
    \normalConeRegular{\feasibleSet}{\varFixed} = \normalCone{\feasibleSet}{\varFixed} = \{\localZero{\varFixed}\}
$;
\item
\uniqueLabel{item:normal_cone:delta}
for $\Xi \subseteq \reals^d$, if $\feasibleSet = \{\delta_x \in \Pp{2}{\reals^d} \st x \in \Xi\}$, then at any $\varFixed=\delta_{\bar x} \in \feasibleSet$ we have
    $\normalConeRegular{\feasibleSet}{\varFixed}
    =
    \{\delta_{\bar x} \times \nu \st \expectedValue{x\sim\nu}{x} \in \normalConeRegular{\Xi}{\bar x}\}$ and
    $\normalCone{\feasibleSet}{\varFixed}=\{\delta_{\bar x} \times \nu \st \expectedValue{x\sim\nu}{x} \in \normalCone{\Xi}{\bar x}\}$,
where $\normalConeRegular{\Xi}{\bar x}$ and $\normalCone{\Xi}{\bar x}$ are the regular and general normal cones in the Euclidean space, respectively.
\end{enumerate}


==> elements/prop_normal_cones_trivial_proof.tex <==
We prove the statements separately.
\begin{enumerate}
\item
It suffices to show that for any generic $\varFixed\in\Pp{2}{\reals^d}$, $\normalConeRegular{\Pp{2}{\reals^d}}{\varFixed}=\{\localZero{\varFixed}\}$, since the limit is then trivially the same.
As already observed in the proof of~\cref{proposition:prop_normal_tangent_cones}, $\localZero{\varFixed} \in \normalConeRegular{\Pp{2}{\reals^d}}{\varFixed}$.
Thus, $\normalConeRegular{\Pp{2}{\reals^d}}{\varFixed}\supseteq\{\localZero{\varFixed}\}$.
For the other inclusion, let $\varTangentFixed \in \normalConeRegular{\Pp{2}{\reals^d}}{\varFixed}$. By definition of regular normal cone, $\varTangentFixed\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$.
{Indeed, every element of the tangent space belongs to the tangent
cone of $\Pp{2}{\reals^d}$ at $\varFixed$: pick $\varTangentFixed^k$ in the set of
\eqref{definition:tangent_space} with
$\wassersteinDistance{\varTangentFixed^k}{\varTangentFixed}{\varFixed}\to 0$ and
$\tau_k \fromAbove 0$ below the corresponding $\bar\varepsilon$, and set
$\varGeneric_k \coloneqq \pushforward{(\projection{1}{} +
\tau_k\projection{2}{})}{\varTangentFixed^k}$; then $\tau_k\varTangentFixed^k \in
\pushforward{(\projection{1}{}, \projection{2}{} -
\projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric_k}}$,
$\wassersteinDistance{\varGeneric_k}{\varFixed}{2} \leq
\tau_k\norm{\varTangentFixed^k}_{\varFixed} \to 0$, and
$\wassersteinDistance{\tfrac{1}{\tau_k}(\tau_k\varTangentFixed^k)}{\varTangentFixed}{\varFixed}
\to 0$, as required by \cref{definition:def_tangent_cone}.}
By~\cref{proposition:prop_normal_tangent_cones}, $\innerProduct{\varTangentFixed}{\varTangentFixed}_{\varFixed}\leq 0$. Thus, with~\cref{proposition:prop_wasserstein_geom}\ref{item:wass_geom:cauchy_schwarz}-\ref{item:zero_iff_zero}, $\norm{\varTangentFixed}_{\varFixed}^2\leq 0$ and $\varTangentFixed\localEquiv{\varFixed}\localZero{\varFixed}$. This proves $\normalConeRegular{\Pp{2}{\reals^d}}{\varFixed}\subseteq\{\localZero{\varFixed}\}$, which concludes the proof.

\item
{
As $\localZero{\varFixed} \in \normalConeRegular{\feasibleSet}{\varFixed}$ (again by the proof of~\cref{proposition:prop_normal_tangent_cones}), it suffices to prove $\normalConeRegular{\feasibleSet}{\varFixed}\subseteq\{\localZero{\varFixed}\}$.
Let $\varTangentFixed \in \normalConeRegular{\feasibleSet}{\varFixed}$.
{Pick $\varTangentFixed^k$ in the set of
\eqref{definition:tangent_space} with
$\wassersteinDistance{\varTangentFixed^k}{\varTangentFixed}{\varFixed}\to0$ and
$\tau_k \fromAbove 0$ below the corresponding $\bar\varepsilon$; then
$\varGeneric_k \coloneqq
\pushforward{(\projection{1}{}+\tau_k\projection{2}{})}{\varTangentFixed^k}$
satisfies
$\wassersteinDistance{\varGeneric_k}{\varFixed}{2}\leq\tau_k\norm{\varTangentFixed^k}_{\varFixed}\to0$,
so $\varGeneric_k\in\feasibleSet$ for $k$ large because $\varFixed\in
\interior{\feasibleSet}{\wassersteinDistance{}{}{2}}$; since moreover
$\tau_k\varTangentFixed^k\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric_k}}$
and
$\wassersteinDistance{\tfrac{1}{\tau_k}(\tau_k\varTangentFixed^k)}{\varTangentFixed}{\varFixed}\to0$,
\cref{definition:def_tangent_cone} gives
$\varTangentFixed\in\tangentCone{\feasibleSet}{\varFixed}$.}
Then, the statement follows analogously to \ref{item:normal_cone:no_constraints}.
{For $\normalCone{\feasibleSet}{\varFixed}$, note that any
$\varGeneric_n\in\feasibleSet$ with
$\varGeneric_n\convergenceWasserstein\varFixed$ eventually lies in
$\interior{\feasibleSet}{\wassersteinDistance{}{}{2}}$, so
$\normalConeRegular{\feasibleSet}{\varGeneric_n}=\{\localZero{\varGeneric_n}\}$
for $n$ large and the only possible limit is $\localZero{\varFixed}$.}}

\item
We have that $\varTangentFixed \in \normalConeRegular{\feasibleSet}{\varFixed}$ if and only if $\varTangentFixed\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ and for all $\varGeneric_n = \delta_{x_n} \in \feasibleSet$, $\varGeneric_n \convergenceWasserstein \varFixed = \delta_{\bar{x}}$, $\varTangent_n \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric_n}} = \{\delta_{\bar{x}}\times\delta_{(x_n - \bar{x})}\}$ we have $\innerProduct{\varTangentFixed}{\varTangent_n}_{\varFixed}\leq\onotation{\norm{\varTangent_n}_{\varFixed}}$.
{The
requirement $\varTangentFixed \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$ is automatically satisfied: since
$\setPlans{\delta_{\bar x}}{\varGeneric}$ is a singleton, hence its element is
optimal, for every $\varGeneric$, any $\varTangentFixed$ with
$\pushforward{\projection{1}{}}{\varTangentFixed} = \delta_{\bar x}$ belongs to
\eqref{definition:tangent_space}.
We now check the regular normal cone inequality (cf. \cref{definition:def_normal_cone}):}
\begin{align*}
    0 \geq
    \limsup_{n \to\infty}
    \frac{\innerProduct{\varTangentFixed}{\varTangent_n}_{\varFixed}}{\norm{\varTangent_n}_{\varFixed}}
    &=
    \limsup_{n \to\infty}
    \frac{1}{\norm{x_n-\bar x}}\max_{\varTangentCoupling \in \setPlansCommonMarginal{\varTangentFixed}{\varTangent_n}{1}}
    \\
    &\hphantom{{}={}}
    \int_{\reals^d\times\reals^d\times\reals^d}
    \innerProduct{\varTangentReals}{\varTangentReals_n}\d\varTangentCoupling(\bar x, \varTangentReals, \varTangentReals_n)
    \\
    &=
    \limsup_{n \to\infty}
    \frac{1}{\norm{x_n-\bar x}}
    \\
    &\hphantom{{}={}}
    \int_{\reals^d\times\reals^d}
    \innerProduct{\varTangentReals}{x_n - \bar x}\d\varTangentFixed(\bar x, \varTangentReals).
\end{align*}
{We restrict attention to sequences with $x_n \neq \bar x$;
for $x_n = \bar x$ the defining inequality holds trivially, since
$\varTangent_n \localEquiv{\varFixed} \localZero{\varFixed}$.}
Since by \cref{definition:def_normal_cone} it also holds $\pushforward{\projection{1}{}}{\varTangentFixed} = \delta_{\bar x}$ and thus $\varTangentFixed = \delta_{\bar x} \times \varTangent$ for some $\varTangent \in \Pp{2}{\reals^d}$, the condition reads
    $0 \geq \limsup_{n \to\infty}
    \frac{1}{\norm{x_n-\bar x}}
    \int_{\reals^d}
    \innerProduct{\varTangentReals}{x_n - \bar{x}}\d\varTangent(\varTangentReals)
    =
    \limsup_{n \to\infty}
    \frac{\innerProduct{\expectedValue{\varTangentReals\sim\varTangent}{\varTangentReals}}{x_n - \bar{x}}}{\norm{x_n-\bar x}}$,
which is true if and only if ${\expectedValue{\varTangentReals\sim\varTangent}{\varTangentReals}} \in \normalConeRegular{\Xi}{\bar x}$ (cf. \cite[Definition 6.3]{rockafellar2009variational}).
The statement for the general normal cone follows taking the limit and by continuity of the inner product in $\reals^d$ and of the expected value in Wasserstein.
{Conversely, if
$v \coloneqq \expectedValue{x\sim\nu}{x} \in \normalCone{\Xi}{\bar x}$, take
$x_n \to \bar x$ in $\Xi$ and $v_n \in \normalConeRegular{\Xi}{x_n}$ with $v_n
\to v$, and set $\nu_n \coloneqq \pushforward{(\identity{} + v_n - v)}{\nu}$;
then $\expectedValue{x\sim\nu_n}{x} = v_n$, so $\delta_{x_n}\times\nu_n \in
\normalConeRegular{\feasibleSet}{\delta_{x_n}}$ by the first part, and
$\delta_{x_n}\times\nu_n \convergenceWasserstein \delta_{\bar x}\times\nu$ since
$\wassersteinDistance{\delta_{x_n}\times\nu_n}{\delta_{\bar x}\times\nu}{2}^2
\leq \norm{x_n - \bar x}^2 + \norm{v_n - v}^2$, whence $\delta_{\bar x}\times\nu
\in \normalCone{\feasibleSet}{\varFixed}$.}
\end{enumerate}


==> elements/prop_normal_cones_trivial_title.tex <==
Trivial normal cones%

==> elements/prop_normal_tangent_cones_body.tex <==
At any $\varFixed \in \feasibleSet \subseteq \Pp{2}{\reals^d}$, the sets $\normalConeRegular{\feasibleSet}{\varFixed}$ and $\normalCone{\feasibleSet}{\varFixed}$ are nonempty closed cones{, with respect
to $\wassersteinDistance{}{}{\varFixed}$ and in Wasserstein, respectively}. Additionally, if
$
\varTangentFixed \in \normalConeRegular{\feasibleSet}{\varFixed}
$
then
$
\innerProduct{\varTangentFixed}{\varTangent}_{\varFixed} \leq 0
$
for all
$
\varTangent \in \tangentCone{\feasibleSet}{\varFixed}.
$


==> elements/prop_normal_tangent_cones_proof.tex <==
First, we notice that $\localZero{\varFixed} \in \normalConeRegular{\feasibleSet}{\varFixed}, \normalCone{\feasibleSet}{\varFixed}$: For all $\varTangentOther \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$
\begin{align*}
\innerProduct{\localZero{\varFixed}}{\varTangentOther}_{\varFixed}
&=
\max_{\varTangentCoupling \in \setPlansCommonMarginal{\localZero{\varFixed}}{\varTangentOther}{1}}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{\varTangentReals_1}{\varTangentReals_2}\d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
\\&=
\max_{\varTangentCoupling \in \setPlansCommonMarginal{\localZero{\varFixed}}{\varTangentOther}{1}}
\int_{\reals^d\times\reals^d\times\reals^d}
\innerProduct{0}{\varTangentReals_2}\d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
=
0
\leq
\onotation{\norm{\varTangentOther}_{\varFixed}}.
\end{align*}
In particular, $\normalConeRegular{\feasibleSet}{\varFixed}, \normalCone{\feasibleSet}{\varFixed}$ are nonempty.
By \cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:homogeneity} and \cref{proposition:prop_sum_scale_well_defined}, which guarantees $\lambda\varTangent \in \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$, we conclude that $\varTangent \in \normalConeRegular{\feasibleSet}{\varFixed}$ implies $\lambda\varTangent \in \normalConeRegular{\feasibleSet}{\varFixed}$ for all $\lambda \geq 0$, i.e., $\normalConeRegular{\feasibleSet}{\varFixed}$ is a cone.
The following approximation argument proves the analogous result for $\normalCone{\feasibleSet}{\varFixed}$. Given any sequences $(\varGeneric_n)_{n \in \naturals} \subseteq \feasibleSet$, $\varGeneric_n \to \varFixed$, $(\varTangent_n)_{n \in \naturals} \subseteq \Pp{2}{\reals^d}$ so that $\varTangent_n \in \normalConeRegular{\feasibleSet}{\varGeneric_n}$ and $\varTangent_n \convergenceWasserstein \varTangent$, we have, for all $\phi \in \C{0}{\reals^d\times\reals^d}{\reals}$ with at most quadratic growth,
    $\lim_{n \to \infty}
    \int_{\reals^d\times\reals^d}\phi(x, y)\d(\lambda\varTangent_n)(x, y)
    =
    \lim_{n \to \infty}
    \int_{\reals^d\times\reals^d}\phi(x, \lambda y)\d\varTangent_n(x, y)
    =
    \int_{\reals^d\times\reals^d}\phi(x, \lambda y)\d\varTangent(x, y)
    =
    \int_{\reals^d\times\reals^d}\phi(x, y)\d(\lambda\varTangent)(x, y)$.
%
Thus, $\lambda\varTangent_n \convergenceWasserstein \lambda\varTangent$~\cite[Definition 6.8]{villani2009optimal} and so $\lambda \varTangent \in \normalCone{\feasibleSet}{\varFixed}$.
{
To prove that $\normalConeRegular{\feasibleSet}{\varFixed}$ is closed, let $\varTangent_n \in \normalConeRegular{\feasibleSet}{\varFixed}$ with $\wassersteinDistance{\varTangent_n}{\varTangent}{\varFixed}\to 0$. Since $\tangentCone{\Pp{2}{\reals^{d}}}{\varFixed}$ is closed by definition with respect to $\wassersteinDistance{}{}{\varFixed}$, $\varTangent \in \tangentCone{\Pp{2}{\reals^{d}}}{\varFixed}$. We show that $\varTangent \in \normalConeRegular{\feasibleSet}{\varFixed}$.
Let $(\varGeneric_m)_{m\in\naturals}\subseteq \feasibleSet$ with $\varGeneric_m\convergenceWasserstein \varFixed$ and
$\varTangentOther_m \in
\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{
\setPlansOptimal{\varFixed}{\varGeneric_m}
}$. Since $\varTangent_n\in \normalConeRegular{\feasibleSet}{\varFixed}$, for every fixed $n$ we have
$\limsup_{m\to\infty}
\frac{\innerProduct{\varTangent_n}{\varTangentOther_m}_{\varFixed}}
{\norm{\varTangentOther_m}_{\varFixed}}
\le 0.$
Let $\varTangentCoupling_n \in \setPlansCommonMarginal{\varTangent}{\varTangent_n}{1}$ attain $\wassersteinDistance{\varTangent}{\varTangent_n}{\varFixed}$ and define $\varTangentCoupling_n' \coloneqq \pushforward{(\projection{1}{},\projection{2}{},-\projection{3}{})}{\varTangentCoupling_n}$, $\varTangentCoupling_n''
\coloneqq
\pushforward{(\projection{1}{},\projection{3}{},\projection{2}{}-\projection{3}{})}{\varTangentCoupling_n}$.
Then, $\varTangentCoupling_n'' \in \setPlansCommonMarginal{\varTangent_n}{\varTangent \localSum{\varTangentCoupling_n'} (-\varTangent_n)}{1}$ and
$
\varTangent_n \localSum{\varTangentCoupling_n''}
\bigl(\varTangent \localSum{\varTangentCoupling_n'}(-\varTangent_n)\bigr)
=
\pushforward{(\projection{1}{},\projection{2}{}+\projection{3}{})}{\varTangentCoupling_n''}
=
\pushforward{(\projection{1}{},\projection{3}{}+(\projection{2}{}-\projection{3}{}))}{\varTangentCoupling_n}
=\pushforward{(\projection{1}{},\projection{2}{})}{\varTangentCoupling_n}
=
\varTangent.
$
Thus, by \cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:sublinear} and \ref{item:wass_geom:cauchy_schwarz},
\begin{align*}
\frac{\innerProduct{\varTangent}{\varTangentOther_m}_{\varFixed}}
{\norm{\varTangentOther_m}_{\varFixed}}
&=
{\frac{\innerProduct{\varTangent_n \localSum{\varTangentCoupling_n''}
(\varTangent \localSum{\varTangentCoupling_n'}
(-\varTangent_n))}{\varTangentOther_m}_{\varFixed}}
{\norm{\varTangentOther_m}_{\varFixed}}}
\\&\leq
\frac{\innerProduct{\varTangent_n}{\varTangentOther_m}_{\varFixed}}
{\norm{\varTangentOther_m}_{\varFixed}}
+
\frac{\innerProduct{\varTangent \localSum{\varTangentCoupling_n'} (-\varTangent_n)}{\varTangentOther_m}_{\varFixed}}
{\norm{\varTangentOther_m}_{\varFixed}}
\\&\le
\frac{\innerProduct{\varTangent_n}{\varTangentOther_m}_{\varFixed}}
{\norm{\varTangentOther_m}_{\varFixed}}
+
\norm{\varTangent \localSum{\varTangentCoupling_n'} (-\varTangent_n)}_{\varFixed}.
\end{align*}
Taking the limit superior as $m\to\infty$ yields
$
\limsup_{m\to\infty}
\frac{\innerProduct{\varTangent}{\varTangentOther_m}_{\varFixed}}
{\norm{\varTangentOther_m}_{\varFixed}}
\le
\norm{\varTangent \localSum{\varTangentCoupling_n'} (-\varTangent_n)}_{\varFixed} = \wassersteinDistance{\varTangent}{\varTangent_n}{\varFixed}.
$
Finally, letting $n\to\infty$ and using $\wassersteinDistance{\varTangent}{\varTangent_n}{\varFixed}\to 0$, we obtain
$
\limsup_{m\to\infty}
\frac{\innerProduct{\varTangent}{\varTangentOther_m}_{\varFixed}}
{\norm{\varTangentOther_m}_{\varFixed}}
\le 0.
$
Since the sequence $(\varGeneric_m,\varTangentOther_m)$ is arbitrary, this proves
$\varTangent \in \normalConeRegular{\feasibleSet}{\varFixed}$.
Therefore, $\normalConeRegular{\feasibleSet}{\varFixed}$ is closed.}
%
For the general normal cone, we consider a diagonal argument. Consider $\normalCone{\feasibleSet}{\varFixed} \ni \varTangent_n \convergenceWasserstein \varTangent$. Then, there are $\varGeneric_n^m \convergenceWasserstein \varFixed$ and $\normalConeRegular{\feasibleSet}{\varGeneric_n^m} \ni \varTangent_n^m \convergenceWasserstein \varTangent_n$. Then, $\wassersteinDistance{\varTangent_n^m}{\varTangent}{2} \leq \wassersteinDistance{\varTangent_n^m}{\varTangent_n}{2} + \wassersteinDistance{\varTangent_n}{\varTangent}{2}$ hence, for every $n$ we may pick $m(n)$ with $\wassersteinDistance{\varTangent_n^{m(n)}}{\varTangent_n}{2}\leq\frac{1}{n}$ and $\wassersteinDistance{\varGeneric_n^{m(n)}}{\varFixed}{2}\leq\frac{1}{n}$, so that $\varGeneric_n^{m(n)}\convergenceWasserstein\varFixed$, $\varTangent_n^{m(n)}\in\normalConeRegular{\feasibleSet}{\varGeneric_n^{m(n)}}$, and $\varTangent_n^{m(n)}\convergenceWasserstein\varTangent$. Therefore, $\varTangent \in \normalCone{\feasibleSet}{\varFixed}$.

{
Finally, we prove the relationship between $\normalConeRegular{\feasibleSet}{\varFixed}$ and $\tangentCone{\feasibleSet}{\varFixed}$.
Let $\bar\varTangent \in \normalConeRegular{\feasibleSet}{\varFixed}$
and $\varTangent \in \tangentCone{\feasibleSet}{\varFixed}$, as in the statement.
By definition of tangent cone (\cref{definition:def_tangent_cone}), there exist
sequences $(\varGeneric_n)_{n \in \naturals}\subseteq\feasibleSet$ with
$\varGeneric_n \convergenceWasserstein \varFixed$,
$(\varTangent_n)_{n \in \naturals} \subseteq \tangentCone{\Pp{2}{\reals^d}}{\varFixed}$
with $\varTangent_n \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric_n}}$,
and $(\tau_n)_{n \in \naturals} \subseteq \nonnegativeReals$ with $\tau_n \fromAbove 0$,
such that $\wassersteinDistance{\frac{1}{\tau_n}\varTangent_n}{\varTangent}{\varFixed}\to 0$.
%
Fix $\varepsilon > 0$. Since $\bar\varTangent \in \normalConeRegular{\feasibleSet}{\varFixed}$
and $\varGeneric_n \convergenceWasserstein \varFixed$, there exists $N \in \naturals$
such that
$
    \innerProduct{\bar\varTangent}{\varTangent_n}_{\varFixed}
    \leq \varepsilon \norm{\varTangent_n}_{\varFixed}
$
for all $n \geq N$.
Dividing by $\tau_n > 0$ and using \cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:homogeneity},
\begin{equation*}
    \frac{\innerProduct{\bar\varTangent}{\varTangent_n}_{\varFixed}}{\tau_n}
    = \innerProduct{\bar\varTangent}{\tfrac{\varTangent_n}{\tau_n}}_{\varFixed}
    \leq \varepsilon \norm{\tfrac{\varTangent_n}{\tau_n}}_{\varFixed}
    \quad \text{for all } n \geq N.
\end{equation*}
Passing to the limit, using continuity of the inner product
(\cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:continuity_wass}),
and $\norm{\frac{\varTangent_n}{\tau_n}}_{\varFixed} \to \norm{\varTangent}_{\varFixed}$,
\begin{equation*}
    \innerProduct{\bar\varTangent}{\varTangent}_{\varFixed}
    =
    \lim_{n \to \infty} \innerProduct{\bar\varTangent}{\tfrac{\varTangent_n}{\tau_n}}_{\varFixed}
    \leq
    \limsup_{n\to\infty} \varepsilon\norm{\tfrac{\varTangent_n}{\tau_n}}_{\varFixed}
    =
    \varepsilon \norm{\varTangent}_{\varFixed}.
\end{equation*}
Since $\varepsilon > 0$ is arbitrary, $\innerProduct{\bar\varTangent}{\varTangent}_{\varFixed} \leq 0$.}


==> elements/prop_normal_tangent_cones_title.tex <==
Normal and tangent cones relationships%

==> elements/prop_subgradient_convex_body.tex <==
For any proper, lower semicontinuous, $\lambda$-convex functional $V: \reals^d \to \realsBar$ and any point $x \in \reals^d$ such that $V(x) \in \reals$, we have
$\subgradientRegular{V}(x)
=
\left\{
\varTangentReals \in \reals^d
\st
\forall y \in \reals^d,
V(y)
\geq
V(x) + \innerProduct{\varTangentReals}{y - x} + \frac{\lambda}{2}\norm{y - x}^2
\right\}
=
\subgradient{V}(x)$ and
$\subgradientHzn{V}(x)
\subseteq
\left\{
\varTangentReals \in \reals^d
\st
\forall y \in \reals^d, V(y) \in \reals,
0
\geq
\innerProduct{\varTangentReals}{y - x}
\right\}${.
In particular,} if $V(\reals^d) \subseteq \reals$, $\subgradientHzn{V}(x) = \{0\}$.


==> elements/prop_subgradient_convex_proof.tex <==
The characterization for $\subgradientRegular{V}(x)$ follows by definition of $\lambda$-convexity (cf. \cite[Equation 10.4.10]{ambrosio2005gradient}). Then, for any $\varTangentReals \in \subgradient{V}(x)$ consider any sequences $x_n \to x$, $\varTangentReals_n \to \varTangentReals$, $\varTangentReals_n \in \subgradientRegular{V}(x_n)$. Since $V$ is lower semicontinuous, we have $\liminf_{n \to \infty} V(x_n) \geq V(x)$ and, since it is proper and $\varTangentReals_n \in \subgradientRegular{V}(x_n)$, for all $y \in \reals^d$ and for all $n \in \naturals$,
$V(y) \geq V(x_n) + \innerProduct{\varTangentReals_n}{y - x_n} + \frac{\lambda}{2}\norm{y - x_n}^2$, which implies by continuity of the inner product and of the norm that
$V(y) \geq \liminf_{n \to \infty} \left( V(x_n) + \innerProduct{\varTangentReals_n}{y - x_n} + \frac{\lambda}{2}\norm{y - x_n}^2 \right)
\geq V(x) + \innerProduct{\varTangentReals}{y - x} + \frac{\lambda}{2}\norm{y - x}^2$.
In particular, $\subgradient{V}(x) \subseteq \subgradientRegular{V}(x)$ and, since the other inclusion is immediate, $\subgradient{V}(x) = \subgradientRegular{V}(x)$.
Let now $\varTangentReals \in \subgradientHzn{V}(x)$ and consider the corresponding sequences $\tau_n \fromAbove 0$, $x_n \to x$, $V(x_n) \to V(x)$ and $\tau_n \varTangentReals_n \to \varTangentReals$, $\varTangentReals_n \in \subgradientRegular{V}(x_n)$. For all $y \in \reals^d$, $\varTangentReals_n \in \subgradientRegular{V}(x_n)$ implies $V(y) \geq V(x_n) + \innerProduct{\varTangentReals_n}{y - x_n} + \frac{\lambda}{2}\norm{y - x_n}^2$ and, thus,
$\tau_n V(y) \geq \tau_n V(x_n) + \innerProduct{\tau_n\varTangentReals_n}{y - x_n} + \tau_n\frac{\lambda}{2}\norm{y - x_n}^2$.
{For every $y$ with $V(y) \in
\reals$, letting $n \to \infty$ (using $\tau_n \fromAbove 0$, $V(x_n) \to V(x)
\in \reals$, and $\tau_n \varTangentReals_n \to \varTangentReals$) yields $0
\geq \innerProduct{\varTangentReals}{y - x}$, which is the desired inclusion.}
{Since $V -
\frac{\lambda}{2}\norm{\cdot}^2$ is proper, lower semicontinuous, and convex,
with the same domain as $V$, \cite[Proposition 8.12]{rockafellar2009variational}
together with \cite[Exercise 8.8(c)]{rockafellar2009variational} (horizon
subgradients are unaffected by smooth additions) gives} $
\subgradientHzn{V}(x) = \normalCone{\{y \in \reals^d \st V(y) \in \reals \}}{x},
$
so that if $V(\reals^d) \subseteq \reals$, we conclude $\subgradientHzn{V}(x) = \{0\}$.


==> elements/prop_subgradient_convex_title.tex <==
Subgradients of $\lambda$-convex functions%


==> elements/prop_subgradients_epigraphical_normals_body.tex <==
Let $\objective: \Pp{2}{\reals^d} \to \realsBar$, let $\varFixed \in \Pp{2}{\reals^d}$ at which $\objective(\varFixed) \in \reals$, and let
{$\boldsymbol{\varTangent}\in \normalConeRegular{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$
(resp., $\boldsymbol{\varTangent}\in \normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$)} with $\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}=-1$. Then, $\pushforward{T}{\boldsymbol{\varTangent}}\in\subgradientRegular{\objective}(\varFixed)$ (resp., $\pushforward{T}{\boldsymbol{\varTangent}}\in\subgradient{\objective}(\varFixed)$) with $T$ as in \eqref{equation:extraction-map-epigraph}.


==> elements/prop_subgradients_epigraphical_normals_proof.tex <==
To prove this statement, we proceed in two steps.
We first show the statement for the regular normal cone, namely that for all $\boldsymbol{\varTangent} \in \normalConeRegular{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ with $\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = -1$ it holds that $\pushforward{T}{\boldsymbol{\varTangent}} \in\subgradientRegular{\objective}(\varFixed)$. Then, we prove the statement for the general normal cone.

\emph{Step 1 (regular normal cone).}
For this step, we adapt the proof of \cite[Theorem 1.86]{mordukhovich2006variationalI}.
{First, observe that
$\pushforward{T}{\boldsymbol{\varTangent}}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed}$:
indeed,
$\boldsymbol{\varTangent}\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varFixed\times\delta_{\objective(\varFixed)}}$
by \cref{definition:def_normal_cone}, and
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}
then yields the claim.}
For the sake of contradiction, assume that there exists $\boldsymbol{\varTangent} \in \normalConeRegular{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ with $\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = -1$ for which $\pushforward{T}{\boldsymbol{\varTangent}} \not\in\subgradientRegular{\objective}(\varFixed)$. Then, it follows directly from the definition of subgradient (cf. \cref{definition:def_sub_sup_differentiability}) that there exist $\lambda > 0$ and $\varGeneric_n \convergenceWasserstein \varFixed$, $\varTangentOther_n \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric_n}}$ such that
\begin{equation}
\label{eq:subgradient:contradiction}
\objective(\varGeneric_n) - \objective(\varFixed) - \innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\varTangentOther_n}_{\varFixed} < -\lambda\wassersteinDistance{\varFixed}{\varGeneric_n}{2}.
\end{equation}
We now claim that $\wassersteinDistance{\varTangentOther_n}{\localZero{\varFixed}}{\varFixed}\to 0$ or equivalently $\norm{\varTangentOther_n}_{\varFixed}\to 0$. Indeed, since $\varTangentOther_n= \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\gamma_n}$ for some $\gamma_n\in\setPlansOptimal{\varFixed}{\varGeneric_n}$, we have
    $\norm{\varTangentOther_n}_{\varFixed}^2
    =
    \int_{\reals^d\times\reals^d}\norm{\varTangentReals}^2\d\varTangentOther_n(\bar x,\varTangentReals)
    =
    \int_{\reals^d\times\reals^d}\norm{x_n-\bar x}^2\d\gamma_{n}(\bar x,x_n)
    =
    \wassersteinDistance{\varFixed}{\varGeneric_n}{2}^2\to 0$.
Define
$
\beta_n \coloneqq \objective(\varFixed) + \innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\varTangentOther_n}_{\varFixed} -\lambda\wassersteinDistance{\varFixed}{\varGeneric_n}{2}.
$
%
By continuity of the inner product with respect to the convergence induced by $\wassersteinDistance{\cdot}{\cdot}{\varFixed}$ (cf. \cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:continuity_wass}), $\innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\localZero{\varFixed}}_{\varFixed}=0$ (cf. \cref{proposition:prop_wasserstein_geom}\ref{item:negate_zero_is_zero}).
By continuity of the Wasserstein distance in Wasserstein, we conclude $\beta_n \to \objective(\varFixed)$.
Furthermore, \eqref{eq:subgradient:contradiction} implies $\beta_n > \objective(\varGeneric_n)$ so that $\varGeneric_n\times\delta_{\beta_n} \in \epigraph{\objective}$.
{Since $\varTangentOther_n\times\delta_{(\beta_n -
\objective(\varFixed))}$ is a variation at
$\varFixed\times\delta_{\objective(\varFixed)}$ whose last velocity component is
almost everywhere equal to $\beta_n - \objective(\varFixed)$,
\eqref{eq:deterministic_coordinate:splitting} (cf.
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting}),
together with
$\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = -1$,
yields
\begin{equation*}
\innerProduct{\boldsymbol{\varTangent}}{\varTangentOther_n\times\delta_{(\beta_n - \objective(\varFixed))}}_{\varFixed\times\delta_{\objective(\varFixed)}}
=
\innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\varTangentOther_n}_{\varFixed}-(\beta_n - \objective(\varFixed)).
\end{equation*}}
Using $\norm{\varTangentOther_n}_{\varFixed}=\wassersteinDistance{\varFixed}{\varGeneric_n}{2}$, this yields
\begin{align*}
\frac{\innerProduct{\boldsymbol{\varTangent}}{\varTangentOther_n\times\delta_{(\beta_n - \objective(\varFixed))}}_{\varFixed\times\delta_{\objective(\varFixed)}}}{\wassersteinDistance{\varGeneric_n\times\delta_{\beta_n}}{\varFixed\times\delta_{\objective(\varFixed)}}{2}}
&=
\frac{\innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\varTangentOther_n}_{\varFixed}-(\beta_n - \objective(\varFixed))}{\sqrt{\norm{\varTangentOther_n}_{\varFixed}^2 + \abs{\beta_n - \objective(\varFixed)}^2}}
\\&=
\frac{\lambda\norm{\varTangentOther_n}_{\varFixed}}
{\sqrt{\norm{\varTangentOther_n}_{\varFixed}^2 + \abs{\innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\varTangentOther_n}_{\varFixed} - \lambda\norm{\varTangentOther_n}_{\varFixed}}^2}}
\\&\geq
\frac{\lambda\norm{\varTangentOther_n}_{\varFixed}}
{\norm{\varTangentOther_n}_{\varFixed} + \abs{\innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\varTangentOther_n}_{\varFixed} - \lambda\norm{\varTangentOther_n}_{\varFixed}}}
\\&\geq
\frac{\lambda\norm{\varTangentOther_n}_{\varFixed}}
{\norm{\varTangentOther_n}_{\varFixed} + \abs{\innerProduct{\pushforward{T}{\boldsymbol{\varTangent}}}{\varTangentOther_n}_{\varFixed}} + \lambda\norm{\varTangentOther_n}_{\varFixed}}
\\&\geq
\frac{\lambda\norm{\varTangentOther_n}_{\varFixed}}
{\norm{\varTangentOther_n}_{\varFixed} + \norm{\pushforward{T}{\boldsymbol{\varTangent}}}_{\varFixed}\norm{\varTangentOther_n}_{\varFixed} + \lambda\norm{\varTangentOther_n}_{\varFixed}}
=
\frac{\lambda}
{1 + \norm{\pushforward{T}{\boldsymbol{\varTangent}}}_{\varFixed} + \lambda}
>0,
\end{align*}
where the inequalities follow from subadditivity of the square root, triangle inequality, and~\cref{proposition:prop_wasserstein_geom}\ref{item:wass_geom:cauchy_schwarz}.
{By
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport},
the lifted transport plan
$\pushforward{(\projection{1}{},\objective(\varFixed),\projection{2}{},\beta_n)}{\gamma_n}$
belongs to
$\setPlansOptimal{\varFixed\times\delta_{\objective(\varFixed)}}{\varGeneric_n\times\delta_{\beta_n}}$,
it induces the variation $\varTangentOther_n\times\delta_{(\beta_n -
\objective(\varFixed))}$, and it yields
$\wassersteinDistance{\varGeneric_n\times\delta_{\beta_n}}{\varFixed\times\delta_{\objective(\varFixed)}}{2}^2=\wassersteinDistance{\varFixed}{\varGeneric_n}{2}^2+\abs{\beta_n-\objective(\varFixed)}^2$,
as used above.}
However, this inequality contradicts the assumption that $\boldsymbol{\varTangent} \in \normalConeRegular{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ by the definition of the regular normal cone (cf. \cref{definition:def_normal_cone}), since $\varGeneric_n\times\delta_{\beta_n}\in\epigraph{\objective}$ converges to $\varFixed\times\delta_{\objective(\varFixed)}$ while the left-hand side remains bounded away from zero.

\emph{Step 2 (general normal cone).}
Consider now $\boldsymbol{\varTangent} \in \normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ with $\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = -1$. Then, by \cref{definition:def_normal_cone}, there must exist $\boldsymbol{\tilde{\varTangent}}_n \in \normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\beta_n}}$ for some $\varGeneric_n\times\delta_{\beta_n}\in\epigraph{\objective}$ with $\varGeneric_n \convergenceWasserstein\varFixed$ and $\beta_n\to\objective(\varFixed)$, $\boldsymbol{\tilde{\varTangent}_n} \convergenceWasserstein \boldsymbol{\varTangent}$, $\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals}) \sim \boldsymbol{\tilde{\varTangent}_n}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = -\lambda_n$, and $\lambda_n \to 1$, where we used the continuity of the expected value in Wasserstein.
{Moreover, for $n$ large enough, $\lambda_n>0$ forces
$\beta_n=\objective(\varGeneric_n)$. Indeed, if $\beta_n>\objective(\varGeneric_n)$,
then for all sufficiently small $t>0$ we have
$\varGeneric_n\times\delta_{\beta_n-t}\in\epigraph{\objective}$, and the
variation $\localZero{\varGeneric_n}\times\delta_{-t}$ induced by the optimal
transport plan pairing the Dirac measures {has last velocity component
almost everywhere equal to $-t$
(cf.~\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport}); by
\eqref{eq:deterministic_coordinate:splitting}, together with
$\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\tilde{\varTangent}}_n}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}=-\lambda_n$,
this yields}
$\norm{\localZero{\varGeneric_n}\times\delta_{-t}}_{\varGeneric_n\times\delta_{\beta_n}}=t$
and
$\innerProduct{\boldsymbol{\tilde{\varTangent}}_n}{\localZero{\varGeneric_n}\times\delta_{-t}}_{\varGeneric_n\times\delta_{\beta_n}}=t\lambda_n$,
so \cref{definition:def_normal_cone} requires $t\lambda_n\leq\onotation{t}$ as
$t\to0$, i.e., $\lambda_n\leq0$, a contradiction. In particular
$\objective(\varGeneric_n)=\beta_n\to\objective(\varFixed)$ and
$\objective(\varGeneric_n)\in\reals$.}
Since the regular normal cone is a cone (cf. \cref{proposition:prop_normal_tangent_cones}), we have that $\boldsymbol{\varTangent_n} \coloneqq \frac{\boldsymbol{\tilde{\varTangent}_n}}{\lambda_n} \in \normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}$ and $\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals}) \sim \boldsymbol{{\varTangent_n}}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = -1$. Note that $\boldsymbol{\varTangent_n}$ is well defined since $\lambda_n>0$ for $n$ sufficiently large.
By \emph{Step 1}, we thus have $\pushforward{T}{\boldsymbol{\varTangent_n}} \in \subgradientRegular{\objective}(\varGeneric_n)$. We need to show that $\pushforward{T}{\boldsymbol{\varTangent_n}} \convergenceWasserstein \pushforward{T}{\boldsymbol{\varTangent}}$. Since $T$ is Lipschitz continuous (cf. \cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}), it suffices to show that $\boldsymbol{\varTangent_n} \convergenceWasserstein \boldsymbol{\varTangent}$. With $\boldsymbol{\tilde{\varPlanGeneric}_n} \in \setPlansOptimal{\boldsymbol{\varTangent}}{\boldsymbol{\tilde{\varTangent}_n}}$, define
$
\boldsymbol{\varPlanGeneric_n} \coloneqq \pushforward{(\identity{\reals^{d+1}},\identity{\reals^{d+1}},\identity{\reals^{d+1}}, \frac{1}{\lambda_n}\identity{\reals^{d+1}})}{\boldsymbol{\tilde{\varPlanGeneric}_n}}.
$
Then, $\boldsymbol{\varPlanGeneric_n} \in \setPlans{\boldsymbol{\varTangent}}{\boldsymbol{\varTangent_n}}$ and
\begin{align*}
\wassersteinDistance{\boldsymbol{\varTangent}}{\boldsymbol{\varTangent_n}}{2}^2
&\leq
\int_{(\reals^{d+1}\times\reals^{d+1})\times(\reals^{d+1}\times\reals^{d+1})}
\norm{\boldsymbol{\bar{x}} - \boldsymbol{x}}^2 + \norm{\boldsymbol{\varTangentReals} - \boldsymbol{\varTangentReals'}}^2
\d\boldsymbol{\varPlanGeneric_n}((\boldsymbol{\bar{x}}, \boldsymbol{\varTangentReals}),(\boldsymbol{x},\boldsymbol{\varTangentReals'}))
\\&=
\int_{(\reals^{d+1}\times\reals^{d+1})\times(\reals^{d+1}\times\reals^{d+1})}
\norm{\boldsymbol{\bar{x}} - \boldsymbol{x}}^2 + \norm{\boldsymbol{\varTangentReals} - \frac{1}{\lambda_n}\boldsymbol{\tilde{\varTangentReals}}}^2
\d\boldsymbol{\tilde{\varPlanGeneric}_n}((\boldsymbol{\bar{x}}, \boldsymbol{\varTangentReals}),(\boldsymbol{x},\boldsymbol{\tilde{\varTangentReals}}))
\\&\leq
\int_{(\reals^{d+1}\times\reals^{d+1})\times(\reals^{d+1}\times\reals^{d+1})}
\norm{\boldsymbol{\bar{x}} - \boldsymbol{x}}^2
\\&\qquad\qquad\qquad\qquad\qquad+ \left(\abs{1 - \frac{1}{\lambda_n}}\norm{\boldsymbol{\tilde{\varTangentReals}}} + \norm{\boldsymbol{\tilde{\varTangentReals}} - \boldsymbol{\varTangentReals}}\right)^2
\d\boldsymbol{\tilde{\varPlanGeneric}_n}((\boldsymbol{\bar{x}}, \boldsymbol{\varTangentReals}),(\boldsymbol{x},\boldsymbol{\tilde{\varTangentReals}}))
\\&\leq
\int_{(\reals^{d+1}\times\reals^{d+1})\times(\reals^{d+1}\times\reals^{d+1})}
2\norm{\boldsymbol{\bar{x}} - \boldsymbol{x}}^2 + 2\norm{\boldsymbol{\varTangentReals} - \boldsymbol{\tilde\varTangentReals}}^2
\d\boldsymbol{\tilde{\varPlanGeneric}_n}((\boldsymbol{\bar{x}}, \boldsymbol{\varTangentReals}),(\boldsymbol{x},\boldsymbol{\tilde\varTangentReals}))
\\&\qquad+
2\abs{1 - \frac{1}{\lambda_n}}^2
\int_{(\reals^{d+1}\times\reals^{d+1})\times(\reals^{d+1}\times\reals^{d+1})}
\norm{\boldsymbol{\tilde{\varTangentReals}}}^2
\d\boldsymbol{\tilde{\varPlanGeneric}_n}((\boldsymbol{\bar{x}}, \boldsymbol{\varTangentReals}),(\boldsymbol{x},\boldsymbol{\tilde{\varTangentReals}}))
\\&\leq
2\wassersteinDistance{\boldsymbol{\varTangent}}{\boldsymbol{\tilde{\varTangent}_n}}{2}^2 + 2\abs{1 - \frac{1}{\lambda_n}}^2
\norm{\boldsymbol{\tilde{\varTangent}_n}}^2_{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}.
\end{align*}
Since $\wassersteinDistance{\boldsymbol{\varTangent}}{\boldsymbol{\tilde{\varTangent}_n}}{2}\to0$, $\norm{\boldsymbol{\tilde{\varTangent}_n}}^2_{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}} \to \norm{\boldsymbol{\varTangent}}^2_{\varFixed\times\delta_{\objective(\varFixed)}}$ (since convergence in Wasserstein implies convergence of the second moment), and $\lambda_n \to 1$, we conclude that $\wassersteinDistance{\boldsymbol{\varTangent}}{\boldsymbol{\varTangent_n}}{2}\to0$.


==> elements/prop_subgradients_epigraphical_normals_title.tex <==
Subgradients and epigraphical normals%

==> elements/prop_subgradients_horizon_trivial_body.tex <==
{Let $\objective: \Pp{2}{\reals^d} \to \realsBar$ and $\varFixed \in \Pp{2}{\reals^d}$ with $\objective(\varFixed) \in \reals$. If $\objective$ is \emph{strictly continuous} at $\varFixed$, i.e.,
$\limsup_{\varGeneric_1,\varGeneric_2 \convergenceWasserstein \varFixed} \frac{\abs{\objective(\varGeneric_1) - \objective(\varGeneric_2)}}{\wassersteinDistance{\varGeneric_1}{\varGeneric_2}{2}} < \infty$,}
then the horizon subgradient of $\objective$ at $\varFixed$ is trivial; i.e., $\subgradientHzn{\objective}{(\varFixed)} \localEquiv{\varFixed} \{\localZero{\varFixed}\}$.

==> elements/prop_subgradients_horizon_trivial_proof.tex <==
Let ${\varTangent} \in \subgradientHzn{\objective}(\varFixed)$. Then, by \cref{definition:def_sub_sup_differentiability_horizon}, there is $\boldsymbol{\varTangent} \in \normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ such that $\pushforward{T}{\boldsymbol{\varTangent}} = \varTangent$ and $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = 0$.
Therefore, by the definition of normal cone, there are $\varGeneric_n \convergenceWasserstein \varFixed$, $\beta_n \geq \objective(\varGeneric_n)$, $\beta_n \to \objective(\varFixed)$, $\boldsymbol{\varTangent_n} \in \normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\beta_n}}$ with $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent_n}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = -\lambda_n$ and $\lambda_n\to 0$, and $\boldsymbol{\varTangent_n}\to\boldsymbol{\varTangent}$.

To start, we show that if $\beta_n > \objective(\varGeneric_n)$ then $\pushforward{T}{\boldsymbol{\varTangent_n}} = \localZero{\varGeneric_n}$, which directly implies $\varTangent=\localZero{\varFixed}$.
If $\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}=0$, then $\pushforward{T}{\boldsymbol{\varTangent_n}}=\localZero{\varGeneric_n}$ and there is nothing to prove, so assume $\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}>0$.
By continuity of $\objective$, for all $n$ sufficiently large, there is $\bar\varepsilon_n>0$ such that for all $\varGeneric \in \wassersteinBall{\varGeneric_n}{\bar\varepsilon_n}{2}$ it holds $\beta_n\geq \objective(\varGeneric)$. Thus, for all $\varepsilon\in\left(0, \frac{\bar\varepsilon_n}{\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}}\right)$ we can define $\varGeneric_n^\varepsilon \coloneqq \pushforward{(\projection{1}{} + \varepsilon\projection{2}{})}{\pushforward{T}{\boldsymbol{\varTangent_n}}} \in \wassersteinBall{\varGeneric_n}{\bar\varepsilon_n}{2}$.
%
In particular, $\varGeneric_n^\varepsilon\times\delta_{\beta_n} \in \epigraph{\objective}$.
Suppose initially that $\boldsymbol{\varTangent_n}\in\tangentSpaceInterior{\Pp{2}{\reals^{d+1}}}{\varGeneric_n\times\delta_{\beta_n}}$. Then,
    $\varepsilon(\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_0)
    \in
    \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varGeneric_n\times\delta_{\beta_n}}{\varGeneric_n^\varepsilon\times\delta_{\beta_n}}}$
for all $\varepsilon$ sufficiently small.
{Indeed, since $\boldsymbol{\varTangent_n}\in\tangentSpaceInterior{\Pp{2}{\reals^{d+1}}}{\varGeneric_n\times\delta_{\beta_n}}$,
$\pushforward{(\projection{1}{},\projection{1}{}+\varepsilon\projection{2}{})}{\boldsymbol{\varTangent_n}}$
is an optimal transport plan for all $\varepsilon$ sufficiently small, so by
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport}
its image under $\pushforward{T}{\cdot}$, namely
$\pushforward{(\projection{1}{},\projection{1}{}+\varepsilon\projection{2}{})}{\pushforward{T}{\boldsymbol{\varTangent_n}}}$,
lies in $\setPlansOptimal{\varGeneric_n}{\varGeneric_n^\varepsilon}$. In turn,
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport}
lifts this transport plan to an optimal transport plan between $\varGeneric_n\times\delta_{\beta_n}$ and
the Dirac-marginal target $\varGeneric_n^\varepsilon\times\delta_{\beta_n}$, which
induces the displayed variation.}
Thus, by definition of regular normal cone (cf. \cref{definition:def_normal_cone}),
{%
    \begin{align*}
        &\hspace{-1cm}\onotation{\norm{\varepsilon(\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_0)}_{\varGeneric_n\times\delta_{\beta_n}}}
    \\&\geq
    \innerProduct{\boldsymbol{\varTangent_n}}{\varepsilon(\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_0)}_{\varGeneric_n\times\delta_{\beta_n}}
    \\&=
    \varepsilon\innerProduct{\boldsymbol{\varTangent_n}}{\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_0}_{\varGeneric_n\times\delta_{\beta_n}}
    \\&=
    \varepsilon\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}^2,
    \end{align*}
    where the last equality is
    \eqref{eq:deterministic_coordinate:splitting} applied with $c=0$ to the
    variation
    $\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_0$,
    whose last velocity component vanishes and whose image under
    $\pushforward{T}{\cdot}$ equals $\pushforward{T}{\boldsymbol{\varTangent_n}}$.%
}
Thus, $\varepsilon\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}^2 \leq \onotation{\norm{\varepsilon(\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_0)}_{\varGeneric_n\times\delta_{\beta_n}}}$.
Dividing by $\varepsilon$ and letting $\varepsilon\to 0$, we conclude $\pushforward{T}{\boldsymbol{\varTangent_n}} = \localZero{\varGeneric_n}$.
If $\boldsymbol{\varTangent_n}\notin\tangentSpaceInterior{\Pp{2}{\reals^{d+1}}}{\varGeneric_n\times\delta_{\beta_n}}$,
{fix
$\eta>0$ and define $\boldsymbol{\varTangent_n^\eta}\in\tangentSpaceInterior{\Pp{2}{\reals^{d+1}}}{\varGeneric_n\times\delta_{\beta_n}}$ so that
$\wassersteinDistance{\boldsymbol{\varTangent_n^\eta}}{\boldsymbol{\varTangent_n}}{\varGeneric_n\times\delta_{\beta_n}}<\eta$.
We can proceed analogously, with the displacements
$\varepsilon(\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n^\eta}}\times\delta_0)$
in place of
$\varepsilon(\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_0)$,
to get, for all $\varepsilon>0$ sufficiently small (depending on $\eta$),
$\varepsilon\innerProduct{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\pushforward{T}{\boldsymbol{\varTangent^\eta_n}}}_{\varGeneric_n}
\leq
\onotation{\norm{\varepsilon(\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n^\eta}}\times\delta_0)}_{\varGeneric_n\times\delta_{\beta_n}}}$.
Dividing by $\varepsilon$ and letting $\varepsilon\to 0$ at fixed $\eta$
yields
$\innerProduct{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\pushforward{T}{\boldsymbol{\varTangent^\eta_n}}}_{\varGeneric_n}\leq
0$. Since
$\wassersteinDistance{\pushforward{T}{\boldsymbol{\varTangent_n^\eta}}}{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\varGeneric_n}\leq\wassersteinDistance{\boldsymbol{\varTangent_n^\eta}}{\boldsymbol{\varTangent_n}}{\varGeneric_n\times\delta_{\beta_n}}<\eta$ (cf.~\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}),
letting $\eta\to 0$ and using the continuity of the inner product (cf.
\cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:continuity_wass})
we conclude
$\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}^2\leq0$
and, thus, $\pushforward{T}{\boldsymbol{\varTangent_n}} =
\localZero{\varGeneric_n}$.}

{If $\beta_n > \objective(\varGeneric_n)$ for infinitely many $n \in \naturals$, the previous step gives $\pushforward{T}{\boldsymbol{\varTangent_n}} = \localZero{\varGeneric_n}$ along that subsequence, and passing to the limit yields $\pushforward{T}{\boldsymbol{\varTangent}} = \localZero{\varFixed}$. We may therefore assume $\beta_n = \objective(\varGeneric_n)$ for all $n \in \naturals$.
Since $\boldsymbol{\varTangent_n}\in\normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}\subseteq\normalCone{\epigraph{\objective}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}$, \cref{proposition:prop_epigraph_normal_tangent} gives $\lambda_n\geq 0$.
We again prove that $\pushforward{T}{\boldsymbol{\varTangent_n}} = \localZero{\varGeneric_n}$, which directly implies $\varTangent=\localZero{\varFixed}$.
}
We distinguish two cases, a subsequence of $\lambda_n = 0$ and of $\lambda_n > 0$, which we treat separately:
\begin{itemize}[leftmargin=1.5cm]
    \item[$\lambda_n > 0$.]
By \emph{Step 1} of the proof of \cref{proposition:prop_subgradients_epigraphical_normals}, there exists ${\varTangent}_n \coloneqq \frac{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\lambda_n} \in \subgradientRegular{\objective}(\varGeneric_n)$. For $\varepsilon > 0$ sufficiently small, define $\varGeneric_n^\varepsilon \coloneqq \pushforward{(\projection{1}{} + \varepsilon\projection{2}{})}{\varTangent_n}$, so that $\wassersteinDistance{\varGeneric_n}{\varGeneric_n^\varepsilon}{2} = \varepsilon\norm{\varTangent_n}_{\varGeneric_n}$ and $\varepsilon\varTangent_n \in \pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\setPlansOptimal{\varGeneric_n}{\varGeneric_n^\varepsilon}}$, where, as above, we initially assume that $\varTangent_n\in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varGeneric_n}$.
{Since $\objective$ is strictly continuous at $\varFixed$, there exists $M>0$ so that
\begin{equation*}
    \frac{\objective(\varGeneric_n^\varepsilon) - \objective(\varGeneric_n)}{\wassersteinDistance{\varGeneric_n}{\varGeneric_n^\varepsilon}{2}}
    <
    M
\end{equation*}
for all $n$ sufficiently large and $\varepsilon>0$ sufficiently small.}
Using $\varTangent_n \in \subgradientRegular{\objective}(\varGeneric_n)$, for all $n \in \naturals$ we have
$$
    0 \leq \liminf_{\varepsilon\fromAbove0} \frac{\objective(\varGeneric_n^\varepsilon) - \objective(\varGeneric_n) - \innerProduct{\varTangent_n}{\varepsilon\varTangent_n}_{\varGeneric_n}}{\wassersteinDistance{\varGeneric_n}{\varGeneric_n^\varepsilon}{2}}
    \leq M - \norm{\varTangent_n}_{\varGeneric_n}
    =
    M - \frac{\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}}{\lambda_n}.
$$
However, as $n \to \infty$ this value is negative because $M$ is constant, $\lambda_{n} \fromAbove0$, and $\pushforward{T}{\boldsymbol{\varTangent_n}} \convergenceWasserstein \pushforward{T}{\boldsymbol{\varTangent}}$. This yields a contradiction, unless $\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n} \to 0$ and, thus, $\pushforward{T}{\boldsymbol{\varTangent}} = \localZero{\varFixed}$.
If instead $\varTangent_n\notin\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varGeneric_n}$,
{we
may assume $\norm{\varTangent_n}_{\varGeneric_n}>0$ (otherwise
$\pushforward{T}{\boldsymbol{\varTangent_n}}=\localZero{\varGeneric_n}$ and
there is nothing to prove), fix
$\eta\in(0,\norm{\varTangent_n}_{\varGeneric_n})$, and define
$\varTangent_n^\eta\in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varGeneric_n}$ so that
$\wassersteinDistance{\varTangent_n^\eta}{\varTangent_n}{\varGeneric_n}<\eta$.
With $\varGeneric_n^{\varepsilon,\eta} \coloneqq \pushforward{(\projection{1}{}
+ \varepsilon\projection{2}{})}{\varTangent_n^\eta}$, so that
$\varepsilon\varTangent_n^\eta \in \pushforward{(\projection{1}{},
\projection{2}{} -
\projection{1}{})}{\setPlansOptimal{\varGeneric_n}{\varGeneric_n^{\varepsilon,\eta}}}$
and
$\wassersteinDistance{\varGeneric_n}{\varGeneric_n^{\varepsilon,\eta}}{2}=\varepsilon\norm{\varTangent_n^\eta}_{\varGeneric_n}$
for all $\varepsilon>0$ sufficiently small (depending on $\eta$), this gives
$$
    0 \leq \liminf_{\varepsilon\fromAbove0} \frac{\objective(\varGeneric_n^{\varepsilon,\eta}) - \objective(\varGeneric_n) - \innerProduct{\varTangent_n}{\varepsilon\varTangent_n^\eta}_{\varGeneric_n}}{\wassersteinDistance{\varGeneric_n}{\varGeneric_n^{\varepsilon,\eta}}{2}}
    \leq M - \frac{\innerProduct{\varTangent_n}{\varTangent_n^\eta}_{\varGeneric_n}}{\norm{\varTangent_n^\eta}_{\varGeneric_n}}.
$$
Letting $\eta\to0$, the continuity of the inner product and of the norm (cf.
\cref{proposition:prop_wasserstein_geom}\ref{item:inner_product:continuity_wass})
yields $0\leq M-\norm{\varTangent_n}_{\varGeneric_n} = M -
\frac{\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}}{\lambda_n}$,
and we can conclude as above.}
%
%
\item[$\lambda_n = 0$.]
For all $\varepsilon > 0$, define $\varGeneric_n^\varepsilon \coloneqq \pushforward{(\projection{1}{} + \varepsilon\projection{2}{})}{\pushforward{T}{\boldsymbol{\varTangent_n}}}$.
%
Suppose initially that $\pushforward{T}{\boldsymbol{\varTangent_n}}\in\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varGeneric_n}$.
%
Since $\objective$ is strictly continuous, the sequence of reals $\beta_n^\varepsilon = \frac{\objective(\varGeneric_n^\varepsilon) - \objective(\varGeneric_n)}{\varepsilon}$ is bounded and thus admits a subsequence converging to some $\beta_n^0 \in \reals$.
Thus, we now argue that $\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_{\beta_n^0} \in \tangentCone{\epigraph{\objective}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}$.
%
{
Since $\varGeneric_n^\varepsilon\times\delta_{\objective(\varGeneric_n)+\varepsilon\beta_n^\varepsilon}\in\epigraph{\objective}$
and $\boldsymbol{\varTangent_n}$ belongs to the tangent space at $\varGeneric_n\times\delta_{\objective(\varGeneric_n)}$, the limit as $\varepsilon\fromAbove 0$ yields the result (cf.~\cref{definition:def_tangent_cone}).
}
%
However,
\begin{align*}
    \innerProduct{\boldsymbol{\varTangent_n}}{\pushforward{(\projection{1}{},\ldots,\projection{2d+1}{})}{\boldsymbol{\varTangent_n}}\times\delta_{\beta_n^0}}_{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}
    &=
    \innerProduct{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}
    \\
    &\qquad + \beta_n^0\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent_n}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}
    \\
    &=
    \norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}^2 \geq 0,
\end{align*}
{where the first equality is
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting}
with $c=\beta_n^0$, and the second term vanishes as $\lambda_n=0$.}
If $\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}>0$, we contradict \cref{proposition:prop_normal_tangent_cones}.
Thus, $\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}=0$ and so $\pushforward{T}{\boldsymbol{\varTangent_n}} = \localZero{\varGeneric_n}$.
%
{{Note that
$\pushforward{T}{\boldsymbol{\varTangent_n}}\in\tangentCone{\Pp{2}{\reals^d}}{\varGeneric_n}$
by
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency},
since $\boldsymbol{\varTangent_n}$ belongs to the tangent space at
$\varGeneric_n\times\delta_{\objective(\varGeneric_n)}$ by
\cref{definition:def_normal_cone}.} If instead $\pushforward{T}{\boldsymbol{\varTangent_n}}\notin\tangentSpaceInterior{\Pp{2}{\reals^d}}{\varGeneric_n}$,
 let $\eta>0$ and define $\varTangent_n^\eta$ that does, so that $\wassersteinDistance{\varTangent_n^\eta}{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\varGeneric_n}<\eta$.
Then, as above, we have that $\pushforward{(\projection{1}{},\ldots,\projection{d}{},\objective(\varGeneric_n),\projection{d+1}{},\ldots,\projection{2d}{})}{\varTangent_n^\eta}\times\delta_{\beta_n^0}\in\tangentCone{\epigraph{\objective}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}$ (note that $\varTangent_n^\eta$ belongs to the tangent space at $\varGeneric_n$, and not $\varGeneric_n\times\delta_{\objective(\varGeneric_n)}$, so we need to ``add'' the marginal $\delta_{\objective(\varGeneric_n)}$).
%
With \cref{proposition:prop_normal_tangent_cones}, this gives
\begin{align*}
    0
    &\geq
    \innerProduct{\boldsymbol{\varTangent_n}}{\pushforward{(\projection{1}{},\ldots,\projection{d}{},\objective(\varGeneric_n),\projection{d+1}{},\ldots,\projection{2d}{})}{\varTangent_n^\eta}\times\delta_{\beta_n^0}}
    \\
    &=
    \innerProduct{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\varTangent_n^\eta}_{\varGeneric_n}
    \\
    &\qquad + \beta_n^0\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent_n}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}
    \\
    &=
    \innerProduct{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\varTangent_n^\eta}_{\varGeneric_n}
    \\
    &=
    \frac{1}{2}\left(
    \norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}^2
    -
    \wassersteinDistance{\varTangent_n^\eta}{\pushforward{T}{\boldsymbol{\varTangent_n}}}{\varGeneric_n}^2
    +
    \norm{\varTangent_n^\eta}_{\varGeneric_n}^2
    \right)
    \\
    &\geq
    \frac{1}{2}\left(\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}^2-\eta^2\right),
\end{align*}
where {the first equality is
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting}
with $c=\beta_n^0$ (the second term vanishing as $\lambda_n=0$), and }the last
equality uses~\cref{proposition:prop_wasserstein_geom}\ref{item:distance_norm_innerproduct}.
Thus, $\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}\leq\eta$ and, as $\eta$ is arbitrary, we conclude $\norm{\pushforward{T}{\boldsymbol{\varTangent_n}}}_{\varGeneric_n}=0$ and, with it, $\pushforward{T}{\boldsymbol{\varTangent_n}}=\localZero{{\varGeneric_n}}$.
}
\end{itemize}

Conversely, $\localZero{\varFixed\times\delta_{\objective(\varFixed)}}\in\normalConeRegular{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}\subseteq\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$, with $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \localZero{\varFixed\times\delta_{\objective(\varFixed)}}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = 0$ and $\pushforward{T}{\localZero{\varFixed\times\delta_{\objective(\varFixed)}}}=\localZero{\varFixed}$, so $\localZero{\varFixed}\in\subgradientHzn{\objective}(\varFixed)$.



==> elements/prop_subgradients_horizon_trivial_title.tex <==
Horizon subgradients for strictly continuous functions%

==> elements/prop_wasserstein_geom_body.tex <==
Let $\varFixed \in \Pp{2}{\reals^d}$ and $\varTangent,\varTangent_1, \varTangent_2,\varTangent_3 \in \PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$.
%
The following statements hold:
\begin{enumerate}[leftmargin=*]
\item
\uniqueLabel{item:distance_norm_innerproduct}
$
\wassersteinDistance{\varTangent_1}{\varTangent_2}{\varFixed}^2
=
\norm{\varTangent_1}_{\varFixed}^2
-2\innerProduct{\varTangent_1}{\varTangent_2}_{\varFixed}
+\norm{\varTangent_2}_{\varFixed}^2
$.

\item
\uniqueLabel{item:distance:continuity_wass}
The map $\wassersteinDistance{}{}{\varFixed}$ is continuous in the topology induced by $\wassersteinDistance{}{}{\varFixed}$.

\item
\uniqueLabel{item:inner_product:continuity_wass}
The map $\innerProduct{\cdot}{\cdot}_{\varFixed}$ is continuous in the topology induced by $\wassersteinDistance{}{}{\varFixed}$.

\item
\uniqueLabel{item:inner_product:homogeneity}
$
\innerProduct{\lambda_1\varTangent_1}{\lambda_2\varTangent_2}_{\varFixed}
=
\lambda_1\lambda_2
\innerProduct{\varTangent_1}{\varTangent_2}_{\varFixed}
$
for any $\lambda_1, \lambda_2 \geq0$.

\item \uniqueLabel{item:inner_product:sublinear}
$
\innerProduct{\varTangent_1 \localSum{\varTangentCoupling} \varTangent_2}{\varTangent_3}_{\varFixed}
\leq
\innerProduct{\varTangent_1}{\varTangent_3}_{\varFixed}
+
\innerProduct{\varTangent_2}{\varTangent_3}_{\varFixed}
$
for any $\varTangentCoupling\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}$.

\item
\uniqueLabel{item:negate_zero_is_zero}
$\lambda\localZero{\varFixed} \localEquiv{\varFixed} \localZero{\varFixed}$ and
{$
\innerProduct{\lambda\localZero{\varFixed}}{\varTangent}_{\varFixed}
=
\innerProduct{\localZero{\varFixed}}{\varTangent}_{\varFixed}
=
0
$}
for any $\lambda \in \reals$.

\item
\uniqueLabel{item:wass_geom:sum:commutative}
$
\varTangent_1
\localSum{\varTangentCoupling}
\varTangent_2
=
\varTangent_2
\localSum{\varTangentCoupling'}
\varTangent_1
$
for any $\varTangentCoupling\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}$, $\varTangentCoupling'=\pushforward{(\projection{1}{},\projection{3}{},\projection{2}{})}{\varTangentCoupling}$.

\item
\uniqueLabel{item:wass_geom:sum:zero}
$\varTangent \localSum{\varTangentCoupling} \localZero{\varFixed} = \varTangent$ for any $\varTangentCoupling\in\setPlansCommonMarginal{\varTangent}{\localZero{\varFixed}}{1}$.

\item
\uniqueLabel{item:wass_geom:distributive}
$(\lambda_1+\lambda_2)\varTangent=\lambda_1\varTangent\localSum{\varTangentCoupling}\lambda_2\varTangent$ for any $\lambda_1,\lambda_2\in\reals$, $\varTangentCoupling=\pushforward{(\projection{1}{},\lambda_1\projection{2}{},\lambda_2\projection{2}{})}\varTangent$.

\item
\uniqueLabel{item:wass_geom:cauchy_schwarz}
$\innerProduct{\varTangent_1}{\varTangent_2}_{\varFixed}\leq\norm{\varTangent_1}_{\varFixed}\norm{\varTangent_2}_{\varFixed}$ and $\innerProduct{\varTangent}{\varTangent}_{\varFixed}=\norm{\varTangent}_{\varFixed}^2$.

\item
\uniqueLabel{item:zero_iff_zero}
$\norm{\varTangent}_{\varFixed}=0$ if and only if $\varTangent\localEquiv{\varFixed}\localZero{\varFixed}$.

\item
\uniqueLabel{item:epsclose}
If $\wassersteinDistance{\varTangent_1}{\varTangent_2}{\varFixed} < \varepsilon$, there exist $\varTangent_{12} \in \PpLocal{2}{\reals^d\times\reals^d}{\varFixed}$ with $\norm{\varTangent_{12}}_{\varFixed} \leq \varepsilon$ and $\varTangentCoupling \in \setPlansCommonMarginal{\varTangent_1}{\varTangent_{12}}{1}$ so that $\varTangent_1 \localSum{\varTangentCoupling} \varTangent_{12} = \varTangent_2$.
\end{enumerate}


==> elements/prop_wasserstein_geom_proof.tex <==
We prove the statements separately.
\begin{enumerate}[leftmargin=*]
\item
See \cite[Proposition 12.4.2]{ambrosio2005gradient}.

\item
Every distance is continuous in the topology it induces; see \cite[Theorem 21.1]{munkres2019topology} and \cite[Proposition 12.4.2]{ambrosio2005gradient}.

\item
See \cite[Proposition 4.21]{gigli2008geometry}.

\item
See \cite[Proposition 4.27]{gigli2008geometry}.

\item
See \cite[Proposition 4.27]{gigli2008geometry}.

\item
{By definition of $\localZero{\varFixed}$ and of scaling, $\localZero{\varFixed}=\lambda\localZero{\varFixed}$. Then,
\begin{align*}
\innerProduct{\lambda\localZero{\varFixed}}{\varTangent}_{\varFixed}
    &\coloneqq
    \max_{\varTangentCoupling \in \setPlansCommonMarginal{\lambda\localZero{\varFixed}}{\varTangent}{1}}
    \int_{\reals^d\times\reals^d\times\reals^d}
    \innerProduct{\varTangentReals_1}{\varTangentReals_2}
    \\&\qquad
    \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
    \\&=\max_{\varTangentCoupling \in \setPlansCommonMarginal{\lambda\localZero{\varFixed}}{\varTangent}{1}}
    \int_{\reals^d\times\reals^d\times\reals^d}
    \innerProduct{\lambda 0}{\varTangentReals_2}
    \\&\qquad
    \d\varTangentCoupling(\bar x, \varTangentReals_1, \varTangentReals_2)
    \\&= 0 = \innerProduct{\localZero{\varFixed}}{\varTangent}_{\varFixed}.
\end{align*}}

\item
Commutativity follows directly from commutativity of every operation involved; it suffices to consider the pushforward via the map $(\projection{1}{}, \projection{3}{}, \projection{2}{})$ of the couplings.

\item
See \cite[Proposition 4.22]{gigli2008geometry}.

\item See \cite[Proposition 4.22]{gigli2008geometry}.

\item We have
\begin{align*}
    \innerProduct{\varTangent_1}{\varTangent_2}_{\varFixed}
    &=
    \max_{\varTangentCoupling\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}}
    \int_{\reals^d\times\reals^d\times\reals^d}
    \innerProduct{\varTangentReals_1}{\varTangentReals_2}
    \\&\qquad
    \d\varTangentCoupling(\bar x,\varTangentReals_1,\varTangentReals_2)
    \\
    \overset{\heartsuit}&{\leq}
    \max_{\varTangentCoupling\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}}
    \sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{\varTangentReals_1}^2\d\varTangentCoupling(\bar x,\varTangentReals_1,\varTangentReals_2)}
    \\&\qquad\times
    \sqrt{\int_{\reals^d\times\reals^d\times\reals^d}\norm{\varTangentReals_2}^2\d\varTangentCoupling(\bar x,\varTangentReals_1,\varTangentReals_2)}
    \\
    &\leq
    \max_{\varTangentCoupling\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}}
    \sqrt{\int_{\reals^d\times\reals^d}\norm{\varTangentReals_1}^2\d\varTangent_1(\bar x,\varTangentReals_1)}
    \\&\qquad\times
    \sqrt{\int_{\reals^d\times\reals^d}\norm{\varTangentReals_2}^2\d\varTangent_2(\bar x,\varTangentReals_2)}
    \\
    &=
    \norm{\varTangent_1}_{\varFixed}\norm{\varTangent_2}_{\varFixed},
\end{align*}
where in $\heartsuit$ we used H\"older's inequality. In the case $\varTangent_1=\varTangent_2=\varTangent$, we additionally have
$\pushforward{(\projection{1}{},\projection{2}{},\projection{2}{})}{\varTangent}\in\setPlansCommonMarginal{\varTangent}{\varTangent}{1}$ and
    $\innerProduct{\varTangent}{\varTangent}_{\varFixed}
    \geq
    \int_{\reals^d\times\reals^d\times\reals^d}
    \innerProduct{\varTangentReals_1}{\varTangentReals_2}
    \d(\pushforward{(\projection{1}{},\projection{2}{},\projection{2}{})}{\varTangent})(\bar x,\varTangentReals_1,\varTangentReals_2)
    =
    \int_{\reals^d\times\reals^d}
    \innerProduct{\varTangentReals}{\varTangentReals}
    \d\varTangent(\bar x,\varTangentReals)=\norm{\varTangent}_{\varFixed}^2$.
Thus, $\innerProduct{\varTangent}{\varTangent}_{\varFixed}=\norm{\varTangent}_{\varFixed}^2$.

\item By~\ref{item:wass_geom:cauchy_schwarz} and~\ref{item:negate_zero_is_zero} with $\varTangent\localEquiv{\varFixed}\localZero{\varFixed}$ and $\lambda=1$, $\norm{\localZero{\varFixed}}_{\varFixed}=0$. Suppose now $\norm{\varTangent}_{\varFixed}=0$. Then, $\int_{\reals^d\times\reals^d}\norm{\varTangentReals}^2\d\varTangent(\bar x, \varTangentReals) = 0$ and, thus, $\pushforward{\projection{2}{}}{\varTangent} = \delta_0$. Since $\pushforward{\projection{1}{}}{\varTangent} = \varFixed$, $\varTangent\localEquiv{\varFixed}\localZero{\varFixed}$.

\item {Let $\varTangentCoupling^\ast\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}$ be the optimal coupling in $\wassersteinDistance{\varTangent_1}{\varTangent_2}{\varFixed}$.
With this, define
$\varTangentCoupling\coloneqq\pushforward{(\projection{1}{},\projection{2}{},-\projection{2}{}+\projection{3}{})}{\varTangentCoupling^\ast}$ and
$\varTangent_{12}=\pushforward{(\projection{1}{},\projection{3}{})}{\varTangentCoupling}$. Then, $\varTangentCoupling\in\setPlansCommonMarginal{\varTangent_1}{\varTangent_{12}}{1}$ and $\varTangent_1\localSum{\varTangentCoupling}\varTangent_{12}=\pushforward{(\projection{1}{},\projection{2}{}+\projection{3}{})}{\varTangentCoupling}=
\pushforward{(\projection{1}{},\projection{2}{}+\projection{3}{})}{\pushforward{(\projection{1}{},\projection{2}{},-\projection{2}{}+\projection{3}{})}{\varTangentCoupling^\ast}}=\pushforward{(\projection{1}{},\projection{2}{}+(-\projection{2}{}+\projection{3}{}))}{\varTangentCoupling^\ast}=\pushforward{(\projection{1}{},\projection{3}{})}{\varTangentCoupling^\ast}=\varTangent_2$.
To conclude, $\norm{\varTangent_{12}}_{\varFixed}^2=\int_{\reals^d\times\reals^d}\norm{\varTangentReals}^2\d\varTangent_{12}(\bar x,\varTangentReals)
=
\int_{\reals^d\times\reals^d\times\reals^d}
{\norm{-\varTangentReals_1+\varTangentReals_2}^2\d\varTangentCoupling^\ast(\bar
x,\varTangentReals_1,\varTangentReals_2)}
=
\wassersteinDistance{\varTangent_1}{\varTangent_2}{\varFixed}^2$. Thus, $\norm{\varTangent_{12}}_{\varFixed}<\varepsilon$.}
\end{enumerate}


==> elements/prop_wasserstein_geom_title.tex <==
Properties of the Wasserstein geometry%

==> elements/prop_wassersteindistance_general_subgradient_body.tex <==
For $\varFixed, \varReference \in \Pp{2}{\reals^d}$, $\objective: \Pp{2}{\reals^d} \to \realsBar$, $\objective(\varGeneric) \coloneqq \frac{1}{2}\wassersteinDistance{\varGeneric}{\varReference}{2}^2$, we have
$
    \subgradient{\objective}(\varFixed)
    \neq
    \emptyset
$
and
$
    \subgradient{\objective}(\varFixed)
    \subseteq
    \pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{
    \setPlansOptimal{\varFixed}{\varReference}
    }
$.

==> elements/prop_wassersteindistance_general_subgradient_proof.tex <==
By \cref{proposition:prop_wassersteindistance_regular_subgradient_must_be_plan}, for every $\varGeneric \in \Pp{2}{\reals^d}$ we have either $\subgradientRegular{\objective}(\varGeneric) = \emptyset$ or $\emptyset\neq\subgradientRegular{\objective}(\varGeneric) \subseteq \pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\setPlansOptimal{\varGeneric}{\varReference}}$.
Consider now any (possibly trivial) sequence $(\varGeneric_n)_{n \in \naturals} \subseteq \Pp{2}{\reals^d}$ converging to $\varFixed$ such that $\subgradientRegular{\objective}(\varGeneric_n) \neq \emptyset$ for all $n \in \naturals$. Such a sequence exists because $\Ppabs{2}{\reals^d}$ is dense in $\Pp{2}{\reals^d}$ (cf. \cite[Theorem 2.2.7]{panaretos2020invitation}), {$\objective$ is differentiable at every $\varGeneric \in
\Ppabs{2}{\reals^d}$} (by~\cref{proposition:prop_wassersteindistance_regular_subgradient_must_be_plan}\ref{item:prop_wassersteindistance_regular_subgradient_must_be_plan:differentiable}), and  $\objective(\varGeneric_n)$ converges to $\objective(\varFixed)$ (clearly, the squared Wasserstein distance is continuous in Wasserstein).
%
Specifically, let $(\varTangent_n)_{n \in \naturals} \subseteq \Pp{2}{\reals^d\times\reals^d}$ such that $\varTangent_n \in \subgradientRegular{\objective}(\varGeneric_n)$.
By \cref{proposition:prop_wassersteindistance_regular_subgradient_must_be_plan}\ref{item:prop_wassersteindistance_regular_subgradient_must_be_plan:regular_necessary},
$\varTangentOther_n\coloneqq\pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\varTangent_n}\in\setPlansOptimal{\varGeneric_n}{\varReference}$.
We now claim that, up to a subsequence (not relabeled), $\varTangentOther_n\convergenceWasserstein\varTangentOther$ for some $\varTangentOther\in\setPlansOptimal{\varFixed}{\varReference}$.
%
By~\cite[Theorem 5.20]{villani2009optimal} (see also \cite[Proposition 7.1.3]{ambrosio2005gradient}),
$\varTangentOther_n$ converges narrowly (up to subsequences) to some $\varTangentOther\in\setPlansOptimal{\varFixed}{\varReference}$.
Moreover,
\begin{align*}
\int_{\reals^d\times\reals^d}\norm{x}^2+\norm{y}^2\d\varTangentOther_n(x,y)
&=\int_{\reals^d}\norm{x}^2\d\varGeneric_n(x)+\int_{\reals^d}\norm{x}^2\d\varReference(x)
\\
&\to
\int_{\reals^d}\norm{x}^2\d\varFixed(x)+\int_{\reals^d}\norm{x}^2\d\varReference(x)
\\
&=
\int_{\reals^d\times\reals^d}\norm{x}^2+\norm{y}^2\d\varTangentOther(x,y),
\end{align*}
which proves convergence of the second moment. Thus, $\varTangentOther_n\convergenceWasserstein\varTangentOther$.
%
Since the pushforward via Lipschitz continuous maps is Lipschitz continuous with respect to $\wassersteinDistance{}{}{2}$, we have $\varTangent_n=\pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\varTangentOther_n}\convergenceWasserstein\pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\varTangentOther}\in \pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\setPlansOptimal{\varFixed}{\varReference}}$.
{Moreover, if $\varTangentFixed \in
\subgradient{\objective}(\varFixed)$, let $(\varGeneric_n)_{n\in\naturals}$ and
$(\varTangent_n)_{n\in\naturals}$ be as in the definition of the general
subgradient, so that $\varTangent_n \convergenceWasserstein \varTangentFixed$;
the argument above provides a subsequence of $(\varTangent_n)_{n\in\naturals}$
converging in Wasserstein to an element of
$\pushforward{(\projection{1}{}, \projection{1}{} -
\projection{2}{})}{\setPlansOptimal{\varFixed}{\varReference}}$, and uniqueness
of the Wasserstein limit yields $\varTangentFixed \in
\pushforward{(\projection{1}{}, \projection{1}{} -
\projection{2}{})}{\setPlansOptimal{\varFixed}{\varReference}}$.}
Thus, $\subgradient{\objective}(\varFixed)$ is nonempty and contained in $\pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\setPlansOptimal{\varFixed}{\varReference}}$.


==> elements/prop_wassersteindistance_general_subgradient_title.tex <==
General subgradient of the squared Wasserstein distance%

==> elements/prop_wassersteindistance_regular_subgradient_must_be_plan_body.tex <==
Consider the functional $\objective: \Pp{2}{\reals^d} \to \realsBar$,
$\objective(\varGeneric) \coloneqq \frac{1}{2}\wassersteinDistance{\varGeneric}{\varReference}{2}^2$ for some fixed $\varReference \in \Pp{2}{\reals^d}$. Then, for any $\varFixed \in \Pp{2}{\reals^d}$:
\begin{enumerate}
    \item 
    $-\objective$ is regularly subdifferentiable at $\varFixed$ and all $\pushforward{(\projection{1}{}, \projection{2}{} - \projection{1}{})}{\varPlanGeneric}$ are regular subgradients of $-\objective$ at $\varFixed$, where $\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varReference}$.

    \label{item:prop_wassersteindistance_regular_subgradient_must_be_plan:supergradient}

    \item If $\setPlansOptimal{\varFixed}{\varReference}$ is a singleton and induced by an optimal transport map (e.g., when $\varFixed$ is absolutely continuous), then $\objective$ is regularly subdifferentiable, and thus differentiable, at $\varFixed$. 
    \label{item:prop_wassersteindistance_regular_subgradient_must_be_plan:differentiable}
    
    \item If $\varTangent\in \subgradientRegular{\objective}(\varFixed)$, then $\pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\varTangent} \in \setPlansOptimal{\varFixed}{\varReference}$.
    \label{item:prop_wassersteindistance_regular_subgradient_must_be_plan:regular_necessary}

    \item If $\setPlansOptimal{\varFixed}{\varReference}$ is not a singleton, then $\objective$ is not regularly subdifferentiable at $\varFixed$. 
\end{enumerate}


==> elements/prop_wassersteindistance_regular_subgradient_must_be_plan_proof.tex <==
We prove the statements separately:
\begin{enumerate}
    \item See \cite[Theorem 10.2.2]{ambrosio2005gradient}.
    \item See \cite[Theorem 10.2.6]{ambrosio2005gradient}.
    \item
Let $\varTangent\in\subgradientRegular{\objective}(\varFixed)$.
{By
\ref{item:prop_wassersteindistance_regular_subgradient_must_be_plan:supergradient}
and
\cref{proposition:prop_differentiability_properties}\ref{item:subdifferential-cap-superdifferential}}, $\hat\varTangent \in \pushforward{(\projection{1}{}, \projection{1}{} - \projection{2}{})}{\setPlansOptimal{\varFixed}{\varReference}}$ exists such that $\wassersteinDistance{\varTangent}{\hat\varTangent}{\varFixed} = 0$. In particular, this implies $\varTangent = \hat\varTangent$; see \cite[Proposition 12.4.6]{ambrosio2005gradient}.
{Since the map
$(x,\varTangentReals)\mapsto(x,x-\varTangentReals)$ is an involution,
$\varTangent = \pushforward{(\projection{1}{}, \projection{1}{} -
\projection{2}{})}{\varPlanGeneric}$ for some
$\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varReference}$ yields
$\pushforward{(\projection{1}{}, \projection{1}{} -
\projection{2}{})}{\varTangent} = \varPlanGeneric \in
\setPlansOptimal{\varFixed}{\varReference}$.}

\item
{Without loss of generality, suppose $\wassersteinDistance{\varFixed}{\varReference}{2}>0$; otherwise $\varFixed=\varReference$ and the optimal transport plan is trivially unique.
%
We prove the statement via contraposition, i.e., by showing that if $\objective$ is regularly subdifferentiable at $\varFixed$, then the set of optimal transport plans is a singleton. Suppose $\objective$ is regularly subdifferentiable at $\varFixed$. Then, there exists $\varTangent\in\subgradientRegular{\objective}(\varFixed)$.
Now let $\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varReference}$ be arbitrary. By~\ref{item:prop_wassersteindistance_regular_subgradient_must_be_plan:supergradient},
$\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\varPlanGeneric}$
is a regular subgradient of $-\objective$ at $\varFixed$.
%
Thus, by~\cref{proposition:prop_differentiability_properties}\ref{item:subdifferential-cap-superdifferential} and~\ref{item:prop_wassersteindistance_regular_subgradient_must_be_plan:supergradient} (applied to $\varTangent\in\subgradientRegular{\objective}(\varFixed)$ and $\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\tilde\varPlanGeneric}\in-\subgradientRegular{(-\objective)}(\varFixed)$), $\wassersteinDistance{\varTangent}{\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\tilde\varPlanGeneric}}{\varFixed} = 0$ for all $\tilde\varPlanGeneric\in\setPlansOptimal{\varFixed}{\varReference}$.
Therefore, if $\varPlanGeneric,\tilde{\varPlanGeneric}\in\setPlansOptimal{\varFixed}{\varReference}$, then
\[
\wassersteinDistance{\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\varPlanGeneric}}{\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\tilde{\varPlanGeneric}}}{2}
\leq
\wassersteinDistance{\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\varPlanGeneric}}{\pushforward{(\projection{1}{},\projection{1}{}-\projection{2}{})}{\tilde{\varPlanGeneric}}}{\varFixed}=0.
\]
Since the map $(x,y)\mapsto(x,x-y)$ is injective, this implies $\varPlanGeneric=\tilde{\varPlanGeneric}$.
%
Thus, $\setPlansOptimal{\varFixed}{\varReference}$ is a singleton,
which proves the contrapositive and, thus, the statement.}
\end{enumerate}


==> elements/prop_wassersteindistance_regular_subgradient_must_be_plan_title.tex <==
Subgradients of the squared Wasserstein distance and optimal transport plans%

==> elements/strong_vs_regular_normal_cone_body.tex <==
Let $\varFixed\in\Pp{2}{\reals^d}$.
\begin{enumerate}
\item
    \uniqueLabel{item:strong_vs_regular:subgradient}
    For every functional $\objective:\Pp{2}{\reals^d}\to\realsBar$ with $\objective(\varFixed)\in\reals$, it holds that $\subgradientRegularStrong{\objective}(\varFixed) \subseteq \subgradientRegular{\objective}(\varFixed)$ and, consequently, $\subgradientStrong{\objective}(\varFixed) \subseteq \subgradient{\objective}(\varFixed)$.
\item
    \uniqueLabel{item:strong_vs_regular:normal}
    For every set $\feasibleSet \subseteq \Pp{2}{\reals^d}$ with $\varFixed \in \feasibleSet$, it holds that $\normalConeRegularStrong{\feasibleSet}{\varFixed} \subseteq \normalConeRegular{\feasibleSet}{\varFixed}$ and, consequently, $\normalConeStrong{\feasibleSet}{\varFixed} \subseteq \normalCone{\feasibleSet}{\varFixed}$.
\end{enumerate}


==> elements/strong_vs_regular_normal_cone_proof.tex <==
\emph{Subgradients.} Since $\setPlansOptimal{\varFixed}{\varGeneric}\subseteq\setPlans{\varFixed}{\varGeneric}$ for every $\varGeneric\in\Pp{2}{\reals^d}$, the defining inequality of $\subgradientRegularStrong{\objective}(\varFixed)$ (\cref{definition:def_strong_sub_sup_differentiability}), required for all $\varTangent\in\pushforward{(\projection{1}{}, \projection{2}{}- \projection{1}{})}{\setPlans{\varFixed}{\varGeneric}}$, holds in particular for all $\varTangent\in\pushforward{(\projection{1}{}, \projection{2}{}- \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$. On such optimal transport plans $\norm{\varTangent}_{\varFixed}=\wassersteinDistance{\varFixed}{\varGeneric}{2}$, so this is exactly the inequality defining $\subgradientRegular{\objective}(\varFixed)$ (\cref{definition:def_sub_sup_differentiability}); hence $\subgradientRegularStrong{\objective}(\varFixed)\subseteq\subgradientRegular{\objective}(\varFixed)$. The inclusion for the general subgradients follows: if $\varGeneric_n\to\varFixed$ with $\objective(\varGeneric_n)\to\objective(\varFixed)$ and $\varTangent_n\in\subgradientRegularStrong{\objective}(\varGeneric_n)$ with $\varTangent_n\convergenceWasserstein\varTangentFixed$, then $\varTangent_n\in\subgradientRegular{\objective}(\varGeneric_n)$ by the above, and \cref{definition:def_sub_sup_differentiability} gives $\varTangentFixed\in\subgradient{\objective}(\varFixed)$.

\emph{Normal cones.} Since $\setPlansOptimal{\varFixed}{\varGeneric}\subseteq\setPlans{\varFixed}{\varGeneric}$ for every $\varGeneric\in\feasibleSet$, the defining inequality of $\normalConeRegularStrong{\feasibleSet}{\varFixed}$ (\cref{definition:def_fuzzy_normal_cone}), required for all $\varTangent\in\pushforward{(\projection{1}{}, \projection{2}{}- \projection{1}{})}{\setPlans{\varFixed}{\varGeneric}}$, holds in particular for all $\varTangent\in\pushforward{(\projection{1}{}, \projection{2}{}- \projection{1}{})}{\setPlansOptimal{\varFixed}{\varGeneric}}$, which is the defining inequality of $\normalConeRegular{\feasibleSet}{\varFixed}$ (\cref{definition:def_normal_cone}). The inclusion for the (limiting) normal cones then follows directly: if $\varGeneric_n\convergenceWasserstein\varFixed$ in $\feasibleSet$ and $\varTangent_n\in\normalConeRegularStrong{\feasibleSet}{\varGeneric_n}$ with $\varTangent_n\convergenceWasserstein\varTangentFixed$ as in \cref{definition:def_fuzzy_normal_cone}, then $\varTangent_n\in\normalConeRegular{\feasibleSet}{\varGeneric_n}$ by the above, and \cref{definition:def_normal_cone} gives $\varTangentFixed\in\normalCone{\feasibleSet}{\varFixed}$.


==> elements/strong_vs_regular_normal_cone_title.tex <==
Relationship between strong and regular subgradients and normal cones%

==> elements/th_extremal_principle_body.tex <==
{Let $(\Omega_1,\Omega_2,\varFixed)$ be extremal with
$\Omega_1,\Omega_2$ locally closed around $\varFixed$.
%
Then, for every $\varepsilon>0$, there are probability measures $\varFixed_i\in\Omega_i$ with $\wassersteinDistance{\varFixed_i}{\varFixed}{2}<\varepsilon$, an optimal transport plan $\varPlanGeneric\in\setPlansOptimal{\varFixed_1}{\varFixed_2}$, and a shift $a\in\reals^d$ so that, with $c\coloneqq\wassersteinDistance{\pushforward{(\identity{}+a)}{\varFixed_1}}{\varFixed_2}{2}>0$, the tangent vectors
$
\varTangent_1\coloneqq\tfrac1c\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{}-a)}{\varPlanGeneric}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed_1}
$
and
$
\varTangent_2\coloneqq\tfrac1c\pushforward{(\projection{2}{},\projection{1}{}-\projection{2}{}+a)}{\varPlanGeneric}\in\tangentCone{\Pp{2}{\reals^d}}{\varFixed_2},
$
with $\norm{\varTangent_1}_{\varFixed_1}=\norm{\varTangent_2}_{\varFixed_2}=1$, are $\varepsilon$-close with respect to $\wassersteinDistance{}{}{\varFixed_i}$ to the strong regular normal cones $\normalConeRegularStrong{\Omega_1}{\varFixed_1}$ and $\normalConeRegularStrong{\Omega_2}{\varFixed_2}$, respectively. In particular, there is $\varPlanGeneric_{\varTangent}\in\setPlans{\varTangent_1}{\varTangent_2}$ with $\pushforward{(\projection{1}{},\projection{3}{})}{\varPlanGeneric_{\varTangent}}=\varPlanGeneric$ such that
$\int_{\reals^d\times\reals^d\times\reals^d\times\reals^d}\norm{\varTangentReals_1+\varTangentReals_2}^2\d\varPlanGeneric_{\varTangent}(x_1,\varTangentReals_1,x_2,\varTangentReals_2)=0$.}



==> elements/th_extremal_principle_proof.tex <==
Our proof leverages~\cref{lemma:lemma_fuzzy_optimality_condition} and the Borwein–Preiss variational principle~\cite[Theorem 2.5.2]{borwein2006techniques}.
{Extremality of $(\Omega_1,\Omega_2,\varFixed)$ provides a neighborhood $U$ of $\varFixed$, independent of $\varepsilon$, so that for every $\delta>0$ there is a shift $a\in\reals^d$ with $\norm{a}<\delta$ and $\left(\pushforward{(\identity{}+a)}\Omega_1\right)\cap\Omega_2\cap U=\emptyset$.
Fix $r>0$ small enough that $\closedWassersteinBall{\varFixed}{r}{2}\subseteq U$ and $\Omega_i\cap\closedWassersteinBall{\varFixed}{r}{2}$ is closed for $i\in\{1,2\}$, where $\closedWassersteinBall{\varFixed}{r}{2}$ denotes the closed Wasserstein ball of radius $r$ centered at $\varFixed$.
Clearly, it suffices to prove the claim for $\varepsilon\leq r$.
Fix $\varepsilon\in(0,r]$ and apply the above with $\delta=\frac{\varepsilon^2}{8}$, giving $a\in\reals^d$ with $\norm{a}<\frac{\varepsilon^2}{8}$.}
Let again $W_2^a(\varGeneric_1,\varGeneric_2)\coloneqq\wassersteinDistance{\pushforward{(\identity{}+a)}{\varGeneric_1}}{\varGeneric_2}{2}$.
By definition, $W_2^a(\varFixed,\varFixed)=\norm{a}<\frac{\varepsilon^2}{8}$.
Since $W_2^a(\varGeneric_1,\varGeneric_2)=0$ is equivalent to $\pushforward{(\identity{}+a)}{\varGeneric_1}=\varGeneric_2$, $\left(\pushforward{(\identity{}+a)}\Omega_1\right)\cap\Omega_2\cap U=\emptyset$ is equivalent to $W_2^a(\varGeneric_1,\varGeneric_2)>0$ for all $\varGeneric_1\in\Omega_1$ and $\varGeneric_2\in\Omega_2\cap U$.
%
We now deploy the Borwein–Preiss variational principle~\cite[Theorem 2.5.2]{borwein2006techniques}, with their $X=\Omega_1\times\Omega_2$, their $f$ being $W_2^a$, and their $\varepsilon$ being $\varepsilon^2/8$.
%
Let us verify its assumptions.
First, since the Wasserstein space $\Pp{2}{\reals^d}$ is a complete metric space~\cite[Theorem 6.18]{villani2009optimal}, the Cartesian product $\Pp{2}{\reals^d}\times\Pp{2}{\reals^d}$ is also a complete metric space (endowed with the product distance). Since $\Omega_1$ and $\Omega_2$ are locally closed around $\varFixed$ and all statements are local, we can without loss of generality intersect them with $\closedWassersteinBall{\varFixed}{r}{2}$, so that $X=\Omega_1\times\Omega_2$ is closed and, being a closed subspace of a complete metric space, complete.

Second, $W_2^a$ is nonnegative and continuous in Wasserstein.
Third, the squared Wasserstein distance (scaled by $\frac{1}{2}$) is a gauge-type function, as defined in~\cite[Definition 2.5.1]{borwein2006techniques} (see also~\cite[Theorem 2.5.3]{borwein2006techniques} for an analogous statement in Banach spaces). 
Fourth, in the notation of~\cite[Theorem 2.5.2]{borwein2006techniques}, we consider the sequence $\delta_j=2^{-j}$.
Fifth, $(\varFixed,\varFixed)$ is an approximate minimizer of $W_2^a$. Since $W_2^a\geq0$ and $W_2^a(\varFixed,\varFixed)=\norm{a}<\frac{\varepsilon^2}{8}$, we have $W_2^a(\varFixed,\varFixed)<\inf_{(\varGeneric_1,\varGeneric_2)\in X} W^a_2(\varGeneric_1,\varGeneric_2)+\frac{\varepsilon^2}{8}$.
%
By the Borwein–Preiss variational principle, there are probability measures $(\varFixed_1,\varFixed_2)\in\Omega_1\times\Omega_2$ and a sequence of probability measures $((\tilde\varGeneric_{1,j},\tilde\varGeneric_{2,j}))_{j\in\naturals}\subset\Omega_1\times\Omega_2$ so that:
\begin{itemize}
    \item 
    $
        \frac{1}{2}\wassersteinDistance{\varFixed_i}{\varFixed}{2}^2
        \leq
        \frac{1}{8}\varepsilon^2
    $
    and 
    $
        \frac{1}{2}\wassersteinDistance{\varFixed_i}{\tilde\varGeneric_{i,j}}{2}^2
        \leq
        \frac{2^{-j}}{8}\varepsilon^2
    $
    for all $j\in\naturals$ and $i\in\{1,2\}$;
    \item $(\varFixed_1,\varFixed_2)$ is a local minimizer of the function $\psi:\Omega_1\times\Omega_2\to\nonnegativeReals$ defined by {
    $\psi(\varGeneric_1,\varGeneric_2)
    =
    W_2^a(\varGeneric_1,\varGeneric_2)
    +
    \frac{1}{2}
    \sum_{j=0}^\infty
    2^{-j}
    \left(
    \wassersteinDistance{\varGeneric_1}{\tilde\varGeneric_{1,j}}{2}^2
    +
    \wassersteinDistance{\varGeneric_2}{\tilde\varGeneric_{2,j}}{2}^2
    \right)$;}

    \item $\psi(\varFixed_1,\varFixed_2)\leq W_2^a(\varFixed,\varFixed)<\frac{\varepsilon^2}{8}$.
\end{itemize}
{%
Since $\wassersteinDistance{\varFixed_2}{\varFixed}{2}\leq\tfrac\varepsilon2<r$, we have $\varFixed_2\in\closedWassersteinBall{\varFixed}{r}{2}\subseteq U$. Hence, as above, $W_2^a(\varFixed_1,\varFixed_2)>0$, i.e., $\pushforward{(\identity{}+a)}{\varFixed_1}\neq\varFixed_2$ and $c\coloneqq\wassersteinDistance{\pushforward{(\identity{}+a)}{\varFixed_1}}{\varFixed_2}{2}>0$.
Thus, the hypotheses of~\cref{lemma:lemma_fuzzy_optimality_condition} are met and \cref{lemma:lemma_fuzzy_optimality_condition}, together with $\wassersteinDistance{\varFixed_i}{\varFixed}{2}\leq\tfrac\varepsilon2<\varepsilon$ by the first bullet, yields the desired statement.}



==> elements/th_extremal_principle_title.tex <==
Extremal principle%

==> elements/th_fermat_rule_body.tex <==
If a proper functional $\objective: \Pp{2}{\reals^d} \to \realsBar$ attains a local minimum at $\varOptimal$
with $\objective(\varOptimal) \in \reals$, then
$
    \localZero{\varOptimal} \in \subgradientRegularStrong{\objective}(\varOptimal) \subseteq{} \subgradientRegular{\objective}(\varOptimal),
$
which implies $\localZero{\varOptimal} \in \subgradientStrong{\objective}(\varOptimal) \subseteq{} \subgradient{\objective}(\varOptimal)$. When $\objective$ is differentiable (resp. strongly differentiable), this condition reduces to
$
    \localZero{\varOptimal} \localEquiv{\varOptimal} \gradient{{}}{\objective}(\varOptimal)
$
{(resp. $
    \localZero{\varOptimal} \localEquiv{\varOptimal} \gradientStrong{{}}{\objective}(\varOptimal)
$)}.


==> elements/th_fermat_rule_proof.tex <==
{Since $\varOptimal$ is a local minimum, $\objective(\varGeneric) - \objective(\varOptimal)\geq 0$ for all $\varGeneric$ in a neighborhood of $\varOptimal$ of radius $r > 0$.
Recall from
\cref{proposition:prop_wasserstein_geom}\ref{item:negate_zero_is_zero} that
$\innerProduct{\localZero{\varOptimal}}{\varTangent}_{\varOptimal} = 0$ for
\emph{every} $\varTangent \in
\PpLocal{2}{\reals^d\times\reals^d}{\varOptimal}$ and, in particular, for all
$\varGeneric \in \Pp{2}{\reals^d}$ and all $\varTangent \in
\pushforward{(\projection{1}{}, \projection{2}{} -
\projection{1}{})}{\setPlans{\varOptimal}{\varGeneric}}$ induced by an
arbitrary (not necessarily optimal) plan.
Since
$\objective$ is proper with $\objective(\varOptimal) \in \reals$, the function
$h(\varGeneric) \coloneqq \min\{0, \objective(\varGeneric) -
\objective(\varOptimal)\}$ is real-valued, satisfies $\objective(\varGeneric) -
\objective(\varOptimal) \geq
\innerProduct{\localZero{\varOptimal}}{\varTangent}_{\varOptimal} +
h(\varGeneric)$ for all such $\varGeneric$ and $\varTangent$, and vanishes
whenever $\wassersteinDistance{\varOptimal}{\varGeneric}{2} < r$.
Because $\norm{\varTangent}_{\varOptimal} \geq
\wassersteinDistance{\varOptimal}{\varGeneric}{2}$ for every $\varTangent$
induced by a plan between $\varOptimal$ and $\varGeneric$, the condition
$\norm{\varTangent}_{\varOptimal} < r$ forces $h(\varGeneric) = 0$; hence
$h(\varGeneric) = \onotation{\norm{\varTangent}_{\varOptimal}}$.
As this bound holds along all plans, $\localZero{\varOptimal} \in
\subgradientRegularStrong{\objective}(\varOptimal) \subseteq
\subgradientRegular{\objective}(\varOptimal)$
(\cref{lemma:strong_vs_regular_normal_cone}\ref{item:strong_vs_regular:subgradient}),
which readily implies $\localZero{\varOptimal} \in
\subgradientStrong{\objective}(\varOptimal) \subseteq
\subgradient{\objective}(\varOptimal)$.
Finally, if $\objective$ is differentiable (resp. strongly differentiable)
at $\varOptimal$, then, by
\cref{proposition:prop_differentiability_properties}\ref{item:gradient_uniqueness}
(resp. \cref{definition:def_strong_differentiability} and
\cref{lemma:strong_vs_regular_normal_cone}\ref{item:strong_vs_regular:subgradient}),
$\gradient{{}}{\objective}(\varOptimal) \in
-\subgradientRegular{(-\objective)}(\varOptimal)$
(resp. $\gradientStrong{{}}{\objective}(\varOptimal) \in
-\subgradientRegularStrong{(-\objective)}(\varOptimal) \subseteq
-\subgradientRegular{(-\objective)}(\varOptimal)$).
Combining this with $\localZero{\varOptimal} \in
\subgradientRegular{\objective}(\varOptimal)$ and
\cref{proposition:prop_differentiability_properties}\ref{item:subdifferential-cap-superdifferential}
yields $\localZero{\varOptimal} \localEquiv{\varOptimal}
\gradient{{}}{\objective}(\varOptimal)$
(resp. $\localZero{\varOptimal} \localEquiv{\varOptimal}
\gradientStrong{{}}{\objective}(\varOptimal)$).}

==> elements/th_fermat_rule_title.tex <==
Fermat's rule in the Wasserstein space%

==> elements/th_first_order_optimality_conditions_body.tex <==

If a proper functional $\objective$ attains a local minimum at $\varOptimal \in \feasibleSet \subseteq \Pp{2}{\reals^d}$, with $\objective$ locally lower semicontinuous around $\varOptimal$ and $\objective(\varOptimal)\in\reals$, and $\feasibleSet$ \gls*{acr:snc} at $\varOptimal$ and locally closed around $\varOptimal$,
and the constraint qualification
$\subgradientHzn{\objective}(\varOptimal) \cap\left(-\normalConeStrong{\feasibleSet}{\varOptimal} \right)= \{\localZero{\varOptimal}\}$
holds, then
\begin{equation*}
    \localZero{\varOptimal} \in \subgradient{\objective}(\varOptimal) + \normalConeStrong{\feasibleSet}{\varOptimal}
     \coloneqq
     \left\{\varTangent_1 \localSum{\varTangentCoupling} \varTangent_2 \st \varTangent_1 \in \subgradient{\objective}(\varOptimal), \varTangent_2 \in \normalConeStrong{\feasibleSet}{\varOptimal}, \varTangentCoupling \in \setPlansCommonMarginal{\varTangent_1}{\varTangent_2}{1}\right\}.
\end{equation*}
{In particular, since
$\normalConeStrong{\feasibleSet}{\varOptimal} \subseteq
\normalCone{\feasibleSet}{\varOptimal}$
(\cref{lemma:strong_vs_regular_normal_cone}\ref{item:strong_vs_regular:normal}),
the constraint qualification is implied by
$\subgradientHzn{\objective}(\varOptimal) \cap\left(-\normalCone{\feasibleSet}{\varOptimal} \right)= \{\localZero{\varOptimal}\}$
and, thus, the statement holds, a fortiori, with the normal cone
$\normalCone{\feasibleSet}{\varOptimal}$ in place of the strong normal cone
$\normalConeStrong{\feasibleSet}{\varOptimal}$, both in the constraint
qualification and in the conclusion.}
When $\objective$ is differentiable (resp. strongly differentiable), the constraint qualification is not needed and the optimality condition reads
$
    -\gradient{}{\objective}(\varOptimal)\in \normalCone{\feasibleSet}{\varOptimal}
$
{(resp. $
    -\gradientStrong{}{\objective}(\varOptimal)\in \normalConeStrong{\feasibleSet}{\varOptimal}
$)}
even if $\feasibleSet$ is not \gls*{acr:snc} at $\varOptimal$.


==> elements/th_first_order_optimality_conditions_proof.tex <==
The proof strategy follows \cite[Theorem 8.15]{rockafellar2009variational}.

\emph{Step 1 (reduction to a linear program over the epigraph).} Consider in $\Pp{2}{\reals^{d+1}}$ the sets
$D = \{\boldsymbol{\varGeneric} \in \Pp{2}{\reals^d\times\reals} \st \pushforward{(\projection{1}{},\ldots,\projection{d}{})}{\boldsymbol{\varGeneric}} \in \feasibleSet\}$
and $E = \epigraph{\objective}\cap D$.\footnote{{Since
every element of $\epigraph{\objective}$ has a Dirac last marginal,
$E=\epigraph{\objective}\cap D=\epigraph{\objective}\cap\feasibleSet_e$. We work
here with $D\supsetneq\feasibleSet_e$ rather than $\feasibleSet_e$
because $D$ forces the last velocity component of its (strong) normals to vanish
and inherits \gls*{acr:snc} from $\feasibleSet$ via
\cref{proposition:prop_normal_cone_product}\ref{item:product:cylinder}, whereas
$\feasibleSet_e$ constrains only the mean of the last velocity component
(\cref{proposition:prop_normal_cone_product}\ref{item:product:delta} with
$B=\reals$); its normals may thus have arbitrary zero-mean vertical mass, so
$\feasibleSet_e$ is not \gls*{acr:snc}. This is what makes assumption~(ii) of
\cref{theorem:intersection_rule_strong} verifiable.}}
%
We have already argued that for $\varOptimal \in \feasibleSet$ to be optimal for $\objective$ over $\feasibleSet$, $\varOptimal\times\delta_{\objective(\varOptimal)}$  needs to be optimal for $l(\boldsymbol{\varGeneric}) \coloneqq \expectedValue{\boldsymbol{x} \sim \boldsymbol{\varGeneric}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{x}}}$ over $E$. We can deploy the optimality conditions in \cref{proposition:cor_first_order_optimality_conditions_diff}, since $l$ is strongly differentiable (\cref{lemma:linear_strongly_differentiable}) with gradient $\gradientStrong{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)}) = \gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)}) = (\varOptimal\times\delta_{\objective(\varOptimal)})\times\boldsymbol{\delta_{(0,\ldots,0,1)}}$.

{\emph{Step 2 (the normal cones of the epigraph and the constraint set).} To derive the result from \cref{proposition:cor_first_order_optimality_conditions_diff}, we need to characterize $\normalConeStrong{E}{\varOptimal\times\delta_{\objective(\varOptimal)}}$.
For this, we use \cref{theorem:intersection_rule_strong}.
%
To start, we note that $\epigraph{\objective}$ is locally closed by local lower semicontinuity of $\objective$ and $D$ is locally closed since $\feasibleSet$ is locally closed and the first-marginal map is continuous.
Before verifying assumptions (i) and (ii) in~\cref{theorem:intersection_rule_strong} we evaluate the strong normal cones of $\epigraph{\objective}$ and $D$.
%
For $\epigraph{\objective}$, \cref{proposition:th_subgradients_epigraphical_normals} and \cref{lemma:strong_vs_regular_normal_cone} yield
$
\normalConeStrong{\epigraph{\objective}}{\varOptimal\times\delta_{\objective(\varOptimal)}}
\subseteq
\normalCone{\epigraph{\objective}}{\varOptimal\times\delta_{\objective(\varOptimal)}}
=
G \cup H$
where
\begin{equation}
\label{eq:E0}
\begin{aligned}
    G &\coloneqq
    \biggl\{
    \boldsymbol{\varTangent} \in \PpLocal{2}{\reals^{d+1}\times\reals^{d+1}}{\varOptimal\times\delta_{\objective(\varOptimal)}} \st
    \expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}} = -\lambda < 0,
    \frac{1}{\lambda}\pushforward{T}{\boldsymbol{\varTangent}} \in \subgradient{\objective}(\varOptimal)
    \biggr\}\\
    H &\coloneqq
    \biggl\{
    \boldsymbol{\varTangent} \in \PpLocal{2}{\reals^{d+1}\times\reals^{d+1}}{\varOptimal\times\delta_{\objective(\varOptimal)}} \st
    \expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}} = 0,
    \pushforward{T}{\boldsymbol{\varTangent}} \in \subgradientHzn{\objective}(\varOptimal)
    \biggr\}.
\end{aligned}
\end{equation}
{For the strong normal cone to $D$, we use
\cref{proposition:prop_normal_cone_product}\ref{item:product:cylinder} (with
the unconstrained factor in the last coordinate; the relabeling of the
coordinates is immaterial) to obtain}
$
\normalConeStrong{D}{\varOptimal\times\delta_{\objective(\varOptimal)}}
\subseteq
F$
where
\begin{equation*}
    F
    \coloneqq
    \{
    \boldsymbol{\varTangent} \in \PpLocal{2}{\reals^{d+1}\times\reals^{d+1}}{\varOptimal\times\delta_{\objective(\varOptimal)}} \st
    \pushforward{T}{\boldsymbol{\varTangent}} \in \normalConeStrong{\feasibleSet}{\varOptimal},
    \pushforward{(\projection{d+1}{},\projection{2d+2}{})}{\boldsymbol{\varTangent}}
    =
    \localZero{\delta_{\objective(\varOptimal)}}
    \}.
\end{equation*}}


{\emph{Step 3 (verifying the intersection rule).} We now check assumption (i) of~\cref{theorem:intersection_rule_strong}, namely that $\normalConeStrong{\epigraph{\objective}}{\varOptimal\times\delta_{\objective(\varOptimal)}}\cap\left(-\normalConeStrong{D}{\varOptimal\times\delta_{\objective(\varOptimal)}}\right) = \{\localZero{\varOptimal\times\delta_{\objective(\varOptimal)}}\}$.
{By Step 2 and \eqref{eq:E0},
$\normalConeStrong{\epigraph{\objective}}{\varOptimal\times\delta_{\objective(\varOptimal)}}\cap\left(-\normalConeStrong{D}{\varOptimal\times\delta_{\objective(\varOptimal)}}\right)
\subseteq (G\cup H)\cap(-F)$.}
We observe that $G\cap(-F)=\emptyset$. Indeed, every $\boldsymbol{\varTangent}\in-F$ satisfies $\pushforward{(\projection{d+1}{},\projection{2d+2}{})}{\boldsymbol{\varTangent}}=\localZero{\delta_{\objective(\varOptimal)}}$, so $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}}=0$, whereas every element of $G$ satisfies $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}}<0$.
Thus, $(G\cup H)\cap(-F) = H \cap(-F)$.
%
Let $\boldsymbol{\varTangent}\in H\cap(-F)$.
Since membership in $H$ gives $\pushforward{T}{\boldsymbol{\varTangent}}\in\subgradientHzn{\objective}(\varOptimal)$ and membership in $-F$ gives $\pushforward{T}{\boldsymbol{\varTangent}}\in-\normalConeStrong{\feasibleSet}{\varOptimal}$, the constraint qualification $\subgradientHzn{\objective}(\varOptimal)\cap\left(-\normalConeStrong{\feasibleSet}{\varOptimal}\right)=\{\localZero{\varOptimal}\}$ forces $\pushforward{T}{\boldsymbol{\varTangent}}=\localZero{\varOptimal}$. Membership in $-F$ also gives $\pushforward{(\projection{d+1}{},\projection{2d+2}{})}{\boldsymbol{\varTangent}}=\localZero{\delta_{\objective(\varOptimal)}}$ and so $\boldsymbol{\varTangent}=\localZero{\varOptimal\times\delta_{\objective(\varOptimal)}}$.
Consequently, $H\cap (-F)=\{\localZero{\varOptimal\times\delta_{\objective(\varOptimal)}}\}$, whence, since the zero variation is a strong regular normal to every set at every point (its pairing with any variation vanishes, and it belongs to the tangent cone), $\normalConeStrong{\epigraph{\objective}}{\varOptimal\times\delta_{\objective(\varOptimal)}}\cap\left(-\normalConeStrong{D}{\varOptimal\times\delta_{\objective(\varOptimal)}}\right)=\{\localZero{\varOptimal\times\delta_{\objective(\varOptimal)}}\}$, which is assumption (i).
%
It remains to check assumption (ii): $D$ is \gls*{acr:snc} in virtue of~\cref{proposition:prop_normal_cone_product}\ref{item:product:cylinder}, as $\feasibleSet$ is \gls*{acr:snc} by assumption. Thus,~\cref{theorem:intersection_rule_strong} yields the inclusion
\begin{equation}\label{proof:first_order_optimality:decomposition_normal_cone_E}
\normalConeStrong{E}{\varOptimal\times\delta_{\objective(\varOptimal)}}
\subseteq
\normalConeStrong{D}{\varOptimal\times\delta_{\objective(\varOptimal)}}
+
\normalConeStrong{\epigraph{\objective}}{\varOptimal\times\delta_{\objective(\varOptimal)}}
\subseteq
F + (G \cup H).
\end{equation}}

\emph{Step 4 (ruling out the $F+H$ decomposition).} In light of \cref{proposition:cor_first_order_optimality_conditions_diff}, {we need to show that
$-\gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)}) \in \normalConeStrong{E}{\varOptimal\times\delta_{\objective(\varOptimal)}}$ implies
$\localZero{\varOptimal} \in \subgradient{\objective}(\varOptimal) + \normalConeStrong{\feasibleSet}{\varOptimal}$.}
%
{Given~\eqref{proof:first_order_optimality:decomposition_normal_cone_E}, there are two possibilities:
(a) there are $\boldsymbol{\varTangent_F} \in F, \boldsymbol{\varTangent_H} \in H$, and $\boldsymbol{\varTangentCoupling} \in \setPlansCommonMarginal{\boldsymbol{\varTangent_F}}{\boldsymbol{\varTangent_H}}{1}$ so that $\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_H} = -\gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)})$ or
(b) there are $\boldsymbol{\varTangent_F} \in F, \boldsymbol{\varTangent_G} \in G$, and $\boldsymbol{\varTangentCoupling} \in \setPlansCommonMarginal{\boldsymbol{\varTangent_F}}{\boldsymbol{\varTangent_G}}{1}$ so that $\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_G} = -\gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)})$. We now show that the former is not possible.}
%
To this end, we observe that, for all $\boldsymbol{\varTangent_F} \in F, \boldsymbol{\varTangent_H} \in H$, there is no $\boldsymbol{\varTangentCoupling} \in \setPlansCommonMarginal{\boldsymbol{\varTangent_F}}{\boldsymbol{\varTangent_H}}{1}$ so that $\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_H} = -\gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)})$. This follows by contradiction accounting for the linearity of the expected value:
\begin{align*}
\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim (\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_H})}{\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}}
&=
\int_{\reals^{d+1}\times\reals^{d+1}}
\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}
\d(\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_H})(\boldsymbol{x}, \boldsymbol{\varTangentReals})
\\&=
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}
\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals_F} + \boldsymbol{\varTangentReals_H}}
\d\boldsymbol{\varTangentCoupling}(\boldsymbol{x}, \boldsymbol{\varTangentReals_F}, \boldsymbol{\varTangentReals_H})
\\&=
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}
\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals_F}}
\d\boldsymbol{\varTangentCoupling}(\boldsymbol{x}, \boldsymbol{\varTangentReals_F}, \boldsymbol{\varTangentReals_H})
\\&\qquad+
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}
\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals_H}}
\d\boldsymbol{\varTangentCoupling}(\boldsymbol{x}, \boldsymbol{\varTangentReals_F}, \boldsymbol{\varTangentReals_H})
\\&=
\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent_F}}{\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}}
\\&\qquad+
\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent_H}}{\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}}
\\&=0
\neq-1
=
\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim -\gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)})}{\innerProduct{\boldsymbol{(0, \ldots, 0, 1)}}{\boldsymbol{\varTangentReals}}}.
\end{align*}
We thus conclude that $-\gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)}) \in \normalConeStrong{E}{\varOptimal\times\delta_{\objective(\varOptimal)}}$ implies that $\boldsymbol{\varTangent_F} \in F, \boldsymbol{\varTangent_G} \in G$ and $\boldsymbol{\varTangentCoupling} \in \setPlansCommonMarginal{\boldsymbol{\varTangent_F}}{\boldsymbol{\varTangent_G}}{1}$ exist so that $-\gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)}) = \boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_G}$.

\emph{Step 5 (deriving the optimality condition).}
%
Since $\pushforward{T}{\gradient{}{l}(\varOptimal\times\delta_{\objective(\varOptimal)})}=\localZero{\varOptimal}$, it necessarily holds $\localZero{\varOptimal} = \pushforward{T}{(\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_G})}$.
%
We now show that $\pushforward{T}{(\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_G})} = \pushforward{T}{\boldsymbol{\varTangent_F}} \localSum{\pushforward{\hat{T}}{\boldsymbol{\varTangentCoupling}}} \pushforward{T}{\boldsymbol{\varTangent_G}}$, where $\hat{T}: \reals^{d+1}\times\reals^{d+1}\times\reals^{d+1} \to \reals^{d}\times\reals^{d}\times\reals^{d}$ is defined as
$
\hat{T}(\boldsymbol{x}, \boldsymbol{\varTangentReals_1}, \boldsymbol{\varTangentReals_2})
=
((\projection{1}{}, \ldots, \projection{d}{})(\boldsymbol{x}), (\projection{1}{}, \ldots, \projection{d}{})(\boldsymbol{\varTangentReals_1}), (\projection{1}{}, \ldots, \projection{d}{})(\boldsymbol{\varTangentReals_2}))$. Indeed, for all $\phi \in \Cb{\reals^d\times\reals^d}$,
\begin{align*}
&\int_{\reals^{d}\times\reals^{d}}
\phi(x^\ast, \varTangentReals)\d(\pushforward{T}{(\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_G})})(x^\ast, \varTangentReals)
\\&=
\int_{\reals^{d+1}\times\reals^{d+1}}
\phi(T(\boldsymbol{x^\ast}, \boldsymbol{\varTangentReals}))\d(\boldsymbol{\varTangent_F} \localSum{\boldsymbol{\varTangentCoupling}} \boldsymbol{\varTangent_G})(\boldsymbol{x^\ast}, \boldsymbol{\varTangentReals})
\\&=
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}
\phi(T(\boldsymbol{x^\ast}, \boldsymbol{\varTangentReals_1} + \boldsymbol{\varTangentReals_2}))\d\boldsymbol{\varTangentCoupling}(\boldsymbol{x^\ast}, \boldsymbol{\varTangentReals_1}, \boldsymbol{\varTangentReals_2})
\\&=
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}
\phi((\projection{1}{}, \ldots, \projection{d}{})(\boldsymbol{x^\ast}), (\projection{1}{}, \ldots, \projection{d}{})(\boldsymbol{\varTangentReals_1} + \boldsymbol{\varTangentReals_2}))\d\boldsymbol{\varTangentCoupling}(\boldsymbol{x^\ast}, \boldsymbol{\varTangentReals_1}, \boldsymbol{\varTangentReals_2})
\\&=
\int_{\reals^{d+1}\times\reals^{d+1}\times\reals^{d+1}}
\phi((\projection{1}{}, \ldots, \projection{d}{})(\boldsymbol{x^\ast}),
(\projection{1}{}, \ldots, \projection{d}{})(\boldsymbol{\varTangentReals_1}) + (\projection{1}{}, \ldots, \projection{d}{})(\boldsymbol{\varTangentReals_2}))
\d\boldsymbol{\varTangentCoupling}(\boldsymbol{x^\ast}, \boldsymbol{\varTangentReals_1}, \boldsymbol{\varTangentReals_2})
\\&=
\int_{\reals^{d}\times\reals^{d}\times\reals^{d}}
\phi(x^\ast, \varTangentReals_1 + \varTangentReals_2)
\d(\pushforward{\hat{T}}{\boldsymbol{\varTangentCoupling}})(x^\ast, \varTangentReals_1, \varTangentReals_2)
\\&=
{\int_{\reals^{d}\times\reals^{d}}
\phi(x^\ast, \varTangentReals)
\d(\pushforward{T}{\boldsymbol{\varTangent_F}} \localSum{\pushforward{\hat{T}}{\boldsymbol{\varTangentCoupling}}} \pushforward{T}{\boldsymbol{\varTangent_G}})(x^\ast, \varTangentReals).}
\end{align*}
{The structure of $F$ and $G$ implies that $\pushforward{T}{\boldsymbol{\varTangent_F}} \in \normalConeStrong{\feasibleSet}{\varOptimal}$ and $\frac{1}{\lambda}\pushforward{T}{\boldsymbol{\varTangent_G}} \in \subgradient{\objective}(\varOptimal)$ for some $\lambda>0$.
%
Thus, $\localZero{\varOptimal}\in\normalConeStrong{\feasibleSet}{\varOptimal} + \lambda\subgradient{\objective}(\varOptimal)$.
Since the strong normal cone is a cone (the defining inequality of \cref{definition:def_fuzzy_normal_cone} is positively homogeneous in the normal, and the velocity scaling $\pushforward{(\projection{1}{}, \lambda\projection{2}{})}{}$ is Lipschitz with respect to $\wassersteinDistance{}{}{2}$, so positive scaling is also preserved along the limits), we can scale by $\frac{1}{\lambda}$ and obtain $\localZero{\varOptimal}\in\normalConeStrong{\feasibleSet}{\varOptimal} + \subgradient{\objective}(\varOptimal)$, proving the statement.}

\emph{Step 6 (the (strongly) differentiable case).}
%
To conclude, if $\objective$ is differentiable (resp. strongly differentiable), then~\cref{proposition:cor_first_order_optimality_conditions_diff}\ref{item:cor_first_order:regular} (resp. \cref{proposition:cor_first_order_optimality_conditions_diff}\ref{item:cor_first_order:strong}) directly establishes the result.


==> elements/th_subgradients_epigraphical_normals_body.tex <==
Let $\objective: \Pp{2}{\reals^d} \to \realsBar$ and $\varFixed \in \Pp{2}{\reals^d}$ at which $\objective(\varFixed) \in \reals$. With $T$ as in \eqref{equation:extraction-map-epigraph}, {for
$\boldsymbol{\varTangent}\in\Pp{2}{\reals^{d+1}\times\reals^{d+1}}$ with
$\pushforward{\projection{1}{}}{\boldsymbol{\varTangent}}=\varFixed\times\delta_{\objective(\varFixed)}$}
we have that $\boldsymbol{\varTangent} \in
\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$ if and only if either
\begin{enumerate}[leftmargin=*]
    \item $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = -\lambda, \lambda > 0$ and $\frac{1}{\lambda}\pushforward{T}{\boldsymbol{\varTangent}} \in \subgradient{\objective}(\varFixed)$; or
    \item $\expectedValue{(\boldsymbol{x}, \boldsymbol{\varTangentReals}) \sim \boldsymbol{\varTangent}}{\innerProduct{(0, \ldots, 0, 1)}{\boldsymbol{\varTangentReals}}} = 0$ and $\pushforward{T}{\boldsymbol{\varTangent}} \in \subgradientHzn{\objective}(\varFixed)$.
\end{enumerate}


==> elements/th_subgradients_epigraphical_normals_proof.tex <==
We prove necessity first (\emph{Step 1}), and then sufficiency
(\emph{Steps 2--4}).

\emph{Step 1 (necessity).} Follows combining the necessary condition on epigraphical normals in \cref{proposition:prop_epigraph_normal_tangent} with the general normal cone being a cone and \cref{proposition:prop_subgradients_epigraphical_normals,definition:def_sub_sup_differentiability_horizon}.
{In detail, let
$\boldsymbol{\varTangent}\in\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$
and set
$\lambda\coloneqq-\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangent}}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}$,
so that $\lambda\geq0$ by \cref{proposition:prop_epigraph_normal_tangent}. If
$\lambda>0$, since the general normal cone is a cone (cf.
\cref{proposition:prop_normal_tangent_cones}),
$\frac{1}{\lambda}\boldsymbol{\varTangent}\in\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$,
and its last velocity component has expectation $-1$. Then,
\cref{proposition:prop_subgradients_epigraphical_normals} gives
$\frac{1}{\lambda}\pushforward{T}{\boldsymbol{\varTangent}}=\pushforward{T}{\left(\frac{1}{\lambda}\boldsymbol{\varTangent}\right)}\in\subgradient{\objective}(\varFixed)$,
i.e., condition (i); here, scaling and $\pushforward{T}{\cdot}$ commute since,
by \cref{definition:def_almost_linear_structure_wass}, scaling acts on the
velocities only, while $T$ drops the last component of positions and
velocities alike. If instead $\lambda=0$, then $\boldsymbol{\varTangent}$
itself certifies
$\pushforward{T}{\boldsymbol{\varTangent}}\in\subgradientHzn{\objective}(\varFixed)$
by \cref{definition:def_sub_sup_differentiability_horizon}, i.e., condition
(ii).}

{We prove sufficiency in four steps.
The difficulty specific to the
Wasserstein setting is that $T$ discards the last velocity component, so
conditions (i) and (ii) constrain its law only through its
expectation. The
geometry of the deterministic last coordinate is handled by
\cref{lemma:lemma_deterministic_coordinate}; building on it, we first show
that the regular normal cone inequality is insensitive to any further
information carried by the last velocity component (\emph{Step 2}), and then
construct regular epigraphical normals converging to
$\boldsymbol{\varTangent}$ (\emph{Steps 3 and 4}).}

{\emph{Step 2 (the regular normal cone only sees the
expectation of the last velocity component).} Let
$\varGeneric\times\delta_b\in\epigraph{\objective}$, let
$\boldsymbol{\tilde{\varTangent}}\in\normalConeRegular{\epigraph{\objective}}{\varGeneric\times\delta_b}$,
and let $\boldsymbol{\varTangentFixed}$ be a variation at
$\varGeneric\times\delta_b$ with
$\pushforward{T}{\boldsymbol{\varTangentFixed}}=\pushforward{T}{\boldsymbol{\tilde{\varTangent}}}$
whose last velocity component has the same expectation as that of
$\boldsymbol{\tilde{\varTangent}}$. We claim that
$\boldsymbol{\varTangentFixed}\in\normalConeRegular{\epigraph{\objective}}{\varGeneric\times\delta_b}$.
First,
$\boldsymbol{\tilde{\varTangent}}\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varGeneric\times\delta_b}$
by \cref{definition:def_normal_cone}, so
$\pushforward{T}{\boldsymbol{\tilde{\varTangent}}}\in\tangentCone{\Pp{2}{\reals^d}}{\varGeneric}$
by
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}.
Since
$\pushforward{T}{\boldsymbol{\varTangentFixed}}=\pushforward{T}{\boldsymbol{\tilde{\varTangent}}}$,
$\boldsymbol{\varTangentFixed}\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varGeneric\times\delta_b}$.}
{Next, let
$\varGeneric'\times\delta_\beta\in\epigraph{\objective}$ and
$\boldsymbol{\varTangentOther}\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlansOptimal{\varGeneric\times\delta_b}{\varGeneric'\times\delta_\beta}}$.
By
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport},
the last velocity component of $\boldsymbol{\varTangentOther}$ equals
$\beta-b$ almost everywhere and
$\varTangentOther\coloneqq\pushforward{T}{\boldsymbol{\varTangentOther}}\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlansOptimal{\varGeneric}{\varGeneric'}}$,
so that
$\norm{\varTangentOther}_{\varGeneric}=\wassersteinDistance{\varGeneric}{\varGeneric'}{2}$
because $\varTangentOther$ is induced by an optimal transport plan; by
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting},
$\norm{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_b}^2=\norm{\varTangentOther}_{\varGeneric}^2+\abs{\beta-b}^2$.
Moreover, for every variation $\boldsymbol{\varTangentFixed}'$ at
$\varGeneric\times\delta_b$,
\eqref{eq:deterministic_coordinate:splitting} gives
\begin{equation*}
\innerProduct{\boldsymbol{\varTangentFixed}'}{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_b}
=
\innerProduct{\pushforward{T}{\boldsymbol{\varTangentFixed}'}}{\varTangentOther}_{\varGeneric}
+
(\beta-b)\expectedValue{(\boldsymbol{x},\boldsymbol{\varTangentReals})\sim\boldsymbol{\varTangentFixed}'}{\innerProduct{(0,\ldots,0,1)}{\boldsymbol{\varTangentReals}}}.
\end{equation*}}
{The right-hand side of
\eqref{eq:deterministic_coordinate:splitting} takes the same value for
$\boldsymbol{\varTangentFixed}'=\boldsymbol{\varTangentFixed}$ and for
$\boldsymbol{\varTangentFixed}'=\boldsymbol{\tilde{\varTangent}}$. Therefore,
$\innerProduct{\boldsymbol{\varTangentFixed}}{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_b}=\innerProduct{\boldsymbol{\tilde{\varTangent}}}{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_b}\leq\onotation{\norm{\boldsymbol{\varTangentOther}}_{\varGeneric\times\delta_b}}$,
where the inequality holds because
$\boldsymbol{\tilde{\varTangent}}\in\normalConeRegular{\epigraph{\objective}}{\varGeneric\times\delta_b}$.
By \cref{definition:def_normal_cone}, we conclude
$\boldsymbol{\varTangentFixed}\in\normalConeRegular{\epigraph{\objective}}{\varGeneric\times\delta_b}$.}

{\emph{Step 3 (sufficiency: an approximating sequence of
regular normals).} Suppose now that $\boldsymbol{\varTangent}$ satisfies
condition (i) (with $\lambda>0$) or condition
(ii) (with $\lambda\coloneqq0$). We
claim that in both cases there exist
$\varGeneric_n\times\delta_{\beta_n}\in\epigraph{\objective}$ and
$\boldsymbol{\tilde{\varTangent}}_n\in\normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\beta_n}}$
whose last velocity component has expectation $-\lambda_n$, such that
\begin{equation}
\label{eq:epigraphical_normals:approximants}
\varGeneric_n\times\delta_{\beta_n}\convergenceWasserstein\varFixed\times\delta_{\objective(\varFixed)},
\qquad
\pushforward{T}{\boldsymbol{\tilde{\varTangent}}_n}\convergenceWasserstein\pushforward{T}{\boldsymbol{\varTangent}},
\qquad
\lambda_n\to\lambda.
\end{equation}
Under condition (ii),
\cref{definition:def_sub_sup_differentiability_horizon} provides
$\boldsymbol{\varTangent}'\in\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$
with
$\pushforward{T}{\boldsymbol{\varTangent}'}=\pushforward{T}{\boldsymbol{\varTangent}}$
and last velocity component with zero expectation, and
\cref{definition:def_normal_cone} provides
$\varGeneric_n\times\delta_{\beta_n}\in\epigraph{\objective}$ with
$\varGeneric_n\times\delta_{\beta_n}\convergenceWasserstein\varFixed\times\delta_{\objective(\varFixed)}$
and
$\boldsymbol{\tilde{\varTangent}}_n\in\normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\beta_n}}$
with
$\boldsymbol{\tilde{\varTangent}}_n\convergenceWasserstein\boldsymbol{\varTangent}'$.
Then, \eqref{eq:epigraphical_normals:approximants} holds: the second
convergence because $T$ is $1$-Lipschitz (cf.
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}),
and the third by the continuity of the expected value in Wasserstein.}
{Under condition (i), by
\cref{definition:def_sub_sup_differentiability}\ref{item:subgradient}, there
are $\varGeneric_n\convergenceWasserstein\varFixed$ with
$\objective(\varGeneric_n)\to\objective(\varFixed)$ (in particular,
$\objective(\varGeneric_n)\in\reals$ and
$\varGeneric_n\times\delta_{\objective(\varGeneric_n)}\in\epigraph{\objective}$)
and $\varTangent_n\in\subgradientRegular{\objective}(\varGeneric_n)$ with
$\varTangent_n\convergenceWasserstein\frac{1}{\lambda}\pushforward{T}{\boldsymbol{\varTangent}}$.
Set $\beta_n\coloneqq\objective(\varGeneric_n)$ and let
$\boldsymbol{\tilde{\varTangent}}_n$ be the law of
$((x,\objective(\varGeneric_n)),(\lambda\varTangentReals,-\lambda))$ for
$(x,\varTangentReals)\sim\varTangent_n$; i.e., the variation at
$\varGeneric_n\times\delta_{\objective(\varGeneric_n)}$ obtained by scaling
$\varTangent_n$ by $\lambda$ and appending the deterministic last velocity
component $-\lambda$, so that $\lambda_n=\lambda$ for all $n$. Then,
\eqref{eq:epigraphical_normals:approximants} holds: the first convergence
since
$\wassersteinDistance{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}{\varFixed\times\delta_{\objective(\varFixed)}}{2}^2=\wassersteinDistance{\varGeneric_n}{\varFixed}{2}^2+\abs{\objective(\varGeneric_n)-\objective(\varFixed)}^2\to0$
(cf.~\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:transport}),
and the second from
$\pushforward{T}{\boldsymbol{\tilde{\varTangent}}_n}=\lambda\varTangent_n$,
since scaling the velocity components by $\lambda$ is
$\max\{1,\lambda\}$-Lipschitz with respect to
$\wassersteinDistance{\cdot}{\cdot}{2}$. It remains to show that
$\boldsymbol{\tilde{\varTangent}}_n\in\normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}$.
Since the regular normal cone is a cone (cf.
\cref{proposition:prop_normal_tangent_cones}) and
$\boldsymbol{\tilde{\varTangent}}_n=\lambda\boldsymbol{\hat{\varTangent}}_n$,
with $\boldsymbol{\hat{\varTangent}}_n$ the law of
$((x,\objective(\varGeneric_n)),(\varTangentReals,-1))$ for
$(x,\varTangentReals)\sim\varTangent_n$, it suffices to show that
$\boldsymbol{\hat{\varTangent}}_n\in\normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}$;
i.e., that regular subgradients lift to regular epigraphical normals with
deterministic last velocity component $-1$.}
{For the tangency requirement in
\cref{definition:def_normal_cone}:
$\pushforward{T}{\boldsymbol{\hat{\varTangent}}_n}=\varTangent_n\in\tangentCone{\Pp{2}{\reals^d}}{\varGeneric_n}$
by
\cref{definition:def_sub_sup_differentiability}\ref{item:subgradient:regular},
so
$\boldsymbol{\hat{\varTangent}}_n\in\tangentCone{\Pp{2}{\reals^{d+1}}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}$
by
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:tangency}.
For the inequality, fix $\varepsilon>0$. Unpacking the
$\onotation{\cdot}$ notation in
\cref{definition:def_sub_sup_differentiability}\ref{item:subgradient:regular},
there exists $\delta>0$ such that
$\innerProduct{\varTangent_n}{\varTangentOther}_{\varGeneric_n}\leq\objective(\varGeneric')-\objective(\varGeneric_n)+\varepsilon\wassersteinDistance{\varGeneric_n}{\varGeneric'}{2}$
for all $\varGeneric'\in\Pp{2}{\reals^d}$ with
$\wassersteinDistance{\varGeneric_n}{\varGeneric'}{2}<\delta$ and all
$\varTangentOther\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlansOptimal{\varGeneric_n}{\varGeneric'}}$.
Consider now any $\varGeneric'\times\delta_\beta\in\epigraph{\objective}$ and
$\boldsymbol{\varTangentOther}\in\pushforward{(\projection{1}{},\projection{2}{}-\projection{1}{})}{\setPlansOptimal{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}{\varGeneric'\times\delta_\beta}}$
with
$\norm{\boldsymbol{\varTangentOther}}_{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}<\delta$.
With $\varTangentOther\coloneqq\pushforward{T}{\boldsymbol{\varTangentOther}}$
as in \emph{Step 2}, we have
$\wassersteinDistance{\varGeneric_n}{\varGeneric'}{2}=\norm{\varTangentOther}_{\varGeneric_n}\leq\norm{\boldsymbol{\varTangentOther}}_{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}<\delta$
(cf.
\cref{lemma:lemma_deterministic_coordinate}\ref{item:deterministic_coordinate:splitting})
and, by \eqref{eq:deterministic_coordinate:splitting} together with
$\beta\geq\objective(\varGeneric')$,
\begin{align*}
\innerProduct{\boldsymbol{\hat{\varTangent}}_n}{\boldsymbol{\varTangentOther}}_{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}
&=
\innerProduct{\varTangent_n}{\varTangentOther}_{\varGeneric_n}-(\beta-\objective(\varGeneric_n))
\\&\leq
\objective(\varGeneric')-\beta+\varepsilon\wassersteinDistance{\varGeneric_n}{\varGeneric'}{2}
\leq
\varepsilon\norm{\boldsymbol{\varTangentOther}}_{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}.
\end{align*}
As $\varepsilon>0$ was arbitrary, the inequality in
\cref{definition:def_normal_cone} holds, and
$\boldsymbol{\hat{\varTangent}}_n\in\normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\objective(\varGeneric_n)}}$.}

{\emph{Step 4 (sufficiency: conclusion).} Loosely speaking, we
now transport the conditional law of the last velocity component of
$\boldsymbol{\varTangent}$ onto the approximating regular normals of
\emph{Step 3} and correct its expectation by a vanishing shift; \emph{Step 2}
guarantees that the resulting variations are still regular normals. Let
$\{\boldsymbol{\varTangent}_{(x,\varTangentReals)}\}_{(x,\varTangentReals)\in\reals^d\times\reals^d}\subseteq\Pp{2}{\reals}$
be the disintegration with respect to $(x,\varTangentReals)$ of the law of
$((x,\varTangentReals),u)$ under $\boldsymbol{\varTangent}$, where
$(x,\varTangentReals)\sim\pushforward{T}{\boldsymbol{\varTangent}}$ and
$u\in\reals$ denotes the last velocity component (cf.
\cite[Theorem 5.3.1]{ambrosio2005gradient}). For each $n$, let
$\varPlanGeneric_n\in\setPlansOptimal{\pushforward{T}{\boldsymbol{\tilde{\varTangent}}_n}}{\pushforward{T}{\boldsymbol{\varTangent}}}$,
define $\hat{\varPlanGeneric}_n$ via
$\d\hat{\varPlanGeneric}_n((x_n,\varTangentReals_n),(x,\varTangentReals),u)\coloneqq\d\boldsymbol{\varTangent}_{(x,\varTangentReals)}(u)\d\varPlanGeneric_n((x_n,\varTangentReals_n),(x,\varTangentReals))$,
and let $\boldsymbol{\varTangent}_n$ be the law of
$((x_n,\beta_n),(\varTangentReals_n,u+\lambda-\lambda_n))$ under
$\hat{\varPlanGeneric}_n$. Then, $\boldsymbol{\varTangent}_n$ is a variation
at $\varGeneric_n\times\delta_{\beta_n}$ with
$\pushforward{T}{\boldsymbol{\varTangent}_n}=\pushforward{T}{\boldsymbol{\tilde{\varTangent}}_n}$,
and its last velocity component has expectation
$-\lambda+(\lambda-\lambda_n)=-\lambda_n$, the same as that of
$\boldsymbol{\tilde{\varTangent}}_n$. By \emph{Step 2},
$\boldsymbol{\varTangent}_n\in\normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\beta_n}}$.
Moreover, the law of
$\bigl(((x_n,\beta_n),(\varTangentReals_n,u+\lambda-\lambda_n)),((x,\objective(\varFixed)),(\varTangentReals,u))\bigr)$
under $\hat{\varPlanGeneric}_n$ is a transport plan between
$\boldsymbol{\varTangent}_n$ and $\boldsymbol{\varTangent}$, where for the
second marginal we used that the law of
$((x,\objective(\varFixed)),(\varTangentReals,u))$ under
$\hat{\varPlanGeneric}_n$ reconstructs $\boldsymbol{\varTangent}$, since
$(x,\varTangentReals)\sim\pushforward{T}{\boldsymbol{\varTangent}}$ and
$u\sim\boldsymbol{\varTangent}_{(x,\varTangentReals)}$. Thus,
\begin{equation*}
\wassersteinDistance{\boldsymbol{\varTangent}_n}{\boldsymbol{\varTangent}}{2}^2
\leq
\wassersteinDistance{\pushforward{T}{\boldsymbol{\tilde{\varTangent}}_n}}{\pushforward{T}{\boldsymbol{\varTangent}}}{2}^2
+
\abs{\beta_n-\objective(\varFixed)}^2
+
\abs{\lambda-\lambda_n}^2,
\end{equation*}
which vanishes as $n\to\infty$ by
\eqref{eq:epigraphical_normals:approximants}. Hence,
$\boldsymbol{\varTangent}_n\convergenceWasserstein\boldsymbol{\varTangent}$
with
$\boldsymbol{\varTangent}_n\in\normalConeRegular{\epigraph{\objective}}{\varGeneric_n\times\delta_{\beta_n}}$
and
$\varGeneric_n\times\delta_{\beta_n}\in\epigraph{\objective}$ converging to
$\varFixed\times\delta_{\objective(\varFixed)}$, and
\cref{definition:def_normal_cone} yields
$\boldsymbol{\varTangent}\in\normalCone{\epigraph{\objective}}{\varFixed\times\delta_{\objective(\varFixed)}}$,
concluding the proof.}


==> elements/th_subgradients_epigraphical_normals_title.tex <==
Subgradients and epigraphical normals - cont'd%

==> utils/tikzart.tex <==
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{shapes}

\RequirePackage{tikz}
\usetikzlibrary{patterns}

\pgfplotsset{compat=newest}
\usepgfplotslibrary{colormaps}

\definecolor{bluetteLight}{RGB}{173,216,230}
\definecolor{bluetteDark}{RGB}{0,105,148} 
\definecolor{redLight}{RGB}{240,128,128}
\definecolor{redDark}{RGB}{128,0,0}
\definecolor{orangeLight}{RGB}{255,200,0}
\definecolor{orangeDark}{RGB}{255,140,0}
\definecolor{ETHblue}{RGB}{33,92,175}% blue
\definecolor{ETHpetrol}{RGB}{0,120,148}	% petrol
\definecolor{ETHgreen}{RGB}{98,115,19}% green
\definecolor{ETHbronze}{RGB}{142,103,19}% bronze
\definecolor{ETHred}{RGB}{183,53,45}% red
\definecolor{ETHpurple}{RGB}{163,7,116}	% purple
\definecolor{ETHgray}{RGB}{111,111,111}% gray

\pgfmathdeclarefunction{densitystart}{0}{%
  \pgfmathparse{1/(0.5 * sqrt(2*pi))*exp(-((x +1)^2)/(2 * 0.25))}%
}

\pgfmathdeclarefunction{densityend}{0}{%
    \pgfmathparse{1/(sqrt(2*pi))*exp(-((x - 2)^2)/2)}%
}

\pgfmathdeclarefunction{densityvertical}{1}{%
    \pgfmathparse{#1/100 * (1/(0.5 * sqrt(2*pi))*exp(-((x +1)^2)/(2 * 0.25))) + (1 - #1/100) * (1/(sqrt(2*pi))*exp(-((x - 2)^2)/2)) }%
}

\pgfmathdeclarefunction{densityhorizontal}{1}{%
    \pgfmathparse{1/(((#1 / 100 * (0.5) + (1 - #1/100) * 1)) * sqrt(2*pi))*exp(-((x - (#1 / 100 * (-1) + (1 - #1/100) * 2))^2)/(2 * ((#1 / 100 * (0.5) + (1 - #1/100) * 1))^2)}%
}


\tikzset{remblais/.style={circle, fill=ETHred, inner sep=0pt,minimum size=7pt}}
\tikzset{deblais/.style={fill=ETHblue,minimum size=3pt}}
\tikzset{variation/.style={draw=ETHbronze,-latex,thick}}

% Define a command to create a square with a pattern based on value
\newcommand{\patternedsquare}[3]{% position, value, max value
    \pgfmathsetmacro{\intensity}{#2/#3}
    \definecolor{currentcolor}{rgb}{0.6, 0.7, 1-\intensity}
    \node[draw, fill=currentcolor, minimum size=1cm] at (#1) {};
}

% Define a command to create a circle with a pattern based on value
\newcommand{\patternedcircle}[3]{% position, value, max value
    \pgfmathsetmacro{\intensity}{#2/#3}
    \definecolor{currentcolor}{rgb}{1-\intensity, 0.3, 0.3}
    \node[draw, fill=currentcolor, circle, minimum size=1cm] at (#1) {};
}

%OT
\newcommand{\transportMapContinuous}[2]{
    % raw material
\draw (0,0) -- (4,0);
\draw[fill=gray!25] (0.25,0) to [curve through={(.5,-0.1) . . (1,-0.75) . . (1.5,-0.5) . . (2,-.45) . . (2.75,-1) . . (3.5,-0.25)}] (3.75,0) -- cycle;
\node (nu) at (2,.25) {\ifstrempty{#1}{$\mu$}{#1}};

% construction
\draw (5,0) -- (8,0);
\draw[fill=gray!25] (5.25,0) -- (5.25,1.5) -- (5.75,1.5) -- (5.75,1) -- (6.5,1) -- (6.5,2) -- (7.25,1.5) -- (7.75,1.5) -- (7.75,0) -- cycle;
\node (nu) at (7,-.3) {\ifstrempty{#2}{$\nu$}{#2}};

% transport map
\draw[draw=blue, thick, -latex] (3,-.25) to [bend left] node[midway,above left] {$T(x)$} (6,.5);
}
\newcommand{\transportMapDiscrete}{
    % sources
    \node[deblais] (s1) at (0,0) {};
    \node[deblais] (s2) at (3,2) {};
    \node[deblais] (s3) at (2,-1) {};
    \node[deblais] (s4) at (3,.5) {};
    
    % destinatinons
    \node[remblais] (d1) at (0,2) {};
    \node[remblais] (d2) at (1,1) {};
    \node[remblais] (d3) at (4,0) {};
    
    % transport map
    \draw[draw=blue,-latex] (s1) to (d1);
    \draw[draw=blue,-latex] (s2) to (d2);
    \draw[draw=blue,-latex] (s3) to (d2);
    \draw[draw=blue,-latex] (s4) to (d3);
}

\newcommand{\transportPlanContinuous}[3]{
    % box
    \coordinate (bl) at (2,0);
    \coordinate (tl) at ($(bl) + (0,4)$);
    \draw (bl) -- ($(bl) + (4,0)$) -- ($(bl) + (4,4)$) -- (tl) -- cycle;
    
    % raw material
     \draw[fill=gray!25] ($(bl) + (0,0.25)$) to [curve through={($(bl) + (-0.1,.5)$) . . ($(bl) + (-0.75,1)$) . . ($(bl) + (-0.5,1.5)$) . . ($(bl) + (-.45,2)$) . . ($(bl) + (-1,2.75)$) . . ($(bl) + (-0.25,3.5)$)}] ($(bl) + (0,3.75)$) -- cycle;
    \node[anchor=east] (mu) at ($(bl) + (-.5,1.8)$) {\ifstrempty{#1}{$\mu$}{#1}};
     
    % construction
    \coordinate (shifttl) at ($(tl) + (1,0)$);
    \draw[fill=gray!25] ($(shifttl) + (0.25,0)$) -- ($(shifttl) + (0.25,1.5)$) -- ($(shifttl) + (0.75,1.5)$) -- ($(shifttl) + (0.75,1)$) -- ($(shifttl) + (1.5,1)$) -- ($(shifttl) + (1.5,2)$) -- ($(shifttl) + (2.25,1.5)$) -- ($(shifttl) + (2.75,1.5)$) -- ($(shifttl) + (2.75,0)$) -- cycle;
    \node (nu) at ($(tl) + (2.5,.5)$) {\ifstrempty{#2}{$\nu$}{#2}};
    
    % transport plan
    % TODO make precise... right now marginal make no sense
    \path[draw,use Hobby shortcut,closed=true,fill=blue!25] (4.25,0.5) .. (5,1) .. (5.5,.5) .. (5.5,2) .. (5.5,3) .. (5,3) .. (4,3.25) .. (4,2.5);
    
    \node (gamma) at ($(bl) + (3,2)$) {\ifstrempty{#3}{$\plan{\gamma}$}{#3}};
}

\newcommand{\transportPlanDiscrete}{
    % sources
    \node[deblais] (s1) at (0,0) {};
    \node[deblais] (s2) at (3,2) {};
    \node[deblais] (s3) at (2,-1) {};
    \node[deblais] (s4) at (3,.5) {};
    
    % destinatinons
    \node[remblais] (d1) at (0,2) {};
    \node[remblais] (d2) at (1,1) {};
    \node[remblais] (d3) at (4,0) {};
    
    % transport map
    \draw[draw=blue,-latex] (s1) to (d1);
    \draw[draw=blue,-latex] (s1) to (d2);
    \draw[draw=blue,-latex] (s2) to (d1);
    \draw[draw=blue,-latex] (s2) to (d2);
    \draw[draw=blue,-latex] (s3) to (d2);
    \draw[draw=blue,-latex] (s4) to (d3);
}

\newcommand{\geodesicsOriginalSpace}{
    \node[deblais] (x) at (0,0) {};
    \node[remblais] (y) at (2,0) {};
    
    \draw[dashed] (x) -- (y);
    \draw[dashed] (x) to[bend right=90] (y);
    \draw[blue, -latex] plot [smooth] coordinates {(x.south) (0.5,-.5) (1.5,.5) (y.north)};
}
\newcommand{\geodesicsProbabilitySpaceDiscrete}[1]{
    \node[deblais] (x1) at (0,0) {};
    \node[remblais] (y1) at (2,0) {};
    \node[deblais] (x2) at (0,2) {};
    \node[remblais] (y2) at (2,2) {};
\ifstrempty{#1}{
    \draw[dashed] (x2) to[bend left] (y1);
    \draw[dashed] (x1) -- (y2);
    
    \draw[blue,-latex] plot [smooth] coordinates {(x1.south) (0.5,-.5) (1.5,.5) (y1.north)};;
    \draw[blue,-latex] (x2) -- (y2);
}{
    \draw[dashed] (x2) -- (y2);
    \draw[dashed] plot [smooth] coordinates {(x1.south) (0.5,-.5) (1.5,.5) (y1.north)};
    \draw[red,-latex] (x2) to[bend left] (y1);
    \draw[red,-latex] (x1) -- (y2);
}
}

\newcommand{\geodesicsProbabilitySpaceContinuous}[2]{
    \draw[dashed, thick] (1,-.25) to [bend left=90] (7,.75);
    \draw[dashed, thick] (2,-.25) to [bend right=90] (7,.5);
    
    \transportMapContinuous{#1}{#2}
}

%SPP
% Code adapted from https://tex.stackexchange.com/questions/57668/drawing-a-flag-with-tikz
\newcommand{\destination}[3]{%
\begin{scope}[scale=#2,rotate=#3]
    \draw[fill=brown!60!black,thick] ($#1 + (0,0)$) -- ++ (0,8) arc (180:0:0.4 and 0.1) -- ++ (0,-8) arc (360:180:0.4 and 0.1);
    \draw[thick] ($#1 + (0,8)$) arc (180:360:0.4 and 0.1);
    \draw[fill=blue,thick] ($#1 + (0.8,7.5)$) to[out=-30,in=210] ++(3,0) to[out=30,in=150] ++ (3,0) -- ++ (0,-3) to [out=150,in=30] ++(-3,0) to[out=210,in=-30] ++(-3,0) -- cycle;
\end{scope}
}

\tikzset{
 pics/obstacle/.style={
   code={
   \draw[use Hobby shortcut, draw=black, fill, closed] (0,0) +($(0:1+4*rnd)$)
       \foreach \a in {60,120,...,350} {  .. +($(\a: 1+4*rnd)$) };
   }
}}

% https://github.com/sisl/aircraftshapes
\pgfdeclareshape{quadcopter top}{
\inheritsavedanchors[from=coordinate]
\inheritanchor[from=coordinate]{center}
\backgroundpath{
\begin{pgfscope}
\pgftransformshift{\centerpoint}
\pgfmathdivide{\pgfkeysvalueof{/pgf/minimum width}}{1pt}
\pgftransformscale{\pgfmathresult}
\pgfpathcircle{\pgfpoint{0}{0}}{0.08}
\pgfpathcircle{\pgfpoint{0.26}{0.26}}{0.24}
\pgfpathcircle{\pgfpoint{-0.26}{-0.26}}{0.24}
\pgfpathcircle{\pgfpoint{0.26}{-0.26}}{0.24}
\pgfpathcircle{\pgfpoint{-0.26}{0.26}}{0.24}
\pgfpathcircle{\pgfpoint{0.26}{0.26}}{0.21}
\pgfpathcircle{\pgfpoint{-0.26}{-0.26}}{0.21}
\pgfpathcircle{\pgfpoint{0.26}{-0.26}}{0.21}
\pgfpathcircle{\pgfpoint{-0.26}{0.26}}{0.21}
\pgfpathcircle{\pgfpoint{0.26}{0.26}}{0.25}
\pgfpathcircle{\pgfpoint{-0.26}{-0.26}}{0.25}
\pgfpathcircle{\pgfpoint{0.26}{-0.26}}{0.25}
\pgfpathcircle{\pgfpoint{-0.26}{0.26}}{0.25}
\pgfpathcircle{\pgfpoint{0.26}{0.26}}{0.025}
\pgfpathcircle{\pgfpoint{-0.26}{-0.26}}{0.025}
\pgfpathcircle{\pgfpoint{0.26}{-0.26}}{0.025}
\pgfpathcircle{\pgfpoint{-0.26}{0.26}}{0.025}
\pgfpathmoveto{\pgfpoint{-0.01}{0}}
\pgfpathlineto{\pgfpoint{0.25}{0.26}}
\pgfpathlineto{\pgfpoint{0.27}{0.26}}
\pgfpathlineto{\pgfpoint{0.01}{0}}
\pgfpathclose
\pgfpathmoveto{\pgfpoint{0.01}{0}}
\pgfpathlineto{\pgfpoint{-0.25}{0.26}}
\pgfpathlineto{\pgfpoint{-0.27}{0.26}}
\pgfpathlineto{\pgfpoint{-0.01}{0}}
\pgfpathclose
\pgfpathmoveto{\pgfpoint{-0.01}{0}}
\pgfpathlineto{\pgfpoint{0.25}{-0.26}}
\pgfpathlineto{\pgfpoint{0.27}{-0.26}}
\pgfpathlineto{\pgfpoint{0.01}{0}}
\pgfpathclose
\pgfpathmoveto{\pgfpoint{0.01}{0}}
\pgfpathlineto{\pgfpoint{-0.25}{-0.26}}
\pgfpathlineto{\pgfpoint{-0.27}{-0.26}}
\pgfpathlineto{\pgfpoint{-0.01}{0}}
\pgfpathclose
\end{pgfscope}}}

% Forest ride
\newcommand{\forestRideFlag}[1]{
    \destination{(row#1) + (flags)}{0.04}{22.5};
}
\newcommand{\forestRideAgent}[3]{
    \node [quadcopter top,fill=white,draw=#3,minimum width=0.4cm,rotate=360*rnd] at ($(col#2) + (row#1)$) {};
}
\newcommand{\drawForestRideWorld}{
    \draw[step=.5,black,thin] (-0.25,-0.25) grid (12.75,5.25);
    % YOU SHALL NOT PASS LINE
    \draw[draw=red, thick] (0, -0.25) -- (0,5.25);
    
    % define columns and rows
    \foreach \col in {0,...,24}
        \coordinate (col\col) at (0.25 + 0.5*\col,0);
    \foreach \row in {0,...,9}
        \coordinate (row\row) at (0,4.75 - 0.5*\row);
        
    % TREES
    \foreach \row/\col in {0/11,0/12,0/13,0/14,0/15,0/20,2/13,2/14,4/16,4/17,6/11,6/12,6/13,6/14,8/17,8/18,9/15,9/16,9/17} {
        \pic at ($(col\col) + (row\row)$)  [fill=black!60!green, scale=0.06, rotate=360*rnd]{obstacle};
     }
     
     \coordinate (flags) at ($(col24) + (-0.1,-0.2)$);
}

\newcommand{\IFAheart}{
\draw[ETHblue,thick] (0,0) .. controls (0,0.75) and (-1.5,1.00) .. (-1.5,2)  arc (180:0:0.75);
\draw[ETHblue,thick] (0,0) .. controls (0,0.75) and ( 1.5,1.00) .. ( 1.5,2)  arc (0:180:0.75);
\node[inner sep=0pt] (ifa) at (0,1.5)
    {\includegraphics[width=.2\textwidth]{utils/logos/ifalogo_color.pdf}};
}

\newcommand{\tikzheart}{
\draw[ETHblue,thick] (0,0) .. controls (0,0.75) and (-1.5,1.00) .. (-1.5,2)  arc (180:0:0.75);
\draw[ETHblue,thick] (0,0) .. controls (0,0.75) and ( 1.5,1.00) .. ( 1.5,2)  arc (0:180:0.75);
}

\newcommand{\subgradients}{
\draw [very thick,  domain=0:2, samples=5, smooth, variable=\t]
    plot ({\t}, {-2*\t + 8});
\draw [very thick,  domain=2:4, samples=5, smooth, variable=\t]
    plot ({\t}, {\t*\t*0.25 + 3});
\draw [very thick,  domain=4:8, samples=10, smooth, variable=\t]
    plot ({\t}, {(\t-8)*(\t-8)*5*0.0625 + 2});
\draw [very thick,  domain=8:9, samples=5, smooth, variable=\t]
    plot ({\t}, {2});
\draw [very thick,  domain=9:12, samples=5, smooth, variable=\t]
    plot ({\t}, {9});
\draw[dotted, thin] (9,2) -- (9,9);
\draw[dashed] (0,1) -- (12,1);
\node[mark size=2pt,color=black] at (9,2) {\pgfuseplotmark{*}};
\node[mark size=2pt,color=black] at (9,9) {\pgfuseplotmark{o}};
}
